An Inverse Problem for the Relativistic Boltzmann Equation

We consider an inverse problem for the Boltzmann equation on a globally hyperbolic Lorentzian spacetime $(M,g)$ with an unknown metric $g$. We consider measurements done in a neighbourhood $V\subset M$ of a timelike path $\mu$ that connects a point $x^-$ to a point $x^+$. The measurements are modelled by a source-to-solution map, which maps a source supported in $V$ to the restriction of the solution to the Boltzmann equation to the set $V$. We show that the source-to-solution map uniquely determines the Lorentzian spacetime, up to an isometry, in the set $I^+(x^-)\cap I^-(x^+)\subset M$. The set $I^+(x^-)\cap I^-(x^+)$ is the intersection of the future of the point $x^-$ and the past of the point $x^+$, and hence is the maximal set to where causal signals sent from $x^-$ can propagate and return to the point $x^+$. The proof of the result is based on using the nonlinearity of the Boltzmann equation as a beneficial feature for solving the inverse problem.

==> Sections/MA-collision-kernel.tex <==
%
% Last edited: July 2, 2019
%
% This file contains the theorems and lemmas for the microlocal description of the collision operator and particle interactions.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Microlocal analysis of particle interactions}\label{microlocal-collision}


In this section we consider the gain term $\COLOP_{gain}$ of the collision operator and prove that we can extend $\COLOP_{gain}$ to conormal distributions over a certain class of submanifolds in $\PP M$. 
%{\color{red}($\longleftarrow$ distribution is conormal over a manifold. usually not over a Lagrangian manifold. Lagrangian manifolds appear in the microlocal level. For example, the conormal bundle $N^*S$ is a Lagrangian manifold etc.)} 
% As $\COLOP_{gain}$ is quadratic in its arguments, to define an extension we will need to analyze products of Lagrangian distributions. {\color{red}($\longleftarrow$How are the Lagrangian distributions and quadratic operators related?)} 
%Such products may be defined when the base Lagrangian manifolds {\color{red} ( $\longleftarrow$what is a base Lagrangian manifold?)} satisfy either a transverse or clean intersection property (see \cite{DH1972}, \cite{guillemin1975clean}, \cite{melrose-uhlmann1979}, \cite{guillemin1981}, and \cite{greenleaf-uhlmann}). 
%In this paper, we consider distributions over Lagrangian manifolds  which are the geodesic flowout of some submanifold in $\OVS M$ {\color{red}($\longleftarrow$Again, the Lagrangian manifolds occur in the microlocal level. Not in the base-manifold.)}. With such Lagrangian manifolds in mind, we first describe an intersection property which suits our purpose of extending the operator $\COLOP_{gain}$.
%
%
%Let $S_1$ and $S_2$ be submanifolds of $\OVS M$ with $S_1\cap S_2=\emptyset$, whose respective geodesic flowouts $Y_{1} := K_{S_{1}}$ and $Y_{2}:= K_{S_{2}}$ in $\overline{\PP} M$ have admissible intersection: {\color{red} (There is no $S_1$ or $S_2$ needed in the definition. The manifolds $Y_1$, $Y_2$ dont necessarily need to be $K_{S_j}$, $j=1,2$.)}
%
%
\begin{definition}\label{intersection_coords}[Admissible intersection \antti{property}]
We say that \antti{submanifolds} 
%\footnote{\antti{Please stop adding ''open submanifold'' to everywhere. It does not make sense. In what sense is a curve for example an open manifold? If manifold is not closed it does not mean it is open. Btw. these manifolds here can be closed manifolds so please pay attention. }} 
$Y_1 \subset \PP M$ and $Y_2 \subset \PP M$ have an admissible intersection \antti{property} 
%in $X \subset M$ if the following holds: For every 
at $x_0\in \pi(Y_1)\cap \pi(Y_2)$ if there exists an open neighbourhood \tbl{$U_{x_0} = U\subset M$} of $x_0$ and coordinates
\begin{equation}\label{x_splits}
x = (x',x'') : U \rightarrow \R^\nnn, \quad x' = (x^1,\dots,x^d), \quad x''=(x^{d+1}, \dots, x^\nnn)
\end{equation}
centered at $x_0$ 
% on some neighbourhood 
such that
\begin{equation}\label{turhautuminen1}
\begin{split}
Y_1 \cap TU &= \{ (x,p)   \in TU  : x' = 0  , \ p' = 0, \ p''= (1,0,\dots,0) \}     \\
%Y_2 \cap TU &= \{  (x,p) \in TU : x'' = 0, \ p''= 0, \  p' = (1,0,\dots,0) \}
Y_2 \cap TU &= \{  (x,p) \in TU : x'' = 0, \ p''= 0, \ p'= (1,0,\dots,0) \}
%\\ \quad d &=  \dim K_{M_2} = \nnn -  \dim K_{M_1}.
\end{split}
\end{equation}
in the associated canonical coordinates $(x,p) = (x',x'',p',p'')$ of $TU$. 
Moreover, for $X \subset M$ we say that the pair $Y_1$ and $Y_2$ has the admissible intersection property in $X$ if either the property holds at every $x_0 \in \pi(Y_1)\cap \pi(Y_2) \cap X$ or $ \pi(Y_1)\cap \pi(Y_2) \cap X = \emptyset $. 

Given a neighbourhood $U$ as above we define the following conic Lagrangian submanifolds: 
\[
\Lambda_0 := N^*\{ (0,0) \} = T_{x_0}^* \R^\nnn, \quad \Lambda_1 := N^*  \{ x   \in U  : x' = 0  \} \quad \text{and} \quad \Lambda_2 := N^*  \{ x   \in U  : x'' = 0  \}. 
\]
%Moreover, if $X \subset M$ and the property holds at every $x_0 \in \pi(Y_1)\cap \pi(Y_2) \cap X$ we say that the pair $Y_1$ and $Y_2$ has the admissible intersection property in $X$. 
\end{definition}
%\antti{Notice that any two submanifolds $Y_1$, $Y_2$ in $\PP M$ with $\pi(Y_1)\cap \pi(Y_2) \cap X = \emptyset$ have admissible intersectiion property in $X$.}

We remark that our statement of Definition \ref{intersection_coords} is motivated by the following case which arises in our proof of Theorem \ref{themain}. Let $V\subset M$ be as in Theorem \ref{themain}. \antti{ In the proof of the theorem we will consider two delta-type distributions supported over a submanifold $S_{1}\subset \PP^+ V$ of dimension $(n-2)$ and a single point space $S_{2}=\{(x,p)\} \subset \PP^+ V$. The submanifold $S_{1}$  is constructed  in \antti{Corollary \ref{coro_renerew} using Lemma \ref{lemma_renerew}} %(see also Lemma \ref{two_manifold_jacobi_const}) 
so that 
%its projection to $M$ is a Cauchy surface {\color{red}($\longleftarrow$ this is not true)} and such that 
the geodesic flowouts $Y_{1} := K_{S_{1}}$ and $Y_{2}:= K_{S_{2}}$ have admissible intersection property in $\pi \text{supp}A$ and hence transverse intersection when projected to the base manifold $M$ in both settings $(M,g)  = (M_j,g_j)$, $j=1,2$ simultaneously.  
%\tbl{In the coordinates $(x',x'')$ of Definition~\ref{intersection_coords}, the tangent vectors ( i.e. the fiber components) in $Y_1$ and $Y_2$ with base points in $\pi(Y_1)$ and $\pi(Y_2)$ are represent by the constant vector fields $p''=(1,0,\ldots,0)$ and $p'=(1,0,\ldots,0)$ respectively.} 
This intersection is a finite number of \antti{discrete points}. % in the ``unknown'' submanifolds $W_{1}$ and $W_{2}$ of Theorem \ref{themain}. %\footnote{\tbl{Explain what are $Y_1$ and $Y_2$ in practice. $d=1$. Say that the projection to base manifold intersect transversally. Explain that if $Y_1$ and $Y_2$ are tangent spaces of transversally intersecting submanifolds of $M$.}}
Moreover, due to admissible intersection property,  the fibre component $T_x M \cap Y_j$  of $Y_j$ at each point $x$ sufficiently near an intersection point $x_0 \in \pi Y_1 \cap \pi Y_2 \cap (\pi \text{supp}A)$ is a single vector (the vector $(1,0,\dots,0)$ in coordinates) and hence the map $\pi :TM \to M$ defines diffeomorphism from $Y_j$ to the projection $G_{S_j} := \pi K_{S_j}$ in that neighbourhood for both $j=1,2$. 
Globally the set $G_{S_1}$ (also $G_{S_2}$ if $S_2$ is not required to be a single point space) may fail to be manifold due to caustic effects. 
}
%Thus, one may perceive the intersection property as a transversality between $K_{S_1}$ and $K_{S_2}$, although the manifolds do not 
%}
%Through the diffeomorphism one may identify $K_{S_j}$ as the set $G_{S_j}$ near the points in $G_{S_1} \cap G_{S_2}$. 

%With the above situation in mind, we next show that in the case when $\pi S_1\in M$ is a point and $\pi S_2 \subset M$ is a Cauchy surface{\color{red}($\longleftarrow$ again, not true)}, the geodesics flowouts of $S_1$ and $S_2$ have admissible intersection.
% 
%\begin{lemma}
%Let $\mathcal{C}$ be a Cauchy surface of a Lorentzian manifold $(M,g)$. Let $(x_0,p_0)\in \PP^+ \mathcal{C}$ {\color{red} (have you defined this? if not then it is a subbundle of $T\mathcal{C}$ which should not be the case. Compare to $\PP M \subset TM$.)} and denote $S_1=(x_0,p_0)$. Let $q$ be a vector field defined on a submanifold $L$ of $\mathcal{C}$. Let us denote by $S_2$ the submanifold $q(L)$ of $\PP^+ \mathcal{C}$ {\color{red}(makes sense only if $q$ is time-like)}. Assume that $z\in \pi(K_{S_1})\cap \pi(K_{S_2})$. Assume also that $\pi(K_{S_1})$ and $\pi(K_{S_2})$ are submanifolds of $M$ on a neighbourhood of $z$ and that $\pi(K_{S_1})$ and $\pi(K_{S_2})$ intersect transversally at $z$. 
%{\color{red} (Is this lemma really necessary? For such choices of $Y_j$ the transversality assumption is pretty much the same thing as your claim.) }
%
%Then, there is a neighbourhood $U\subset M$ of $z$ and local coordinates $(x',x'')$ , with $x':U\to \R$ and $x'':U\to \R^{n-1}$, such that $Y_1= K_{S_1}$ and $Y_2=K_{S_2}$ may be expressed as in \eqref{turhautuminen1}.
%%. The coordinates $(x',x'')$ have the following properties
%% \[
%%  x = (x',x'') : U \rightarrow \R^\nnn, \quad x' = (x^1,\dots,x^d), \quad x''=(x^{d+1}, \dots, x^\nnn)
%% \]
%%\begin{equation}\label{turhautuminen1}
%%\begin{split}
%%Y_1 \cap TU &= \{ (x,p)   \in TU  : x' = 0  , \ p' = 0, \ p''=1 \}  \\
%%%Y_2 \cap TU &= \{  (x,p) \in TU : x'' = 0, \ p''= 0, \  p' = (1,0,\dots,0) \}
%%Y_2 \cap TU &= \{  (x,p) \in TU : x'' = 0, \ p''= 0, \ p'=(1,0,\dots,0) \}
%%%\\ \quad d &=  \dim K_{M_2} = \nnn -  \dim K_{M_1}.
%%\end{split}
%%\end{equation}
%%in the associated canonical coordinates $(x,p) = (x',x'',p',p'')$ of $TU$.
%\end{lemma}
%\begin{proof}
% Let $y'$ be coordinates on $L\subset \mathcal{C}$. % neighborhood of $y_0$. 
%%Consider the map
%% \[
%%  (t,y')\mapsto \exp_{y'}(t\, q(y')).
%% \]
% 
%Consider $z$ in $\pi(K_{S_1})\cap \pi(K_{S_2})$. By assumption $\pi(K_{S_1})$ and $\pi(K_{S_2})$ intersect transversally at $z$ and  $\pi(K_{S_2})$ is a manifold on a neighbourhood of $z$. It follows that there is a vector field $\hat{q}$ of $TM$, which is defined on a neighbourhood of $z$ in $\pi(K_{S_2})$ and which is transversal {\color{red}($\longleftarrow$ what is transversality between a vector field and a manifold? do you mean $\hat{q} \notin T\pi(K_{S_2})$ ?)} to $\pi(K_{S_2})$. {\color{red} ($\longleftarrow$ with my interpretation of transversality (previous comment) this claim holds for every submanifold of any manifold with greater dimension.)}
% 
% There is a point $(t_0,y_0')\in \R\times \mathcal{C}$ such that $z=\exp_{y_0'}(t_0\, q(y_0'))$. Let us denote 
% \[
% Q(t,y')=\exp_{y'}((t_0+t)\, q(y'))                                                                                                                                                                             
% \]                                 
% and define the map
% \begin{equation}\label{def_of_admissible_coords}
%  (s, t,y')\mapsto \exp_{Q(t, y')}(s\, \hat{q}(Q(t, y'))).
% \end{equation}
% This map is well-defined on a neighbourhood of $(0, t_0,y_0')\in\R\times \R\times \mathcal{C}$. %We claim that this mapping defines coordinates on a neighborhood of $z$ with the desired properties. 
% The map~\eqref{def_of_admissible_coords} is a local diffeomorphism since $\pi(K_{S_1})$ and $\pi(K_{S_2})$ are submanifolds of $M$ on a neighbourhood of $z$ and since $\pi(K_{S_1})$ and $\pi(K_{S_2})$ intersect transversally at $z$. Thus~\eqref{def_of_admissible_coords} defines a local coordinate system on a neighbourhood $U$ of $M$. By setting $x'=s$ and $x''=(t,y')$ we see that~\eqref{turhautuminen1} holds. {\color{red} (According to what you claim in this proof, the set $\pi Y_1$ should lie in $\{ x' = 0\} = \{ (s,t,y') : s= 0\} = \{ \exp_{Q(t, y')}(0 \hat{q}(Q(t, y'))) \} = \{ Q(t,y') : (t,y') \ \text{free variable} \  \} $. This can not be true since $Y_1$ should be 1-dimensional. Maybe $Y_1$ and $Y_2$ whould be other way around here. Moreover, according to your proof, $\pi Y_2$ should lie in $\{ x'' = 0\} = \{ (s,t,y') : (t,y') = 0\} = \{ \exp_{Q(0,0)}(s\, \hat{q}(Q(0,0))) : s \text{ free variable}   \}$ which cant even be corrected by swapping $Y_1$ and $Y_2$. Non of the elements $\hat{q}$, $y' = 0$ etc. is explicitly fixed so the claim cant hold as it is. I can only guess that $Q(0,0)$ is suppose to be in the curve $Y_1 = \dot\gamma_{(x_0,p_0)}$ or something like that...)}
%\end{proof}


%\begin{property}\label{intersection_coords}[Admissible intersection]
%We say that submanifolds $Y_1$ and $Y_2$ of $\PP M$ have admissible intersection property if the following holds: If $z\in \pi(Y_1)\cap \pi(Y_2)$, there is an open neighbourhood $U$ of $z$ and a local coordinate system $x=(x',x'')$ on $U$ such that~\eqref{turhautuminen1} holds.  
%% \begin{equation}\label{x_splits}
%% x = (x',x'') : U \rightarrow \R^\nnn, \quad x' = (x^1,\dots,x^d), \quad x''=(x^{d+1}, \dots, x^\nnn)
%% \end{equation}
%% % on some neighbourhood 
%% such that
%% \begin{equation}\label{turhautuminen1}
%% \begin{split}
%% Y_1 \cap TU &= \{ (x,p)   \in TU  : x' = 0  , \ p' = 0 \}  \\
%% %Y_2 \cap TU &= \{  (x,p) \in TU : x'' = 0, \ p''= 0, \  p' = (1,0,\dots,0) \}
%% Y_2 \cap TU &= \{  (x,p) \in TU : x'' = 0, \ p''= 0, \ p'=\textit{constant vector} \}
%% %\\ \quad d &=  \dim K_{M_2} = \nnn -  \dim K_{M_1}.
%% \end{split}
%% \end{equation}
%% in the associated canonical coordinates $(x,p) = (x',x'',p',p'')$ of $TU$.~\footnote{\tbl{Later on we need to prove that such coordinates exist for $K_{S_1}$ and $K_{S_2}$.}} 
%In this case we define the conic Lagrangian submanifolds of $U$ by using the coordinate $(x',x'')$ as
%\[
%\Lambda_0 := T_{0}^* \R^\nnn, \quad \Lambda_1 := N^*  \{ x   \in U  : x' = 0  \} \quad \text{and} \quad \Lambda_2 := N^*  \{ x   \in U  : x'' = 0  \}. 
%\]
%% \footnote{\tbl{Explain what are $Y_1$ and $Y_2$ in practice. $d=1$. Say that the projection to base manifold intersect transversally. Explain that if $Y_1$ and $Y_2$ are tangent spaces of transversally intersecting submanifolds of $M$.}}
%\end{property}



%Since $\overline{\PP} M $ is a manifold with boundary, an extension of 
Our goal is to extend the operator $\COLOP_{gain}[\ccdot,\ccdot] : C^\infty_c( \PP M)\times C^\infty_c( \PP M) \rightarrow C^\infty( \overline{\PP} M) $ to conormal distributions over submanifolds 
%{\color{red} ($\longleftarrow $ again, not Lagrangian submanifolds. 
%Distribution is conormal over a manifold. The singularities are on Lagrangian manifolds.)} 
of $\PP M$, such as those described above. %However, the extended operator would take values in $\mathcal{D}'( \overline{\PP} M)$. 
The analysis of such an extension requires microlocal analysis on manifolds with boundary, since $\overline{\PP} M$ has a boundary given by the collection of lightlike vectors. %is a manifold with boundary,  and its %(x,p)$ for $(x,p)\in \overline{\PP} M$ and 
%analysis 
%of $\COLOP_{gain}[\ccdot,\ccdot](x,p)$ for $(x,p)\in \overline{\PP} M$ 
%requires microlocal analysis on manifolds with boundary, which 
The analysis of distributions over manifolds with boundary can be involved and technical. \tbl{We are able to avoid difficulties related to manifolds with boundary by introducing an auxiliary vector field and composing it with $\COLOP_{gain}$. This is explained next.} % wish to avoid the potential complexities in microlocal analysis on manifold with boudary. %However, this level of complexity is not required for our purposes. 

Fix an open set $U\subset M$ and a smooth vector field \tjb{$P: U\to \overline{\PP} U$}\f{changed F to P. This change was done throughout this section (and hence the document).}. Let $u,v\in C_c^\infty(\PP M)$, and let $x\in U$. We define the operator $\COLOP_{gain}^P: C_c^\infty(\PP M)\times C_c^\infty(\PP M)\to C^\infty(U)$ as 
\begin{equation}\label{def_of_QF}
% \COLOP_{gain}^P:=F^*\COLOP_{gain}, \qquad 
\COLOP_{gain}^P[u,v](x)=\COLOP_{gain}[u,v](P(x)).
\end{equation}
%Here $F^*$ denotes the pull back of functions by $F$.
\tbl{We will see in this section that we are able to analyze $\COLOP_{gain}^{P}$ operator by using standard techniques such as those in~\cite{duistermaat2010fourier}. }\tjb{The analysis of $\COLOP^{P}_{gain}$ presented in this section will be used to study the singular structure of solutions $\Phi_{L^{+}V}f$ to \eqref{boltzmann} for given sources $f$ which are constructed in Section \ref{main-proof}. We note now that in Section \ref{main-proof},  we we will choose a specific $P$, which we will denote by $P_{e}$.}%~\f{There are now $F$, $P$, $P_e$, $P_{e'}$. Remove some. I think $P$ and $P_e$ should suffice. -Tony} %We will also analyse the 
% 
% the operators 
% \[
%  \COLOP_{gain}[\ccdot,\ccdot](x,F(x)) \text{ and } \COLOP_{gain}[\IX(\ccdot),\IX(\ccdot)](x,F(x)), \quad x\in U
% \]
%\COLOP_{gain}[\ccdot,\ccdot](x,F(x))$ and $$, defined for $x\in U$.
% '
%Before doing so, we first record a couple of lemmas, whose proofs we have placed in the appendix.

We first record a couple of auxiliary lemmas. \tbl{The first lemma considers the conormal bundle of a submanifold of $U\times \PP U\times \PP U$. The points of $U\times \PP U\times \PP U$ are denoted by % consisting of points 
$(x,y,z,p,q) = (x,(y,p), (z,q))$.} % $x\in U$, $(y,p)\in \PP U$ and $(z,q)\in \PP U$.%  \{ x\} \times  \PP_xU \times \PP_xU$
\begin{lemma}\label{Lambda_R-lemma}
Let $Y_1$ and $Y_2$ and $U$ be as in Definition~\ref{intersection_coords} and adopt also the associated notation.
% of Property~\ref{intersection_coords}. %be an open subset of a smooth Lorentzian manifold $(M,g)$ and 
Define
\[
\Lambda_R =   N^* \Big( \bigcup_{x\in U}  \{ x\} \times  \PP_xU \times \PP_xU  \Big).
\]
%We identify $T^*(U \times  \PP U  \times \PP U )$ locally as a subset of $(U^3 \times \R^{2\nnn} ) \times \R^{5\nnn} $ by using canonical coordinates on $U$. In these canonical coordinates,
%In canonical coordinates of $T^*(U \times  \PP(U) \times \PP(U) )$, identified as a subset of $(U^3 \times \R^{2\nnn} ) \times \R^{5\nnn} $, 
The submanifold $\Lambda_R$ of $T^*( U \times \PP U \times \PP U) \setminus \{0 \}$ equals the set
\begin{align*}%\label{uuUUU90777}
\Lambda_R = \{ %(x,y,z, p,q\, ; \, \xi^x, \xi^y , \xi^z, \xi^p,\xi^{q} )
\big(x, y, z,p, q \, ; \, \xi^x, \xi^y, \xi^z,\xi^p,\xi^{q} \big) \in \  &T^*(U \times \PP U \times  \PP U) \setminus \{0\}  :  \\
%&  \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad %%<---u kidding? just move the & in the previous line.
&  \xi^x + \xi^y +\xi^z = 0 , \ \xi^p = \xi^{q} = 0, \ x=y=z  \}.
\end{align*}

\tbl{We have
\begin{align}\label{lambda_R_prime}%\label{hauska122211}
\Lambda_R' &%= \{ (x,y,z, p,q\, ; \, \xi^x, \xi^y , \xi^z, \xi^p,\xi^{q} )  : x=y=z, \ \xi^x + \xi^y +\xi^z = 0 , \ \xi^p = \xi^{q} = 0  \} \\
  =\{ \big((x ; \xi^x), (y, z,p, q \, ; \, \xi^y, \xi^z,\xi^p,\xi^{q} )\big) \in \ T^*U \times T^* ( \PP U \times  \PP U) \setminus \{0\}   : \nonumber  \\
 &  \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \xi^x =\xi^y+ \xi^z \neq 0, \
   \xi^p =  \xi^{q} =0 , \ 
    x=y=z \}.
\end{align}
}
% 
% \begin{equation}\label{lambda_R_prime}
% \begin{split}
% \Lambda_R' %= \{ (x,y,z, p,q\, ; \, \xi^x, \xi^y , \xi^z, \xi^p,\xi^{q} )  : x=y=z, \ \xi^x + \xi^y +\xi^z = 0 , \ \xi^p = \xi^{q} = 0  \} \\
%   :=\{ \big((x ; \xi^x), (y, z,p, q \, ; \, \xi^y, \xi^z,\xi^p,\xi^{q} )\big) \in \  T^*U \times & T^* ( \PP U \times  \PP U)  \setminus \{0\}   :   \\
% % &  \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \xi^x =\xi^y+ \xi^z \neq 0, \ %%<---u kidding? just move the & in the previous line.
%  & \xi^p =  \xi^{q} =0 , \ 
%     x=y=z \}.
%     \end{split}
% \end{equation}
The spaces $\Lambda'_R \times ( N^*[Y_1 \times  Y_2] ) $ and $T^*U \times \text{diag}\, T^*( \PP M \times \PP M) $ intersect transversally in $T^*U \times T^*(\PP M \times \PP M) \times  T^*(\PP M \times \PP M)$.

\end{lemma}
Please see Appendix \ref{appendixa1} for a proof. 
\medskip



%\begin{lemma}\label{tensorlemma}
%Let $Y_j\subset TM$, $j=1,2$, be as in in Definition \ref{intersection_coords}, and let $f_j  \in  I^{m_j} (N^* Y_j )$. Then,~\f{Tensor product of distributions added.}
%\[
%\begin{split}
%f_1 \otimes f_2 \in I^{m_1+m_2 + \nnn,  -m_2- \nnn} \big( N^* [Y_1  \times \PP M] , N^* [Y_1  \times  Y_2]   \big) \\
% +  I^{m_1+m_2+ \nnn, -m_1-\nnn} \big( N^*[\PP M \times  Y_2 ] , N^* [Y_1  \times  Y_2]   \big). 
%%+ I^{\tilde\mu,\mu} \big(  \PP \times K_{M_2}  ,  K_{M_1}  \times K_{M_2}   \big)
%\end{split}
%\]
% \end{lemma}

% We will next consider submanifolds $Y_1$ and $Y_2$ of $\overline{\PP} M$ intersecting transversally. If $(x_0,p_0)$ is in the intersection of $Y_1$ and $Y_2$, there is an open neighbourhood $U$ of $x_0$ and coordinates $x$~\footnote{\tbl{Check this and clean.}} %on $U$ with the following properties:
% \begin{equation}\label{x_splits}
% x = (x',x'') : U \rightarrow \R^\nnn, \quad x' = (x^1,\dots,x^d), \quad x''=(x^{d+1}, \dots, x^\nnn)
% \end{equation}
% % on some neighbourhood 
% such that
% \begin{equation}\label{turhautuminen1}
% \begin{split}
% Y_1 \cap TU &= \{ (x,p)   \in TU  : x' = 0  , \ p' = 0,  \ p'' = (1,0,\dots,0)  \}  \\
% Y_2 \cap TU &= \{  (x,p) \in TU : x'' = 0, \ p''= 0, \  p' = (1,0,\dots,0) \}
% %\\ \quad d &=  \dim K_{M_2} = \nnn -  \dim K_{M_1}.
% \end{split}
% \end{equation}
% in the associated canonical coordinates $(x,p) = (x',x'',p',p'')$ of $TU$. 
% 
% ÂŽintersect transversally, if $ is an intersection point there are coordinates $x$ on an We introduce some notation. Let $(U,x)$ be coordinate neighbourhood of $M$. The
%  

For the next theorem let $Y_1,Y_2 \subset \PP M$ be smooth manifolds which satisfy the properties in Definition \ref{intersection_coords}. Fix $x_0 \in \pi(Y_1) \cap \pi(Y_2) \cap X$ (below we choose $X= \pi \text{supp}A $) and let $\Lambda_j$, $j=1,2$, be the Lagrangian manifolds specified in the definition. In canonical coordinates $(x,\xi) = (x',x'', \xi', \xi'')$ on $T^*U$ we obtain the expressions
\begin{align}
\Lambda_0 = \{ (x,\xi) : x' = 0, \ x'' = 0 \}, \\
\Lambda_1 = \{ (x,\xi) : x' = 0, \ \xi'' = 0 \}, \\
\Lambda_2 = \{ (x,\xi) : x''= 0, \ \xi' = 0 \}.
\end{align}
Thus, the elements of the manifolds $\Lambda_0,\Lambda_1, \Lambda_2$ can be parametrized by the free coordinates $(\xi',\xi'')$, $(x'',\xi')$, and $(x',\xi'')$, respectively. In the canonical coordinates \\ $(x,p ; \xi^x,\xi^p) = (x',x'',p',p'' ; (\xi^x)',(\xi^x)'',(\xi^p)',(\xi^p)'' )$ in $T^*TU$ we have that
\begin{align}
N^*Y_1 = \{ (x,p ; \xi^x,\xi^p) : x'= 0, \ p'=0, \ p''=(1,0,\dots,0), \ (\xi^x)'' = 0\},\\
N^*Y_2 = \{ (x,p ; \xi^x,\xi^p) : x''= 0, \ p''=0, \ p'=(1,0,\dots,0), \ (\xi^x)' = 0\},
\end{align}
so the manifolds $N^* Y_1$ and $N^* Y_2 $ are locally parametrized by the \tbl{coordinates $(x'', ( \xi^x)', \xi^p)$ and $(x', ( \xi^x)'', \xi^p)$ respectively. 
%The trivialisations above are considered in 
The identity \eqref{symboiu} in the next theorem is written in terms of the coordinates $(x'', ( \xi^x)', \xi^p)$, $(x', ( \xi^x)'', \xi^p)$ and $((\xi^x)',(\xi^x)'')$ for the symbols $\sigma(f_1)$, $\sigma(f_2)$ and $\sigma ( \COLOP_{gain}^P[f_1,f_2])$ respectively. }

We extend $\COLOP_{gain}^P$ to conormal distributions as follows. % captured in the following proposition.

%To avoid dealing with operators on a manifold with boundary we would like to extend the operator $\COLOP_{gain}[ \ \cdot \ , \ \cdot \ ] (x,p)$ for fixed variable $p \in \OVS$. 
%However, this  creates a slight technical issue since the domain of $p = F(x)$ now depends on the base point $x$. We circumvent this problem by employing local coordinates, where we can identify $T_xM = \R^n$. Fixing $p \in \R^n$ then corresponds to a smooth local section $x \mapsto (x, p^\alpha \partial_\alpha |_x)$ in the bundle $\pi: \OVS \rightarrow \R \times N$. Motivated by this, we proof the following:

\begin{theorem}\label{sofisti}   
Let $(M,g)$ be a globally hyperbolic Lorentzian manifold.  
Let $Y_1,\, Y_2 \subset \PP M$, 
%S^{r_j}_{t_j}$, $t_j \in \R$, $r_j > 0$ , $j=1,2$  
be smooth manifolds that have the admissible intersection \antti{property} (Definition \ref{intersection_coords}) at some $x_0 \in \pi Y_1 \cap \pi Y_2$ and let $\Lambda_l$, $l=0,1,2$, and $U\subset M$ be as in Definition~\ref{intersection_coords}. %Let also $m_1,\,m_2\in \R$. %By using the coordinates~\eqref{x_splits},~\eqref{turhautuminen1} % that 
%for each $x_0 \in \text{supp} ( x \mapsto A(x,\cdot,\cdot,\cdot , \cdot) ) \cap G_{M_1} \cap G_{M_2}$ 
%there is an open neighbourhood $ U \subset M$ and local coordinates 
% \[
% x = (x',x'') : U \rightarrow \R^\nnn, \quad x' = (x^1,\dots,x^d), \quad x''=(x^{d+1}, \dots, x^\nnn)
% \]
% % on some neighbourhood 
% satisfying~\footnote{\tbl{Does this exactly mean that $Y_1$ and $Y_2$ intersect transversally (on $U$)? If so we could put it into a lemma.}}
% \begin{equation}\label{turhautuminen1}
% \begin{split}
% Y_1 \cap TU &= \{ (x,p)   \in TU  : x' = 0  , \ p' = 0,  \ p'' = (1,0,\dots,0)  \}  \\
% Y_2 \cap TU &= \{  (x,p) \in TU : x'' = 0, \ p''= 0, \  p' = (1,0,\dots,0) \}  , 
% %\\ \quad d &=  \dim K_{M_2} = \nnn -  \dim K_{M_1}.
% \end{split}
% \end{equation}
% in the associated canonical coordinates $(x,p) = (x',x'',p',p'')$ of $TU$. 
%Using the coordinates $(x,p)$, 
% define the conic Lagrangian submanifolds 
% \[
% \Lambda_0 := T_{0}^* \R^\nnn, \quad \Lambda_1 := N^*  \{ x   \in U  : x' = 0  \} \quad \text{and} \quad \Lambda_2 := N^*  \{ x   \in U  : x'' = 0  \}. 
% \]
%
Let $P$  be a smooth section of the bundle $\pi: \overline{\mathcal{P}}U \rightarrow U$  %, that is, a smooth function $F : U \rightarrow \overline{\mathcal{P}} U$ such that $\pi \circ F(x) = x$. %That is, in 
and  $\COLOP$ be the collision operator with an admissible collision kernel. 
%\begin{enumerate}
%\item[i)] 

Then the operator $\COLOP_{gain}^P: C_c^\infty (\PP M ) \times C_c^\infty (\PP M ) \rightarrow C^\infty ( U )$ defined in~\eqref{def_of_QF}
% \begin{align*}
% \COLOP_{gain}  [h_1,h_2]_F (x) :=\COLOP_{gain} [h_1,h_2] (x ,p(x) ), 
% \end{align*}
%given by
%\[
%\COLOP_{gain}  [h_1,h_2]_F (x) =\COLOP_{gain} [h_1,h_2] (x ,p(x) ) 
%\]
extends into a continuous map
\[
 I^{m_1}_{comp} ( \PP M ;\, N^*Y_1 )\times I^{m_2}_{comp} (\PP M ;\, N^*Y_2 ) \rightarrow \mathcal{D}' (U), \quad m_1,m_2 \in \R.
 % I^{m_2-\nnn/4,m_1+ \nnn/2} (  \Lambda_0, \NG_{M_1} ,   ; U )+I^{m_1-\nnn/4,m_2 + \nnn/2} ( \Lambda_0,  \NG_{M_2}  ;  U  )
\]
%\item
%\item[ii)]  

For $(f_1 , f_2) \in I^{m_1}_{comp} ( \PP M ;\, N^*Y_1)\times I^{m_2}_{comp} (\PP M ;\, N^*Y_2)$ we have that 
\[
WF(\COLOP_{gain}^P[f_1,f_2]) \subset \Lambda_0 \cup \Lambda_{1} \cup \Lambda_{2}. 
%\end{split}
\]
%where the product type symbol class is defined in the sense of \cite{guillemin1981}.
%\item[]
Moreover, microlocally away from both $\Lambda_{1}$ and $\Lambda_{2} $, we have that 
%\begin{align}
\begin{equation}\label{si3478}
\COLOP_{gain}^P [f_1,f_2]\in I^{m_1+m_2+3\nnn/4} (U;\,\Lambda_0 \setminus( \Lambda_{1} \cup \Lambda_{2}) )
\end{equation}
together with the symbol 
\begin{equation}\label{symboiu}
\begin{split}
 \sigma ( \COLOP_{gain}^P [f_1,f_2]) \tbl{((\xi^x)',(\xi^x)'')} = 
%c A(x, \hat{p}(x) ,  p_x+q_x- \hat{p}(x) , p_x,q_x)  
 C \sigma( f_1) (0 ;  \tbl{(\xi^x)' , 0  ) \sigma(f_2) ( 0 ;  (\xi^x)''} , 0) , %\\  (\xi',\xi'') \in \R^\nnn \setminus (  \{0\} \times \R^\nnn  \ \cup \    \R^\nnn \times \{ 0\} ) 
 \end{split}
\end{equation}
where $C$ is given in the canonical coordinates $p = (p',p'')$ and $q=(q',q'')$ by 
\[
C = c\s A(x_0, \hat{p} (x_0) , p+q- \hat{p}(x_0) , p,q) \big|_{p = (1,0,\dots,0), \ q=(1,0,\dots,0) } , 
\] 
and $\hat{p}(x_0) \in \overline{\PP}_{x_0} U$ is such that $P(x_0) = ( x_0, \hat{p}(x_0)) $. 
%for some constant $c\neq 0$ and the unique vectors $p,q \in \PP_x M$ satisfying $(x,p) \in Y_1 \cap T_x U$ and $(x,q) \in Y_2 \cap T_x U$. 
Here $c$ is some non-zero constant and the manifolds $\Lambda_0 \setminus( \Lambda_{1} \cup \Lambda_{2})$, $T^* U \cap N^* Y_1$, and $T^* U \cap N^* Y_2$ are parametrised by the canonical coordinates \tbl{$((\xi )',(\xi^x)'')$}, $(x'', (\xi^x)',\xi^p)$ and $(x' , (\xi^x)'', \xi^p)$ respectively. 
%for every $(f_1 , f_2) \in I^{m_1}_{comp} (  N^*Y_1 ; \overline{\mathcal{P}} M  )\times I^{m_2}_{comp} ( N^*Y_2 ;  \overline{\mathcal{P}} M )$.
%
%\item[iii)] 


%\end{enumerate}
\end{theorem}


%\subsection{Proof of Proposition \ref{sofisti}}
 

%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Theorem for Q[X^{-1} . , X^{-1} . ](x, F(x))
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%


\begin{proof}[Proof of Theorem \ref{sofisti}]
%Let us  now continue to the proof of Proposition \ref{sofisti}. 
We write $I^m (\PP M ;\, \Lambda) = I^m(\Lambda)$ for a Lagrangian manifold $\Lambda \subset T^* (\PP M)$ and $m \in \R$. 
To prove the claims of the proposition, %that $\COLOP_{gain}^P [ f_1,f_2 ]$ can be extended to compactly supported conormal distributions $f_j  \in  I^{m_j}_{comp} (N^* Y_j )$, $j=1,2$, and that the extension has the claimed properties, 
we first represent $\COLOP_{gain}^P [ f_1, f_2 ]$ as a composition of a Fourier integral operator and a tensor product of $f_1$ and $f_2$. Then we appeal to results for Fourier integral operators in~\cite{duistermaat2010fourier} to conclude the proof. %in particular to \cite[Theorem 2.4.1]{duistermaat2010fourier} and  \cite[Corollary 1.3.8]{duistermaat2010fourier}. 
The majority of the proof consists of demonstrating that the Fourier integral operators we use to decompose $\COLOP_{gain}^P [ f_1,f_2 ]$ satisfy the conditions required by~\cite[Theorem 2.4.1]{duistermaat2010fourier} and~\cite[Corollary 1.3.8]{duistermaat2010fourier}. 
%By the definition of $\COLOP_{gain}^P [ f_1,f_2 ]$ it suffi

%{\color{gray}Before we begin, we remark that the shorthand notation $\PP:= \PP U$ is used extensively in this proof.} {\color{red}($\leftarrow$ Lets not do this. Too dangerous notation.)}


Let $(x,p) = (x',x'',p',p'')$ be local coordinates in $TU$, where $U$ is an open neighbourhood of $x_0$, as described in Definition~\ref{intersection_coords}. %be a coordinates described in~\eqref{x_splits} and \eqref{turhautuminen1}. 
 Let us define an % Fourier 
 integral operator 
\[
R : C^\infty_c  ( \PP M  \times \PP M  ) \rightarrow \mathcal{D}' ( U  )
\]
by the formula%~\footnote{Need to choose one domain for $\delta_\Sigma$. The notation is funny, because not it looks like a pairing of $\phi$. I'd recommend $\delta_\Sigma[\phi]$. Also, I guess the target of $\Delta_\Sigma$ can be taken to be smooth functions.}
\[
\begin{split}
%\langle \delta_\Sigma ( x,p \, ; \,\cdot\,  ) ,  \phi \rangle = \int_{\Sigma_{x,p}} \phi (y,z,w,q,p',q')\, dV (y,z,w,q,p',q'), \ \phi \in C^\infty_c ( \mathcal{C}^3 ).
%\langle \delta_\Sigma ( x,p \, ; \,\cdot\,  ) ,  \phi \rangle  
\langle R [\phi] , \psi \rangle =&  \int_{  \PP U \oplus \PP U } \phi ( x, p , x , q) \psi(x) \, dv (x,p,q) \\
%= & \int_{\Sigma} \psi(x,p)  \phi (z,p',w,q') \, d\Sigma
%V (y,z,w,q,p',q').%, \ \phi \in C^\infty_c ( \mathcal{C}^3 ).
\end{split}
\]
%where $(x,p) \mapsto dV_{x,p}$ is a volume form on $T_{(x,x)} ( \R \times N)^2$
where $dv$ is \tbl{the induced volume form on the direct sum bundle $\PP U \oplus \PP U := \{ \big((x,p), (y,q) \big) \in \PP U \times \PP U : x = y \}$ and where $\phi\in C^\infty_c  ( \PP M  \times \PP M  )$ and $\psi\in C_c^\infty(U)$. The induced volume form $dv$ is given by considering $\PP U \oplus \PP U$ as a submanifold of $\PP U\times \PP U$ equipped with product Liouville volume form.} %Since $R$ is intgration over a submanifold of $\PP M \times \PP M$, we have that $R\in I^{-\nnn/4}( U, \PP M \times \PP M , \Lambda'_R)$.

% and $d\Sigma$~\footnote{Make precise later. Check Choque-Bruhat.} is the induced volume form on 
%\[
%\Sigma_{x,p} := \{ \vec{p} \in \{ (x,p) \} \times T(\R \times N)^3 : x= y=z=w  , \quad q  + p = p'+q'  \}.
%% \quad \text{ ($(x,p)$ fixed) }
%\]
%
%Then $\delta_\Sigma$ is a Fourier integral operator with kernel is the delta function $\Sigma$ 
%Here the notation $\Sigma$ refers to the set defined in~\eqref{Sigma_union} as
%The notation refers to the manifold
%\begin{align}%\label{def_sigma}
% \Sigma&:=\bigcup_{(x,p)\in T(\R \times N)} \Sigma_{x,p} =\{\,\vec{p}\in T(\R\times N)^4:\, x=y=z=w, \  p + q = p' + q' \}.\nonumber
%\end{align}
%from the definition of the collision operator. 
Let $P$ be a smooth local section of the bundle $\pi: \overline{\mathcal{P}}U \rightarrow U$. We represent $P$ as $P(x)=(x,\hat{p}(x))$ by using the coordinates $x$. Next, consider the operator	
\[
 \langle R_A [\phi] , \psi \rangle = \int_{  \PP U \oplus \PP U } A(x,\hat{p}(x),\, p+q - \hat{p}(x) ,\, p,\,q)\phi ( x, p , x , q ) \psi(x) \, dv (x,p,q) 
\]
% 
% 
% \[
% R_A (x \, ; \, z,p',w,q') := 
% %\bigg( \int_{L^+_x(\R \times N)} A(x,p , p'+q' - p , p',q') dw_x(p) \bigg) \cdot R (x \ ;  z,p',w,q') 
% A(x,p(x),\, p'+q' - p(x) ,\, p',\,q') \cdot R (x \, ;\,  z,p',w,q'). 
% \]
%Here the symbol $\cdot$ refers to multiplication by a smooth function. 
Notice that
\begin{equation}\label{uusi7878782}
%R_A (x \, ;  \, z,p',w,q') [ h_1 (z,p')  h_2(w,q') ] 
R_A[h_1 \otimes h_2]= 
%\pi_{L^+}^* 
\COLOP_{gain}^P [h_1, h_2] , \quad h_1,h_2 \in C_c^\infty( \PP M ).
\end{equation}
Here $h_1\otimes h_2$ is the tensor product of $h_1$ and $h_2$\tbl{, i.e. $(h_1\otimes h_2)((x,p),(y,q))= h_1(x,p)h_2(y,q)$.}
%for volume forms $dw_x$ and $dv$ such that $dw_x \wedge dv$ corresponds to the volume form in the definition of the collision operator under the parametrization
%of $\Sigma$ by variables $(x,p,q',p') \mapsto (x,p, p'+q'-p,p' ,q') \in \Sigma$.  
%Above
%Where the symbol $\cdot$ refers to multiplication by a smooth function. 
%Notice that the choice of volume form does not affect to microlocal properties since each volume form differs from others by multiplication of positive smooth function. 
%
\tbl{The distribution kernel associated to the operator $R $ is
%has the associated  kernel 
\[
k_R  \in \mathcal{D}' ( U \times  \PP M \times \PP M ). 
%, \quad 
%\langle  k_R  , \tilde{\phi}  \rangle :=  \int_{  \PP U \oplus \PP U } \tilde{\phi} (x, x, p,x,q ) dv %(x,p,q) , 
\]}
%where $\tilde{\phi} \in C^\infty_c ( U \times  \PP M \times \PP M)$. 
%The kernel is  a conormal distribution of class 
Since \tbl{$k_R$} is a delta distribution over the submanifold 
\[
 \bigcup_{x\in U}  \{ x\} \times  \PP_x M \times \PP_x M \  \subset \ U  \times  \PP M \times \PP M,
\]
it can be viewed as a conormal distribution
\begin{align*}
k_R &\in  I^{-\nnn/4 }(\tbl{U  \times  \PP M \times \PP M \s;  \Lambda_R }), \\
\Lambda_R &:=   N^* \Big( \bigcup_{x\in U}  \{ x\} \times  \PP_x M \times \PP_x M \Big).
\end{align*}
Hence $R$ is a Fourier integral operator %of order $-\nnn/2$ in the sense that
%\[
 of class $I^{-\nnn/4}( U, \PP M \times \PP M , \Lambda'_R)$. Since the collision kernel $A$ is smooth, $R_A$ is also of class $I^{-\nnn/4}( U, \PP M \times \PP M , \Lambda'_R)$. %belongs to the same class of Fourier integral operators as $R$.~\footnote{\tbl{We haven't shown that $R$ is a Fourier integral operator. Move this sentence later.}}
 %
By Lemma \ref{Lambda_R-lemma}, %(see Appendix \ref{appendix-al}), 
the Lagrangian manifold $\Lambda_R$ is given by
\begin{align*}%\label{uuUUU90777}
\Lambda_R = \{ %(x,y,z, p,q\, ; \, \xi^x, \xi^y , \xi^z, \xi^p,\xi^{q} )
\big(x, y, z,p, q \, ; \, \xi^x, \xi^y, \xi^z,\xi^p,\xi^{q} \big) \in \  & T^*(U \times \PP U \times  \PP U) \setminus \{0\}  : \\
%&  \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad <--- please use & to avoid this --Antti
& \xi^x + \xi^y +\xi^z = 0 , \ \xi^p = \xi^{q} = 0, \ x=y=z  \}.
\end{align*}
%\[
%\Lambda_R = \{ (x,y,z, p,q\, ; \, \xi^x, \xi^y , \xi^z, \xi^p,\xi^{q} )  :\, x=y=z, \ \xi^x + \xi^y +\xi^z = 0 , \ \xi^p = \xi^{q} = 0  \} .
%\]
%
Further, we have that $WF'(R_A) \subset \Lambda_R'$, where $\Lambda_R'$ equals by its definition~\eqref{relation_defn} the set %in~\eqref{lambda_R_prime}
\begin{align}\label{hauska12221}%\label{lambda_R_prime}
\Lambda_R' %= \{ (x,y,z, p,q\, ; \, \xi^x, \xi^y , \xi^z, \xi^p,\xi^{q} )  : x=y=z, \ \xi^x + \xi^y +\xi^z = 0 , \ \xi^p = \xi^{q} = 0  \} \\
  =\{ \big((x ; \xi^x), (y, z,p, q \, ; \, \xi^y, \xi^z,\xi^p,\xi^{q} )\big) & \in \  T^*U \times T^* ( \PP U \times  \PP U) \setminus \{0\}   : \nonumber  \\
 %&  \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad %%<--- please use & to avoid this --Antti
 & \xi^x =\xi^y+ \xi^z \neq 0, \
   \xi^p =  \xi^{q} =0 , \ 
    x=y=z \}.
\end{align}


% 
% \begin{align}%\label{hauska12221}
% %\resizebox{0.91\hsize}{!}{$
% %\Lambda'_R= \{ ((x ; \xi^x), (y, z,q, p' \ ; \ \xi^y, \xi^z,\xi^q,\xi^{p'} )) \in T^*(U) \times T^* ( \PP(U) \times  \PP(U)) \setminus \{0\}   : \xi^x =\xi^y+ \xi^z \neq 0, \ \xi^p = 0, \  \xi^{q} =0 , \  x=y=z \} 
% %$%
% %}%
% %\begin{split}
% %%\begin{split}
%   \{ \big((x ; \xi^x), (y, z,p, q \, ; \, \xi^y, \xi^z,\xi^p,\xi^{q} )\big) \in \ &T^*U \times T^* ( \PP U \times  \PP U) \setminus \{0\}   : \nonumber  \\
%  & \xi^x =\xi^y+ \xi^z \neq 0, \
%    \xi^p =  \xi^{q} =0 , \ 
%     x=y=z \}.
%  %\end{split}
% \end{align}
%(c.f. the expression in ~\eqref{relation_defn}).
%\]
%where the relation satisfies
%of order $0$~\footnote{Define order here, or define in the intro and refer there. This needs some details still.} with relation % (by definition~\cite{})
% \[
% \begin{split}
% \Lambda'_R &\subset T^* (U) \times T^* ( \PP U \times \PP U) \setminus \{0\} ,
% %\quad  \Lambda'_F = \{ ((x,p\  ; \ \xi), (z,w,p',q' \ ; \ \eta)) : (x,z,w,p,p',q' \ ; \ \xi, -\eta))\in \Lambda'_F \} 
% %&\approx ( T^* U \times T^* \R^{\nnn} )\times( T^* U^3 \times T^* \R^{3\nnn}),
% \end{split}
% \]
%defined by (\ref{relationss}), 
%and has the coordinate form 

 

Now we show % (such as that contained in \cite{duistermaat2010fourier}),
%we next show 
that $\COLOP_{gain}^P [\ccdot, \ccdot]$ can be extended to the set of compactly supported conormal distributions $I^{m_1}_{comp} (N^* Y_1 )\times I^{m_2}_{comp} (N^* Y_2 )$, for $m_1,m_2\in \R$. In fact, by \cite[Corollary 1.3.8]{duistermaat2010fourier}, it is sufficient to demonstrate that 
\begin{equation}\label{intersection_of_wavefronts_empty}
WF_{\PP M \times \PP M}'(R_A)\cap WF(f_1 \otimes f_2)=\emptyset.
\end{equation}
% 
% the composition $R_A \circ( f_1 \otimes f_2)$ is well-defined 
% 
for $(f_1,f_2)\in I^{m_1}_{comp} (N^* Y_1 )\times I^{m_2}_{comp} (N^* Y_2 )$. 
%Note that $WF_{\PP M \times \PP M}'(R_A) = WF_{\PP M \times \PP M}'(R)$ since the collision kernel $A$ is smooth.  
%
%We check that the required conditions in \cite[Corollary 1.3.8]{duistermaat2010fourier} on the respective wavefront sets associated to the operators $R_A$ and $( f_1 \otimes f_2)$ are satisfied. First we will show that $WF_{\PP M \times \PP M}'(R_A)$ does not meet the wave front set $WF(f_1 \otimes f_2) $.
% % % 
% % % The wavefront set of $F$ is denoted by $WF'(F)$ and is the set
% % % \begin{align}
% % % WF'(F)&=\{(x,\xi^x,y,\xi^y)\in (T^*X\times T^*Y)\setminus \{0\} \,:\, (x,y,\xi^x,-\xi^y)\in WF(G)\},\label{wf_set_fio}
% % % \end{align}
% % % where $WF(G)$ is the wavefront set of the distribution kernel  $G$ of $F$. We also define the restricted wavefront sets of $F$ as 
% % % \begin{align}
% % % WF'_X(F)&= \{(x,\xi^x)\in (T^*X)\setminus \{0\} \,:\, (x,y,\xi^x,0)\in WF(G)\},\label{wf_set_fio_image}\\
% % % %
% % % WF'_Y(F)&= \{(y,\xi^y)\in (T^*Y)\setminus \{0\} \,:\, (x,y,0,\xi^y)\in WF(G)\}\label{wf_set_fio_domain}.
% % % \end{align}
%
Since the wavefront set of $f_j \in I^m(N^* Y_j)$, $j=1,2$ is contained in $N^* Y_j$, we have by \cite[Proposition 1.3.5]{duistermaat2010fourier} that the wavefront set of the tensor product $f_1 \otimes f_2$ satisfies 
\[
WF(f_1 \otimes f_2) \subset (N^* Y_1 \times \{0\}_{\PP M }) \cup (\{0\}_{\PP M} \times N^*Y_2) \cup (N^*Y_1 \times N^*Y_2 ),
\]
where $\{0\}_{\PP M} \subset T^* (\PP M)$ is the zero bundle over $\PP M$. 
%Notice that in the above, the right hand side is a union of closed cones in $TTM$, and thus a closed cone itself.<----UNION OF CLOSED IS NOT NECESSARILY CLOSED --Antti
 By using the fact that $WF(k_R)\subset \Lambda_R$ and the equation~\eqref{hauska12221}, the set $WF_{\PP M \times \PP M}'(R) \subset  T^* ( \PP U \times  \PP U) \setminus \{0 \} $, defined in~\eqref{wf_set_fio_domain}, satisfies
\begin{align}\label{restricted_WF_calc}
 WF_{\PP M \times \PP M}'(R) &= \{ (y,z, p, q \; \xi^y, \xi^z,\xi^p,\xi^{q})\in T^*(\PP M\times \PP M)\setminus \{0\}:  \nonumber \\ 
&\qquad\quad \text{ there is }
%\text{there exists} \
x \in  U
\text{ such that } \big((x\;0), (y,z, p, q \; \xi^y, \xi^z,\xi^p,\xi^{q}) \big) \in WF(k_R) \} \nonumber
\\
& \subset \{ (x,x,p, q \; \xi^y, -\xi^y,0,0)\in T^*(\PP M\times \PP M)\setminus \{0\} :  p,q \in \PP_x U, \  \xi^y \in \R^\nnn \setminus \{0 \} \}.%,\\
%&=:\mathcal{V}.
\end{align}
%Here we used~\eqref{hauska12221} and the definition of the wavefront set~\cite[eq. (1.3.19)]{duistermaat2010fourier}~\footnote{\tbl{Place definitions of the wavefront sets in preliminarie section.}}
Since $Y_1$ and $Y_2$ satisfy Definition \ref{intersection_coords}, pairs of elements in the fibers of $N^*Y_1$ and $N^*Y_2$ are linearly independent. They are also non-zero by the definition of a normal bundle. Thus an element of $N^*Y_1\times N^*Y_2$ cannot be of the form $(x,x, p, q \; \xi^y, -\xi^y,0,0)$.
%unless $\xi^y=0$. %%%<-- which is also impossible as zero does not belong to the normal bundle --Antti.
 We deduce that $WF_{\PP M \times \PP M }'(R) \cap (N^*Y_1 \times N^*Y_2 )= \emptyset$. By a similar consideration, we see that the set in~\eqref{restricted_WF_calc} does not intersect $(N^* Y_1 \times \{0\}_{\PP M}) \cup (\{0\}_{\PP M} \times N^*Y_2 )$. In particular, we have~\eqref{intersection_of_wavefronts_empty}. % that the wavefront set 
% \begin{equation}\label{intersection_of_wavefronts_empty}
% WF(f_1 \otimes f_2)\cap WF_{\PP M \times \PP M}'(R)=\emptyset.
% \end{equation}
%
%
% % % % 
% % % % 
% % % % \begin{lemma}\label{Lambda_R-lemma}
% % % % Let $U$ be an open subset of a smooth Lorentzian manifold $(M,g)$ and let \[\Lambda_R =   N^* ( \bigcup_{x\in U}  \{ x\} \times  \PP_xU \times \PP_xU  ).\]
% % % % We identify $T^*(U \times  \PP U  \times \PP U )$ locally as a subset of $(U^3 \times \R^{2\nnn} ) \times \R^{5\nnn} $ by using canonical coordinates. In these canonical coordinates,
% % % % %In canonical coordinates of $T^*(U \times  \PP(U) \times \PP(U) )$, identified as a subset of $(U^3 \times \R^{2\nnn} ) \times \R^{5\nnn} $, 
% % % % the submanifold $\Lambda_R$ of $T^*( M \times \PP U \times \PP U) \setminus \{0 \}$ equals the set
% % % % \begin{equation*}%\label{uuUUU90777}
% % % % \Lambda_R = \{ (x,y,z, p,q\ ; \ \xi^x, \xi^y , \xi^z, \xi^p,\xi^{q} )  : x=y=z, \ \xi^x + \xi^y +\xi^z = 0 , \ \xi^p = \xi^{q} = 0  \} .
% % % % \end{equation*}
% % % % % Let $U$ be an open subset of a smooth Lorentzian manifold $(M,g)$ and let \[\Lambda_R =   N^* ( \bigcup_{x\in U}  \{ x\} \times  \PP_xU \times \PP_xU  ).\]
% % % % % In canonical coordinates of $T^*(U \times  \PP(U) \times \PP(U) )$, identified as a subset of $(U^3 \times \R^{2\nnn} ) \times \R^{5\nnn} $, the submanifold $\Lambda_R$ of $T^*( M \times \PP U \times \PP U) \setminus \{0 \}$ equals the set
% % % % % \begin{equation}\label{uuUUU90777}
% % % % % \Lambda_R = \{ (x,y,z, p,q\ ; \ \xi^x, \xi^y , \xi^z, \xi^p,\xi^{q} )  : x=y=z, \ \xi^x + \xi^y +\xi^z = 0 , \ \xi^p = \xi^{q} = 0  \} .
% % % % % \end{equation}
% % % % \end{lemma}
% % % % \begin{lemma}\label{dimension-transverse-lemma}
% % % % The spaces $\Lambda'_R \times ( N^*Y_1 \times  N^*Y_2 ) $ and $T^*U \times \text{diag}\, T^*( \PP M \times \PP M) $ intersect transversally in $T^*U \times T^*(\PP M \times \PP M) \times  T^*(\PP M \times \PP M)$.
% % % % \end{lemma}
% % % % 
% % % % \begin{proof}
% % % % Recall that for any linear subspaces $L_1,L_2$ of a finite dimensional real vector space,
% % % % \begin{equation}\label{jksadss}
% % % % \dim (L_1 + L_2) = \dim L_1 + \dim L_2 - \dim (L_1 \cap L_2).
% % % % \end{equation}
% % % % In particular, if this gives the dimension of the underlying vector space then the subspaces intersect transversally. 
% % % % The local expression (\ref{hauska12221}) and coordinates (\ref{turhautuminen1}) imply that the space
% % % % \[
% % % % (\Lambda'_R \times (  N^*Y_1 \times  N^*Y_2) ) \cap (T^*U \times \textrm{diag}\,T^*( \PP M \times \PP M) )
% % % % \]
% % % % equals in the associated canonical coordinates $((x,\xi)(y,z,q,p'; \xi^y,\xi^z, \xi^q,\xi^{p'}))$ the punctured $\nnn$-dimensional plane
% % % % \[
% % % % L:= \big\{ ( (0;\xi^x  ) , \text{diag} (0,0, e_1, e_2 ; \xi^x_1,\dots \xi^x_d, 0, \dots, 0 ,\xi_{d+1}^x ,\dots, \xi^x_\nnn ,0,\dots,0 ) ) : \xi^x \in \R^\nnn \setminus \{0 \} \big\}  
% % % % \]
% % % % where  and $e_1 := (0,\dots,0,1,0,\dots,0) \in \R^\nnn$ and $e_2 := (1,\dots,0)\in \R^\nnn$. In particular, it is a manifold and 
% % % % \[
% % % % \begin{split}
% % % % \dim ( \Lambda'_R \times ( N^*Y_1 \times  N^*Y_2) ) + \dim (T^*(U) \times \text{diag} T^*( \PP M \times \PP M) ) - \dim L \\
% % % % = 9 \nnn  + 10 \nnn - \nnn = 18\nnn = \dim ( T^*U \times T^*(\PP M \times \PP M) \times  T^*(\PP M \times \PP M) )
% % % % \end{split}
% % % % \]
% % % % from which we obtain the claim by applying (\ref{jksadss}) to  tangent spaces. 
% % % % 
% % % % \end{proof}
% % % % 
% % % % \begin{lemma}\label{tensorlemma}
% % % % Let $f_j  \in  I^{m_j} (N^* Y_j )$, $j=1,2$. Then,
% % % % \[
% % % % \begin{split}
% % % % f_1 \otimes f_2 \in I^{m_1+m_2 + \nnn,  -m_2- \nnn} \big( N^* Y_1  \times \{ 0 \}_{\PP} , N^* Y_1  \times N^* Y_2   \big) \\
% % % %  +  I^{m_1+m_2+ \nnn, -m_1-\nnn} \big( \{ 0 \}_{\PP} \times N^* Y_2  , N^* Y_1  \times N^* Y_2   \big) 
% % % % %+ I^{\tilde\mu,\mu} \big(  \PP \times K_{M_2}  ,  K_{M_1}  \times K_{M_2}   \big)
% % % % \end{split}
% % % % \]
% % % %  in the sense of \cite{greenleaf-uhlmann} (cf. \cite{guillemin1981,melrose-uhlmann1979}).\footnote{\tbl{Add these comormal spaces to the preliminary section.}}
% % % %  \end{lemma}
% % % %  We prove this lemma in Appendix \ref{appendix-al}.
% % % % 
% % % % % We will next consider submanifolds $Y_1$ and $Y_2$ of $\overline{\PP} M$ intersecting transversally. If $(x_0,p_0)$ is in the intersection of $Y_1$ and $Y_2$, there is an open neighbourhood $U$ of $x_0$ and coordinates $x$~\footnote{\tbl{Check this and clean.}} %on $U$ with the following properties:
% % % % % \begin{equation}\label{x_splits}
% % % % % x = (x',x'') : U \rightarrow \R^\nnn, \quad x' = (x^1,\dots,x^d), \quad x''=(x^{d+1}, \dots, x^\nnn)
% % % % % \end{equation}
% % % % % % on some neighbourhood 
% % % % % such that
% % % % % \begin{equation}\label{turhautuminen1}
% % % % % \begin{split}
% % % % % Y_1 \cap TU &= \{ (x,p)   \in TU  : x' = 0  , \ p' = 0,  \ p'' = (1,0,\dots,0)  \}  \\
% % % % % Y_2 \cap TU &= \{  (x,p) \in TU : x'' = 0, \ p''= 0, \  p' = (1,0,\dots,0) \}
% % % % % %\\ \quad d &=  \dim K_{M_2} = \nnn -  \dim K_{M_1}.
% % % % % \end{split}
% % % % % \end{equation}
% % % % % in the associated canonical coordinates $(x,p) = (x',x'',p',p'')$ of $TU$. 
% % % % % 
% % % % % ÂŽintersect transversally, if $ is an intersection point there are coordinates $x$ on an We introduce some notation. Let $(U,x)$ be coordinate neighbourhood of $M$. The
% % % % %  
% % % % We extend $\COLOP_{gain}^P$ to conormal distributions as follows. % captured in the following proposition.
% % % % 
% % % % %To avoid dealing with operators on a manifold with boundary we would like to extend the operator $\COLOP_{gain}[ \ \cdot \ , \ \cdot \ ] (x,p)$ for fixed variable $p \in \OVS$. 
% % % % %However, this  creates a slight technical issue since the domain of $p = F(x)$ now depends on the base point $x$. We circumvent this problem by employing local coordinates, where we can identify $T_xM = \R^n$. Fixing $p \in \R^n$ then corresponds to a smooth local section $x \mapsto (x, p^\alpha \partial_\alpha |_x)$ in the bundle $\pi: \OVS \rightarrow \R \times N$. Motivated by this, we proof the following:
% % % % 
% % % % \begin{proposition}\label{sofisti}   
% % % % Let $(M,g)$ be a geodesically complete,~\footnote{\tbl{Do we use completeness smoewhere?}} globally hyperbolic Lorentzian manifold.  
% % % % Let $Y_1,\, Y_2 \subset  \overline{\PP} M\subset TM$,
% % % % %S^{r_j}_{t_j}$, $t_j \in \R$, $r_j > 0$ , $j=1,2$  
% % % % be smooth submanifolds that satisfy Property \ref{intersection_coords} . Let $(x_0,p_0)\in Y_1\cap Y_2$ and adopt the notation in Propoerty~\ref{intersection_coords}. Let also $m_1,\,m_2\in \R$. %By using the coordinates~\eqref{x_splits},~\eqref{turhautuminen1} % that 
% % % % %for each $x_0 \in \text{supp} ( x \mapsto A(x,\cdot,\cdot,\cdot , \cdot) ) \cap G_{M_1} \cap G_{M_2}$ 
% % % % %there is an open neighbourhood $ U \subset M$ and local coordinates 
% % % % % \[
% % % % % x = (x',x'') : U \rightarrow \R^\nnn, \quad x' = (x^1,\dots,x^d), \quad x''=(x^{d+1}, \dots, x^\nnn)
% % % % % \]
% % % % % % on some neighbourhood 
% % % % % satisfying~\footnote{\tbl{Does this exactly mean that $Y_1$ and $Y_2$ intersect transversally (on $U$)? If so we could put it into a lemma.}}
% % % % % \begin{equation}\label{turhautuminen1}
% % % % % \begin{split}
% % % % % Y_1 \cap TU &= \{ (x,p)   \in TU  : x' = 0  , \ p' = 0,  \ p'' = (1,0,\dots,0)  \}  \\
% % % % % Y_2 \cap TU &= \{  (x,p) \in TU : x'' = 0, \ p''= 0, \  p' = (1,0,\dots,0) \}  , 
% % % % % %\\ \quad d &=  \dim K_{M_2} = \nnn -  \dim K_{M_1}.
% % % % % \end{split}
% % % % % \end{equation}
% % % % % in the associated canonical coordinates $(x,p) = (x',x'',p',p'')$ of $TU$. 
% % % % %Using the coordinates $(x,p)$, 
% % % % % define the conic Lagrangian submanifolds 
% % % % % \[
% % % % % \Lambda_0 := T_{0}^* \R^\nnn, \quad \Lambda_1 := N^*  \{ x   \in U  : x' = 0  \} \quad \text{and} \quad \Lambda_2 := N^*  \{ x   \in U  : x'' = 0  \}. 
% % % % % \]
% % % % 
% % % % Let $F$  be a smooth local section of the bundle $\pi: \overline{\mathcal{P}}U \rightarrow U$. %, that is, a smooth function $F : U \rightarrow \overline{\mathcal{P}} U$ such that $\pi \circ F(x) = x$. %That is, in 
% % % % Let $\COLOP$ be the collision operator with an admissible kernel.
% % % % The operator $\COLOP_{gain}^P: C_c^\infty (\overline{\mathcal{P}} M ) \times C_c^\infty (\overline{\mathcal{P}}M ) \rightarrow C^\infty ( U )$ defined in~\eqref{def_of_QF}
% % % % % \begin{align*}
% % % % % \COLOP_{gain}  [h_1,h_2]_F (x) :=\COLOP_{gain} [h_1,h_2] (x ,p(x) ), 
% % % % % \end{align*}
% % % % %given by
% % % % %\[
% % % % %\COLOP_{gain}  [h_1,h_2]_F (x) =\COLOP_{gain} [h_1,h_2] (x ,p(x) ) 
% % % % %\]
% % % % extends into a continuous map
% % % % \[
% % % %  I^{m_1}_{comp} (  N^*Y_1 ;\, \overline{\mathcal{P}} M  )\times I^{m_2}_{comp} ( N^*Y_2 ; \, \overline{\mathcal{P}} M ) \rightarrow \mathcal{D}' (U). 
% % % %  % I^{m_2-\nnn/4,m_1+ \nnn/2} (  \Lambda_0, \NG_{M_1} ,   ; U )+I^{m_1-\nnn/4,m_2 + \nnn/2} ( \Lambda_0,  \NG_{M_2}  ;  U  )
% % % % \]
% % % % 
% % % % Let $(f_1 , f_2) \in I^{m_1}_{comp} (  N^*Y_1 ;\, \overline{\mathcal{P}} M  )\times I^{m_2}_{comp} ( N^*Y_2 ; \, \overline{\mathcal{P}} M )$.
% % % % We have that
% % % % \[
% % % % WF(\COLOP_{gain}^P[f_1,f_2]) \subset \Lambda_0 \cup \Lambda_{1} \cup \Lambda_{2}
% % % % %\end{split}
% % % % \]
% % % % %where the product type symbol class is defined in the sense of \cite{guillemin1981}.
% % % % and, microlocally away from $\Lambda_{1} \cup \Lambda_{2} $, we have that~\footnote{\tbl{Define microlocally away}} 
% % % % %\begin{align}
% % % % \[
% % % % \COLOP_{gain}^P [f_1,f_2]\in I^{m_1+m_2+3\nnn/4} (\Lambda_0 \setminus( \Lambda_{1} \cup \Lambda_{2}) ;\,U ).
% % % % \]
% % % % %for every $(f_1 , f_2) \in I^{m_1}_{comp} (  N^*Y_1 ; \overline{\mathcal{P}} M  )\times I^{m_2}_{comp} ( N^*Y_2 ;  \overline{\mathcal{P}} M )$.
% % % % \end{proposition}
% % % % 
% % % % 
% % % % %\subsection{Proof of Proposition \ref{sofisti}}
% % % %  
% % % % 
% % % % %
% % % % %
% % % % %
% % % % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % %
% % % % % Theorem for Q[X^{-1} . , X^{-1} . ](x, F(x))
% % % % %
% % % % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % %
% % % % %
% % % % %
% % % % 
% % % % 
% % % % \begin{proof}[Proof of Proposition \ref{sofisti}]
% % % % %Let us  now continue to the proof of Proposition \ref{sofisti}. 
% % % % Let us denote $I^m ( \Lambda   ; \PP M ) = I^m(\Lambda)$ for a Lagrangian manifold $\Lambda \subset T^* (\PP M)$ and $m \in \R$. 
% % % % To prove the claims of the proposition, %that $\COLOP_{gain}^P [ f_1,f_2 ]$ can be extended to compactly supported conormal distributions $f_j  \in  I^{m_j}_{comp} (N^* Y_j )$, $j=1,2$, and that the extension has the claimed properties, 
% % % % we first represent $\COLOP_{gain}^P [ \ccdot,\ccdot ]$ as a composition of Fourier integral operators. Then we appeal to standard results for Fourier integral operators in~\cite{duistermaat2010fourier} to finish the proof. %in particular to \cite[Theorem 2.4.1]{duistermaat2010fourier} and  \cite[Corollary 1.3.8]{duistermaat2010fourier}. 
% % % % The bulk of the proof consists of demonstrating that the corresponding Fourier integral operators satisfy the intersection and mapping conditions of \cite[Theorem 2.4.1]{duistermaat2010fourier} and  \cite[Corollary 1.3.8]{duistermaat2010fourier}.
% % % % 
% % % % %{\color{gray}Before we begin, we remark that the shorthand notation $\PP:= \PP U$ is used extensively in this proof.} {\color{red}($\leftarrow$ Lets not do this. Too dangerous notation.)}
% % % % 
% % % % 
% % % % Let $(x_0,p_0)\in Y_1\cap Y_2$ and $(U,x)$ as in the statement. %be a coordinates described in~\eqref{x_splits} and \eqref{turhautuminen1}. 
% % % %  Let us define an % Fourier 
% % % %  integral operator 
% % % % \[
% % % % R : C^\infty_c  ( \PP M  \times \PP M  ) \rightarrow \mathcal{D}' ( U  )
% % % % \]
% % % % by the formula%~\footnote{Need to choose one domain for $\delta_\Sigma$. The notation is funny, because not it looks like a pairing of $\phi$. I'd recommend $\delta_\Sigma[\phi]$. Also, I guess the target of $\Delta_\Sigma$ can be taken to be smooth functions.}
% % % % \[
% % % % \begin{split}
% % % % %\langle \delta_\Sigma ( x,p \, ; \,\cdot\,  ) ,  \phi \rangle = \int_{\Sigma_{x,p}} \phi (y,z,w,q,p',q')\, dV (y,z,w,q,p',q'), \ \phi \in C^\infty_c ( \mathcal{S}^3 ).
% % % % %\langle \delta_\Sigma ( x,p \, ; \,\cdot\,  ) ,  \phi \rangle  
% % % % \langle R [\phi] , \psi \rangle =&  \int_{  \PP U \oplus \PP U } \phi ( x, p' , x , q') \psi(x) \, dv (x,p',q') \\
% % % % %= & \int_{\Sigma} \psi(x,p)  \phi (z,p',w,q') \, d\Sigma
% % % % %V (y,z,w,q,p',q').%, \ \phi \in C^\infty_c ( \mathcal{S}^3 ).
% % % % \end{split}
% % % % \]
% % % % %where $(x,p) \mapsto dV_{x,p}$ is a volume form on $T_{(x,x)} ( \R \times N)^2$
% % % % where $dv$ is a volume form on the direct sum bundle $\PP U \oplus \PP U := \{ \big((x,p) (y,q) \big) \in \PP U \times \PP U : x = y \}$ induced by the volume form on $\PP U$, and where $\phi\in C^\infty_c  ( \PP M  \times \PP M  )$ and $\psi\in C_c^\infty(U)$. %Since $R$ is intgration over a submanifold of $\PP M \times \PP M$, we have that $R\in I^{-\nnn/4}( U, \PP M \times \PP M , \Lambda'_R)$.
% % % % 
% % % % % and $d\Sigma$~\footnote{Make precise later. Check Choque-Bruhat.} is the induced volume form on 
% % % % %\[
% % % % %\Sigma_{x,p} := \{ \vec{p} \in \{ (x,p) \} \times T(\R \times N)^3 : x= y=z=w  , \quad q  + p = p'+q'  \}.
% % % % %% \quad \text{ ($(x,p)$ fixed) }
% % % % %\]
% % % % %
% % % % %Then $\delta_\Sigma$ is a Fourier integral operator with kernel is the delta function $\Sigma$ 
% % % % %Here the notation $\Sigma$ refers to the set defined in~\eqref{Sigma_union} as
% % % % %The notation refers to the manifold
% % % % %\begin{align}%\label{def_sigma}
% % % % % \Sigma&:=\bigcup_{(x,p)\in T(\R \times N)} \Sigma_{x,p} =\{\,\vec{p}\in T(\R\times N)^4:\, x=y=z=w, \  p + q = p' + q' \}.\nonumber
% % % % %\end{align}
% % % % %from the definition of the collision operator. 
% % % % Let $F$ be a smooth local section of the bundle $\pi: \overline{\mathcal{P}}U \rightarrow U$ and let $A$ be the collision kernel of $\COLOP$. We represent $F$ as $F(x)=(x,p(x))$ by using the coordinates $x$. Let us then consider the operator~\footnote{\tbl{This is just a kernel. We need to specify which variables will be integrated, i.e. where does the operator act.}}
% % % % \[
% % % %  \langle R_A [\phi] , \psi \rangle = \int_{  \PP U \oplus \PP U } A(x,p(x),\, p'+q' - p(x) ,\, p',\,q')\phi ( x, p' , x , q' ) \psi(x) \, dv (x,p',q') 
% % % % \]
% % % % % 
% % % % % 
% % % % % \[
% % % % % R_A (x \, ; \, z,p',w,q') := 
% % % % % %\bigg( \int_{L^+_x(\R \times N)} A(x,p , p'+q' - p , p',q') dw_x(p) \bigg) \cdot R (x \ ;  z,p',w,q') 
% % % % % A(x,p(x),\, p'+q' - p(x) ,\, p',\,q') \cdot R (x \, ;\,  z,p',w,q'). 
% % % % % \]
% % % % %Here the symbol $\cdot$ refers to multiplication by a smooth function. 
% % % % Notice next that
% % % % \begin{equation}\label{uusi7878782}
% % % % %R_A (x \, ;  \, z,p',w,q') [ h_1 (z,p')  h_2(w,q') ] 
% % % % R_A[h_1\,h_2]= 
% % % % %\pi_{L^+}^* 
% % % % \COLOP_{gain}^P [h_1,h_2] , \quad h_1,h_2 \in C_c^\infty( \PP M ).
% % % % \end{equation}
% % % % Here $h_1\,h_2$ is just the product of $h_1$ and $h_2$.
% % % % %for volume forms $dw_x$ and $dv$ such that $dw_x \wedge dv$ corresponds to the volume form in the definition of the collision operator under the parametrization
% % % % %of $\Sigma$ by variables $(x,p,q',p') \mapsto (x,p, p'+q'-p,p' ,q') \in \Sigma$.  
% % % % %Above
% % % % %Where the symbol $\cdot$ refers to multiplication by a smooth function. 
% % % % %Notice that the choice of volume form does not affect to microlocal properties since each volume form differs from others by multiplication of positive smooth function. 
% % % % 
% % % % The kernel associated to the operator $R $ is
% % % % %has the associated  kernel 
% % % % \[
% % % % k_R  \in \mathcal{D}' ( U \times  \PP M \times \PP M )  , \quad 
% % % % \langle  k_R  , \tilde{\phi}  \rangle :=  \int_{  \PP U \oplus \PP U } \tilde{\phi} (x, x, p,x,q ) dv (x,p,q) , 
% % % % \]
% % % % where $\tilde{\phi} \in C^\infty_c ( U \times  \PP M \times \PP M)$. 
% % % % %The kernel is  a conormal distribution of class 
% % % % The kernel $k_R$ can be viewed as a conormal distribution (cf. Section~\ref{lagrangian-dist})~\footnote{\tbl{Proof?}} 
% % % % \begin{align*}
% % % % k_R &\in  I^{-\nnn/4 }(  \Lambda_R ;\,  U  \times  \PP M \times \PP M  ), \\
% % % % \Lambda_R &=   N^* \Big( \bigcup_{x\in U}  \{ x\} \times  \PP_x M \times \PP_x M \Big).
% % % % \end{align*}
% % % % Hence $R$ is a Fourier integral operator %of order $-\nnn/2$ in the sense that
% % % % %\[
% % % %  of class $I^{-\nnn/4}( U, \PP M \times \PP M , \Lambda'_R)$. Since the collision kernel $A$ is smooth, $R_A$ is also of class $I^{-\nnn/4}( U, \PP M \times \PP M , \Lambda'_R)$. %belongs to the same class of Fourier integral operators as $R$.~\footnote{\tbl{We haven't shown that $R$ is a Fourier integral operator. Move this sentence later.}}
% % % %  
% % % % By Lemma \ref{Lambda_R-lemma}, %(see Appendix \ref{appendix-al}), 
% % % % the Lagranian manifold $\Lambda_R$ has the local coordinate expression 
% % % % \[
% % % % \Lambda_R = \{ (x,y,z, p,q\, ; \, \xi^x, \xi^y , \xi^z, \xi^p,\xi^{q} )  :\, x=y=z, \ \xi^x + \xi^y +\xi^z = 0 , \ \xi^p = \xi^{q} = 0  \} .
% % % % \]
% % % % 
% % % % Further, we have that $WF'(R_A) \subset \Lambda_R'$, where locally $\Lambda_R'$ is by definition (see~\eqref{relation_defn}) the set
% % % % \begin{align}\label{hauska12221}
% % % % %\resizebox{0.91\hsize}{!}{$
% % % % %\Lambda'_R= \{ ((x ; \xi^x), (y, z,q, p' \ ; \ \xi^y, \xi^z,\xi^q,\xi^{p'} )) \in T^*(U) \times T^* ( \PP(U) \times  \PP(U)) \setminus \{0\}   : \xi^x =\xi^y+ \xi^z \neq 0, \ \xi^p = 0, \  \xi^{q} =0 , \  x=y=z \} 
% % % % %$%
% % % % %}%
% % % % %\begin{split}
% % % % %%\begin{split}
% % % %   \{ \big((x ; \xi^x), (y, z,p, q \, ; \, \xi^y, \xi^z,\xi^p,\xi^{q} )\big) \in \ &T^*U \times T^* ( \PP U \times  \PP U) \setminus \{0\}   : \nonumber  \\
% % % %  & \xi^x =\xi^y+ \xi^z \neq 0, \
% % % %    \xi^p =  \xi^{q} =0 , \ 
% % % %     x=y=z \}.
% % % %  %\end{split}
% % % % \end{align}
% % % % %(c.f. the expression in ~\eqref{relation_defn}).
% % % % %\]
% % % % %where the relation satisfies
% % % % %of order $0$~\footnote{Define order here, or define in the intro and refer there. This needs some details still.} with relation % (by definition~\cite{})
% % % % % \[
% % % % % \begin{split}
% % % % % \Lambda'_R &\subset T^* (U) \times T^* ( \PP U \times \PP U) \setminus \{0\} ,
% % % % % %\quad  \Lambda'_F = \{ ((x,p\  ; \ \xi), (z,w,p',q' \ ; \ \eta)) : (x,z,w,p,p',q' \ ; \ \xi, -\eta))\in \Lambda'_F \} 
% % % % % %&\approx ( T^* U \times T^* \R^{\nnn} )\times( T^* U^3 \times T^* \R^{3\nnn}),
% % % % % \end{split}
% % % % % \]
% % % % %defined by (\ref{relationss}), 
% % % % %and has the coordinate form 
% % % % 
% % % %  
% % % % 
% % % % Now we show % (such as that contained in \cite{duistermaat2010fourier}),
% % % % %we next show 
% % % % that $\COLOP_{gain}^P [\ccdot, \ccdot]$ can be extended to the set of compactly supported conormal distributions $I^{m_1}_{comp} (N^* Y_1 )\times I^{m_2}_{comp} (N^* Y_2 )$, for $m_1,m_2\in \R$. In fact, by \cite[Corollary 1.3.8]{duistermaat2010fourier}, it is sufficient to demonstrate that the composition $R_A \circ( f_1 \otimes f_2)$ is well-defined for $(f_1,f_2)\in I^{m_1}_{comp} (N^* Y_1 )\times I^{m_2}_{comp} (N^* Y_2 )$. 
% % % % 
% % % % We check that the required conditions in \cite[Corollary 1.3.8]{duistermaat2010fourier} on the respective wavefront sets associated to the operators $R_A$ and $( f_1 \otimes f_2)$ are satisfied. First we will show that $WF_{\PP M \times \PP M}'(R_A)$ does not meet the wave front set $WF(f_1 \otimes f_2) $.
% % % % 
% % % % Since the wavefront set of $f\in I^m(\Lambda)$ is contained in $\Lambda$, by \cite[Proposition 1.3.5]{duistermaat2010fourier} we see that the wavefront set of the tensor product $f_1 \otimes f_2$ satisfies 
% % % % \[
% % % % WF(f_1 \otimes f_2) \subset (N^* Y_1 \times \{0\}_{\PP M }) \cup (\{0\}_{\PP M} \times N^*Y_2) \cup (N^*Y_1 \times N^*Y_2 ),
% % % % \]
% % % % where $\{0\}_{\PP M} \subset T^* (\PP M)$ is the zero bundle over $\PP M$. Notice that in the above, the right hand side is a union of closed cones in $TTM$, and thus a closed cone itself.
% % % % 
% % % %  Since $WF(k_R)\subset \Lambda_R$, the wavefront set $WF_{\PP M \times \PP M}'(R) \subset  T^* ( \PP U \times  \PP U) \setminus \{0 \} $ has a local expression which satisfies
% % % % \begin{align*}
% % % %  WF_{\PP M \times \PP M}'(R) &= \{ (y,z, q, p' ; \xi^y, \xi^z,\xi^q,\xi^{p'}):  \\ 
% % % % &\qquad\qquad\qquad \text{ there is }
% % % % %\text{there exists} \
% % % % x \in  U
% % % % \text{ such that } \big((x,0), (y,z, q, p' ; \xi^y, \xi^z,\xi^q,\xi^{p'}) \big) \in WF(k_R) \} 
% % % % \\
% % % % & \subset \{ (x,x, q, p' ; \xi^y, -\xi^y,0,0) :  (x,q,p') \in \PP U \oplus \PP U, \  \xi^y \in \R^\nnn \setminus \{0 \} \},\\
% % % % &=:\mathcal{V}.
% % % % \end{align*}
% % % % Here we used~\eqref{hauska12221} and the defintion of the wavefront set~\cite[eq. (1.3.19)]{duistermaat2010fourier}~\footnote{\tbl{Place definitions of the wavefront sets in preliminarie section.}}
% % % % 
% % % % Since $Y_1$ and $Y_2$ have the admissible intersection property, Property \ref{intersection_coords}, pairs of elements in the fibers of $N^*Y_1$ and $N^*Y_2$ are linearly independent. Thus an element of $N^*Y_1\times N^*Y_2$ cannot be of the form $(x,x, q, p' ; \xi^y, -\xi^y,0,0)$ unless $\xi^y=0$. We deduce that $WF_{\PP M \times \PP M }'(R) \cap (N^*Y_1 \times N^*Y_2 )= \emptyset$. Additionally, the set $\mathcal{V}$ does not intersect $(N^* Y_1 \times \{0\}_{\PP M}) \cup (\{0\}_{\PP M} \times N^*Y_2 )$. In particular, we have that the wavefront set 
% % % % \[
% % % % WF(f_1 \otimes f_2)\cap WF_{\PP M \times \PP M}'(R)=\emptyset.
% % % % \]
% % % % We also have $WF_{\PP M \times \PP M}'(R_A) = WF_{\PP M \times \PP M}'(R)$. 
%
%
%From ,
%~\footnote{\tbl{Place definitions of the wavefront sets in preliminarie section.}}
 %
 The  set $WF_{U}'(R) \subset  T^* U \setminus \{0 \}$, defined in~\eqref{wf_set_fio_image}, satisfies
%Since $WF(k_R)\subset \Lambda_R$ we have by definition~\cite[eq. (1.3.18)]{duistermaat2010fourier} that 
\begin{align*}
 WF_{U}'(R) &= \{ (x,\xi^x) \in T^*U: \,\text{ there is } \\ 
&\qquad\qquad
%\text{there exists} \
(y,p,z, q) \in  \PP U\times \PP U
\text{ such that } \big((x\; \xi^x), (y,z, p, q\, ;\, 0, 0,0,0) \big) \in WF(k_R) \}.
  \end{align*}
  By using the fact that $WF(k_R)\subset \Lambda_R$ and~\eqref{hauska12221}, we see that if $\big((x\; \xi^x), (y,z, p, q\, ;\, 0, 0,0,0) \big) \in WF(k_R)$, then $\xi^x=0$. 
%If $(x\; \xi^x)\in WF_{U}'(R)\neq \emptyset$, then $\xi^x$ in the brackets above must satisfy $\xi^x=-\xi^y-\xi^z=0$. But this implies $\xi^x=0$, which is a contradiction since $WF_{U}'(R)$ does not contain the zero vector by definition. 
Thus $WF_{U}'(R)= \emptyset$.
%
By \cite[Corollary 1.3.8]{duistermaat2010fourier} the composition $R_A \circ( f_1 \otimes f_2)$ is well defined and we obtain the desired continuous extension for $\COLOP_{gain}^P [ f_1,f_2 ] \in \mathcal{D}'(U)$.
%By \cite[Corollary 1.3.8]{duistermaat2010fourier} we obtain the desired continuous extension for $\COLOP_{gain}^P [ f_1,f_2 ] \in \mathcal{D}'(U)$.
The second claim of the proposition follows directly from \cite[Corollary 1.3.8]{duistermaat2010fourier} and the facts $WF_{U}'(R_A) \subset WF_U'(R)= \emptyset$ and $WF(R_A)\subset \Lambda_R'$: %we also achieve the second claim of the Proposition:
\begin{equation}\label{wave_front_calc_in_prop4}
WF ( \COLOP_{gain}^P [ f_1,f_2 ] ) \subset \Lambda_R' \circ  \Big( (N^* Y_1 \times \{0\}_{\PP M}) \cup (\{0\}_{\PP M} \times N^*Y_2) \cup (N^*Y_1\times N^*Y_2) \Big).
\end{equation}
%\tbl{stopped here.}


By using the coordinate description \eqref{hauska12221}, we show next that
\begin{equation}\label{lambda_composed_with_Y1}
 \Lambda'_R \circ (  N^*Y_1 \times \{0\}_{\tbl{ \PP M}}) = \Lambda_{1}, \quad \Lambda'_R \circ ( \{0\}_{\tbl{\PP M}} \times N^*Y_2) = \Lambda_{2}.
\end{equation}
 By definition (see \eqref{relation_of_composition}), we have that  %and by using local coordinates
\begin{align}\label{lambda_composed_with_Y2}
\Lambda'_R \circ (  N^*Y_1 \times \{0\}_{\tbl{ \PP M }})&=\{ (x,\xi^x)\in T^*U: \text{ such that } \big((x,\xi^x), (y,p \; \xi^y, \xi^p), (z,q \; \xi^z, \xi^q)\big)\in \Lambda_R' \nonumber \\
& \text{ where } (y,p \; \xi^y, \xi^p)\in N^*Y_1 \text{ and } \xi^z=\xi^q=0 \}.
\end{align}
By using~\eqref{hauska12221}, it follows that in the expression above, we must have that $(x,\xi^x)$ is any element of the form $(y,\xi^y)$, where $(y,p\; \xi^y, 0)\in N^*Y_1$ for some $p$.~\f{The condition $(\xi^x)''=0$ was indeed missing. Removed.}  Thus we have $\Lambda'_R \circ (  N^*Y_1 \times \{0\}_{\tbl{\PP M}}) = \Lambda_{1}$. We similarly have $\Lambda'_R \circ ( \{0\}_{\tbl{\PP M}} \times N^*Y_2) = \Lambda_{2}$. We have proven~\eqref{lambda_composed_with_Y1}.	

By using the coordinates $(x,p)=(x',x'',p',p'')$ we may also write any $(x,\xi)\in T^*U$ as $(x,\xi)=(x',x'',\xi',\xi'')$. %described in Property~\ref{intersection_coords}. By using the property of $Y_1$ and $Y_2$ and the coordinates in~\eqref{turhautuminen1} 
We have that  
%in canonical coordinates $(x,\xi^x) $,  $x = ( x^1,\dots,x^\nnn)$, 
%we may write
\begin{align*}
\Lambda_{1} &= \{ (x\;\xi)\in T^*U : x'=0, \ \xi''=0 \}, \\ % x^1=  \dots = x^d = 0, \ \xi_{d+1}^x = \dots = \xi_\nnn^x = 0 \} \\
\Lambda_{2} &= \{ (x\;\xi)\in T^*U : x''= 0, \ \xi'=0 \}.% \dots = x^\nnn = 0, \ \xi_{1}^x = \dots = \xi_d^x = 0 \}.
\end{align*}
We calculate similarly as in~\eqref{lambda_composed_with_Y2} 
\begin{align}\label{lambda_composed_with_Y3}
\Lambda'_R \circ (  N^*Y_1 \times N^*Y_2)&=\{ (x,\xi^y+\xi^z)\in T^*U: \text{ such that } \big((x,\xi^x), (x,p \; \xi^y, 0), (x,q \; \xi^z, 0)\big)\in \Lambda_R' \nonumber \\
& \quad\quad\quad \text{ where } (x,p \; \xi^y, 0)\in N^*Y_1 \text{ and } (x,q \; \xi^z, 0)\in N^*Y_2 \} \nonumber \\
%and therefore
%\[
% \Lambda'_R \circ (  N^*Y_1 \times N^* Y_2 ) 
 &= \{ (x', x'' \; \xi', \xi'')\in T^*U \setminus \{0 \} :  x'= x'' = 0 \} = \Lambda_0.
\end{align}
Here we used again~\eqref{hauska12221}.
By combining~\eqref{wave_front_calc_in_prop4},~\eqref{lambda_composed_with_Y2} and~\eqref{lambda_composed_with_Y3}, we have shown that 
\[
WF ( \COLOP_{gain}^P [ f_1,f_2 ]) \subset  \Lambda_0 \cup \Lambda_{1} \cup \Lambda_{2}. 
\]
%Lastly, we finish the proof by showing that the final claim of the proposition holds. 

We are left to show the last claims of the theorem. Fix arbitrary conic neighbourhoods $\Gamma_1,\Gamma_2$ of $\Lambda_1$ and $\Lambda_2 $, respectively. 
Let $\epsilon>0$ be small enough to satisfy
\begin{equation}\label{zskla}
   \Big\{ (x,\xi) \in T U :  \| x' \| < \epsilon , \    \|\xi''\| < \epsilon \|\xi' \| \Big\} \subset \Gamma_1 
\end{equation}
and
\[
\Big\{ (x,\xi) \in T U :   \| x'' \| < \epsilon , \|\xi' \|  < \epsilon \| \xi'' \|  \Big\} \subset \Gamma_2 .
\]
By multiplying the amplitude in the oscillatory integral representation of $f_1 \otimes f_2$ by
\[
1 = \phi + (1-\phi) , 
\]
where $\phi \in C^\infty( T^*( \PP M \times \PP M) \setminus \{0\} )$ is positively homogeneous of degree $0$ and equals $1$ near $N^*[Y_1 \times \PP M] = N^* Y_1 \times \{ 0 \}_{\PP M}$ and $0$ near $N^* [\PP M \times Y_2] = \{ 0 \}_{\PP M} \times N^* Y_2$,~\f{To Matti's question, I don't know.}     
we write 
\[
f_1 \otimes f_2  \equiv v_1+ v_2 
\]
where
\begin{align}
&v_1    \in I^{m_1+m_2 + \nnn, - m_2 - \nnn}_{comp} \big( N^* Y_1  \times \{0\}_{\PP M},   N^* [Y_1  \times  Y_2]  \big), \\
 &v_2 \in I^{m_1 + m_2+ \nnn,-m_1-\nnn}_{comp} \big( \{0\}_{\PP M} \times N^*Y_2  , N^* [Y_1  \times  Y_2]  \big), 
\end{align}
%and 
%\begin{align}
%\sigma(v_1) &=  \phi  \sigma(f_1) \otimes \sigma(f_2), \\ 
%\sigma(v_2)& =  (1-\phi) \sigma(f_1) \otimes \sigma(f_2).
%\end{align}
% \antti{ far from origin}. 
%on $N^* [Y_1 \times Y_2]$. 
%Moreover, we choose $\phi$ such that it equals $1$ in a neighbourhood of the set
%\[
%J_1 := \Big\{ (x,p,y,q; \xi^x,\xi^p,\xi^y,\xi^q) \in T^* ( \PP M \times \PP M)   :  x=x_0 = y, \ \frac{| (\xi^x)' | }{| \xi^x |} < \epsilon  \Big\}
%\]
%and zero in a neighbourhood of the set 
%\[
%J_2 := \Big\{ (x,p,y,q; \xi^x,\xi^p,\xi^y,\xi^q) \in T^* ( \PP M \times \PP M)   :  x=x_0 = y, \ \frac{| (\xi^y)'' | }{| \xi^x |} < \epsilon  \Big\}.
%\]
To prove \eqref{si3478} it is sufficient to show that for both $j=1,2$ there is a decomposition $R_A \circ v_j = u_j + r_j$, where $u_j$ is a Lagrangian distribution over $ \Lambda_0$ and $WF(r_j) \subset \Gamma_j$. %The symbol identity \eqref{symboiu} follows from \cite[eq. (4.2.10)]{duistermaat2010fourier}. 
We only consider the $v_1$ component of $f_1\otimes f_2$ and write $v=v_1$. The argument for the other component is similar. 
%\\
%{\color{red} 
%------------------------------------------------------------------------------------------------------\\
%Several things below need to be fixed. Please find the details below and compare them to what was written in my original proof. --Antti \\
%------------------------------------------------------------------------------------------------------\\
%}
%By~\eqref{lagrangian_pairs} %the above~\eqref{} and by greenleaf uhlmann (1.4) 
Fix small $\delta_1,\delta_2 \in (0,1)$ with $\frac{2\delta_1}{1-\delta_2}< \epsilon$, and 
let $\psi \in C^\infty (T^* ( \PP M \times \PP M) \setminus \{0\})$ be positively homogeneous of degree 0 such that it equals $1$ on the conic neighbourhood
\[ 
\begin{split}
X_1:= \Big\{ (x,p,y,q; \xi^x,\xi^p,\xi^y,\xi^q) \in T^* ( \PP U \times \PP U) \setminus \{0\}   :  \| (\xi^x)'' \| < \frac{\delta_1}{2} \| (\xi^x)' \| , \\
 \| x' \| < \frac{\epsilon}{2} , \  \| (\xi^y)'' \| < \frac{\delta_1}{2} \| (\xi^x)' \|,  \ 
\| (\xi^y)' \| < \frac{\delta_2}{2} \| (\xi^x)' \| \Big\} 
\end{split}
\] of $N^*Y_1 \times \{0 \}_{\PP M}$ 
and vanishes in the exterior of the larger neighbourhood
\[
\begin{split}
X_2:= \Big\{ (x,p,y,q; \xi^x,\xi^p,\xi^y,\xi^q) \in T^* ( \PP U \times \PP U) \setminus \{0\}   :  \| (\xi^x)'' \| < \delta_1 \| (\xi^x)' \| , \\
 \| x' \| < \epsilon , \  \| (\xi^y)'' \| < \delta_1 \| (\xi^x)' \|, 
\| (\xi^y)' \| < \delta_2 \| (\xi^x)' \| \Big\} .
\end{split}
\]
By dividing the amplitude in the oscillatory integral according to $1 = \psi + (1-\psi)$ we obtain the decomposition $v = v' + v''$, where $v'  \in I_{comp}^{m_1+m_2 + n} ( N^*[Y_1 \times Y_2])$ and $WF(v'') \subset X_2$. Moreover, 
\[
\sigma(v') = (1-\psi) \sigma(v) = \sigma(v)= c \phi (\sigma(f_1) \otimes \sigma(f_2) )\quad \text{on} \quad  (N^*[Y_1 \times Y_2]) \setminus X_2. 
\]
Applying \cite[Corollary 1.3.8]{duistermaat2010fourier} and $WF(v'') \subset X_2$ we deduce
\[
\begin{split}
WF( R_A \circ v'') \subset    WF'(R_A) \circ WF(v'') \cup WF_U'(R_A) \subset  ( \pi \text{supp} A ) \cap   ( \Lambda_R' \circ WF(v'')) \\ 
 \subset ( \pi \text{supp} A )  \cap   ( \Lambda_R' \circ X_2) 
\end{split}
\]
By definition, an element $(x,\eta)$ in $( \Lambda_R' \circ X_2)$ satisfies  $\| x' \| < \epsilon$ and 
\[
\eta = \xi^x+ \xi^y, \quad  \| (\xi^x)'' \| < \delta_1 \| (\xi^x)' \| , 
 \  \| (\xi^y)'' \| < \delta_1 \| (\xi^x)' \|,  \ 
\| (\xi^y)' \| < \delta_2 \| (\xi^x)' \|. 
\]
By using the triangle inequality and the inequalities above one computes
\[
\frac{ \| \eta'' \| }{\| \eta' \| } \leq \frac{ \| (\xi^x)'' \| + \| (\xi^y)'' \|  }{| \| (\xi^x)' \| - \| (\xi^y)'\| |  } < \frac{2 \delta_1 }{ 1-\delta_2 } < \epsilon
% \quad \Rightarrow \quad \| \eta'' \| < \epsilon \| \eta' \|.
\]
which implies $ \| \eta'' \| < \epsilon \| \eta' \|$. 
Thus, by \eqref{zskla}, we conclude
\[
WF( R_A \circ v'') \subset  \Gamma_1
\]
%
% we have that 	
%\[
% v\in I^{m_1+m_2 + \nnn}_{comp} \big(N^* (Y_1  \times  Y_2)  \big)
%\]
%{\color{red} ($\longleftarrow$ Not true.) \\
%(Let..? $\longrightarrow$ )}
%us define 
%\begin{align}
%\Sigma :=  (N^* Y_1 \times \{0\}_{\PP M}) \cup (\{0\}_{\PP M} \times N^*Y_2 ).
%\end{align}
%{\color{red} (consider referring to $N^*[ Y_1  \times \PP M] = N^* Y_1 \times \{0\}_{\PP M}$ or stick to either one of these elements. Notice that you had changed $N^* Y_1 \times \{0\}_{\PP M}$ into $N^*[ Y_1  \times \PP M]$ in Lemma  \ref{tensorlemma})}
%Let $\Gamma$ be a conical neighbourhood of $\Sigma$ and let $\chi$ a smooth cutoff function that vanishes on $\Gamma$. 
%%and let $ \chi(x,p,y,q ; \xi ) : (\PP M \times \PP M ) \times \R^{4\nnn} \rightarrow [0,1]$ be a smooth function homogeneous of order $0$ with respect to the Fourier variable $\xi$. Assume that $\chi(x,p,y,q ; \xi )$ vanishes on some conical neighbourhood $\Gamma$ of $\Sigma$. 
%%We separate $v_1$ and $v_2$ microlocally by multiplying their symbols by the partition of unity 
%%\begin{align}
%%1= \chi(x,p,y,q ; \xi ) + (1-\chi(x,p,y,q ;  \xi )).
%%\end{align}
%%This separation allows us to write
%Set
%\begin{align}
%%f_1 \otimes f_2  
%v &=  u + r, %\text{ where } u=\chi v \text{ and } r=(1-\chi) v	
%\end{align}
%where $u=\chi v$, $r=(1-\chi) v$, and {\color{red} ($\longleftarrow$ here you multiply a distribution in $\PP M \times \PP M$ with a function on $T^*(\PP M \times \PP M)$. How do you define that? Is this $\chi$ actually considered as a pseudo-differential operator $\chi(x,p,y,q,D_x,D_p,D_y,D_q)$? What if $\chi$ is neither in a symbol class or positively homogeneous? Then this would fail to be $\Psi$DO or even well defined. Also, if you want to use $\Psi$DOs here then you'd have to refer to some composition calculus for $\Psi$DOs. In my proof I divided the symbol inside the operator, that is; $a(x,p,y,q, D_x,D_p,D_y,D_q) = (\chi a) (x,p,y,q,D_x,D_p,D_y,D_q) + ((1-\chi)a)  (x,p,y,q,D_x,D_p,D_y,D_q) $ where $a$ is a symbol and $\chi$ is a positively homogeneous of degree $0$ w.r.t. $(\xi^x,\xi^p,\xi^y,\xi^q)$. 
%To be precise, the division $a(x,p,y,q,D_x,D_p,D_y,D_q) = \chi(x,p,y,q,D_x,D_p,D_y,D_q)   a(x,p,y,q,D_x,D_p,D_y,D_q)  + (1- \chi(x,p,y,q,D_x,D_p,D_y,D_q)   )a(x,p,y,q,D_x,D_p,D_y,D_q) $ holds only modulo smooth functions, assuming that $\chi$ defines $\Psi$DO. --Antti)}
%\begin{equation}\label{nops}
%u \in I^{m_1+m_2 + \nnn}_{comp} 
%\big( 
% N^*(Y_1 \times Y_2 ) 
% \setminus \Sigma \big) .  
%\end{equation}
%{\color{red} ($\longleftarrow$Again, not well defined without extra conditions on $\chi$. You would also need $\chi$ to be $\Psi DO$ of order $0$ for the order to not change when multiplying with $\chi$. This is usually ensured by using cut-offs with positive homogeneity of degree 0 (Notice that for $\Psi DOs$ the order of symbol equals the order of the operator: $0 + n/2 - 2n/4 = 0$).  --Antti)}
%By construction the residual term  $r$ is a compactly supported distribution on $\PP M \times \PP M$ which satisfies
%\begin{align}
%WF(r)  \subset    \Sigma \cup ( \Gamma \cap N^*(Y_1 \times Y_2 )) . 
%\end{align}
%%A consequence of the propagation of singularities result given in \cite[Corollary 1.3.8]{duistermaat2010fourier} combined~\footnote{\tbl{Argue that the conditions are valid and add equation numbers.}} with the fact $WF_{U}'(R_A) = \emptyset$ (shown in \cite[eq. (1.3.18)]{duistermaat2010fourier}) implies that
%We have shown earlier  {\color{red} ($\longleftarrow$ not true. $r$ was just defined. --Antti)} that $WF_{\PP M \times \PP M}'(R_A)\cap WF(r)=\emptyset$ and $WF_{U}'(R_A) = \emptyset$. Thus, from~\cite[Corollary 1.3.8]{duistermaat2010fourier}, we deduce
%\begin{align}
%\begin{split}
%WF( R_A \circ r ) \subset
% (\Lambda_R' \circ \Sigma)  \cup ( ( \Lambda_R' \circ  \Gamma) \cap (\Lambda_R' \circ N^*(Y_1 \times Y_2) )) \\
% =(\Lambda_{1} \cup  \Lambda_{2} )  \cup ( ( \Lambda_R' \circ  \Gamma) \cap \Lambda_0 ).
% \end{split}
%\end{align}
%We show next that if $\widetilde{\Gamma}$ is a conical neighbourhood of $\Lambda_1\cup \Lambda_2$, then by redefining $\Gamma$ smaller if necessary, we obtain $WF( R_A \circ r )\subset \widetilde{\Gamma}$. This is equivalent {\color{red} (really equivalent? --Antti)}  to demonstrating that microlocally away (see Definition \ref{microlocally_away_defn}) from $(\Lambda_{1} \cup  \Lambda_{2} ) $, the element $R_A \circ (f_1 \otimes f_2)$ reduces to $R \circ u$ up to a smooth residual term. %there is a conical neighbourhood of $\Gamma$ of $\Sigma$ such that $(\Lambda_R' \circ  \Gamma)  \cap \Lambda_0\subset \widetilde{\Gamma}$.
%Set $\epsilon>0$ to be a small parameter and use it to define a restriction $\Gamma_\epsilon$ of the neighbourhood $\Gamma$. We take $\epsilon$ sufficiently small so that $\Gamma_\epsilon$ can be expressed in local coordinates near $Y_1$ and $Y_2$ (\ref{turhautuminen1}) as  $\Gamma_\epsilon \cap T^*U = \Gamma_{1,\epsilon} \cup \Gamma_{2,\epsilon}$ {\color{red}($\longleftarrow$ This statement is not true. The identity should be the definition of the neighbourhood $\Gamma_\epsilon$. Also, I suggest that we dont ''redefine'' or ''restrict'' the neighbourhood $\Gamma$ as it was never really explicitly fixed. Instead, I would just say that ''we fix $\Gamma$ in the following way..'' or something like that. Then you wouldnt really need the extra notation $\Gamma_\epsilon$ etc. This is perhaps just a matter of taste. --Antti)}, where
%\begin{align}
%\Gamma_{1,\epsilon} :=  \{ (x,y,p,q ; \xi^x , \xi^y , \xi^p, \xi^q ) :    | \xi^x \cdot v | \leq  \epsilon \| \xi^x \| \| v \| , \  \forall v \in \R^d \times \{0,\dots,0\}  \},
%\end{align}
%and
%\begin{align}
% \Gamma_{2,\epsilon} :=  \{ (x,y,p,q ; \xi^x , \xi^y , \xi^p, \xi^q ) :    | \xi^x \cdot v | \leq  \epsilon \| \xi^x \| \| v \| , \  \forall v \in \{ 0, \dots, 0 \} \times \R^{\nnn-d}  \}.
%\end{align}
%The local representation (\ref{hauska12221}) yields
%\begin{align}
%\begin{split}
%(\Lambda_R' \circ  \Gamma)  \cap \Lambda_0 = 
%\{ (0, \xi^x ) :    | \xi^x \cdot v | \leq  \epsilon \| \xi^x \| \| v \| , \  \forall v \in \R^d \times \{0,\dots,0\}  \} \\
% \cup \{ (0 ; \xi^x  ) :    | \xi^x \cdot v | \leq  \epsilon \| \xi^x \| \| v \| , \  \forall v \in \{ 0, \dots, 0 \} \times \R^{\nnn-d}  \}.  
%\end{split}
%\end{align}
%From this we see that for sufficiently small $\epsilon > 0$, the set $(\Lambda_R' \circ  \Gamma)  \cap \Lambda_0$
%%converges to $(\Lambda_{M_1} \cup  \Lambda_{M_2} ) \cap \Lambda_0$ as $\epsilon \longrightarrow 0+$ and hence 
%is contained in $\widetilde{\Gamma}$. 
%%any given conical neighbourhood of $(\Lambda_{1} \cup  \Lambda_{2} )$.  Thus, away from $(\Lambda_{1} \cup  \Lambda_{2} ) $ the element $R_A \circ (f_1 \otimes f_2)$ reduces to $R \circ u$ up to a smooth residual term. 
To finish the proof we are left to show that the conditions of \cite[Theorem 2.4.1]{duistermaat2010fourier} (cf. the global formulation  \cite[Theorem 4.2.2]{duistermaat2010fourier}) for the composition of $v'$ and $R_A$ are satisfied. 
% (cf. the global formulations for the transversal intersection calculus \cite[Theorem 4.2.2]{hormander1971fourier1}, \cite[Theorem 4.2.2]{duistermaat2010fourier} and for the clean intersection calculus \cite[Theorem II]{guillemin1975clean}).   
The symbol identity \eqref{symboiu} follows from \cite[eq. (4.2.10)]{duistermaat2010fourier}. 
% and
%\[
%\sigma(v_1') + \sigma(v_2') = c \phi ( \sigma(f_1 ) \otimes \sigma( f_2) )  +(1-\phi) c  ( \sigma(f_1 ) \otimes \sigma( f_2) )   = c ( \sigma(f_1 ) \otimes \sigma( f_2) )
%\]
%Since the admissible collision kernel $A$ is compactly supported with respect to the base point $x\in M$ it follows that $R_A$ is properly supported. 
%\antti{(removed an old line from here -antti)} \footnote{\antti{removed an old line here as it was not true --antti}}
The condition \cite[eq. (2.4.8)]{duistermaat2010fourier}  is satisfied since $v'$ is compactly supported. The  conditions \cite[eq. (2.4.9), (2.4.10)]{duistermaat2010fourier} follow from the definitions (\ref{turhautuminen1}) and (\ref{hauska12221}). The last condition  \cite[eq. (2.4.11)]{duistermaat2010fourier} follows from Lemma \ref{lambda_R_prime}.
%
%
% \begin{lemma}\label{dimension-transverse-lemma}
% The spaces $\Lambda'_R \times ( N^*Y_1 \times  N^*Y_2 ) $ and $T^*U \times \text{diag}\, T^*( \PP M \times \PP M) $ intersect transversally in $T^*U \times T^*(\PP M \times \PP M) \times  T^*(\PP M \times \PP M)$.
% \end{lemma}
% 
% \begin{proof}
% Recall that for any linear subspaces $L_1,L_2$ of a finite dimensional real vector space,
% \begin{equation}\label{jksadss}
% \dim (L_1 + L_2) = \dim L_1 + \dim L_2 - \dim (L_1 \cap L_2).
% \end{equation}
% In particular, if this gives the dimension of the underlying vector space then the subspaces intersect transversally. 
% The local expression (\ref{hauska12221}) and coordinates (\ref{turhautuminen1}) imply that the space
% \[
% (\Lambda'_R \times (  N^*Y_1 \times  N^*Y_2) ) \cap (T^*U \times \text{diag} T^*( \PP M \times \PP M) )
% \]
% equals in the associated canonical coordinates $((x,\xi)(y,z,q,p'; \xi^y,\xi^z, \xi^q,\xi^{p'}))$ the punctured $\nnn$-dimensional plane
% \[
% L:= \big\{ ( (0;\xi^x  ) , \text{diag} (0,0, e_1, e_2 ; \xi^x_1,\dots \xi^x_d, 0, \dots, 0 ,\xi_{d+1}^x ,\dots, \xi^x_\nnn ,0,\dots,0 ) ) : \xi^x \in \R^\nnn \setminus \{0 \} \big\}  
% \]
% where  and $e_1 := (0,\dots,0,1,0,\dots,0) \in \R^\nnn$ and $e_2 := (1,\dots,0)\in \R^\nnn$. In particular, it is a manifold and 
% \[
% \begin{split}
% \dim ( \Lambda'_R \times ( N^*Y_1 \times  N^*Y_2) ) + \dim (T^*(U) \times \text{diag} T^*( \PP M \times \PP M) ) - \dim L \\
% = 9 \nnn  + 10 \nnn - \nnn = 18\nnn = \dim ( T^*U \times T^*(\PP M \times \PP M) \times  T^*(\PP M \times \PP M) )
% \end{split}
% \]
% from which we obtain the claim by applying (\ref{jksadss}) to  tangent spaces. 
% 
% \end{proof}
%
Since the conditions of \cite[Theorem 2.4.1]{duistermaat2010fourier} are met, we have that $R_A \circ v'$ is a well-defined oscillatory integral of order $m_1+m_2 + 3\nnn/4$ with the canonical relation $\Lambda'_R \circ (  N^*(Y_1 \times Y_2)) = \Lambda_0$. 
In conclusion, for arbitrary conic neighbourhoods $\Gamma_1,\Gamma_2$ of $\Lambda_1$ and $\Lambda_2$ there is the decomposition
\[
 \COLOP_{gain}^P [ f_1,f_2 ] = u + r, \quad u := R_A \circ (v_1'+v_2') \in I_{comp}^{m_1+ m_2 +3\nnn/4}( \Lambda_0) , \quad  r:=  R_A \circ (v_1''+v_2'') ,
\]
such that $WF(r) \subset \Gamma_1 \cup \Gamma_2$ and the symbol identity  \eqref{symboiu} holds on $\Lambda_0 \setminus (\Gamma_1 \cup \Gamma_2)$. 
%We show next that  $ \Lambda'_R \circ (  N^*(Y_1 \times Y_2)\setminus \Sigma)= \Lambda_0\setminus(\Lambda_1\cup \Lambda_2)$.
%By definition (eq. \eqref{relation_of_composition}) we have
%\[
%\begin{split}%\label{lambda_composed_with_Y2}
%\Lambda'_R \circ (  N^*(Y_1 \times Y_2)\setminus \Sigma)=\{ (x,\xi^x)\in T^*U: \ & \exists \big((y,p \; \xi^y, \xi^p),(z,q \; \xi^z, \xi^q)\big)\in N^*(Y_1 \times Y_2)\setminus \Sigma \nonumber \\
%& \text{such that }
% \big((x,\xi^x), (y,p, z,q \; \xi^y, \xi^p, \xi^z, \xi^q)\big)\in \Lambda_R' \}.
%\end{split}
%\]
%
%Let $(x,\xi^x) \in \Lambda'_R \circ (  N^*Y_1 \times N^*Y_2\setminus \Sigma)$. From \eqref{hauska12221},  $\big((x,\xi^x), (y,p, z,q \; \xi^y, \xi^p, \xi^z, \xi^q)\big)\in \Lambda_R'$ implies that 
%\begin{align*}
% \xi^x&=\xi^y+\xi^z\ne0, \\
% \xi^p&=\xi^q=0, \text{ and}\\
% x&=y=z
%\end{align*}
%must hold. From the coordinate representation of $Y_1$ and $Y_2$ in \eqref{turhautuminen1}, $(y,p\; \xi^y,0)\in N^*Y_1$ satisfies $y'=0$ and $(\xi^y)''=0$. Similarly, $(z,q\; \xi^z,0)\in N^*Y_2$ satisfies $z''=0$ and $(\xi^z)'=0$. Thus for $\xi^x$ to not vanish, we must have $(\xi^y)'\ne0$, and $(\xi^z)''\ne0$. Then, from the expressions for $\Lambda_1$ and $\Lambda_2$ given in equations \eqref{lambda_composed_with_Y1} and \eqref{lambda_composed_with_Y2} respectively,  we deduce that $(x,\xi^x)\notin \Lambda_1$ and $(x,\xi^x)\notin \Lambda_2$. 
%That is, we have shown  $\Lambda'_R \circ (  N^*(Y_1 \times Y_2) \setminus \Sigma) \subset \Lambda_0\setminus (\Lambda_1\cup \Lambda_2)$.
%By a similar argument we also obtain $\Lambda_0\setminus (\Lambda_1\cup \Lambda_2) \subset \Lambda'_R \circ (  N^*(Y_1 \times Y_2)\setminus \Sigma)$.
%%
%%
%%Thus elements in $\Lambda'_R \circ (  N^*Y_1 \times N^*Y_2\setminus \Sigma)$ must have the form 
%%\begin{align*}
%% (\xi^y)^{''}&=0, \text{ and } (\xi^z)^{'}=0 \\ 
%% (\xi^y,\xi^z) &\text{ is not of the form } (\xi^y, 0 ) \text{ where } \xi^y\in \Lambda_1 \\
%% (\xi^y,\xi^z) &\text{ is not of the form } (0, \xi^z) \text{ where } \xi^y\in \Lambda_2
%%\end{align*}
%%This means that $\xi^x\in \Lambda_0\setminus (\Lambda_1\cup \Lambda_2)$.
%In conclusion, we have shown
%\[
%R \circ u \in I^{m_1+m_2 + 3\nnn/4} ( \Lambda_0 \setminus (\Lambda_{1} \cup \Lambda_{2} ) ).
%\]
%which completes the proof. 
\end{proof}





%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Theorem for Q[X^{-1} . , X^{-1} . ](x, F(x))
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
%As heuristically argued in Section \ref{Bman-model}, the second linearization of our source-to-solution map data determines terms of the form $\IX\COLOP_{gain}[\IX f_1,\IX f_2]$ for conormal distributions $f_1,f_2$. We now extend $\COLOP_{gain}$ to distributions of the form $\IX f$, where $f$ is a Lagrangian distribution over the geodesic flowout of some submanifold in $\OVS M$.



Theorem \ref{sofisti} together with the microlocal properties of the geodesic vector field yields the following corollary:

%Putting together the microlocal properties of the geodesic vector field reviewed in Section \ref{Vlasov}, and the analysis of Theorem \ref{sofisti} additionally yields the following result:


\begin{corollary}[Extension to distributions solving Vlasov's equation]\label{sofisti_further}
%Let $(M,g)$ be geodesically complete, globally hyperbolic Lorentzian manifold.  
%Let $S_j \subset P^{r_j}_{t_j}$, $t_j \in \R$, $r_j > 0$ , $j=1,2$  
%be smooth manifolds such that    
% \[
% \PP(U)  \cap (S_1 \cup  S_2) = \emptyset,  
% \]
% and for $Y_j := K_{S_j}$, $j=1,2$, there is an open neighbourhood $ U \subset M$ and local coordinates 
%\[
%x = (x',x'') : U \rightarrow \R^\nnn, \quad x' = (x^1,\dots,x^d), \quad x''=(x^{d+1}, \dots, x^\nnn)
%\]
%% on some neighbourhood 
%satisfying
%\begin{equation}\label{turhautuminen2}
%\begin{split}
%Y_1 \cap TU &= \{ (x,p)   \in TU  : x' = 0  , \ p' = 0,  \ p'' = (1,0,\dots,0)  \}  \\
%Y_2 \cap TU &= \{  (x,p) \in TU : x'' = 0, \ p''= 0, \  p' = (1,0,\dots,0) \}  , 
%%\\ \quad d &=  \dim K_{M_2} = \nnn -  \dim K_{M_1}.
%\end{split}
%\end{equation}
% in the associated canonical coordinates $(x,p) = (x',x'',p',p'')$ of $TU = U \times \R^\nnn$. 
%Further, define
%\[
%\Lambda_0 := T_{0}^* \R^\nnn, \quad \Lambda_1 := N^*  \{ x   \in U  : x' = 0  \} \quad \text{and} \quad \Lambda_1 := N^*  \{ x   \in U  : x'' = 0  \} . 
%\]
%Let $F(x)= (x,p(x))$,  be a smooth local section of the bundle $\pi: \overline{\mathcal{P}}(U) \rightarrow U$.
%
%Let $(M,g)$ be a globally hyperbolic Lorentzian manifold.  


\tbl{Let $(M, g)$ be a globally hyperbolic Lorentzian manifold and let $\mathcal{C}$ be a Cauchy surface of $(M,g)$. %, $K\subset \OVS \mathcal{C}^+$ be compact and $k\ge 0$.
Let $S_1, S_2 \subset \PP^+ \mathcal{C} $} be smooth manifolds such that 
%\begin{itemize}
%\item $\pi (\overline{S}_1 \cup \overline{S}_2) \cap  U = \emptyset$ .
%\item
the geodesic flowouts $Y_1 := K_{S_1}$ and $Y_2:= K_{S_2}$ have an admissible intersection \antti{property} (see Definition \ref{intersection_coords}) in $\pi \text{supp} A$. Let $U$ be a small neighbourhood of some $x_0 \in \pi Y_1 \cap \pi Y_2 \cap \pi \text{supp} A$ as in the definition of admissible intersection, let $P : U \rightarrow \OVS U$ be a smooth section of $\OVS U$ and assume \tbl{additionally} that $S_1,S_2 \subset \PP M \setminus \PP \overline{U} $. %\footnote{\antti{added bar over U. --antti}}
%\end{itemize}
Additionally, for $f_j \in   I_{comp}^{l_j}(\PP M ;\,N^*S_j)$, $j=1,2$,
 let $ u( f_j) $ solve the Vlasov's equation with source $f_j$ \tbl{and which vanish in $\mathcal{C}^-$.}
%Let $S_j \subset P^{r_j}_{t_j} M$, $t_j \in \R$, $r_j > 0$, $j=1,2$, 
%\[
%(\overline{S}_1 \cup \overline{S}_2) \cap  \overline{U} = \emptyset .
%\]
%Let $F : U \rightarrow \overline{\PP} U$ be a local section as in the proposition and set $\Lambda_j = \Lambda_{S_j} \cap T^*U$. 
%Let $S_1, S_2 \subset \PP M$, $\overline{S}_1 \cup \overline{S}_2) \cap  \overline{U} = \emptyset .$
%be smooth manifolds such that the conditions of Proposition \ref{sofisti} are satisfied for $Y_j := K_{S_j}$  and 
%\[
%(\overline{S}_1 \cup \overline{S}_2) \cap  \overline{U} = \emptyset .
%\]
%Let $F : U \rightarrow \overline{\PP} U$ be a local section as in the proposition and set $\Lambda_j = \Lambda_{S_j} \cap T^*U$. 
 %
%For 
%\[
%(h_j, f_j) \in  C^\infty_c (\PP_0 M ) \times I_{comp}^{l_j}(N^*S_j ; \PP M ),  \quad j=1,2, %\quad  \PP_0 := \PP \cap T_0 \R \times TN ,
%\]
% let $ v(h_j, f_j) \in \mathcal{D}' (\PP M)$ be defined by 
%\begin{align}
%\mathcal{X} v(h_j, f_j) = f_j,  \quad v(h_j,f_j)|_{\PP_0}  = h_j.
%% \quad 
%% \in C^\infty (\SP_0 )
%\end{align} 
 %
%\begin{align}
%\mathcal{X} u( f_j) = f_j,  \quad v(h_j,f_j)|_{\PP_0}  = 0.
%% \quad 
%% \in C^\infty (\SP_0 )
%\end{align} 
%
%(i.e.  $v(f_0,f) = \IX f + \XX_0^{-1}f_0$).
% where  
 %$\SP_0 := \SP \cap T_0 \R \times TN$, 
%and
% the restriction is defined via the pull-back of the inclusion $\PP_0 \hookrightarrow  \PP$. 
%
% Then, the operator 
% \[
%  \COLOP_{gain} [ v , v ]_F   ( h_1 , h_2  , f_1, f_2 ) := \COLOP_{gain} [ v ( h_1 , f_1 ), v (  h_2 , f_2 )]_F  
%  \]
% defines a continuous  map
% \[
% \begin{split}
%\COLOP_{gain} [ v , v ]_F   
% : C^\infty_c (\PP_0 M  ) \times C^\infty_c (\PP_0 M  ) 
%%\times  C^\infty_c (\PP_0 (M \setminus \overline{U} ) ) 
%\times I^{l_1}_{comp} (  N^*S_1 ; \PP M ) )\times I^{l_2}_{comp} ( N^*S_2 ; \PP M )\rightarrow \mathcal{D}' (U). 
%\end{split}
%\]
%

 
 Then, the operator \tbl{$\COLOP_{gain}^P [ u(\ccdot) , u(\ccdot) ]$, defined in~\eqref{def_of_QF},}
% \[
%  \COLOP_{gain} [ v , v ]_F   ( h_1 , h_2  , f_1, f_2 ) := \COLOP_{gain} [ v ( h_1 , f_1 ), v (  h_2 , f_2 )]_F  
%  \]
 defines a continuous  map
 \[
 \begin{split}
%\COLOP_{gain} [ u(\cdot) , u(\cdot) ]_F   
I^{l_1}_{comp} ( \PP M ;\, N^*S_1) )\times I^{l_2}_{comp} (\PP M ;\, N^*S_2)\rightarrow \mathcal{D}' (U). 
\end{split}
\]

Moreover, microlocally away from both $\Lambda_{1}$ and $\Lambda_{2} $, we have that 
%\begin{align}
\begin{equation}
\COLOP_{gain}^P [u(f_1),u(f_2)]\in I^{l_1+l_2+3\nnn/4-1/2} (U;\,\Lambda_0 \setminus( \Lambda_{1} \cup \Lambda_{2}))
\end{equation}
together with the symbol 
\begin{equation}\label{symbol_in_the_corollary}
\begin{split}
 \sigma ( \COLOP_{gain}^P [u(f_1),u(f_2)]) (\xi',\xi'') = 
%c A(x, \hat{p}(x) ,  p_x+q_x- \hat{p}(x) , p_x,q_x)  
 C \sigma( u(f_1) ) (0;\xi',0) \sigma(u(f_2)) ( 0 ;  \xi'' , 0) , %\\  (\xi',\xi'') \in \R^\nnn \setminus (  \{0\} \times \R^\nnn  \ \cup \    \R^\nnn \times \{ 0\} ) 
 \end{split}
\end{equation}
where the constant $C$ is given in the canonical coordinates $p = (p',p'')$ and $q=(q',q'')$ by 
\[
C = c A(x_0, \hat{p} (x_0) , p+q- \hat{p}(x_0) , p,q) \big|_{p = (1,0,\dots,0), \ q=(1,0,\dots,0) } , 
\] 
and $\hat{p}(x_0) \in \overline{\PP}_{x_0} U$ is such that $P(x_0) = ( x_0, \hat{p}(x_0)) $. 
%for some constant $c\neq 0$ and the unique vectors $p,q \in \PP_x M$ satisfying $(x,p) \in Y_1 \cap T_x U$ and $(x,q) \in Y_2 \cap T_x U$. 
Here $c$ is some non-zero constant and the manifolds $\Lambda_0 \setminus( \Lambda_{1} \cup \Lambda_{2})$, $T^*U \cap N^* Y_1$, and $T^* U \cap N^* Y_2$ are parametrised by the canonical coordinates $(\xi',\xi'')$, $(x''; (\xi^x)',\xi^p  )$, and $(x' ; (\xi^x)'', \xi^p)$, respectively.


%\[
% \COLOP_{gain} [ v ( f_1 ), v ( f_2 )]_F \in I^{l_1+l_2+ 3\nnn /4 - \tbl{1}} (\Lambda_0 \setminus( \Lambda_{1} \cup \Lambda_{2}) ;U ) .
%\]
%for every $( h_1, h_2, f_1  , f_2 )) \in  C^\infty_c (\PP_0 M )  \times  C^\infty_c (\PP_0 M )  \times I^{l_1}_{comp} (  N^*Y_1 ; \PP M  )\times I^{l_2}_{comp} ( N^*Y_2 ; \PP M )$.
% \tbl{* check the order of the distribution space}
\end{corollary}


\begin{proof}%[Proof of Proposition \ref{sofisti_further}]

%We assume for simplicity that $(M,g)$ is geodesically complete. 

For $j=1,2$, let $f_j \in I^{l_j}_{comp} ( N^* S_j ; \PP M )$. Choose a cut-off function $\chi \in C^\infty_c (M) $ so that $\chi =1 $ on $U \cap \text{supp} (x \mapsto A(x,\ccdot))$ and \tbl{$\chi=0$} on a neighbourhood of $\pi(S_1 \cup S_2) \subset M \setminus \overline{U}$ 
%\footnote{\antti{added bar over U. --antti}}. 


Now, for each $j=1,2$, by Lemma \ref{vlasov_ext_conormal}, there exists a solution $u(f_j)$ to the Vlasov equation with source $f_j$ and initial data $0$. Moreover, as $Y_j = K_{S_j}$, \antti{the sources $f_j$ are compactly supported and time-like geodesics can not be trapped} we get $\chi u(f_j) \in I_{comp}^{l_j -1/4} (\PP M ;\,N^*Y_j )$.

% and may be expressed as~\f{I think the integral is not well defined for distributions and it should be removed.}
% \[
% u(f_j)(x,p) = \int_{-\infty}^0 f_j( \gamma_{(x,p)}(s) , \dot\gamma_{(x,p)}(s) )  ds, 
% \]
% where the integration is understood in sense of distributions. 
% Since a globally hyperbolic manifold is causally disprisoning, we have that $\chi u(f_j)$ is compactly supported and vanishes near $S_j$ for both $j=1,2$.  Thus, one deduces $\chi u(f_1) \in I_{comp}^{l_1 -1/4} (N^*Y_1 ; \PP M )$ and $\chi u ( f_2) \in I_{comp}^{l_2 -1/4} (N^*Y_2 ; \PP M )$

%Then, 
Substituting $u = \chi u  + (1-\chi) u$ into $\COLOP_{gain}$, we obtain that 
 \[
 \begin{split}
 \COLOP_{gain}^P [ u(f_1), u(f_2)]    \equiv & \COLOP_{gain}^P [\chi  u(f_1), \chi  u(f_2)].  
 \end{split}
 \]
Thus we have reduced to the setting of Proposition \ref{sofisti} and obtain the desired results.





% TJB Edit 1
%For $j=1,2$, let $f_j \in I^{l_j}_{comp} ( N^* S_j ; \PP M )$. 
%
%As stated in Section \ref{mla_vlasov}, $-i\XX$ has principal symbol $p^\alpha \xi^x_\alpha   - \Gamma^\alpha_{\lambda \mu} (x)  p^\lambda  p^\mu  \xi^p_\alpha$, and hence $-i\XX\in \Psi^{1}_{1,0}(\PP M)$ is a first order pseudodifferential operator of real principal type. Thus, as shown in \cite{melrose-uhlmann1979}[Proposition 6.6] (see also \cite{DH1972}[Theorem 6.5.3]), there is a left (or alternatively right) parametrix $\IX$ for $\XX$ which satisfies 
%\[
%\IX\in I^{-\frac12,-\frac12}(\Delta_{T^*\PP M},\Lambda_\XX).%\IX\in I^{\frac12 -1,-\frac12}(\Delta_{T^*\PP M},\Lambda_\XX).
%\]
%Here $\Delta_{T^*\PP M} \subset (T^*\PP M\setminus 0)\times (T^*\PP M\setminus 0)$ denotes the diagonal, and 
%\begin{align}
%\Lambda_\XX &= \{  ((x,p \, ; \, \xi^x,\xi^p) ,(y,q \, ; \, \xi^y,\xi^q)) \in T^* TM \times T^*  TM\,:\,  (x,p \, ; \, \xi^x,\xi^p)\text{ and }(y,q \, ; \, \xi^y,\xi^q) \notag\\
%&\qquad \text{ lie on the same bicharacteristic strip of }\XX\}.
%\end{align}
%
%By \cite{greenleaf-uhlmann}[Proposition 2.1], $\IX f_j \in I^{l_j-\frac12,-\frac12}(N^*S_j,\Lambda_\XX\circ N^*S_j)$. In particular, this means that microlocally away from $E=(\Lambda_\XX\circ N^*S_j)\cap N^*S_j$,
%\[
%\IX f_j \in I^{l_j-\frac14}(N^*S_j\setminus E) \text{ and } \IX f_j \in I^{l_j-\frac12}(\Lambda_\XX\circ N^*S_j\setminus E).
%\]
%
%%\tbl{Above have I got the orders correct?}
%Recall that $(x,p \, ; \, \xi^x,\xi^p)\in T^*  TM$ and $(y,q \, ; \, \xi^y,\xi^q)\in T^*  TM$ lie on the same bicharacteristic strip of $\XX$ if 
%\[
%(y,q) = \gamma_{x,p}(s) \,\text{for some } s\in \R,
%\]
%and there exists $\psi\in C^\infty(TM)$ such that $\psi$ is constant along geodesics in $M$ and 
%\[
%d\psi|_{(x,p)}= (\xi^x,\xi^p) \, \text{ and } d\psi|_{(y,q)} = (\xi^y,\xi^q).
%\]
%From these definitions we see that 
%\begin{align*}
%\Lambda_\XX\circ N^*S_j &= \{(x,p,\xi^x,\xi^p) \in T^*(\PP M)\,:\, \exists\, (y,q,\xi^y,\xi^q)\in N^*S_j \text{ s.t. } (x,p,\xi^x,\xi^p, y,q,\xi^y,\xi^q) \in \Lambda_\XX\}\\
%&= N^*K_{S_j}.
%\end{align*}
%
%As $N^*K_{S_j} = \Lambda_\XX\circ N^*S_j$, setting $Y_j= K_{S_j}$ we have derived $\IX f_j \in I^{l_j-\frac12}(N^*Y_j)$ for $j=1,2$. Since we assume that $Y_1$ and $Y_2$ satisfy the intersection property \ref{intersection_coords}, by Theorem \ref{sofisti} we obtain the stated claims.
% {vlasov-ext-conormal}
% $u_j\in I^{l_j-\frac12,-\frac12}(N^*S_j,\Lambda_\XX\circ N^*S_j)$








% OLD VERSION

%Consider initial and source data
%\[
%(h_j,f_j) \in C^\infty_c (\PP_0 M) \times I^{l_j}_{comp} ( N^* S_j ; \PP M ) , \quad j=1,2.
%\]
%By (\ref{supp121}), $\text{supp} ( \IX f_j  + \mathcal{X}^{-1}_0 h_j ) \subset K_{\text{supp}(f_j)}^+ \cup K_{\text{supp}(h_j)}^+$, where
%\[
%K_{\text{supp}(f_j)}^+ := \{  (x,p) \in TM : (x,p) =  \dot\gamma_{(y,q)}(s) ,  \ \text{for some} \ (y,q) \in  \text{supp}(f_j), \ s \geq 0 \} \subset \PP M.
%\]
%and
%\[
%K_{\text{supp}(h_j)}^+ := \{  (x,p) \in TM : (x,p) =  \dot\gamma_{(y,q)}(s) ,  \ \text{for some} \ (y,q) \in  \text{supp}(h_j), \ s \geq 0 \} \subset \PP M.
%\]
%Let $f_j \in I^{l_j}_{comp} ( N^* S_j ; \PP M )$, $j=1,2$. By (\ref{supp121}), $\text{supp} ( \IX f_j  + \mathcal{X}^{-1}_0 h_j ) \subset K_{\text{supp}(f_j)}^+ \cup K_{\text{supp}(h_j)}^+$, where
%\[
%K_{\text{supp}(f_j)}^+ := \{  (x,p) \in TM : (x,p) =  \dot\gamma_{(y,q)}(s) ,  \ \text{for some} \ (y,q) \in  \text{supp}(f_j), \ s \geq 0 \} \subset \PP M.
%\]
%
%
%Thus, outside $K_{\text{supp}(f_j)}^+ \cup K_{\text{supp}(h_j)}^+$ the distribution $v(h_j,f_j) =\mathcal{X}_0^{-1} h_j +  \IX f_j$ is zero.
%
%Further, since each time-like geodesic escapes permanently from a compact set \cite[Proposition 1]{MR1216526} and $ \text{supp} (x \mapsto A(x,\cdot,\cdot,\cdot,\cdot))$ is compact, we conclude that the sets
%\[
%\text{supp} (v(h_j,f_j))  \cap 
%\{ (x,p) \in T M : x \in \text{supp} (x \mapsto A(x,\cdot,\cdot,\cdot,\cdot)) \cap \overline{U} \}
%, \quad j=1,2
%\]
%\[
%\begin{split}
% \PP(K_j; M) \cap \text{supp} (v(h_j,f_j))     \subset& \PP (K_j ; M) \cap [ \Lambda_{\mathcal{X}}' \circ ( \text{supp}(h_j) \cup \text{supp}(f_j)) ], 
%\\
% &\PP (K_j ; M) := \{ (x,p) \in \PP M :  x\in K_j \}
%% \{ (x,p) \in \mathcal{S}(K) :  \  (x,p)  = \dot\gamma_{(y,q)} (s)  ,  \ (y,q) \in \text{supp}(f) \cup \text{supp}(f_0), \ s>0 \} ,
%%=\bigcup_{(x,p) \in \text{supp}(h_j) } \Big( \gamma_{(x,e(p))} , \sqrt{-g(p,p)} \dot\gamma_{(x,e(p))} \Big) [-S,0]  \cap \mathcal{S}(K),
%\end{split}
%\]
%are compact. {\color{red} (if doesn't work then let's put $h_j =0$ --antti)}
%In addition, they do not intersect $\overline{S}_1 \cup \overline{S}_2$ by the assumptions. 
% 
%Thus, we can choose 
%$\chi \in C_c^\infty ( T M )$ such that $\chi(x,p) = 1$ on a relatively compact neighbourhood of
% \[
% \begin{split}
%& [\text{supp} (v(h_1,f_1)) \cup \text{supp} (v(h_2,f_2))  ]\cap 
%\{ (x,p) \in T M : x \in \text{supp} (x \mapsto A(x,\cdot,\cdot,\cdot,\cdot)) \cap  \overline{U} \}
%\PP ( \text{supp} (x \mapsto A(x,\cdot,\cdot,\cdot,\cdot)) ; U )  
%\\
%& \PP ( \text{supp} (x \mapsto A(x,\cdot,\cdot,\cdot,\cdot)) ; U )   := \{ (x,p) \in \mathcal{P} U : x \in \text{supp} (x \mapsto A(x,\cdot,\cdot,\cdot,\cdot)) \}
%\end{split}
% \] 
%and $\chi(x,p) = 0$ on some neighbourhood of 
%\[
%\begin{split}
%&[\overline{S}_1 \cup \overline{S}_2] \cap [\text{supp} (v(h_1,f_1)) \cup \text{supp} (v(h_2,f_2))  ] .\\
%&\subset [\overline{S}_1 \cup \overline{S}_2] \cap [ K_{\text{supp}(f_1)}^+ \cup K_{\text{supp}(h_1)}^+  \cup K_{\text{supp}(f_2)}^+ \cup K_{\text{supp}(h_2)}^+] \\
%&= [S_1 \cup S_2] \cap [\text{supp} (f_1) \cup \text{supp} (h_1) \cup  \text{supp} (f_2) \cup \text{supp} (h_2) ]. 
%\end{split}
%\]
% Notice that here we need the condition $\pi M_1 \cap \pi M_2 = \emptyset$. 
%By (\ref{prprp1}) and compactness of the support,
%% the distributions $\chi v(f_0,f) $, $\chi v (\tilde{f}_0, \tilde{f})$ are compactly supported conormal particle clouds with initial manifolds in $M_1,M_2$, respectively. 
%%More precisely,  
%\[
%\chi v(h_1,f_1) \in I_{comp}^{l_1 -1/4} (N^*Y_1 ; \PP M ) \quad \text{and} \quad \chi v (h_2, f_2) \in I_{comp}^{l_2 -1/4} (N^*Y_2 ; \PP M )
%\]
% for $( h_1 ,  h_2  , f_1, f_2 ) \in C^\infty_c (\PP_0 M ) \times C^\infty_c (\PP_0 M ) \times  I_{comp}^{l_1}(N^*S_1 ; \PP M)\times  I_{comp}^{l_2}(N^*S_2 ;  \PP M) $. 
%% The source term of the collision operator extends naturally to the pair $( v(f_0,f), v (\tilde{f}_0, \tilde{f}) )$ by splitting integration over $\Sigma_{x,p}$ into parts according to 
%% $v(\cdot) = \chi v(\cdot)  + (1-\chi) v(\cdot)$.  
%Substituting $v(\cdot) = \chi v(\cdot)  + (1-\chi) v(\cdot)$ we obtain
% \[
% \begin{split}
% \COLOP_{gain} [ v(h_1,f_1), v(h_2, f_2)]_F   =& \COLOP_{gain} [\chi  v(h_1,f_1), \chi  v(h_2, f_2)]_F  
% % + \underbrace{\COLOP_{gain} [\chi  v(h_0,h),(1- \chi)  v(\tilde{h}_0,\tilde{h})]}_{= 0} \\
%% +& \underbrace{ \COLOP_{gain} [(1 -\chi)  v(h_0,h), \chi  v(\tilde{h}_0,\tilde{h})] }_{=0}+  \COLOP_{gain} [(1 -\chi)  v(h_0,h), (1- \chi)  v(\tilde{h}_0,\tilde{h})] \\
%%\equiv  & \COLOP_{gain} [\chi  v(h_0,h), \chi v(\tilde{h}_0,\tilde{h})]  \mod C^\infty (T(\R \times N))  \\
% \end{split}
% \]
% for smooth  $h_1,f_2$ and hence 
%the claim follows by Proposition \ref{sofisti} and 
% continuity of the inverse map $(h,f) \mapsto v(h,f ) = \XX_0^{-1}h + \IX f $. 

\end{proof}



==> Sections/introduction-new.tex <==
%%%
%%%. Introduction
%%%
%%%. Date: May 11 2020
%%%
%%%
\section{Introduction}

% MODEL \\
% MOTIVATION\\
% INVERSE PROBLEM\\
% RESULT\\
% EARLIER RESULTS\\
% SKETCH OF PROOF\\

% % % % % % % % % % % {\color{gray}
% % % % % % % % % % % The question ``From what information can an observer in a physical system determine properties of that system?'' is a fundamental one, and seeking an answer such a question is the archetypal expression of an inverse problem.  While there is a considerable amount of literature on the study of inverse problems for wave or linear transport equations, little is known for inverse problems involving key nonlinear transport equations. In this paper, we address an inverse problem for the nonlinear kinematic behaviour of particles of matter or radiation in some media. %From observer measurements, we show that we can uniquely determine certain physical properties of the media studied.
% % % % % % % % % % % }
%A common goal in all inverse problems is to recover information from indirect, incomplete or noisy observations.

In this paper we study what information can be recovered from indirect measurements of a system governed by the \tjb{Boltzmann equation.} The Boltzmann equation describes nonlinear particle dynamics
% in a physical system determine properties of that system?'' is a fundamental one, and seeking an answer such a question is the archetypal expression of an inverse problem.  
% 
% While there is a considerable amount of literature on the study of inverse problems for wave or linear transport equations, little is known for inverse problems involving key nonlinear transport equations. In this paper, we address an inverse problem for the nonlinear kinematic behaviour of particles of matter or radiation in some media. %From observer measurements, we show that we can uniquely determine certain physical properties of the media studied.
%Nonlinear particle dynamics 
which arise in many areas of \tjb{physics, such as} atmospheric chemistry, cosmology and condensed matter physics. \tjb{For example, in} cosmology, the Boltzmann equation describes how radiation is scattered by matter such as dust, stars and plasma on an Einstein spacetime. In condensed matter physics, the Boltzmann \tjb{equation may describe the transportation} of electrons or electron-phonon excitations in a media, which can be a metal or a semiconductor. In such situations, the geometry of the spacetime or resistivity of the media may be described by a Lorentzian manifold. % governs free propagation of light and matter in the media and . %, which governs free propagation of light and matter in the media. % $g$ on a manifold $M$ which models the spacetime.
%
%In both of these cases, free propagation of light and matter is governed by a Lorentzian manifold, which in the
%latter case models the resistivity of the media.
%In the former case, the Lorentzian manifold is of course the Einstein's spacetime and in the latter Lorentzian metric models resistivity of the media. 
\tjb{In particular, we investigate} the inverse problem of recovering the corresponding Lorentzian manifold of a system behaving according to the Boltzmann equation by making measurements in a confined, possibly small, area in space and time. 

In the kinetic theory we adopt, %fparticles is characterized by two principles. The first is causal one, namely that 
particles travel on a Lorentzian manifold $(M,g)$ along trajectories defined by either future-directed timelike geodesics (for positive mass particles) or future-directed lightlike geodesics (in the case of zero mass particles). In the absence of collisions and external forces, the kinematics of a particle density distribution $u\in C^\infty (TM)$ is captured by the \emph{Vlasov equation} \cite{Ringstrom}, \cite{Rendall} (or Liouville-Vlasov equation \cite{Choquet-Bruhat})  
\[
\XX u(x,p) =0 \quad \text{for } (x,p)\in \OVS M.
\]
Here $\OVS M$ is the subset of $TM$ of the future directed causal (i.e. not spacelike) vectors and $\mathcal{X}: C^\infty (TM) \rightarrow C^\infty (TM)$ is the geodesic vector field. 
%The integral curves of $\XX$ are geodesic velocity curves in the tangent space $TM$. 
In terms of the Christoffel symbols $\Gamma_{\lambda\mu}^\alpha$, the latter is given as
\[
\mathcal{X} = \sum_{\alpha,\lambda,\mu}  p^\alpha  \frac{\partial}{\partial x^\alpha}  -  \Gamma^\alpha_{\lambda \mu}   p^\lambda  p^\mu  \frac{\partial}{\partial p^\alpha }.
\]
%The in
The behaviour of binary collisions is characterized by a \emph{collision operator} %$\COLOP[u,v]$
 \begin{equation}\label{collision_operator_formula_intro}
\COLOP [u, v] (x,p)  
%=  A(x,p,q, p', q')  \delta_{\tilde\Sigma } 
=\int_{\Sigma_{x, p }}  \left[u (x,p) v (x,  q )  - u (x,p' ) v (x,  q' ) \right] A(x,p,q, p', q') dV (x,p \; q,p',q'),
\end{equation}
where   $u,v \in C^\infty( \OVS M)$.
%where
%\[
%\Sigma_{x,p} := \{ ( p', q' , q) \in   T_x(\R \times N)^3 : p + q = p' + q' \}.
%\]
Here $ dV (x,p \; q,p',q') $ is the induced volume form on the submanifold
\[
\Sigma_{x,p} := \{p\}\times  \{ (q,p',q')\in ( \overline{\mathcal{P}}_x M )^3  \,:\, p+q = p'+q'\} \subset (T_x M)^4
\]
%\[
% \overline{\mathcal{P}}_x^+ M := \{ (x,p) \in T_x M \setminus \{0 \} : -g(p,p)\geq 0, \ p \  \text{future-directed} \  \},
%\]
and for each $(x,p)\in \OVS M$ the function
\[
A(x,p, \cdot,\cdot,\cdot )\in C^\infty(\Sigma_{x, p }) 
\]
is called a \emph{collision kernel} (or a shock cross-section). %Essentially, this operator averages the numbers of 

We assume that $(M,g)$ is a globally hyperbolic $C^\infty$ smooth Lorentzian manifold (see Section~\ref{prelim}). Global hyperbolicity allows us to impose an initial state for the particle density function $u$ by using a Cauchy surface $\mathcal{C}\subset M$.
%Putting these concepts together, 
Given an initial state of no particles in the causal past $\mathcal{C}^-$ of $\mathcal{C}$, and a particle source $f$, supported in the causal future $\mathcal{C}^+$ of $\mathcal{C}$, the kinematics of a distribution of particles $u$ is given by the \emph{relativistic Boltzmann equation} \cite{Choquet-Bruhat}, \cite{Ringstrom}, \cite{Rendall},
\begin{equation}\label{boltzmann}
 \begin{split}
\mathcal{X}u(x,p)-\COLOP[u,u](x,p)&= f(x,p), \quad  (x,p)\in
\OVS M  \\
u(x,p)&= 0, \quad\quad\quad \ \  (x,p)\in \OVS \mathcal{C}^-.
 \end{split}
\end{equation}
%Here $\mathcal{C}^-\subset M$ is the causal past of the Cauchy surface $\mathcal{C}$. 
Though we do not consider it in this paper, Boltzmann's H-Theorem (which states that the entropy flux is nonincreasing in time) can be shown to hold for the relativistic Boltzmann kinematic model \eqref{boltzmann} when the collisions are reversible ($A(x,p,q, p', q') = A(x,p',q', p, q)$). We refer the reader to the works of \cite{Choquet-Bruhat}, \cite{Ringstrom}, or \cite{Rendall} for more details on this matter.

%the physical quantities of total mass~\fottnote{Here mass refers to the quantity $\int,~\f{What is this specifically? Invariant mass might refer to ADM mass, which is not what we are discussing.} total energy, and total momentum can be defined and shown to be conserved under the relativistic Boltzmann kinematic model (see \cite{Choquet-Bruhat}, \cite{Ringstrom}, or \cite{Rendall} for more details).

%Here and below write $L^+V \subset TM$ for the bundle of lightlike future directed vectors over a set $V$ and 

We study an inverse problem where we make observations in an open neighbourhood $V$ of a timelike geodesic in $M$. We assume that $V$ has compact closure without further notice. The observations are captured by the 
\emph{source-to-solution map for light observations},%~\f{We use $\mathcal{L}^+$ and $L^+$. Let's pick one. TB: the first is the projection of $L^+$ to the base.} %which is the assignment
\begin{equation}\label{light-source-soln}
 \Phi_{L^+V} : B \rightarrow C_b( L^+V ) ,\quad \Phi_{L^+V}(f) := \Phi(f)|_{L^+V}.
\end{equation}
Here $\Phi$ is the \emph{source-to-solution map} for the relativistic Boltzmann equation
%{\color{red}(I cleaned this a little bit and restricted the image into the light-like bundle --Antti)}
\begin{equation}\label{supposedtolooklikethis}
\Phi : B \rightarrow 
%C_{\OVS([0,\infty)\times N) }^0  ( \OVS V ) 
C_b( \OVS M ), \quad \Phi(f) = u,
\end{equation}
where $u$ solves \eqref{boltzmann} with a source $f$. The set $B$ is a neighbourhood of the origin in $C_K( \OVS \mathcal{C}^+)= \{f\in C(\OVS \mathcal{C}^+)\,:\, \text{supp}(f)\subset K\}$ for a fixed compact set $K\subset \OVS \mathcal{C}^+$ and $C_b(\OVS M)=\{f\in C(\OVS M): f \text{ is bounded}\}$. We also denote by $L^+V \subset TM$ the bundle of light-like future directed vectors whose base points are in $V$.
% and $\mathcal{C}^+\subset M$ is the causal future of $\mathcal{C}$.
%((0,\infty) \times N) \big)$, and $B_V = B \cap C_c^\infty(\SP V )$. 
%Here we define $\SP V = \OVS P\setminus L^+V$. 
Loosely speaking, the operator $\Phi_{L^+V}$ corresponds to measuring the photons received in $V\subset M$ from particle interactions governed by the Boltzmann equation \eqref{boltzmann}.

Known uniqueness and existence results to \eqref{boltzmann} depend inextricably on the properties of the collision kernel $A$. For general collision kernels, existence of solutions to \eqref{boltzmann} is not known. Complicating the analysis is the fact that it is not completely known what are the physical restrictions on the form of the collision kernel \cite[p. 155]{Ringstrom}. Further, in the case of Israel molecules, where one has a reasonable description of what the collision kernel should be, the collision operator can not be seen as a continuous map
% 
% term~\f{We use both $dV(x,p; q, p',q')$ and $dV_{x,p}(q,p',q')$. Let's pick one.} 
% \[
% \COLOP_{loss}[u, v] (x,p):= u (x,p) \int_{\Sigma_{x, p }}   v (x,  q ) A(x,p,q, p', q') dV_{x,p} (q,p',q'). %dV (x,p \ ; \ q,p',q') 
% \]
% cannot be written as a continuous map 
% 
between weighted $L^p$ spaces~\cite[Appendix F]{Ringstrom}. It is not always clear what is the relationship between conditions on the collision operator $\COLOP$ and the induced conditions on its collision kernel $A$. %Thus, current results for existence and uniqueness of solutions to \eqref{boltzmann} have imposed various restrictions on the collision kernel, as well as on the geometry and the data. 

To address the well-posedness of \eqref{boltzmann}, we consider collision kernels of the following type. Here we denote
\[
 \Sigma := \bigcup_{(x,p) \in \overline{\PP}M} \Sigma_{x,p} \subset TM^{ 4}
\]
and $L^+M$ and $\PP M$ are the bundles of light-like and timelike vectors over $M$ respectively.% $\PP M$ the bundle of t
\begin{definition}[Admissible Kernels]\label{good-kernels}
%Let $( M = \R\times N,g)$ be a Lorentzian spacetime, $r_1,r_2>0$ and $\hat\mu : [-1,1] \rightarrow (0,\infty) \times N$ be a smooth timelike curve.  For $-1< s^{-} < s^{+} < 1$, set $x^{\pm}:= \hat\mu (s^{\pm})$ and $W :=  I^-(x^{+}) \cap I^+(x^{-})$. 
We say that $A:\Sigma\subset T M^4\to\R$ is an \emph{admissible collision kernel} with respect to a  relatively compact open set 
%\footnote{Note that we have added `relatively compact open set' and removed the property that $W$ is a proper subset on Sep. 6, 2021. - Matti} 
 $W\subset M$ if $A$ satisfies
\begin{enumerate}
     \item\label{conditiony} $A\in C^\infty(\Sigma  )$. 
     
     \item\label{conditionyyyyy} The set $\pi \text{supp}  A$ is compact and contains $W$ as a subset. 
     
     \item\label{condition4}  $A(x, p, q ,p',q')>0$, for all $(x,p,q,p',q') \in \Sigma \cap (L^+W \times \overline{\PP} W \times \PP W \times  \PP W)$. 
     % \footnote{\antti{removed c. --antti}}
     %\tbl{TB: Changed from $A(x, p, q ,p',q')>0$, for all $(x,p,q,p',q') \in \Sigma \cap (L^+W \times TW \times P^{m_1}W \times  P^{m_2}W)$}
     %$A(x, p, q ,p',q')>0$, for all $(x,p,q,p',q') \in \Sigma \cap (L^+W \times TW \times P^{m_1}W \times  P^{m_2}W)$.
     
     %
     
     %
     \item\label{conditionyy} There is a constant $C>0$ such that for all $(x,p) \in \OVS M$,
     \[
      \|A(x,p, \cdot,\cdot,\cdot)\|_{L^1(\Sigma_{x,p})} :=   \int_{\Sigma_{x,p}} | A(x,p, q, p',q')  | dV(x,p \; q,p',q')\leq C.
      %\quad \text{for} \quad ,
     \]
% 
%      
%      \|A(x,p, \cdot, \cdot, \cdot)\|_{L^1(\Sigma_{x,p})} \leq C,$ for every $(x,p) \in \OVS M$.
%       %
     \item\label{conditionyyyy} For every $(x,p) \in \OVS M$ the function $F_{x,p}(\lambda) :=  \|A(x,\lambda p, \cdot, \cdot, \cdot)\|_{L^1(\Sigma_{x,\lambda p})}$, \tbl{$\lambda\in \R$}, is continuously differentiable at $\lambda=0$ and satisfies $F_{x,p}(0) = 0$. 
 \end{enumerate}
\end{definition}
If there is no reason to emphasize the set $W$ we just use the term \emph{admissible collision kernel}. The most important case is when $W$ is a time-like diamond as in the main theorem, see Figure~\ref{fig:W_pic}. The reader may take this as an assumption, although many of the steps in our main proof can be carried through for more general $W$. 
%Although many steps apply 
%Although many of the 
%We
% In Definition \ref{good-kernels}, we set $L^+W$ to be the light-like bundle of future-directed vectors over $W$, $\PP W  = \overline{\PP} W \setminus L^+ W$,
%   \[
%   \|A(x,p, \cdot,\cdot,\cdot)\|_{L^1(\Sigma_{x,p})} :=   \int_{\Sigma_{x,p}} | A(x,p, q, p',q')  |dV(x,p ; q,p',q'), \quad \text{for} \quad (x,p) \in \OVS M,
%  \]
%  and
%  \[
% \text{supp} (x \mapsto A(x, \cdot, \cdot, \cdot, \cdot ) ) := \text{cl} \{ x \in M :  \exists (p,q,p',q' ) \in T_x M^4 \text{ such that }  A(x,p,q,p',q') \neq 0 \}   ,
% \]
% where $\text{cl}$ refers to the topological closure.

%Conditions (\ref{conditiony}) and (\ref{condition4}) in Definition \ref{good-kernels} ensure that the kernel defines reasonable binary collisions in the unknown set $W$. 
We note that the condition \eqref{condition4} ensures that  colliding  particles traveling at less than the speed of light scatters lightlike particles.  
%  \footnote{Our proofs carry through with the following weaker assumption: For each $x \in W$, let $\gamma_{(x,p)}$ be the geodesic with initial data $(x,p)$, and suppose there exists a set $l=l_x  \subset  L^+_x M$ of future-directed light-like vectors such that $G_{l}^+ := \{ y \in M : y = \gamma_{(x,p)} (s), \ s\in [0,\infty), \  p \in l \}$ satisfies $G_{l}^+ = \mathcal{L}^+(x)$ and $A(x, p , q , p' , q' ) > 0$ for every $p \in l$ and $ p',q' \in \mathcal{P}_x^+W$ in our notation. }
%  ~\f{TB: how is this wording? {\color{red} ''massive particle'' means something else in physics. I changed ''massive'' to ''with mass'' -A}} 
The conditions
%(\ref{conditiony})
%-(\ref{conditionyy}) and (\ref{conditionyyyy})
(\ref{conditionyy}) and (\ref{conditionyyyy}) are imposed to have control of collisions of relatively high and low momenta particles. 
These conditions are required in our proof of the well-posedness of the Cauchy problem for the Boltzmann equation \eqref{boltzmann}: 

%With the assumption that the collision kernel is admissible, we prove well-posedness of \eqref{boltzmann}:
\begin{theorem}\label{boltz-exist}

Let $(M, g)$ be a globally hyperbolic $C^\infty$-smooth Lorentzian manifold. Let also $\mathcal{C}$ be a Cauchy surface of $M$ and $K\subset \OVS \mathcal{C}^+$ be compact. % and $\XX$ its associated geodesic vector field. %$\compp$ be a compact set in $\OVS ((0, \infty) \times N) $ and set 
Assume that $A: \Sigma \to \mathbb{R}$ is an admissible collision kernel in the sense of Definition \ref{good-kernels}.
%Assume also that $\text{supp}(x \mapsto A(x,\cdot,\cdot,\cdot,\cdot))$ is compact. 

Then, there are open neighbourhoods $B_1 \subset C_K(\OVS \mathcal{C}^+ )$ and $B_2\subset C_b( \OVS  M )$ of the respective origins such that if $f \in B_1$, the relativistic Boltzmann problem \eqref{boltzmann} with source $f$ has a unique solution $u\in B_2$. Further, there is a constant $c_{A,K}>0$ such that~\f{Norm symbols changed.}
\[ \tjb{\|u\|_{C( \OVS M )}\le c_{A,K}\|f\|_{C(\OVS M)}.}\]

\end{theorem}

The well-posedness of~\eqref{boltzmann} has also been addressed in the following works. For exponentially bounded data, and an $L^1$-type bound on the cross-section of the collision kernel, it was shown in \cite{Bichteler} that a short-time unique solution to \eqref{boltzmann} exists in the setting of a $4$-dimensional, globally hyperbolic spacetime. Also for globally hyperbolic geometries, under conditions which require the collision operator to be a continuous map between certain weighted Sobolev spaces, it was proven in \cite{Bancel} that a unique short-time solution exists to \eqref{boltzmann} in arbitrary dimension. If the geometry of $(M,g)$ is close to Minkowski in a precise sense, the collision kernel satisfies certain growth bounds and the initial data satisfied a particular form of exponential decay, then unique global solutions exist to the Cauchy problem for the Boltzmann equation~\cite{Glassey}. We refer to~\cite{Choquet-Bruhat}, \cite{Ringstrom} and \cite{Rendall} for more information about the well-posedness of~\eqref{boltzmann}. Also, the recent paper~\cite{lai-uhlmann-yang}, related to our work, contains a well-posedness result in Euclidean spaces.

We are now ready to present our main theorem. In our theorem, measurements of solutions to the Boltzmann equation are made on a neighborhood $V$ of a timelike geodesic $\hat\mu$ in $(M,g)$.  We prove that measurements made on $V$ both determines a subset $W$ of $M$ and the restriction of the metric to $W$ (up to isometry). The subset $W$ is naturally limited by the finite propagation speed of light. The situation is illustrated in Figure~\ref{fig:W_pic} below. 
 \begin{figure}[ht!]
    \centering
    \includegraphics[scale=0.3]{scattering-boltzmann3.pdf}
    \caption{Illustration of the timelike geodesic $\hat\mu$, known set $V$, and the yet unknown set $W$.}
    \label{fig:W_pic}
\end{figure}%, of the Lorentzian manifold $(M,g)$, which is naturally 

\tbl{Before we continue, we introduce our notation. We consider source-to-solutions maps of the Bolzmann equation \eqref{boltzmann} defined on sources, which are supported on different compact sets $K\subset \OVS M$. As follows from Theorem \ref{boltz-exist}, for each such $K$ the source-to-solution map $B_1\to B_2\subset C_b(\OVS M)$ of the Boltzmann equation is well defined, where $B_1\subset C_K(\OVS \mathcal{C}^+)$. In this case, we denote $B_{1,K}=B_K$. In the next theorem we consider source-to-solution maps of Boltzmann equations defined on
\begin{equation}\label{union_domain}
 \mathcal{B}:=\bigcup_{\{K:\s \pi(K)\subset Z\}} B_{1,K} \subset C_c(\OVS \mathcal{C}^+),
 \end{equation}
 where $Z$ is a fixed compact subset of $M$.}


% Below in the theorem $e$ will be some auxiliary Riemannian metric on $M$, $K\subset \OVS M$ a compact set and $B_r$, $r>0$, the bundle of balls of radius $r$ of $TM$ in the metric $e$. In this case, $B_1\setminus B_{1/2}$ is a bundle over $M$ whose fibers look like hollow balls. The set $K$ is chosen so that we may approximate lightlike vectors (of length between $1/2$ and $1$ in the metric $e$) by timelike vectors of $K$. We also denote $K_\pi:=\pi(K)$.
% We will assume $(B_1\setminus B_{1/2})\cap \OVS \pi(K) \subset K$ so that we may approx

\begin{theorem}\label{themain}
Let $(M_1, g_1)$ and $(M_2,g_2)$ be globally hyperbolic $C^\infty$-smooth Lorentzian manifolds of dimension $\geq 3$.~\f{Dimension added.} Assume that $V$ is a mutual open subset of $M_1$ and $M_2$ and that $g_1|_V=g_2|_V$. Let $\mu : [-1,1] \rightarrow V$ be a smooth timelike curve. Let also $-1< s^{-} < s^{+} < 1$, and define $x^{\pm}:= \mu(s^{\pm})$ and 
\[
W_j :=  I_j^-(x^{+}) \cap I_j^+(x^{-}), \quad j=1,2. %is a relatively compact open set. 
\]
% Let $K\subset \OVS M$ be compact set such that $\mu[-1,1]\subset \subset \pi(K)\subset V$ and $(B_1\setminus B_{1/2}) \s \cap\s \OVS (K_\pi) \subset K$.
% $(B_1\setminus B_{1/2})\cap \OVS M\subset K$.

Let $Z\subset V\subset M$ be a compact set such that $\mu[-1,1]\subset\subset Z$.

\tbl{Suppose that $A_1$ and $A_2$ are admissible kernels in the sense of Definition \ref{good-kernels}. Assume that the source-to-solution maps  of the Boltzmann equation on $(M_1,g_1)$ and $(M_2,g_2)$ with kernels $A_1$ and $A_2$ respectively agree,
\[
 \Phi_{2,\,L^+V}  = \Phi_{1,\,L^+V},
\]
on $\mathcal{B}$. Here $\mathcal{B}$ is as in \eqref{union_domain}.
% explained before the the union $\cup_K B_{1,K}\subset C_c(\OVS \mathcal{C}^+)$, where $K\subset \OVS M$ is any compact set such that $\mu[-1,1]\subset\subset \pi(K)$ and $B_{1,K}\subset C_K(\OVS \mathcal{C}^+)$ is the set $B_1\subset C_K(\OVS \mathcal{C}^+)$ in Theorem \ref{boltz-exist}.
}
% % % % % 
% % % % % \begin{enumerate}
% % % % % %    \item there exist open neighbourhoods $V_{\lambda} \subset M_\lambda$ of $\mu_{\lambda}$ and a diffeomorphism \\$\Xi :V_{1} \rightarrow V_{2}$  such that $g_{1}|_{V_{1}} = \Xi^* g_{2}|_{V_{2}}$ and $\mu_{1} = \Xi \circ \mu_{2}$;
% % % % %     \item $A_{j}\in C^\infty(\Sigma_{j})$ are admissible kernels %(see Definition \ref{good-kernels}) 
% % % % %     %for the Boltzmann equation 
% % % % %     %in $(\R\times N_\lambda,g_\lambda, \mu_\lambda)$;
% % % % %     \item \tbl{For all compact sets $K\subset \OVS M$ with $\pi_K:=\pi(K)\subset Z$, the source-to-solution maps $\Phi_{j,\,L^+V} : B_K \rightarrow C_b(L^+ V)$ for light observations} 
% % % % % %     \[
% % % % % %     \]
% % % % % %     
% % % % % of the Boltzmann equation \eqref{boltzmann} with kernel $A_j$, and  where $B_K$ is an open neighborhood of the origin in $C_K(\OVS V)$, satisfy %on $\OVS(M_\lambda)$ satisfy
% % % % % \[
% % % % % \Phi_{2,\,L^+V}  = \Phi_{1,\,L^+V}. % (T \Xi^{-1})^* \circ \Phi_{1,\,L^+V} \circ T\Xi^* .
% % % % % \]
% % % % % 
% % % % % %in a neighbourhood of origin in $C_c^\infty (\SP V_\lambda )$. 
% % % % % %{\color{red} (...on smooth test functions, or on distributions of %the form $h(x,p) = \delta(x_\R - t) f(x,p), \  f\in %C_c^\infty(TV), \ t\in \R $, or whatever we like )}.
% % % % % \end{enumerate}
%\end{enumerate}
Then there is an isometric $C^\infty$-smooth diffeomorphism $F: W_1 \rightarrow W_2$,
\[
 F^*g_2=g_1 \text{ on } W_1.
\]
% 
% F: W_1 \rightarrow W_2$ such that $F^* g_{2}$ is conformal to $g_{1}$. Moreover, writing $F^* g_{2} = c(x)g_1$, we have $c(x)\equiv 1$ for $x\in W_1$.
\end{theorem}

% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % ---------------------
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % % We will consider particles which undergo binary collisions. In this case, a second governing kinematic principle is conservation of momentum under collisions (also called \emph{elastic collisions}). That is, for particles of momenta $p$ and $q$ in $\OVS(M)$ which collide and result in two new particles of momenta $p'$ and $q' $(respectively), we assume that \[ p+q = p' + q'.\]
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % The behaviour of binary elastic collisions is characterized by a \emph{collision operator} %$\COLOP[u,v]$
% % % % % % % % % % % % % % % % % % %  \[
% % % % % % % % % % % % % % % % % % % \COLOP [u, v] (x,p)  
% % % % % % % % % % % % % % % % % % % %=  A(x,p,q, p', q')  \delta_{\tilde\Sigma } 
% % % % % % % % % % % % % % % % % % % =\int_{\Sigma_{x, p }}  \left[u (x,p) v (x,  q )  - u (x,p' ) v (x,  q' ) \right] A(x,p,q, p', q') dV (x,p \ ; \ q,p',q'),
% % % % % % % % % % % % % % % % % % % \]
% % % % % % % % % % % % % % % % % % % %where
% % % % % % % % % % % % % % % % % % % %\[
% % % % % % % % % % % % % % % % % % % %\Sigma_{x,p} := \{ ( p', q' , q) \in   T_x(\R \times N)^3 : p + q = p' + q' \}.
% % % % % % % % % % % % % % % % % % % %\]
% % % % % % % % % % % % % % % % % % % where $ dV (x,p \ ; \ q,p',q') $ is non-zero volume form on the submanifold 
% % % % % % % % % % % % % % % % % % % \[
% % % % % % % % % % % % % % % % % % % \Sigma_{x,p} := \{p\}\times  \{ (q,p',q')\in ( \overline{\mathcal{P}}_x M )^3  \,:\, p+q = p'+q'\} \subset (\overline{\mathcal{P}}_x M)^4,
% % % % % % % % % % % % % % % % % % % \]
% % % % % % % % % % % % % % % % % % % %\[
% % % % % % % % % % % % % % % % % % % % \overline{\mathcal{P}}_x^+ M := \{ (x,p) \in T_x M \setminus \{0 \} : -g(p,p)\geq 0, \ p \  \text{future-directed} \  \},
% % % % % % % % % % % % % % % % % % % %\]
% % % % % % % % % % % % % % % % % % % and $A\in C^\infty(\Sigma_{x, p })$ is a \emph{collision kernel} (also called a shock cross-section). %Essentially, this operator averages the numbers of 
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % For example, in a cosmological model, information may be observed radiation which is scattered by matter (dust, stars, plasma, etc.) present in the universe, and one might seek to determine the spacetime geometry. In condensed matter physics, one my be examining the behaviour of electron transport or electron-phonon excitations in a metal or semiconductor and wish to know what is the electrical resistivity of the media. In such situations, the geometry or resistivity may be described by a Lorentzian metric $g$ on a manifold $M$ which models the spacetime. Given observer measurements of particles on an open set $V\subset M$, our goal is to recover the metric $g$ and its conformal class on a larger region $W\supset V$. In this paper, we present a setting for which this is possible.
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % %, where the measurements recorded by an observer are the introduction of known sources of particles into the system at at some time and location and particles received at some detecting region at a later time. 
% % % % % % % % % % % % % % % % % % % % Information about the particle dynamics is recorded by an observer who may introduce known sources of particles into the system at at some time location and who may measure particles at some detecting region at a later time. 
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % %Before we formulate our main theorem, let us introduce some additional concepts. Let $V\subset M$ be open and let $\hat\mu : [-1,1] \rightarrow V$ be smooth timelike curve that represents an observer in the spacetime $(M,g)$. We assume that $V$ and the restrictoin
% % % % % % % % % % % % % % % % % % % We now formulate this setting precisely. We assume that the system (which includes the observer, particles, and media) is modelled by a $C^\infty$-smooth, globally hyperbolic Lorentzian spacetime $(M, g)$. The Lorentzian metric $g$ is a smooth $(0,2)-$tensor with signature $(-, +, \dots, +)$ (which we think of as describing gravity or resistivity). Global hyperbolicity implies that there is a Cauchy hypersurface $N\subset M$ such that $(M,g)$ can be expressed as the product $M = \R\times N$ and $g = -g_{00}dt^2 + g_t$ for some $C^\infty$-smooth function $g_{00}:M\to (0,\infty)$ and family Riemannian metrics $g_t$ on $N$, for $t\in \R$. An observer in this spacetime is represented by a $C^\infty$-smooth timelike curve $\hat\mu : [-1,1] \rightarrow M$. We assume that we know the metric $g$ in a small open neighbourhood $V$ of $\hat\mu$, where the observer may take measurements.  
% % % % % % % % % % % % % % % % % % % %Our goal is to recover the metric $g$ on a region of media $W\subset M$ from the observer's measurements.
% % % % % % % % % % % % % % % % % % % The region of media $W\subset M$ we seek to understand is defined as follows. For $-1< s^{-} < s^{+} < 1$, set $x^{\pm}:= \hat\mu(s^{\pm})$. Then  $W :=  I^-(x^{+}) \cap I^+(x^{-})$. See Figure \ref{fig:W_pic}.
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % %  \begin{figure}
% % % % % % % % % % % % % % % % % % % %     \centering
% % % % % % % % % % % % % % % % % % % %     \includegraphics[scale=0.25]{pictures/scattering-boltzmann3.pdf}
% % % % % % % % % % % % % % % % % % % %     \caption{Illustration of the timelike geodesic $\hat\mu$, known set $V$, and the yet unknown set $W$.}
% % % % % % % % % % % % % % % % % % % %     \label{fig:W_pic}
% % % % % % % % % % % % % % % % % % % % \end{figure}
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % %We will consider particles\footnote{For our purposes, we refer to particles (photons, electrons, dust, etc.) and quasiparticles (phonons, plasmons, etc.) as simply \emph{particles}.} (photons, electrons, dust, phonons, plasmons, etc.) which undergo binary collisions. 
% % % % % % % % % % % % % % % % % % % We represent particles\footnote{For our purposes, we refer to particles (photons, electrons, dust, etc.) and quasiparticles (phonons, plasmons, etc.) as simply \emph{particles}.} (photons, electrons, dust, phonons, plasmons, etc.) as either a distribution $u\in\mathcal{D}'(S)$ or conormal distribution $u\in I^{l}(N^*S)$, $l\in \R$, for some submanifold $S$ of \emph{phase space}. We denote the particle phase space of all nonzero causal vectors $p\in TM$ by $\overline{\PP} M$ and the fibre of this vector bundle at $x\in M$ by $\overline{\PP} _x M$. We write $\OVS M\subset TM$ for the restriction of $\overline{\PP} M$ to future-directed causal vectors.
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % %One can think of such distributions as an average of an ensemble of collections of possible particle states.
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % The kinetic theory we adopt for particles is characterized by two principles. The first is causal one, namely that particles travel along trajectories defined by either future-directed timelike geodesics (for positive mass particles) or future-directed lightlike geodesics (in the case of zero mass particles). 
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % In the absence of collisions and external forces, the kinematics of a particle distribution $u$ is captured by the \emph{Vlasov equation} \cite{Ringstrom}, \cite{Rendall} (or Liouville-Vlasov equation \cite{Choquet-Bruhat})  
% % % % % % % % % % % % % % % % % % % \[
% % % % % % % % % % % % % % % % % % % \XX u(x,p) =0 \quad \text{for } (x,p)\in \OVS M,
% % % % % % % % % % % % % % % % % % % \]
% % % % % % % % % % % % % % % % % % % where $\mathcal{X}: C^\infty (TM) \rightarrow C^\infty (TM) $ is the geodesic vector field. Here $\OVS M$ is the the subset of $TM$ of the future directed causal vectors. 
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % We will consider particles which undergo binary collisions. In this case, a second governing kinematic principle is conservation of momentum under collisions (also called \emph{elastic collisions}). That is, for particles of momenta $p$ and $q$ in $\OVS(M)$ which collide and result in two new particles of momenta $p'$ and $q' $(respectively), we assume that \[ p+q = p' + q'.\]
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % The behaviour of binary elastic collisions is characterized by a \emph{collision operator} %$\COLOP[u,v]$
% % % % % % % % % % % % % % % % % % %  \[
% % % % % % % % % % % % % % % % % % % \COLOP [u, v] (x,p)  
% % % % % % % % % % % % % % % % % % % %=  A(x,p,q, p', q')  \delta_{\tilde\Sigma } 
% % % % % % % % % % % % % % % % % % % =\int_{\Sigma_{x, p }}  \left[u (x,p) v (x,  q )  - u (x,p' ) v (x,  q' ) \right] A(x,p,q, p', q') dV (x,p \ ; \ q,p',q'),
% % % % % % % % % % % % % % % % % % % \]
% % % % % % % % % % % % % % % % % % % %where
% % % % % % % % % % % % % % % % % % % %\[
% % % % % % % % % % % % % % % % % % % %\Sigma_{x,p} := \{ ( p', q' , q) \in   T_x(\R \times N)^3 : p + q = p' + q' \}.
% % % % % % % % % % % % % % % % % % % %\]
% % % % % % % % % % % % % % % % % % % where $ dV (x,p \ ; \ q,p',q') $ is non-zero volume form on the submanifold 
% % % % % % % % % % % % % % % % % % % \[
% % % % % % % % % % % % % % % % % % % \Sigma_{x,p} := \{p\}\times  \{ (q,p',q')\in ( \overline{\mathcal{P}}_x M )^3  \,:\, p+q = p'+q'\} \subset (\overline{\mathcal{P}}_x M)^4,
% % % % % % % % % % % % % % % % % % % \]
% % % % % % % % % % % % % % % % % % % %\[
% % % % % % % % % % % % % % % % % % % % \overline{\mathcal{P}}_x^+ M := \{ (x,p) \in T_x M \setminus \{0 \} : -g(p,p)\geq 0, \ p \  \text{future-directed} \  \},
% % % % % % % % % % % % % % % % % % % %\]
% % % % % % % % % % % % % % % % % % % and $A\in C^\infty(\Sigma_{x, p })$ is a \emph{collision kernel} (also called a shock cross-section). %Essentially, this operator averages the numbers of 
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % Putting these concepts together, given an initial state of no particles on a Cauchy surface $\mathcal{C}\subset M$ and a particle source $f\in \mathcal{D}'( \OVS M)$, the kinematics of a distribution of particles $u \in \mathcal{D}'( \OVS M)$ is given by the \emph{relativistic Boltzmann equation} \cite{Choquet-Bruhat}[p. 328, Eq. 7.1], \cite{Ringstrom}[p. 154, Eq. 10.6], \cite{Rendall}[p. 44, Eq. 3.38]
% % % % % % % % % % % % % % % % % % % \begin{alignat}{2}\label{boltzmann}
% % % % % % % % % % % % % % % % % % % %\begin{gathered}
% % % % % % % % % % % % % % % % % % % \mathcal{X}u(x,p)-\COLOP[u,u](x,p)&= f(x,p), \quad && (x,p)\in
% % % % % % % % % % % % % % % % % % % \OVS M \nonumber \\
% % % % % % % % % % % % % % % % % % % u(x,p)&= 0, \quad && (x,p)\in \OVS \mathcal{C}^-,
% % % % % % % % % % % % % % % % % % % %\end{gathered}
% % % % % % % % % % % % % % % % % % % \end{alignat}
% % % % % % % % % % % % % % % % % % % where $\mathcal{C}^-\subset M$ is the causal past of the Cauchy surface $\mathcal{C}$. Though we do not consider them, the physical quantities of invariant mass, total energy, and total momentum can be defined and shown to be conserved under the relativistic Boltzmann kinematic model (see \cite{Choquet-Bruhat}, \cite{Ringstrom}, or \cite{Rendall} for more details).
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % Observer measurements in $V$ about the particle system are captured by the \emph{source-to-solution map for light observations}, which is the assignment
% % % % % % % % % % % % % % % % % % % \begin{equation}\label{light-source-soln}
% % % % % % % % % % % % % % % % % % %  \Phi_{L^+V} : B_V \rightarrow C( L^+V ) ,\quad \Phi_{L^+V}(f) := \Phi(f)|_{L^+V},
% % % % % % % % % % % % % % % % % % % \end{equation}
% % % % % % % % % % % % % % % % % % % where $L^+V \subset TM$ is the bundle of lightlike causal vectors on $V$, $\Phi$ is the \emph{source-to-solution map} for the relativistic Boltzmann equation
% % % % % % % % % % % % % % % % % % % %{\color{red}(I cleaned this a little bit and restricted the image into the light-like bundle --Antti)}
% % % % % % % % % % % % % % % % % % % \begin{equation}\label{supposedtolooklikethis}
% % % % % % % % % % % % % % % % % % % \Phi : B \rightarrow 
% % % % % % % % % % % % % % % % % % % %C_{\OVS([0,\infty)\times N) }^0  ( \OVS V ) 
% % % % % % % % % % % % % % % % % % % C( \OVS M ), \quad \Phi(f) = u,
% % % % % % % % % % % % % % % % % % % \end{equation}
% % % % % % % % % % % % % % % % % % % for $u \in  C( \OVS M )$ which solves \eqref{boltzmann} with source $f$, $B$ is a neighbourhood of the origin in $C_c^\infty \big( \SP ((0,\infty) \times N) \big)$, and $B_V = B \cap C_c^\infty(\SP V )$. Here we define $\SP V = \OVS P\setminus L^+V$. Loosely speaking, the operator $\Phi_{L^+V}$ corresponds to measuring the photons received in our known set $V$ from particle interactions governed by the Boltzmann equation \eqref{boltzmann}.
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % %The existence of the sets $B$ and $B_V$ are given and source-to-solution maps $\Phi$ and $ \Phi_{L^+V}$ are well defined when the Boltzmann equation \eqref{boltzmann} has a unique solution. 
% % % % % % % % % % % % % % % % % % % Known uniqueness and existence results to \eqref{boltzmann} depend inextricably on the properties of the collision kernel $A$. For general collision kernels, local existence of solutions to \eqref{boltzmann} is not known. Complicating the analysis is the fact that there are very few known physical restrictions on the form of the collision kernel \cite[p. 155]{Ringstrom}. Further, in the case of Israel molecules, where one has a reasonable description of what the collision kernel should be, the term 
% % % % % % % % % % % % % % % % % % % \[
% % % % % % % % % % % % % % % % % % % \COLOP_{loss}[u, v] (x,p):= u (x,p) \int_{\Sigma_{x, p }}   v (x,  q ) A(x,p,q, p', q') dV_{x,p} (q,p',q'). %dV (x,p \ ; \ q,p',q') 
% % % % % % % % % % % % % % % % % % % \]
% % % % % % % % % % % % % % % % % % % cannot be written as a continuous map between weighted $L^p$ spaces (see Appendix F in \cite{Ringstrom} for details). It is not eiher always clear what is the relationship between conditions on the collision operator $\COLOP$ and the induced conditions on its collision kernel $A$.
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % Thus, current results for existence and uniqueness of solutions to \eqref{boltzmann} have imposed various restrictions on the collision kernel, as well as on the geometry and the data. We highlight a selected few representatives of the literature next. For small-data and an $L^1$-type bound on the collision kernel, it was shown in \cite{Bichteler} that a short-time unique solution to \eqref{boltzmann} exists in the globally hyperbolic setting. Also for globally hyperbolic geometries, under conditions which require the collision operator to be a continuous map between certain weighted Sobolev spaces, it was proven in \cite{Bancel} that a unique short-time solution exists to \eqref{boltzmann}. If the geometry of $(M,g)$ is close to Minkowski in a precise sense, the collision kernel satisfies certain growth bounds, and the initial data satisfied a particular form of exponential decay, then unique global solutions exist to the Boltzmann Cauchy problem \cite{Glassey}. For more information on the Cauchy problem \eqref{boltzmann}, please consult the refernces \cite{Choquet-Bruhat}, \cite{Ringstrom}, and \cite{Rendall}.
% % % % % % % % % % % % % % % % % % %  
% % % % % % % % % % % % % % % % % % % To address the problem of uniqueness of solutions to \eqref{boltzmann}, in this paper we consider collision kernels of the following type.
% % % % % % % % % % % % % % % % % % % \begin{definition}[Admissible Kernels]\label{good-kernels}
% % % % % % % % % % % % % % % % % % % %Let $( M = \R\times N,g)$ be a Lorentzian spacetime, $r_1,r_2>0$ and $\hat\mu : [-1,1] \rightarrow (0,\infty) \times N$ be a smooth timelike curve.  For $-1< s^{-} < s^{+} < 1$, set $x^{\pm}:= \hat\mu (s^{\pm})$ and $W :=  I^-(x^{+}) \cap I^+(x^{-})$. 
% % % % % % % % % % % % % % % % % % % Let $\Sigma := \bigcup_{(x,p) \in \overline{\PP}M} \Sigma_{x,p} \subset TM^4$. We say that $A:\Sigma\subset T M^4\to\R$ is an \emph{admissible collision kernel} if $A$ satisfies
% % % % % % % % % % % % % % % % % % % \begin{enumerate}
% % % % % % % % % % % % % % % % % % %      \item\label{conditiony} $A\in C^\infty(\Sigma  )$. 
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % %      \item\label{condition4}  $A(x, p, q ,p',q')>0$, for all $(x,p,q,p',q') \in \Sigma \cap (L^+W \times \overline{\PP} W \times \PP W \times  \PP W)$. \tbl{TB: Changed from $A(x, p, q ,p',q')>0$, for all $(x,p,q,p',q') \in \Sigma \cap (L^+W \times TW \times P^{m_1}W \times  P^{m_2}W)$}
% % % % % % % % % % % % % % % % % % %      %$A(x, p, q ,p',q')>0$, for all $(x,p,q,p',q') \in \Sigma \cap (L^+W \times TW \times P^{m_1}W \times  P^{m_2}W)$.
% % % % % % % % % % % % % % % % % % %      
% % % % % % % % % % % % % % % % % % %      %
% % % % % % % % % % % % % % % % % % %      \item\label{conditionyyyyy} $\text{supp} (x \mapsto A(x, \cdot, \cdot, \cdot, \cdot ) )$ is compact.
% % % % % % % % % % % % % % % % % % %      %
% % % % % % % % % % % % % % % % % % %      \item\label{conditionyy} There exists a constant $C>0$ such that $\|A(x,p, \cdot,\cdot,\cdot)\|_{L^1(\Sigma_{x,p})} \leq C,$ for every $(x,p) \in \OVS M$.
% % % % % % % % % % % % % % % % % % %       %
% % % % % % % % % % % % % % % % % % %      \item\label{conditionyyyy} For every $(x,p) \in \OVS M$ the function $F_{x,p}(\lambda) :=  \|A(x,\lambda p, \cdot,\cdot,\cdot)\|_{L^1(\Sigma_{x,\lambda p})}$ is continuously differentiable at $\lambda=0$ and satisfies $F_{x,p}(0) = 0$. 
% % % % % % % % % % % % % % % % % % %  \end{enumerate}
% % % % % % % % % % % % % % % % % % % \end{definition}
% % % % % % % % % % % % % % % % % % % In Definition \ref{good-kernels}, we set $L^+W$ to be the light-like bundle of future-directed vectors over $W$, $\PP W  = \overline{\PP} W \setminus L^+ W$,
% % % % % % % % % % % % % % % % % % %   \[
% % % % % % % % % % % % % % % % % % %   \|A(x,p, \cdot,\cdot,\cdot)\|_{L^1(\Sigma_{x,p})} :=   \int_{\Sigma_{x,p}} | A(x,p, q, p',q')  |dV(x,p ; q,p',q'), \quad \text{for} \quad (x,p) \in \OVS M,
% % % % % % % % % % % % % % % % % % %  \]
% % % % % % % % % % % % % % % % % % %  and
% % % % % % % % % % % % % % % % % % %  \[
% % % % % % % % % % % % % % % % % % % \text{supp} (x \mapsto A(x, \cdot, \cdot, \cdot, \cdot ) ) := \text{cl} \{ x \in M :  \exists (p,q,p',q' ) \in T_x M^4 \text{ such that }  A(x,p,q,p',q') \neq 0 \}   ,
% % % % % % % % % % % % % % % % % % % \]
% % % % % % % % % % % % % % % % % % % where $\text{cl}$ refers to the topological closure.
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % Conditions (\ref{conditiony}) and (\ref{condition4}) in Definition \ref{good-kernels} ensure that the kernel defines reasonable binary collisions in the unknown set $W$. In particular, we note that condition \eqref{condition4} ensures that colliding particles of masses $r_1$, $r_2>0$ and positive energies in $W$ scatters light in every spatial direction  \footnote{Our proofs carry through with the following weaker assumption: For each $x \in W$, let $\gamma_{(x,p)}$ be the geodesic with initial data $(x,p)$, and suppose there exists a set $l=l_x  \subset  L^+_x M$ of future-directed light-like vectors such that $G_{l}^+ := \{ y \in M : y = \gamma_{(x,p)} (s), \ s\in [0,\infty), \  p \in l \}$ satisfies $G_{l}^+ = \mathcal{L}^+(x)$ and $A(x, p , q , p' , q' ) > 0$ for every $p \in l$ and $ p',q' \in \mathcal{P}_x^+W$ in our notation. }. The continuity conditions 
% % % % % % % % % % % % % % % % % % % %(\ref{conditiony})
% % % % % % % % % % % % % % % % % % % %-(\ref{conditionyy}) and (\ref{conditionyyyy})
% % % % % % % % % % % % % % % % % % % (\ref{conditionyyyyy})-(\ref{conditionyyyy}) 
% % % % % % % % % % % % % % % % % % % are those we required to show unique local existence of solutions to problem \eqref{boltzmann}. 
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % % With the assumption that the collision kernel is admissible, we prove a uniqueness result to \eqref{boltzmann}:
% % % % % % % % % % % % % % % % % % % % \begin{theorem}\label{boltz-exist}
% % % % % % % % % % % % % % % % % % % % Let $(M, g)$ be a globally hyperbolic $C^\infty$-smooth Lorentzian manifold, $\mathcal{C}$ be a Cauchy surface of $M$, and  $\mathcal{C}^+ $ be the causal future of the surface $\mathcal{C}$.  Assume that $A: \Sigma \to \mathbb{R}$ is an admissible collision kernel in the sense of Definition \ref{good-kernels}.
% % % % % % % % % % % % % % % % % % % % %Assume also that $\text{supp}(x \mapsto A(x,\cdot,\cdot,\cdot,\cdot))$ is compact. 
% % % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % % Then, there are open neighbourhoods $B_1 \subset C_c(\OVS \mathcal{C}^+ )$ and $B_2\subset C( \OVS  M )$ of the respective origins such that if $f \in B_1$, the relativistic Boltzmann problem \eqref{boltzmann} with source $f$ has a unique solution $u\in B_2$. Further, there is a constant $C>0$ such that
% % % % % % % % % % % % % % % % % % % % \[ ||u||_{C( \OVS M )}\le C||f||_{C(\OVS M)}.\]
% % % % % % % % % % % % % % % % % % % % \end{theorem}
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % From Theorem \ref{boltz-exist} we obtain that our measurement data $ \Phi_{L^+V}$ is then a well-defined map. In this case, we prove that the source to solution map $ \Phi_{L^+V}$ uniquely determines the Lorentzian metric $g$ and its conformal class.
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % \begin{theorem}\label{themain}
% % % % % % % % % % % % % % % % % % % Let $(M_\lambda, g_\lambda)$, $\lambda =1,2$ be two globally hyperbolic, $C^\infty$-smooth, Lorentzian manifolds. Let $\mu_{\lambda} : [-1,1] \rightarrow (0,\infty) \times N_\lambda$ be given smooth timelike curves, and for $-1< s^{-} < s^{+} < 1$, set $x_{\lambda}^{\pm}:= \mu^{\lambda}(s^{\pm})$ and $W_\lambda :=  I^-(x_{\lambda}^{+}) \cap I^+(x_{\lambda}^{-}).$ %is a relatively compact open set.
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % Suppose that 
% % % % % % % % % % % % % % % % % % % \begin{enumerate}
% % % % % % % % % % % % % % % % % % %     \item there exist open neighbourhoods $V_{\lambda} \subset M_\lambda$ of $\mu_{\lambda}$ and a diffeomorphism \\$\Xi :V_{1} \rightarrow V_{2}$  such that $g_{1}|_{V_{1}} = \Xi^* g_{2}|_{V_{2}}$ and $\mu_{1} = \Xi \circ \mu_{2}$;
% % % % % % % % % % % % % % % % % % %     \item $A_{\lambda} \in C^\infty(\Sigma_{\lambda})$ are admissible kernels %(see Definition \ref{good-kernels}) 
% % % % % % % % % % % % % % % % % % %     %for the Boltzmann equation 
% % % % % % % % % % % % % % % % % % %     %in $(\R\times N_\lambda,g_\lambda, \mu_\lambda)$;
% % % % % % % % % % % % % % % % % % %     \item The source-to-solution maps for light observations,   
% % % % % % % % % % % % % % % % % % %     \[\Phi_{\lambda,\,L^+V} : B_\lambda \rightarrow C( \mathcal{L}^+ V ), \ \ \lambda = 1,2,
% % % % % % % % % % % % % % % % % % %     \]
% % % % % % % % % % % % % % % % % % %     of the Boltzmann equation \eqref{boltzmann} on $\OVS(M_\lambda)$ satisfy
% % % % % % % % % % % % % % % % % % % \[
% % % % % % % % % % % % % % % % % % % \Phi_{2,\,L^+V}  =  (T \Xi^{-1})^* \circ \Phi_{1,\,L^+V} \circ T\Xi^* .
% % % % % % % % % % % % % % % % % % % \]
% % % % % % % % % % % % % % % % % % % %in a neighbourhood of origin in $C_c^\infty (\SP V_\lambda )$. 
% % % % % % % % % % % % % % % % % % % %{\color{red} (...on smooth test functions, or on distributions of %the form $h(x,p) = \delta(x_\R - t) f(x,p), \  f\in %C_c^\infty(TV), \ t\in \R $, or whatever we like )}.
% % % % % % % % % % % % % % % % % % % \end{enumerate}
% % % % % % % % % % % % % % % % % % % 
% % % % % % % % % % % % % % % % % % % Then there is a diffeomorphism $F: W_1 \rightarrow W_2$ such that $F^* g_{2}$ is conformal to $g_{1}$. Moreover, writing $F^* g_{2} = c(x)g_1$, we have $c(x)\equiv 1$ for $x\in W_1$.
% % % % % % % % % % % % % % % % % % % \end{theorem}

\tbl{Note that %we could also prove a slightly more general theorem. 
alternative to $V$ being a mutual open set of $M_1$ and $M_2$, we could instead assume that there are open sets $V_1\subset M_1$ and $V_2\subset M_2$ and an isometry $\mathcal{I}:V_1\to V_2$ so that the corresponding source-to-solution maps $\Phi_{j,L^+V_j}$, $j=1,2$, satisfy $\Phi_{1,L^+V_1}\mathcal{I}^*=\mathcal{I}^*\Phi_{2,L^+V_2}$. In this case there would be an isometry $W_1\to W_2$. We work with the assumption that $V$ is a mutual open set for simplicity.}

Inverse problems have been studied for equations with various nonlinearity types. Many of the earlier works rely on the fact that a solution to a related linear inverse problem exists. However, it was shown in Kurylev-Lassas-Uhlmann~\cite{Kurylev2018} that the nonlinearity can be used as a beneficial tool to solve inverse problems for nonlinear equations. They proved that local measurements of the scalar wave equation with a quadratic nonlinearity on a Lorentzian manifold determines \tjb{topological, differentiable, and conformal structure of the Lorentzian manifold}. Our proof of Theorem~\ref{themain}, which we explain shortly in the next section, builds upon this work ~\cite{Kurylev2018}. %We explain shortly the proof in the next section.

Recently, Lai, Uhlmann and Yang \cite{lai-uhlmann-yang} studied an inverse problem for the Boltzmann equation in the Euclidean setting. With an $L^1$ bound and symmetry constraint on the collision kernel, they show that one may reconstruct the collision kernel from boundary %the Albedo operator~ --  that is, 
measurements. % of the incoming and outgoing particle flux and the boundary of the Euclidean manifold.  
% Also recently, for compact manifolds with boundary, Oksanen, Salo, Stefanov, and Uhlmann \cite{OSSU} have shown that is it possible to determine the scattering relation, X-ray transform, and boundary expansion of operators of real principal type from Cauchy data on the boundary.
% 
% 
% There is a richer history for the study of inverse problems for linear versions of the Boltzmann equation. 
Linear equations such as Vlasov, radiative transfer (also called linear Boltzmann), or generalized transport equations model kinematics of particles which do not undergo collisions. We list a very modest selection of the literature on inverse problems for these equations next.  In Euclidean space, Choulli and Stefanov \cite{CS-1} showed that one can recover the absorption and production parameters of a radiative transfer equation from measurements of the particle scattering. They also showed that an associated boundary operator, \tjb{called the} Albedo operator, determines the absorption and production parameters for radiative transfer equations in \cite{CS-2} and \cite{CS-3}. Other results for the recovery of the coefficients of a radiative transfer equation in Euclidean space from the Albedo operator have been proven by Tamasan \cite{Tamasan}, Tamasan and Stefanov \cite{TamasanStefanov}, Stefanov and Uhlmann \cite{StefanovUhlmann}, Bellassoued and Boughanja \cite{BellassouedBoughanja}, and Lai and Li \cite{LaiLin}. Under certain curvature constraints on the metric, an inverse problem for a radiative transfer equation was studied in the Riemannian setting by McDowall \cite{McDowall1}, \cite{McDowall2}. A review of some of these and other inverse problems for radiative transfer and linear transportation equations is given by Bal \cite{GBal-1}. %\cite{Bal-LM}, \cite{Bal-J1}, \cite{Bal-J2}

The mentioned work~\cite{Kurylev2018} invented a \emph{higher order linearization method} for inverse problems of nonlinear equations in the Lorentzian setting for the wave equation. Other works studying inverse problems for nonlinear hyperbolic equations by using the higher order linearization method include: Lassas, Oksanen, Stefanov and Uhlmann \cite{lassas-oksanen-stefanov-uhlmann}; Lassas, Uhlmann and Wang \cite{lassas-uhlmann-wang-semi}, \cite{lassas-uhlmann-wang-emeq}; and Wang and Zhou \cite{wang-zhou}; Lassas, Liimatainen, Potenciano-Machado and Tyni~\cite{lassas2020uniqueness}. The higher order linearization method in inverse problems for nonlinear elliptic equations was used recently in Lassas, Liimatainen, Lin and Salo~\cite{lassas2019inverse} and Feizmohammadi and Oksanen~\cite{feizmohammadi2020inverse}, and in the partial data case in Krupchyk and Uhlmann~\cite{krupchyk2020remark} and Lassas, Liimatainen, Lin and Salo~\cite{lassas2019partial}.

%These results adapt a method of proof first appearing in the excellent work of \cite{Kurylev2018}. We also build upon the work of \cite{Kurylev2018}. Below we motivate our approach to the proof of Theorem \ref{themain}. %we now summarize the main ideas we use from \cite{Kurylev2018}.

%From light which radiates out from an unknown, compact domain of the spacetime and whose signal is received in a neighbourhood of the observer, Kurylev, Lassas, and Uhlmann \cite{Kurylev2018} proved that this information allows one to determine the topological and conformal structure of the unknown region. The authors also considered a wave equation with a quadratic nonlinearity and showed that from knowledge of the source-to-solution map for the wave equation restricted to a known neighbourhood of the observer one can learn the metric in a larger, unknown region of the spacetime. Two key results of this work were that (a) one can parametrize the unknown domain by the ``first observation of light'' sets, and (b) that the presence of the nonlinearity enabled them to obtain a stronger result then what was currently known for the linear problem. 

%which exploits the fact that the source to solution map for the wave problem captures information about the nonlinear terms appearing in the wave equation.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Summary
%


\subsection{Theorem \ref{themain} proof summary}\label{proof_summary_main_thm} Now we will explain the key ideas in our proof of Theorem \ref{themain}. To begin let $\hat\mu:[-1,1]\to M$ be a future directed, timelike geodesic and let $V$ be an open neighbourhood of the graph of $\hat\mu$ where we do measurements. For some $-1<s^-<s^+<1$, let $x^\pm=\mu(s^\pm)$, $W=I^-(x^+)\cap I^+(x^-)$ and $w\in W$. We adapt the method of higher order linearization introduced in~\cite{Kurylev2018} for the nonlinear wave equation to our Boltzmann setting \eqref{boltzmann}. Using this approach, we use the nonlinearity to produce a point source at $w$ for the linearized Boltzmann equation. 

The point source at $w$ is generated formally as follows. Let $\mathcal{C}$ be a Cauchy surface in $M$ and  $f_1,f_2\in C_c(\OVS V)$ be two sources of particles. For sufficiently small parameters $\eps_1$ and $\eps_2$, let $u_{\eps_1f_1+\eps_2f_2}$ be the solution to
\begin{equation}%\label{boltz-intro}
\begin{split}
\mathcal{X}u_{\epsilon_{1}f_1+\epsilon_{2}f_2}-\COLOP[u_{\epsilon_{1}f_1+\epsilon_{2}f_2},u_{\epsilon_{1}f_1+\epsilon_{2}f_2}]&= \epsilon_{1}f_1 +\epsilon_{2}f_2\quad  \text{in} \quad  \OVS M \\%\text{on }K_{Q,T}\\
 u_{\epsilon_{1}, \epsilon_{2}}(x,p)&= 0 \quad\quad\quad\quad\quad \ \text{in} \quad  \OVS \mathcal{C}^- %\text{if } x\in(-\infty,0]\times N
\end{split}
\end{equation}
By computing the mixed derivative 
\[
 \Phi^{2L}(f_1,f_2):=\frac{\p}{\p \eps_1}\frac{\p}{\p \eps_2}\Big|_{\eps_1=\eps_2=0} u_{\eps_1 f_1 + \eps_2 f_2},
\]
we show that $\Phi^{2L}(f_1,f_2)$ solves the equation
\begin{align}\label{2nd_lin_source}
%\Phi^L(f_j) &= \IX f_j, \; j=1,2, \notag \\
\XX \big(\Phi^{2L}(f_1,f_2)\big) &=  \COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]+  \COLOP [ \Phi^L (f_2),  \Phi^L( f_1)]% \label{second-ss-intro}
%\in C^\infty (\mathcal{S}),
\end{align}
on $\OVS M$. Here the functions $\Phi^L(f_l)$, $l=1,2$, are solutions to the linearization of the Boltzmann equation at $u=0$, which solve
\tbl{
\begin{equation}\label{transport_intro}
\begin{split}
\XX \big(\Phi^L(f_l)\big) &= f_l \s\quad \text{in}\quad \OVS M. \\%\text{on }K_{Q,T}\\
 \Phi^L(f_l)&= 0 \quad \  \text{in} \quad  \OVS \mathcal{C}^- %\text{if } x\in(-\infty,0]\times N
\end{split}
\end{equation}}
% 
% \begin{equation}\label{transport_intro}
%  \XX \big(\Phi^L(f_l)\big) = f_l \quad \text{on } \OVS M.
% \end{equation}
The transport equation \eqref{transport_intro} is also called the \emph{Vlasov equation}.
%which is the linearization of the Boltzmann equation at $0$ solution. 

Next, we build particular functions $f_1$ and $f_2$ such that the right hand side of \eqref{2nd_lin_source}, 
\[
\COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]+  \COLOP [ \Phi^L (f_2),  \Phi^L( f_1)],\]
 is a point source at $w$. To do this, we note that since $w\in W$, there exists lightlike geodesics $\eta$ and $\tilde\eta$, initialized in our measurement set $V$, which have their first intersection at $w$. We choose timelike geodesics $\gamma_{(\hat{x},\hat{p})}$ and $\gamma_{(\hat{y},\hat{q})}$ with initial data $(\hat{x},\hat{p})$ and $(\hat{y},\hat{q})$ in the bundle $\SP V$ of future-directed timelike vectors and which approximate the geodesics $\eta$ and $\tilde\eta$. %We then choose timelike directions $(\hat{x},\hat{p})$ and $(\hat{y},\hat{q})$ in $\SP V$ such that the geodesics arising from such initial data, $\gamma_{\hat{x},\hat{p}}$ and $\gamma_{\hat{y},\hat{q}}$ also have their first intersection at $w$ and are close to $\delta$ and $\tilde\delta$. 
Then, in Lemma \ref{coro_renerew}, we create $\dim(M)-2$  Jacobi fields on the geodesic $\gamma_{(\hat{y},\hat{q})}$ such that the variation of $\dot\gamma_{(\hat{y},\hat{q})}$ generated by the Jacobi fields is a submanifold $Y_2\subset \SP W\subset TM$. In particular, since $Y_2$ and $Y_1:=\text{graph}(\gamma_{(\hat{x},\hat{p})})\subset TM$ are geodesic flowouts, they can be considered as distributional solutions to the linear transport equation~\eqref{transport_intro}. The Jacobi fields are also constructed so that the projection of $Y_2\subset TM$ to $M$ near the intersection points of $\gamma_{(\hat{x},\hat{p})}$ and $\gamma_{(\hat{y},\hat{q})}$ is a $\dim(M)-1$ dimensional submanifold of $M$ which intersects the other geodesic $\gamma_{(\hat{x},\hat{p})}$ transversally in $M$. This transversality condition enables us to employ microlocal techniques to show in 
% and results (the bulk of which is done in 
Theorem \ref{sofisti} and Corollary \ref{sofisti_further} that $\COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]+  \COLOP [ \Phi^L (f_2),  \Phi^L( f_1)]$ represents a point source. 

To differentiate $u_{\eps_1f_1+\eps_2f_2}$ with respect to both $\eps_1$ and $\eps_2$, we also prove that the source to solution map of the Boltzmann equation \eqref{boltzmann} is two times Frech\'et differentiable in Lemma~\ref{deriv}. To analyze the nonlinear term $\COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]+  \COLOP [ \Phi^L (f_2),  \Phi^L( f_1)]$ when $\Phi^L(f_1)$ and $\Phi^L( f_2)$ are distributions in $\mathcal{D}'(TM)$, namely the delta distributions of the submanifolds $Y_1$ and $Y_2$ of $TM$, we view them as conormal distributions in $I^{k_l}(N^*Y_l)$ for some $k_l\in \R$ and $l=1,2$.  This allows us to compute the terms $\COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]$ and $\COLOP [ \Phi^L (f_2),  \Phi^L( f_1)]$ by using the calculus of Fourier integral operators. Slight complications to this analysis are due the fact that the distributions $\COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]$ and $\COLOP [ \Phi^L(f_2),  \Phi^L( f_1) ]$ have relations (in the sense of the theory of Fourier integral operators) in the bundle of causal vectors, which is a manifold with boundary.  

% have relations~\f{Say more clearly.} which lie over a Lagrangian manifold with boundary. 
%{\color{red}(This is not an issue as these objects are zero on the boundary anyway (incoming particles are timelike). The boundary is present in the variable $p$ (outgoing 4-momentum or 4-velocity) of the collision operator $\COLOP[,] (x,p)$. --Antti)}
We circumvent these complications by only measuring lightlike signals. This means that we compose the source to solution map with a 
%signals received at $V$, and in doing so compose $\Phi^{2L}$ with a smooth, local, 
lightlike section $P:V_e\subset V\to L^+V$, where $V_e$ open subset of $V$. % can be connected to $w$ by a future-directed, lightlike geodesic and $V_e$ is a small open set about $e$. 
This reduces our analysis of the term $\COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]$ in \eqref{2nd_lin_source}, $\COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]$,
to an analysis of the term
%\[ 
%\XX\big(\Phi^{2L}_{L^+V}(f_1,f_2)(x,P(x))\big) =  \COLOP_{gain} [ \Phi^L(f_1),  \Phi^L( f_2) ](x,P(x))+  \IX \COLOP_{gain} [ \Phi^L %(f_2), \Phi^L (f_1)](x,P(x)), 
%\]
%where 
\[
- \int_{\Sigma_{x, p}} \Phi^L(f_1) (x,p' ) \Phi^L(f_2) (x,  q' )  A(x,p,q, p', q') dV_{x,p} (q,p',q'), %dV (x,p \ ; \ q,p',q'), 
\]  
where $x$ lies in the open subset $V_e\subset M$ and $p=P(x)\in L^+V$, since the other part of the collision operator~\eqref{collision_operator_formula_intro} in this case yields zero. We analyze similarly the second right hand side term in \eqref{2nd_lin_source}. %, $\COLOP [ \Phi^L(f_2),  \Phi^L( f_1) ]$.

By the above construction, we construct a singularity at $w\in W\subset M$, which we may observe the singularity by using the source to solution map for light observations $\Phi_{L^+V}$.   
%we learn the locations in $V$ where we observe light particles which emanated from the interaction of the sources we constructed at $w$. 
Similar to \cite{Kurylev2018}, from our analysis we may recover the so-called 
%adopt a label these light observation locations in $V$ by functions, called 
\tbl{\emph{earliest observation time functions}} from the knowledge of $\Phi_{L^+V}$. Time separation function at $w$ compute the optimal travel time of light signal received from $w$. The collection of all \tbl{earliest observation time functions} from $w$ determines the \emph{earliest light observation set} that is the set of points $y\in \mathcal{U}$ that can be connected to $w$ by lightlike geodesics which have no interior cut points. This set is denoted by $\mathcal{E}_{\mathcal{U}}(w)$. Here $\mathcal{U}$ is an open subset of $V$ and we consider $\mathcal{E}_{\mathcal{U}}(w)$ as the map \tbl{$w\in W\mapsto \mathcal{E}_{\mathcal{U}}(w)$}.  We refer to Section \ref{time_sep_fnct} or~\cite{Kurylev2018} for explicit definitions. 

We apply the above to construct and measure point sources on two different Lorentzian manifolds $(M_1,g_1)$ and $(M_2,g_2)$ to prove:
%e then construct a smaller open set $\mathcal{U}\subset V$ foliated by timelike geodesics. Writing $\mathcal{E}^j_{\mathcal{U}}: w\in W_{\lambda}\mapsto \mathcal{E}^j_{\mathcal{U}}(w)$ for $j =1,2$, we prove
\begin{proposition} \label{ss_map_first_obs}
Let $\Phi_{1,\,L^+V}$ and $\Phi_{2,\,L^+V}$ be the source-to-solution maps for light observation satisfying the conditions in Theorem \ref{themain}.  Assume that the conditions of Theorem \ref{themain} are satisfied for the Lorentzian manifolds $(M_1,g_1)$ and $(M_2,g_2)$.
%, fix $w_{M_1}\in W_1$ and let $w_{M_2}\in W_2$ be as described above. 
Then $\Phi_{2,\,L^+V}  = \Phi_{1,\,L^+V}$ implies
\[
\{\mathcal{E}^1_{\mathcal{U}}({w_1}):\ w_1\in W_1\} = \{\mathcal{E}^2_{\mathcal{U}}({w_2}):\ w_2\in W_2\}. 
%\mathcal{E}^2_{\mathcal{U}}({W_2}). % (w_{M_2})
\]
\end{proposition}

As shown in \cite[Theorem 1.2]{Kurylev2018}, the sets $\mathcal{E}^{j}_{\mathcal{U}}(w)$, $j=1,2$, determine the unknown regions $W_{j}$ and the conformal classes of the Lorentzian metrics $g_j$ on them. That is, there is a diffeomorphism $F:(W_1,g_1|_{W_1})\to (W_2,g_1|_{W_2})$ such that $F^*g_2=c\s g_1$ on $W_1$. 
 %and the Lorentzian metrics  use the result \cite{Kurylev2018} which shows that this parametrization uniquely recovers the topological structure and Lorentzian structure $g|_W$ up to conformal class. 
After the reconstruction of the conformal class of the metric $(W,g|_W)$, we conclude the proof of Theorem \ref{themain} by showing that the source-to-solution map in $V$ uniquely determines the conformal factor $c(x)$ in $W$. This implies that the source-to-solution map in the set $V$ determines uniquely the isometry type of the Lorentzian manifold $(W,g|_W)$.  
%
% with an elementary argument which employs geodesic %parametrization to show we may recover the conformal class of %$g|_W$.~\f{This last sentence needs to be said better. Why can %re recover the conformal, while~\cite{Kurylev2018} can't. Let's %discuss that by a couple of sentences here. I ended here % 12.11.2020 -Tony}
% % % % % % % % % % % 
% % % % % % % % % % % 
% % % % % % % % % % % % \gamma_{(\hat{x},\hat{p})}for which there are 
% % % % % % % % % % % 
% % % % % % % % % % % %The Jacobi fields %
% % % % % % % % % % % 
% % % % % % % % % % % directions $(\hat{x},\hat{p})$ and $(\hat{y},\hat{q})$ in $\SP V$ such that the geodesics $\gamma_{(\hat{x},\hat{p})}$ and $\gamma_{(\hat{y},\hat{q})}$ with initial data $(\hat{x},\hat{p})$ and $(\hat{y},\hat{q})$ respectively, %$\gamma_{\hat{x},\hat{p}}$ and $\gamma_{\hat{y},\hat{q}}$ 
% % % % % % % % % % % also have first intersection at $w$ and are close to $\delta$ and $\tilde\delta$.
% % % % % % % % % % % 
% % % % % % % % % % % 
% % % % % % % % % % % 
% % % % % % % % % % % 
% % % % % % % % % % % , which we can observe by using the source to solution map of the Boltzmann equation.
% % % % % % % % % % % 
% % % % % % % % % % % 
% % % % % % % % % % % 
% % % % % % % % % % % We will use the second linearization of the source to solution map to generate 
% % % % % % % % % % % 
% % % % % % % % % % % We first explain how we can recover $a$ from the DN map $\Lambda$ of the equation~\eqref{eq:intro_wave-eq}.
% % % % % % % % % % % %This method can be used to %by presenting a formal argument how to 
% % % % % % % % % % % %recover $a$ from the knowledge of the DN map $\Lambda$ of the equation~\eqref{eq:intro_wave-eq} as follows.
% % % % % % % % % % %  Let us consider the case $m=2$. Let $f_1,\s f_2\in H^{s+1}(\Sigma)$, and let us denote by $u_{\eps_1f_1+\eps_2f_2}$ the solution to~\eqref{eq:intro_wave-eq} with boundary data $\eps_1f_1+\eps_2f_2$, where $\eps_1,\eps_2$ are sufficiently small parameters. By taking the mixed derivative of the equation~\eqref{eq:intro_wave-eq} with respect to the parameters $\eps_1$ and $\eps_2$, and of the solution $u_{\eps_1f_1+\eps_2f_2}$, we see that 
% % % % % % % % % % % \[
% % % % % % % % % % %  w:=\frac{\p}{\p \eps_1}\frac{\p}{\p \eps_2}\Big|_{\eps_1=\eps_2=0} u_{\eps_1 f_1 + \eps_2 f_2}
% % % % % % % % % % % \]
% % % % % % % % % % % solves 
% % % % % % % % % % % \begin{equation}\label{eq:second_deriv}
% % % % % % % % % % %  \square w   = -2a v_{1}v_2
% % % % % % % % % % % \end{equation}
% % % % % % % % % % %  with zero initial and boundary data. 
% % % % % % % % % % %  %Here $v_1$ and $v_2$ are solutions to the linearized equation $\square v=0$ with $v_1|_\Sigma=f_1$ and $v_2|_\Sigma=f_2$. 
% % % % % % % % % % %  Here the functions $v_j$ solve
% % % % % % % % % % %  \begin{equation}
% % % % % % % % % % %  \begin{cases}
% % % % % % % % % % %  \square v_j = 0, &\text{in } \Omega\times [0,T],\\ 
% % % % % % % % % % %  v_j = f_j, &\text{on } \p\Omega\times[0,T],\\
% % % % % % % % % % %  v_j\big|_{t=0} = \p v_j\big|_{t=0} = 0, &\text{in } \Omega,
% % % % % % % % % % %  \end{cases}
% % % % % % % % % % %  \end{equation}
% % % % % % % % % % %  for $j=1,2$.  %In the literature, taking mixed mixed derivatives of the equationthe solution $u_{\eps_1f_1+\eps_2f_2}$ of the non-linear equation with respect to $\eps_1$ and $\eps_2$ is known as the higher order linearization method.
% % % % % % % % % % %   This way we have produced new linear equations from the non-linear equation \eqref{eq:intro_wave-eq}. Studying these new equations in inverse problems for non-linear equations is known as the higher order linearization method.
% % % % % % % % % % % 
% % % % % % % % % % %  If we assume that the DN map is known, then the normal derivative of $w$ is also known on $\Sigma$ since  %Taking the mixed derivative of the DN map yields
% % % % % % % % % % %   \[
% % % % % % % % % % %    \p_\nu w = \p^2_{\eps_1\eps_2}|_{\eps_1=\eps_2=0}\s \Lambda(\eps_1f_1+\eps_2f_2).
% % % % % % % % % % %  \]
% % % % % % % % % % % % \[
% % % % % % % % % % % %  \p_\nu w 
% % % % % % % % % % % % \]
% % % % % % % % % % % % is also known on $\Sigma$ as it is the mixed derivative $\p^2_{\eps_1\eps_2}\Lambda(\eps_1f_1+\eps_2f_2)$ at $\eps_1=\eps_2=0$. 
% % % % % % % % % % % We let $v_0$ be an auxiliary function solving $\square v=0$ with $v_0|_{t=T} =\p_t v_0|_{t=T} = 0$ in  $\Omega$. The function $v_0$ will compensate the fact we know $\p_\nu w$ only on the lateral boundary $\Sigma$. Then, by multiplying~\eqref{eq:second_deriv} by $v_0$, and integrating by parts on $\Omega\times [0,T]$, we have the integral identity
% % % % % % % % % % %  \begin{equation}\label{eq:integral_identity_derivitve}
% % % % % % % % % % %   \int_{\Sigma}v_0\s \p^2_{\eps_1\eps_2}|_{\eps_1=\eps_2=0}\Lambda(\eps_1f_1+\eps_2f_2)\s \d S=\int_{\Omega\times [0,T]} \s v_0\s \square w \s \d x \s \d t  =-2\int_{\Omega\times [0,T]}a\s v_0\s v_1\s v_2\s \d x \s \d t. 
% % % % % % % % % % %  \end{equation}
% % % % % % % % % % %  Thus the quantity
% % % % % % % % % % %  \begin{equation}\label{eq:integral_denisty}
% % % % % % % % % % %   \int_{\Omega\times [0,T]} a\s v_0\s v_1\s v_2 \s \d x \s \d t 
% % % % % % % % % % %  \end{equation}
% % % % % % % % % % %  is known from the knowledge of the DN map. Since $v_1$ and $v_2$ were arbitrary solutions to $\square v=0$, we may choose suitable solutions $v_1$ and $v_2$ so that the products of the form $v_0v_1v_2$ become dense in $L^1(\Omega\times [0,T])$. This recovers $a$. 
% % % % % % % % % % %  
% % % % % % % % % % % Heuristically, in $1+1$ dimensions it would be sufficient to have $v_1=\delta((x-x_0)-(t-t_0))$ and $v_2=\delta((x-x_0)+(t-t_0))$ to recover $a(x_0,t_0)$ for $(x_0,t_0)\in \R^{1+1}$. Here $\delta$ is the $1$-dimensional delta function. In this case $v_1v_2$ is the delta function $\delta_{(x_0,t_0)}$ of $\R^{1+1}$ with mass at $(x_0,t_0)$. 
% % % % % % % % % % % However, since delta distributions do not correspond to a family of solutions of the non-linear wave equation, we will instead use \emph{approximate delta functions}.
% % % % % % % % % % %   In higher dimensions, different choices of $v_1$ and $v_2$ reduce the integral~\eqref{eq:integral_denisty} to a Radon transformation of $a$ on $\R^n$, which is stably invertible.
% % % % % % % % % % % %  To obtain stability, instead of taking derivatives of the equation~\eqref{eq:intro_wave-eq} with respect to the parameters $\eps_1$ and $\eps_2$ we will take finite differences.
% % % % % % % % % % % 
% % % % % % % % % % % 
% % % % % % % % % % %  
% % % % % % % % % % %  %To obtain stability instead of uniqueness, we take mixed finite difference
% % % % % % % % % % % Instead of differentiating equation~\eqref{eq:intro_wave-eq}, to obtain stability we will take the mixed finite difference
% % % % % % % % % % %   $D_{\eps_1,\eps_2}^2$ of $u_{\eps_1f_1+\eps_2f_2}$. In this case, we have the following integral identity % instead of mixed derivative, to have that $w$ satisifies
% % % % % % % % % % % %  \[
% % % % % % % % % % % %  w=D_{\eps_1\eps_2}^2\Big|_{\eps_1=\eps_2=0} u_{\eps_1 f_1 + \eps_2 f_2}+ \mathcal{O}(\langle\eps_1,\eps_2\rangle^3).
% % % % % % % % % % % % \]
% % % % % % % % % % % \begin{equation}
% % % % % % % % % % % \begin{aligned}
% % % % % % % % % % %   \int_{\Omega\times [0,T]} a\s v_0\s v_1\s v_2\s \d x \s \d t &=\int_{\Sigma}v_0\s D_{\eps_1\eps_2}^2\Big|_{\eps_1=\eps_2=0}\Lambda(\eps_1f_1+\eps_2f_2) \s \d S\\
% % % % % % % % % % %   &\qquad  + \frac{1}{\eps_1\eps_2}\int_{\Omega\times [0,T]} v_0\square\s R\s \d x \s \d t ,
% % % % % % % % % % %   \end{aligned}
% % % % % % % % % % %  \end{equation}
% % % % % % % % % % % where $R=\mathcal{O}_{E^{s+2}}(\langle\eps_1,\eps_2\rangle^3)$ in an energy space norm, for details see \eqref{eq:energy_norm} and \eqref{eq:tildeR}--\eqref{est:square_tildeR}. Here we denote by $\langle\eps_1,\eps_2\rangle^3$ homogeneous polynomials of order $3$ in $\eps_1$ and $\eps_2$. Stability result Theorem \ref{thm:stability} will follow by optimizing in $\eps_1$ and $\eps_2$ and parameters related to the solutions $v_1$ and $v_2$. The proof of Theorem~\ref{thm:noise} follows from a similar argument.
% % % % % % % % % % % 
% % % % % % % % % % % 
% % % % % % % % % % % 
% % % % % % % % % % % 
% % % % % % % % % % % 
% % % % % % % % % % % 
% % % % % % % % % % % We show that the source-to-solution map for the Boltzmann equation \eqref{boltzmann} captures information about the nonlinear collision operator $\COLOP$, and then use this data to gain information about the spacetime. As in \cite{Kurylev2018}, we obtain a relationship between the source-to-solution map and the nonlinearity $\COLOP$ by linearizing the equation \eqref{boltzmann}. This procedure, combined with analysis of the microlocal properties of $\COLOP$, enables us to use the source-to-solution map to determine if particle sources interact in the unknown region $W$ (for notional simplicity, we suppress the subscript $\lambda$ in the following outline, as the same construction will be applied both manifolds). 
% % % % % % % % % % % 
% % % % % % % % % % % For every $w \in W$, we show that we may build two sources of particles which will produce a point source singularity at $w$. Indeed, if $w\in W$, there exists future-directed, lightlike geodesics $\delta$ and $\tilde\delta$, initialized in the known set $V$, which have first intersection at $w$. We then choose timelike directions $(\hat{x},\hat{p})$ and $(\hat{y},\hat{q})$ in $\SP V$ such that the geodesics arising from such initial data, $\gamma_{\hat{x},\hat{p}}$ and $\gamma_{\hat{y},\hat{q}}$ also have first intersection at $w$ and are close to $\delta$ and $\tilde\delta$. We construct $\dim(M)-2$ Jacobi fields on the geodesic $\gamma_{\hat{y},\hat{q}}$ such that the variation generated by the Jacobi fields is a submanifol $S\subset \SP V$. 
% % % % % % % % % % % 
% % % % % % % % % % % We then use $\gamma_{\hat{x},\hat{p}}$ and Jacobi fields over $\gamma_{\hat{y},\hat{q}}$ to construct a submanifold $S\subset \SP V $, such that $(\hat{x},\hat{p})\notin S$ and $(\hat{y},\hat{q})\in S$. We will take care to ensure that the projection to $M$ of the geodesic flowout $Y_2$ of $S$ and $Y_1 = \gamma_{\hat{x},\hat{p}}$ have transverse intersection at $\{w\}\subset M$ and each intersection point of $\gamma_{\hat{x},\hat{p}}$ and $\gamma_{\hat{y},\hat{q}}$ in $W$ (this is done in Lemmas \ref{manifold_jacobi_const} and \ref{two_manifold_jacobi_const}). Finally, we construct a source $f_1$ which approximates a delta distribution over $ \{(\hat{x},\hat{p})\}$ and another source $f_2$ which approximates a delta distribution over $S$. %each of which behaves like a delta distribution:  $f_1\in I^{\nnn/2}(\{(\hat{x},\hat{p})\})$ and $f_2\in I^1(S)$.
% % % % % % % % % % % 
% % % % % % % % % % % %Next, we choose two sources $f_1\in I^{l_1}(N^*Y_1)$ and $f_2\in I^{l_2}(N^*Y_2)$, for $l_j\in \R$, $j=1,2$, each which behaves like a smoothened delta distribution. 
% % % % % % % % % % % 
% % % % % % % % % % % We consider the particle interactions arising from 
% % % % % % % % % % % \begin{equation}\label{boltz-intro}
% % % % % % % % % % % \begin{gathered}
% % % % % % % % % % % \mathcal{X}u_{\epsilon_{1}, \epsilon_{2}}-\COLOP[u_{\epsilon_{1}, \epsilon_{2}},u_{\epsilon_{1}, \epsilon_{2}}]= \epsilon_{1}f_1 +\epsilon_{2}f_2\quad \text{on } \OVS M \\%\text{on }K_{Q,T}\\
% % % % % % % % % % % u_{\epsilon_{1}, \epsilon_{2}}(x,p)= 0 \quad \text{if } x\in(-\infty,0]\times N
% % % % % % % % % % % \end{gathered}
% % % % % % % % % % % \end{equation}
% % % % % % % % % % % where $\COLOP$ has admissible kernel as in Definition \ref{good-kernels}.
% % % % % % % % % % % 
% % % % % % % % % % % From our unique local existence results for \eqref{boltz-intro}, the source-to-solution map $\Phi$ for this problem is well-defined in a neighbourhood of the origin.
% % % % % % % % % % % 
% % % % % % % % % % % We show that the singularities of the nonlinear term $\mathcal{X}^{-1}\COLOP[\mathcal{X}^{-1}f_1, \mathcal{X}^{-1}f_2]$ are captured by the second linearization of $\Phi$. We illustrate this concept formally. The perturbed source-to-solution map for \eqref{boltz-intro} takes the form
% % % % % % % % % % % %\[
% % % % % % % % % % % %(\epsilon_1, \epsilon_2 ) \mapsto \Phi ( \epsilon_1 f_1 + \epsilon_2 f_2  ).
% % % % % % % % % % % %\]
% % % % % % % % % % % %Comparing orders in $\epsilon_1$ and $\epsilon_2$,
% % % % % % % % % % % \[
% % % % % % % % % % % \Phi(\epsilon_1 f_1 + \epsilon_2 f_2) = \epsilon_1 \Phi^L(f_1) + \epsilon_2 \Phi^L(f_2) + \epsilon_1\epsilon_2 \Phi^{2L}(f_1,f_2)  + \text{higher order terms}
% % % % % % % % % % % \]
% % % % % % % % % % % where $\Phi^L$ and $\Phi^{2L}$ are the respective first and second linearizations of $\Phi$ and the higher order terms vanish in the limit for parameters $(\epsilon_1, \epsilon_2 )\to (0,0)$. Substituting $\Phi ( \epsilon_1 f_1 + \epsilon_2 f_2  )$ into \eqref{boltz-intro} comparing orders in $\epsilon_1$ and $\epsilon_2$ gives
% % % % % % % % % % % \begin{align}
% % % % % % % % % % % \Phi^L(f_j) &= \IX f_j, \; j=1,2, \notag \\
% % % % % % % % % % % \Phi^{2L}(f_1,f_2) &=  \IX \COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]+  \IX \COLOP [ \Phi^L (f_2),  \Phi^L( f_1)] . \label{second-ss-intro}
% % % % % % % % % % % %\in C^\infty (\mathcal{S}),
% % % % % % % % % % % \end{align}
% % % % % % % % % % % 
% % % % % % % % % % % In this way equation \eqref{second-ss-intro} describes how our measurements $\Phi$ captures information about the singular behaviour of $\COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]$. By applying microlocal techniques, we are be able to measure the lightlike signals received in $V$ from the interactions at the point $w$.
% % % % % % % % % % % 
% % % % % % % % % % % A slight complication to the proposed microlocal analysis is that the distribution $\COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]$ has relations which lie over a Lagrangian manifold with boundary. 
% % % % % % % % % % % %{\color{red}(This is not an issue as these objects are zero on the boundary anyway (incoming particles are timelike). The boundary is present in the variable $p$ (outgoing 4-momentum or 4-velocity) of the collision operator $\COLOP[,] (x,p)$. --Antti)}
% % % % % % % % % % % However, we do not use microlocal techniques adapted to spaces with boundary. Rather, we restrict to only measure light signals received at $V$, and in doing so compose $\Phi^{2L}$ with a smooth, local, lightlike section $P:V_e\subset V\to L^+(V)$, where $e\in V$ can be connected to $w$ by a future-directed, lightlike geodesic and $V_e$ is a small open set about $e$. This reduces our analysis to 
% % % % % % % % % % % \[ \Phi^{2L}_{L^+V}(f_1,f_2)(x,P(x)) =  \IX \COLOP_{gain} [ \Phi^L(f_1),  \Phi^L( f_2) ](x,P(x))+  \IX \COLOP_{gain} [ \Phi^L (f_2), \Phi^L (f_1)](x,P(x)), \]
% % % % % % % % % % % where 
% % % % % % % % % % % \[
% % % % % % % % % % % \COLOP_{gain} [u, v] (x,p) :=- \int_{\Sigma_{x, p }} u (x,p' ) v (x,  q' )  A(x,p,q, p', q') dV_{x,p} (q,p',q'), %dV (x,p \ ; \ q,p',q'), 
% % % % % % % % % % % \]  
% % % % % % % % % % % and $x$ lies in the open submanifold $V_e\subset M$.
% % % % % % % % % % % 
% % % % % % % % % % % We next show that for $\sslimit:= \Phi^{2L}_{L^+V}(f_1,f_2)(x,P(x))$,
% % % % % % % % % % % \[
% % % % % % % % % % % \sslimit \in  I^{\nnn/4 - 1/2} ( N^* (\gamma  ) \cap T^* V_e ;  V_e), \ \ WF (\sslimit)  = N^* (\gamma  ) \cap T^* V_e
% % % % % % % % % % % \]
% % % % % % % % % % % where $\gamma$ is (the image of) a lightlike geodesic from $e$ to $w$. In particular,
% % % % % % % % % % % \[
% % % % % % % % % % % \text{supp}( \sslimit) \subset \mathcal{L}^+   \big[ \gamma_{(\hat{x},\hat{p})} (0,\infty) \cap  \gamma_{(\hat{y},\hat{q})}(0,\infty) \cap W \big].
% % % % % % % % % % % \]
% % % % % % % % % % % That is, the interaction of particles $f_1$ and $f_2$ creates a point source singularity at $w$ which scatters to all future lightlike directions.
% % % % % % % % % % % 
% % % % % % % % % % % From the singularity at $w$ encoded in $\mathcal{S}$, we learn the locations in $V$ where we observe light particles which emanated from the interaction of the sources we constructed at $w$. As in done in \cite{Kurylev2018}, we adopt a label these light observation locations in $V$ by functions, called \emph{time separation functions}, which compute the optimal travel time of the light signal received from $w$.  The collection of all such time separation functions from $w$ is called the \emph{earliest light observation set} and denoted by $\mathcal{E}_{V}(w)$ (see \cite{Kurylev2018} and Section \ref{time_sep_fnct} for explicit definitions). 
% % % % % % % % % % % 
% % % % % % % % % % % We then construct a smaller open set $\mathcal{U}\subset V$ foliated by timelike geodesics. Writing $\mathcal{E}^\lambda_{\mathcal{U}}: w\in W_{\lambda}\mapsto \mathcal{E}^\lambda_{\mathcal{U}}(w)$ for $\lambda =1,2$, we prove
% % % % % % % % % % % \begin{proposition} \label{ss_map_first_obs}
% % % % % % % % % % % Let $\Phi_{1,\,L^+V}$ and $\Phi_{2,\,L^+V}$ be the source-to-solution maps described as in Theorem \ref{themain}.  Assume that the conditions of Theorem \ref{themain} are satisfied for $(M_j,g_j)$, $j=1,2$, fix $w_{M_1}\in W_1$ and let $w_{M_2}\in W_2$ be as described above. Then $\Phi_{2,\,L^+V}  =  (T \Xi^{-1})^* \circ \Phi_{1,\,L^+V} \circ T\Xi^*$ implies
% % % % % % % % % % % \[
% % % % % % % % % % % \mathcal{E}^1_{\mathcal{U}}\big|_{W_1} = \mathcal{E}^2_{\mathcal{U}}\big|_{W_2}. % (w_{M_2})
% % % % % % % % % % % \]
% % % % % % % % % % % \end{proposition}
% % % % % % % % % % % 
% % % % % % % % % % % As shown in \cite{Kurylev2018}, the sets $\mathcal{E}^{\lambda}_{\mathcal{U}}(w)$ parametrize our unknown regions $W_{\lambda}$. We use the result \cite{Kurylev2018}[Theorem 1.2] which shows that this parametrization uniquely recovers the topological structure and Lorentzian structure $g|_W$ up to conformal class. 
% % % % % % % % % % % 
% % % % % % % % % % % We conclude the proof with an elementary argument which employs geodesic reparametrizations to show we may recover the conformal class of $g|_W$.


\textbf{Paper outline.} Section \ref{prelim} contains all the preliminary information. There we introduce our notation (\ref{notation}) and recall Lagrangian distributions (\ref{lagrangian-dist}). We provide some expository material on the collisionless (Vlasov) and Boltzmann models of particle kinematics in Sections \ref{Vlasov} and \ref{Bman-model} respectively.  In Section~\ref{microlocal-collision}, we analyze the operator $\COLOP_{gain}$ from a microlocal perspective. Viewing particles as conormal distributions, we describe fully the wavefront set which arises from particle collisions. Additionally, in Section \ref{travserse-collisions-section} we construct a submanifold $S_2\subset TM$, whose geodesic flowout is $Y_2\subset TM$, such that the graph $Y_1$ of a geodesic and $Y_2$ satisfies the properties discussed in Section~\ref{proof_summary_main_thm}. 
% intersects a given geodesic transversally (in $TM$) through a finite collection of points. 
In Section \ref{main-proof}, we provide the proof of Theorem \ref{themain}, broken down into several key steps:
\begin{enumerate}
\item We show that from our source to solution map data, we can determine if our particle sources interact in $W$. 
\begin{enumerate}
\item[\textbullet] In section \ref{delta_dist_of_subm}, given choices of future-directed timelike vectors $(\hat{x},\hat{p})$ and $(\hat{y},\hat{q})$, as in Section~\ref{proof_summary_main_thm}, we construct the sources $f_1$ and $f_2$ described in Section~\ref{proof_summary_main_thm}.
\item[\textbullet] In this section we additionally construct smooth $C^\infty_c$ approximations $h_1^\epsilon$ and $h_2^\epsilon$, $\eps>0$, of the sources $f_1$ and $f_2$ respectively. This is done mainly for technical reasons, since we only consider the source-to-solution operator of the Boltzmann equation for smooth sources. % are well defined.
% 
% \footnote{For physical considerations, we emphasize that we work with smooth particle densities which approximate the ``real'' statistically defined sources. it is from these approximate measurements that we recover the desired Lorentzian metric and conformal class.}. Here $\epsilon>0$ is the regularization parameter which tells us how close our mollifications are to delta distributions. 
% We use these approximate sources to guarantee that the 
\item[\textbullet] In Section \ref{sca123} we describe \antti{a particular} future-directed lightlike vector field $P_e: V_e\to L^+V_e$, $V_e\subset V$ \antti{that admits as an integral curve a fixed optimal geodesic $\gamma$. We compose it with the collision operator~\eqref{collision_operator_formula_intro} and prove
% \[
% \sslimit \in  I^{\nnn/4 - 1/2} (V_e; N^* (\gamma  ) \cap T^* V_e), \ \ WF (\sslimit)  = N^* (\gamma  ) \cap T^* V_e,
% \]
%\antti{
\[
%\sslimit \in  I^{5\nnn/4}~\f{This might not be correct. Need to be checked. -Tony} (V_e; N^* (\gamma  ) \cap T^* V_e), \ \ 
\text{singsupp} (\sslimit)  =  \gamma   \cap  V_e,
\]
where $\mathcal{S}$ is known from our measurements, namely $\sslimit=\lim_{\epsilon \rightarrow 0}  \Phi^{2L} (h_1^\epsilon, h_2^\epsilon)  \circ P_e $. }
%\tbl{(Here $I^{5\nnn/4} (V_e; N^* (\gamma  ) \cap T^* V_e)$ denotes a class of conormal distributions, which we discuss in Section \ref{lagrangian-dist}.)}
\end{enumerate}
\item In section \ref{ss_elos} we prove Proposition \ref{ss_map_first_obs}, which says that we may determine earliest light observation sets from our measurements of $\mathcal{S}$. %This result is the first step which links the first light observations on $V$ and the data.
\item From the work in Section \ref{ss_elos} which connects  source-to-solution map data to the earliest light observation sets, we show we may determine the conformal class of the metric.
\item  Lastly, in the section \ref{det-of-conform} we finish the proof by showing that we can identify the conformal factor of the metric.
%showing that the conformal factor between the metrics in $W_1$ and $W_2$ is $1$.
\end{enumerate}
 Auxiliary lemmas, which include lemmas on the existence of solutions to the Cauchy problem of the Boltzmann equation with small data and the linearization of the source-to-solution map, among others, are contained in the Appendices.

\textbf{Acknowledgments.} 
The authors were supported by the Academy of Finland (Finnish Centre of Excellence in Inverse Modelling and
Imaging, grant numbers 312121 and 309963) and AtMath Collaboration project.





==> Sections/main-proof.tex <==
%
% Last edited: Oct 08, 2019
%
% This file contains the proof of the main theorem
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\s}{\hspace{0.5pt}}

\section{Proof of Theorem \ref{themain}}\label{main-proof}

In this section we prove our main result Theorem~\ref{themain}. As shown in Section \ref{Bman-model}, the second Frech\'et derivative $\Phi''$ of the source-to-solution map $\Phi$  satisfies
% % % % % \begin{alignat}{2}\label{vlasov1}
% % % % % %\begin{gathered}
% % % % % \mathcal{X}u(x,p)&= f(x,p) \quad &&\text{on} \quad \OVS M \nonumber \\
% % % % % u(x,p)&= 0 \quad &&\text{on} \quad  \OVS \mathcal{C}^- %((-\infty,0] \times N)
% % % % % %\end{gathered}
% % % % % \end{alignat}
\begin{equation}\label{adso00}
\begin{split}
%\Phi_{L^+V}''(h_1,h_2) (x,p) &=
\Phi '' (0; f,h) 
%\\
&= \IX \COLOP [ \IX(f),  \IX( h) ]+  \IX \COLOP [ \IX (h),  \IX(f)] \quad \text{on } \SP M,
\end{split}
\end{equation}
where $f,\, h$ are any compactly supported smooth functions and $\IX$ is the solution operator of the linearized problem~\eqref{vlasov1}. %In our proof of Theorem~\ref{themain}, we will only measure lightlike particles. In that case, the restriction of $\Phi''$ is 
%In the case $(x,p) \in L^+ V$ and $h_{1},h_{2}\in C_c^\infty(\SP V)$, it follows from the definition that this derivative is completely 
%determined by the operator $\Phi_{L^+ V}$.~\footnote{\tbl{Make this sentence better. What was the point?}} %Thus, it is sufficient to show that  $\Phi '' (h_1,h_2) (x,p)$ for $(x,p) \in L^+ V$ and $h_{1},h_{2}\in C_c^\infty(\SP V)$ determines the Lorentzian metric in $W$. 
We use the microlocal properties of the collision operator $\COLOP$ we proved in the previous section to determine the wavefront set of $\Phi''(h_1,h_2)$ for sources $h_{1}$ and $h_{2}$ with singularities. %\in C_c^\infty(\SP V )$. %~\footnote{\tbl{Make this sentence better. There is no wavefront set for smooth sources.}} 
%This is described next.

\subsection{Delta distribution of a submanifold}\label{delta_dist_of_subm}

% {\color{blue}

First, we construct the specific particle sources which we will use in our proofs.
Let $(M,g)$ be a $C^\infty$ smooth globally hyperbolic manifold of dimension $n$. Let $\mathcal{C}$ be a Cauchy surface of $(M,g)$. We introduce a parametrization $\R\times \SP \mathcal{C} \to \SP M$ for $\SP M$ as:% given by
\begin{equation}\label{ll5789}
   \Psi(s, (x,p))= \dot\gamma_{(x,p)}(s), \quad s\in \R, \ (x,p) \in  \SP \mathcal{C}. 
\end{equation}
Here $\SP \mathcal{C}\subset TM$ is the set of future-directed time-like vectors with base points in $\mathcal{C}$. We call the parametrization~\eqref{ll5789} the \emph{flowout parametrization} of $\SP M$. %This slightly abuses the common terminology in that we might not have chosen local coordinates for $\SP \mathcal{C}$. Especially we will speak about coordinate representations of functions, volume forms etc. in the coordinates~\eqref{ll5789}. 
We refer to~\cite[Theorem 9.20]{Lee_2013} for properties of flowouts in general.


%Let $\widetilde{\mathcal{C}}$ be another Cauchy surface of $(M,g)$, such that $\widetilde{\mathcal{C}}=\{\tilde{t}\}\times N$, $\tilde{t}>0$. That is $\widetilde{\mathcal{C}}$ is in the future $\mathcal{C}^+$ of $\mathcal{C}$. 
Let $S$ be a  submanifold \antti{(not necessarily closed) }
%\footnote{\antti{simplified the sentence--Antti}} 
%}
of $\SP\mathcal{C}\subset \SP M$.
%, which either is a compact submanifold or its closure $\overline{S}$ is a submanifold with boundary.
The delta distribution $\delta_S\in \mathcal{D}'(\SP M)$ of the submanifold $S$ on $\SP M$ is defined as usual by
\[
 \delta_S(f)=\int_S \tbl{f(x,p)}\, dS, \text{ for all } f\in C_c^\infty( \PP^+ M),
\]
where $dS$ is the volume form \tbl{ of the submanifold $S$ of $\PP^+M$.} 
For our purposes it will be convenient to consider the delta distribution on $S$, in the case where $S$ is considered as a submanifold $\SP \mathcal{C}$ (instead of $\SP M$). \tbl{We distinguish this case and denote by $\check{\delta}_S\in \mathcal{D}'(\SP \mathcal{C})$ the distribution $\check{\delta}_S(\check{f})=\int_S \check{f}(x,p)\, dS$  for all  $\check{f}\in C_c^\infty(\SP \mathcal{C})$. 
%where $dS_{\PP^+\mathcal{C}}$ is the volume form induced from $\PP^+\mathcal{C}$ to $S$.
The representation of $\delta_S$ in the flowout parametrization~\eqref{ll5789} of $\SP M$ is then 
\[
 \delta_S=\delta_0\otimes\check{\delta}_S,
\]
where $\delta_0\in \mathcal{D}'(\R)$ is the delta distribution on the real line with its support at the $0\in \R$, and $\check{\delta}_S\in \mathcal{D}'(\SP \mathcal{C})$ is as above. We will write simply $\delta_S(s,(x,p))=\delta_0(s)\s \check{\delta}_S(x,p)$, $s\in \R$ and $(x,p)\in \SP \mathcal{C}$. We write similarly for other products of pairs of distributions %on a product space in cases the distributions of the pairs are 
supported in mutually separate variables.}% \footnote{\antti{lots of text, nothing happens}} %components of the product space. 

% where $a>0$ is the coordinate representation of the volume form up to normalization.
 \tbl{We would like to view $\delta_S$ as a conormal distribution of the class $I^{m}(\SP M; N^*S)$. However, this is not strictly speaking possible due to the possible bonudary points of $\overline{S}$. 
 %
 %\tbl{For this, we need to discuss the technicality that in our application $\overline{S}$ might be a submanifold with non-empty boundary in $\SP M$. }
%
To deal with the possible boundary points of the submanifold $\overline{S}$, we are going to consider the product of a cutoff function and $\delta_S$ as follows. Let $(y,q)\in S$ and let $(s',s'')\in \R^{\dim{(\SP \mathcal{C})}-\dim{(S)}}\times  \R^{\dim{(S)}}$ be coordinates on a neighborhood $B\subset \SP \mathcal{C}$ of $(y,q)$ such that $S$ corresponds to the set $\{s'=0\}$ and $S$ is parametrized by the $s''$ variable. Let $\chi_R=\chi_R(s'')$ to be a cutoff function, which is supported in a small ball of radius $R$ and outside a neighborhood of the boundary of submanifold $\overline{S}$. We have that %$\chi_R\check{\delta}_S\in \mathcal{D}'(\SP \mathcal{C})$ and  
$\chi_R\delta_S =\chi_R(\delta_0\otimes\check{\delta}_S)\in \mathcal{E}'(\SP M)$ in the flowout parametrization is the oscillatory integral
%\begin{equation}\label{delta_as_oscillory}
%  (\chi_R\check{\delta}_S)(s',s'')= \chi_R(s'')\int e^{i s' \cdot \xi'} a(s'')d\xi',
% \end{equation}
\begin{equation}\label{delta_as_oscillory2}
 (\chi_R\delta_S)(s,s',s'')=\chi_R(s'')a(s'')\iint e^{is\s \xi} e^{i s' \cdot \xi'} d\xi d\xi'.
\end{equation}
Here $a(s'')$ corresponds the volume form of $S$ and the integration is over $\xi\in \R$ and $\xi'\in \R^{\dim{(\SP \mathcal{C})}-\dim{(S)}}$. 
}

By the above definition, $\chi_R(x,p)\delta_S(x,p)$ %equals $\chi_R\s \delta_S$ and it 
is a conormal distribution in the class $I^{m}_{comp}(\SP M; N^*S)$, where the order $m$ is 
\begin{equation}\label{order_m}
 m=\codim(S)/2-\dim(\SP M)/4,
\end{equation}
see Section~\ref{lagrangian-dist} for the definition of the order $m$. Here $\codim(S)=\dim(\SP M) -\dim(S)$. % is with respect to the dimension $2n$ of $\SP M$.
In the proof of Theorem~\ref{themain}, the submanifold $S$ will be either of dimension $0$ or $n-2$, and thus $m$ will be either $n/2$ or $1$ respectively. We remark that when $S$ is of dimension $0$ the cutoff function in~\eqref{delta_as_oscillory2} can be omitted.


\subsubsection{Approximate delta distributions}\label{approx_delta_dists}
% {\color{blue}

We will use $C^\infty$ smooth sources that approximate delta distributions \tbl{$\delta_{S_1}$ and $\delta_{S_2}$ (multiplied by cutoff functions), where $S_1$ and $S_2$ are  submanifolds of $\SP \mathcal{C}$.} The dimension of $S_1$ will be $n-2$ and $S_2$ will be a point. These approximations are described next.

Let $S$ be a submanifold of $\SP \mathcal{C}\subset \SP M$ and let $\delta_S$ and $\chi_R$ be as in Section~\ref{delta_dist_of_subm} above. By using standard (Friedrichs) mollification, see e.g.~\cite{friedlander1998}, we have that there is a sequence $(h^\eps)$, $\eps>0$, of functions $C_c^\infty(\SP M)$ such that
\begin{equation}\label{regu}
 h^\eps \to \chi_R\s \delta_{S} \text{ in } \mathcal{D}'(\SP M),
\end{equation}
as $\eps\to 0$. %We have similarly a sequence $(h_2^\eps)$ of functions in $C_c^\infty(\SP M)$, with $h_2^\eps \to \delta_{S_2}$ in $\mathcal{D}'(\SP M)$ as $\eps\to 0$. 
Let $u^\eps=\IX h^\eps\in C^\infty(\SP M)$ be the solution to
\begin{equation}\label{approx_sol}
 \begin{split}
\XX u^\eps  &= h^\epsilon \text{ on } \SP M \\
u^\eps &= 0 \text{ on } \SP \mathcal{C}^-.
\end{split}
\end{equation}
By the representation formula of solutions to~\eqref{approx_sol} given in Theorem~\ref{vlasov-exist} we have that %~\footnote{\tbl{Insert specific reference. Put a representation formula of solution to the existence of Vlasov.}}
%Expressing $\IX h_1^\epsilon$ and $\IX h_2^\epsilon$ in an integral form or directly by referring to the properties of $\IX$ in Section \ref{mla_valsov} one obtains 
\begin{equation}\label{approx_sol_prop}
u^\eps \geq 0, \quad \text{supp}(u^\eps) \subset K_{\text{supp}(h^\epsilon)}.
\end{equation}
By considering only small enough $\eps>0$, the support of the solutions $u^\epsilon$ can be taken to be in any neighborhood of $K_S$ chosen beforehand. %and $ K_{\{ (\hat{x},\hat{p})\}} = \dot\gamma_{(\hat{x},\hat{p})} $ as $\epsilon \longrightarrow 0$.~\footnote{\tbl{Is this needed? If, there might be need for some compactness statement.}} 

Let $\widetilde{\mathcal{C}}$ be another Cauchy surface of $(M,g)$, which is in the past $\mathcal{C}^-$ of $\mathcal{C}$. Note that $u^\eps$ is then also a solution to $\XX u^\eps=h^\eps$ with \tbl{ $u^\eps =0$ on $\SP \widetilde{\mathcal{C}}^{-}$}. By Lemma~\ref{vlasov_ext_conormal}, $u^\eps$ is  unique. We also have that $WF(\chi_R\s\delta_S)\cap N^*(\SP \widetilde{\mathcal{C}})\subset N^*S\cap N^*(\SP \widetilde{\mathcal{C}})=\emptyset$.
By applying Lemma~\ref{vlasov_ext_conormal} again, we obtain % $\IX$ has a unique continuous extension to $\{\}$, and thus it follows that%~\footnote{\tbl{Insert specific result which gives this after Section 3.1.1 has been finalized.}}
\[
\lim_{\epsilon \rightarrow 0} u^\eps
%= \lim_{\epsilon \rightarrow 0}\IX (\rho^\epsilon *  \delta_{S_1}) (r, r')   
= u
\]
%and
%\[
%\lim_{\epsilon \rightarrow 0} \IX h_2^\epsilon =  \lim_{\epsilon \rightarrow 0} \IX (\rho^\epsilon * f) (s, s' , s'') =  \IX f (s, s' , s'')
%\]
in the space of distributions $\mathcal{D}'(\SP M)$. Here $u=\IX (\chi_R\s\delta_{S})$ solves
\begin{equation}\label{solution_with_delta_source}
\begin{split}
\XX u = \chi_R\s\delta_S \text{ on } \SP M \\
u = 0 \text{ on } \SP \widetilde{\mathcal{C}}.
\end{split}
\end{equation}
Finally, if $\chi\in C_c^\infty(\SP M)$ is a cutoff such that $\supp{\chi}\subset\subset \SP M\setminus S$, we have that $\chi u\in I^{m-1/4}(\SP M; N^*K_S)$, with $m$ given in~\eqref{order_m}.

\subsection{\tbl{Nonlinear interaction in the inverse problem}}\label{sca123}
Throughout this Section~\ref{sca123} we assume that $(M,g)$ is a globally hyperbolic manifold of dimension $n$ and that $\mathcal{C}$ is a Cauchy surface of $(M,g)$. We also assume that the submanifolds $S_1\subset \PP^+ \mathcal{C}$ and $S_2=\{(x_0,p_0)\}\in \PP^+ \mathcal{C}$, $x_0 \notin \overline{S}_1$,  are such that the flowouts $K_{S_1}$ and $K_{S_2}$ satisfy the admissible intersection property (Definition~\ref{intersection_coords}) in $\pi\text{supp}A$, where $A$ is an admissible collision kernel.  
\antti{As shown simultaneously for two manifolds in Corollary \ref{coro_renerew}, such a pair of submanifolds can be constructed around any distinct base points on the Cauchy surface. }
Further, let $\hat\mu : [-1,1] \rightarrow M$ be $C^\infty$-smooth timelike curve and $V\subset M $ be an open neighbourhood of $\hat{\mu}$.

%Let us recall some semi-Riemannian geometry concepts. 
%The $(M,g)$ be a Lorentzian manifold. 
The length of a piecewise smooth causal path $\alpha : [a,b] \rightarrow M$ is defined  as %be defined by 
\begin{equation}\label{lengtyht}
l(\alpha) := \sum_{j=0}^{m-1} \int_{a_j}^{a_{j+1}} \sqrt{ -g( \dot\alpha(s), \dot\alpha(s)) } ds,
\end{equation}
where $a_0<a_1< \cdots<a_{m-1} < a_m$ are chosen such that $\alpha$ is smooth on each interval $(a_j,a_{j+1})$ for $j=0,\dots,m-1$. \tbl{The time separation function, see e.g.~\cite{oneill1983semiriemannian}, is denoted by $\tau : M \times M \rightarrow [0, \infty)$ and defined as 
% \[
% \tau(x,y) :=\begin{cases}  \sup \int_0^1 \sqrt{ -g( \dot\alpha (s) , \dot\alpha (s))  } ds, & x<y \\
% 0, & \text{otherwise.}
% \end{cases}
% \] 
\[
\tau(x,y) :=\begin{cases}  \sup l(\alpha) , & x<y \\
0, & \text{otherwise,}
\end{cases}
\] 
where the supremum 
%of the length function % ~\eqref{lengtyht},
%\begin{equation*}%\label{lengtyht}
%$
%l(\alpha) = \sum_{j=0}^{m-1} \int_{b_j}^{b_{j+1}} \sqrt{ -g( \dot\alpha(s), \dot\alpha(s)) } ds 
%$ %\end{equation*}
is taken over all piecewise smooth lightlike and timelike curves $\alpha : [0,1] \rightarrow M$, which are smooth on each interval $(b_j,b_{j+1})$, and that satisfy $\alpha(0)  = x$ and $\alpha(1) = y$. %where $a_0<a_1< \cdots<a_{m-1} < a_m$ are chosen such that 
%$\alpha$ is . % for $j=0,\dots,m-1$. 
%The causality notation $x<y$ was defined in the introduction.
%}
%
%%
%
%\tbl{The time separation function is $\tau(x,y) = \sup l(\alpha)$, where $x,y\in M$ and 
%$l$ is the semi-Riemannian length   (\ref{lengtyht}) and 
%the supremum is taken over causal piecewise smooth paths connecting $x$ to $y$ and $\tau(x,y) = 0$ if there are no such paths. 
If $\tau(x,y)=0$ and there is a lightlike geodesic $\gamma$ connecting points $x,y\in M$, we call $\gamma$ \emph{optimal}.
By~\cite[Proposition 14.19]{oneill1983semiriemannian}, we have that if $(M,g)$ is globally hyperbolic and if $x,y\in M$ satisfy $\tau(x,y)=0$, then an optimal lightlike geodesic $\gamma$ always exists. 
%If $\tau(x,y)=0$, then $\gamma$ is lightlike.
}
%We simplify the notation by denoting the image of a given curve $\gamma (s)$ in $M$ by $\gamma$. 

The main result of this Section~\ref{sca123} is the following:
\begin{proposition}\label{kooasu} 
%Let $Y_1,\, Y_2 \subset \PP M$,
%S^{r_j}_{t_j}$, $t_j \in \R$, $r_j > 0$ , $j=1,2$  
%be smooth manifolds that have admissible intersection according to Definition \ref{intersection_coords}.
%%
%
Let $(M,g)$ be a globally hyperbolic manifold, $A:TM^4\to \R$ an admissible collision kernel with respect to a relatively compact subset $W \subset M$. 
%$W\subset M$ be an open relatively compact set where $A$ is strictly positive\footnote{Positivity of $A$ is added on Sep. 6 - Matti} 
Let $\mathcal{C}\subset M$ be a Cauchy surface, $S_1$ be a submanifold of $\PP^+ \mathcal{C}$, and $S_2=\{(x_0,p_0)\}\in \PP^+ \mathcal{C}$, $x_0\notin \overline{S}_1$. Assume that
%\footnote{Set $W$ added on Sep. 6, 2021. - Matti} 
$K_{S_1}$ and $K_{S_2}$ have the admissible intersection property in $\pi \text{supp} A$ according to Definition \ref{intersection_coords}. Assume also that $\pi(K_{S_1})$ and $\pi(K_{S_2})$  intersect  in $ \pi \text{supp} A$ first time at $z_1\in W$. Let $\gamma$ be \tbl{an optimal} future-directed light-like geodesic in $M$ such that $\gamma(0) = z_1$ and $e := \gamma(T)$. % that maximizes the length %Assume furthermore that $\gamma :[0,T]\to M$ maximizes length 
%over all piecewise smooth causal paths from $z_1$ to $e$.%~\f{We could use the optimal geodesic term here.}

Additionally, let $h_{1}^{\epsilon},\s h_{2}^{\epsilon}\in C_c^\infty(\PP^+M)$ be the  approximations of the distributions $\chi_{R}\s\delta_{S_1}$ and $\delta_{S_2}$, \tbl{where $S_2$ is a point}, as described 
% lightlike curves $\delta_{S_1}$ and $\delta_{S_2}$ as described 
in Section~\ref{approx_delta_dists}. %sources in Section \ref{regu}.
 
Then, there is a section $P_{e}: V_e\to L^+V_e$ on a neighborhood $V_e$ of $e$ %of the point $e$ and a section  % $x \mapsto P_e (x) \in L^+(V_e)$, $x\in V_e$ 
such that the limit%~\f{$\mathcal{C}$ has no double meaning. Have to fix this in the end.}
% \[
%  \sslimit:=\lim_{\epsilon \rightarrow 0} (  \Phi'' (0;h_1^\epsilon, h_2^\epsilon)  \circ P_e ) \in  I^{\nnn/4 - 1/2} (V_e; N^* (\gamma ) \cap T^* V_e)
%  \]
\[
 \sslimit:=\lim_{\epsilon \rightarrow 0} (  \Phi'' (0;h_1^\epsilon, h_2^\epsilon)  \circ P_e ) 
 %\in  I (V_e; N^* (\gamma ) \cap T^* V_e)
 \]
  exists and 
  \antti{ 
  %is a conormal distribution over $\gamma$ in $V_e$ with singularities
%Then there is a neighbourhood $U_{a} \subset V$ of $a$ such that 
\[
  \text{singsupp} ( \sslimit)   = \gamma  \cap V_e
\]
}
%In particular, $\mathcal{E}_{V'} (z_1)$ is obtained from the source-to-solution data for any open $V' \subset V$.
%{\color{gray}Precisely, $\sslimit$ is a delta distribution over the part of the graph of $\gamma$ in $V_e$.}
\end{proposition}
%Notice here that since $(M,g)$ is globally hyperbolic, the graph of $\gamma$ in the proposition is a submanifold of dimension $1$. In particular, the conormal bundle $N^* (\gamma )$  is well defined. 
In the context of the main theorem the proposition above can be used to detect rays of light propagating from the unknown set $W$ to the measurement neighbourhood $V$. In that setting $z_1\in W$ whereas $e \in V$ and $V_e \subset V$.
The situation is pictured in \tbl{Figure~\ref{fig:light_obs2}} below.
\begin{figure}[ht!]\label{fig:kooasu}
    \centering
%
% New picture
\begin{tikzpicture}
    \draw [fill=lightgray] (0,0) ellipse (1cm and 5cm);
    \draw[thick] (0,4) -- (0,-4);
    \node at (-0.2,0) {$\hat\mu$} ;
     \node(dot) at (0, 2) {\textbullet};
    \node at (-0.2,2) {$e$} ;
        \node at (1.4,0.3) {$\gamma$} ;
       \node at (2,0) {\textbullet} ;
         \node at (2.3,0) {$z_1$} ;
         \draw[thick] (2,0) -- (0,2);
        \node at (-2,0) {$W$} ;
                \node at (0,-4.4) {$V$} ;
    \draw (0,4) -- (4,0) -- (0,-4) -- (-4,0) -- (0,4);
\end{tikzpicture}
   \caption{\antti{The setup of Proposition \ref{kooasu} can be used to detect singularities propagating along rays of light in $V$.} }
    \label{fig:light_obs2}
\end{figure}

Before proceeding with the proof of Proposition \ref{kooasu}, \antti{we state the following supporting result which follows from a simple dimension argument similar to the one used in Lemma \ref{lemma_renerew}. In other words, there is so much freedom for variation that caustic effects can be avoided at finite number of fixed points. 
The vector field $P_e$ in Proposition \ref{kooasu} is constructed as a restriction of $P$ in the lemma below for convenient choice of the vectors $(x_j,p_j)$. }
%\footnote{\antti{I removed the gray stuff from here}} %, which are Lemma~\ref{hhaovg}, Lemma~\ref{ooiiuu} and Lemma~\ref{shortcut_lemma}. 

%The next lemma is
\begin{lemma}\label{ooiiuu}
%Let $s\mapsto \gamma(s)  \in \R \times N$ be a future-directed light-like geodesic and fix $(x_0,p_0):=\dot\gamma(s_0)$,  $(y_0,q_0):=\dot\gamma(s_1)$ where $s_0<s_1$. 
Let $(x_j,p_j)  \in L^+(M)$, $j=1,\dots,m$, be a finite set of vectors. 
There is an open (possibly disconnected) neighborhood $ Q  $ of $\{x_1,\dots,x_m\}$  in $M$ and a smooth local section 
 $P : Q \rightarrow L^+Q$,  $P(x) = (x,p(x))$,
of the bundle $\pi : L^+M  \rightarrow M$ such that for \tbl{$x\in Q$ and $s\in \R$ such that $\gamma_{(x,p(x))} (s) \in  Q$
%it contains the vectors $(x_j,p_j)$, $j=0,\dots,k$ and has geodesics as integral curves. That is,
\begin{equation}\label{conditions_for_P}
 \begin{split}
P( x_j ) &= (x_j,p_j)  \\  
%\text{if}
% \quad (x,p) = P(x) , \ \gamma_{(x,p)} (s) \in U, \quad \text{then} \quad
\dot\gamma_{(x,p(x))} (s) &= P( \gamma_{(x,p(x))} (s) ). % , \quad \text{for}  \quad x\in Q, \quad \gamma_{(x,p(x))} (s) \in  Q.
\end{split}
\end{equation}
}
%%%%
\end{lemma}

\begin{comment}

\begin{proof}[Proof of Lemma \ref{ooiiuu}]\label{prooffff123}

We obtain the existence of the vector field $\widetilde{P}$ via a dimensionality argument. First, we may assume that the geodesics $\gamma_{(x_j,p_j)} $ and $ \gamma_{(x_l,p_l)}$, are identical as sets for every $l,j \in \{ 1, \dots, m\}$. The general case can be divided into distinct cases of this type.

For $j=1,\ldots,m$, let $\mathcal{C}_j\subset M$ be Cauchy surfaces such that $\mathcal{C}_{j} =\{t_{j} \}\times N$ for some $t_{j}\in \R$ and $x_j\in \mathcal{C}_j$. Let $B$ be an open subset of the lightlike bundle $P^0 \mathcal{C}_1$ such that $B\ni (x_1,p_1)$. Define 

\[
\phi_j: B\to P^0 \mathcal{C}_j
, \qquad  \phi_j(x,p)=\dot{\gamma}_{(x,p)}(s_j(x,p)),
\]
where $s_j(x,p)\in \R$ is the parameter value for which the geodesic $\gamma_{(x,p)}$ intersects the Cauchy surface $\mathcal{C}_j$. 

We write $\pi:TM\to M$ for the standard projection map. We also write  
\[
D_{(x_1,p_1)}(\pi\circ \phi_j):T_{(x_1,p_1)}P^0\mathcal{C}_1 \to T_{x_j}M
\]
for the derivative (pushforward) of $\pi\circ \phi_j$. Notice that the linear subspaces $ \text{ker}\,D_{(x_1,p_1)}(\pi\circ \phi_j)  $ are $(n-1)$ dimensional. This follows by observing that  the domain of the local diffeomorphism $\phi_j$ is $2n-2$ dimensional and that $\phi_j$ maps to the lightlike bundle, which has fibres of dimension $n-1$.

%\tbg{Let $B \subset P_{t}^0 M$, $t=x_1^0$, $j=1,\dots,m$ be a open neighbourhood of $(x_1,p_1)$ such that the embedding $\phi_j : B \rightarrow P^0_{t_j} M$, $t_j := x_j^0$ ($t_1=t$),  $\phi_j ( x, p) = \dot\gamma_{(x,p)}( (\gamma_{(x,p)}^0)^{-1} (t_j) ) $ ($\phi_1 = id_B$), is well defined for $j=1,\dots,m$. 
%The planes $\text{ker}T_{(x_0,p_0)} (\pi \circ \phi_j)$ $j=1,\dots,m$ are $(\nnn-1)$-dimensional linear subspaces of the space $T_{(x_0,p_0)}P_{t}^0 M$ which is of dimension $2\nnn-2$.}
By the above, the codimension of each linear subspace $\text{ker}\,D_{(x_1,p_1)}(\pi\circ \phi_j)\subset T_{(x_1,p_1)}P^0\mathcal{C}_1$ is $(2\nnn-2) - (\nnn-1) = \nnn-1$. It follows that we may choose an $(n-1)$-dimensional subspace $L$ of $T_{(x_1,p_1)}P^0\mathcal{C}_1$ such that it meets each of the subspaces $\text{ker}\s(D_{(x_1,p_1)}(\pi\circ \phi_j))$ only at the origin, $j=1,\dots,m$. That is, we choose an % that there is an 
$(\nnn - 1)$-dimensional subspace $L \subset T_{(x_1,p_1)}P^0\mathcal{C}_1$ such that 
\begin{equation}\label{L_not_intersect}
L \cap \bigg( \bigcup_{j=1}^m \text{ker}\s(D_{(x_1,p_1)} (\pi \circ \phi_j)) \bigg) = \{0\}. 
\end{equation}
Let $G \subset P^0\mathcal{C}_1$ be a smooth submanifold such that $L$ equals the tangent space of $G$ at $(x_1,p_1)$. %$L= T_{(x_1,p_1)}G$.~\footnote{\tbl{Explain what is the tangent space of submanifold.}} 
 From the choice of $L$, see~\eqref{L_not_intersect}, the maps $D_{(x_1,p_1)} ( \pi \circ \phi_j |_G ) =D_{(x_1,p_1)} ( \pi \circ \phi_j) |_L $ are injective. Therefore, there is an open set $\widetilde{B}\subset G$ with $(x_1,p_1)\in \widetilde{B}$ such that the maps
 \[
 \pi \circ \phi_j |_{\widetilde{B}}:\widetilde{B} \to  \pi \circ \phi_j(\widetilde{B})\subset M,
\]
are diffeomorphism onto their images. Further, the dimension of the submanifold $(\pi \circ \phi_j) (\widetilde{B})$ of $M$ is $\nnn-1$, which is equal to the dimension of $\mathcal{C}_j$. 

We next construct the desired set $Q\subset M$ and vector field \tbl{$\widetilde{P}:Q\to  L^+Q$} by considering the geodesic flowout $K_{\phi_j(\widetilde{B})} \subset L^+M$ of $\phi_j(\widetilde{B})$ for $j=1,\dots, m$. As argued in Remark \ref{flowout-is-manifold}, since $(M,g)$ is smooth, there is an open set $V_j\subset TM$ such that 
\[
U_j = K_{\phi_j(\widetilde{B})}\cap V_j, \quad j=1,\ldots,m.
\]
is a smooth submanifold of $L^+M$ and $\pi(U_j)$ is a smooth $n$-dimensional submanifold of $M$ foliated by lightlike geodesics.

Finally, we set  $Q=\bigcup_{j=1}^m \pi(U_j)$ and 
\[
 \widetilde{P}(x)= p \ \ \text{if } (x,p)\in \bigcup_{j=1}^m U_j.
\]
As each $U_j$ is the local flowout of $\phi_j(\widetilde{B})$ by lightlike geodesics, the conditions~\eqref{conditions_for_P} hold.

\end{proof}

\end{comment}

%{\color{gray}
%The \emph{time separation function} is $\tau(x,y) = \sup l(\alpha)$ where $l$ is the semi-Riemannian length   (\ref{lengtyht}) and the sup is taken over causal piecewise smooth paths connecting $x$ to $y$ and $\tau(x,y) = 0$ if there are no such paths.
%}
%\footnote{\antti{removed gray stuff}}

\tbl{Following~\cite{oneill1983semiriemannian},} we say a path $\alpha([t_1,t_2])$ is a pre-geodesic if  $\alpha(t)$ is a $C^1$-smooth
curve such that $\dot\alpha(t)\not =0$ 
on $t\in [t_1,t_2]$, and there exists a \tbl{reparametrization} of $\alpha([t_1,t_2])$ so that it becomes a geodesic. 
Proposition 10.46 of \cite{oneill1983semiriemannian} implies the existence of a shortcut path between points which are not connected by lightlike pre-geodesics: 

\begin{lemma}[Shortcut Argument]\label{shortcut_lemma}
\tbl{Let $(M,g)$ be globally hyperbolic and }$x,y,z\in M$. Suppose that $x$ can be connected to $y$ by a future-directed lightlike geodesic $\gamma_{x\to y}$, and $y$ can be connected to $z$ by a  future-directed lightlike geodesic $\gamma_{y\to z}$. Additionally, assume that $\gamma_{x\to y}\cup\gamma_{y\to z}$ is not a lightlike pre-geodesic.
Then, there exists a timelike geodesic connecting $x$ to $z$.~\f{Let's say what the shortcut argument implies, and where it is used.}
\end{lemma}

%\begin{proof}
%The proof uses an elementary geometric fact.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Proof of Proposition \ref{kooasu}
%
%
We now prove Proposition \ref{kooasu}:

\begin{proof}[Proof of Proposition \ref{kooasu} ]\label{89347jjaa}
%\textbf{Step 1.}
%Let $\mathcal{C}$ be a Cauchy surface of $(M,g)$.
Let $U$ be an open neighborhood of $z_1$, small enough so that $G_{S_1}\cap U$ and $G_{S_2}\cap U$ are manifolds and that $U\cap (\pi(S_1)\cup \pi(S_2))=\emptyset$. 
% % % \tbg{is a manifold~\f{Do we need the subscript in $U$? I removed it elsewhere in the proof.} be a coordinate neighbourhood that is centered at the first intersection point $z_1$ and of the form (\ref{turhautuminen1}) for $Y_1 = \{ \hat{x}, \hat{p} \}$, $Y_2 = K_{S_2}$, $j=1,2$,~\f{What is $Y_1$ now?} (cf. conditions of Theorem \ref{sofisti_further}). 
% % % Again, this is possible due to our construction of $S$ which comes from Lemma \ref{two_manifold_jacobi_const}.}
% % % %Throughout the proof we shall denote $U= U_{z_1}$.w_{M_2}
Let $P: U\to L^+(U)$ be an arbitrary smooth section on $U$. We remark that we will choose a specific $P$ later in the proof. %and we will also redefine $U$ smaller if that is necessary. \tbg{by restricting the section $\tilde{P}$ from Lemma $\ref{ooiiuu}$ to a certain neighbourhood).}

% {\color{blue}

Let $h_1^\eps$ and $h_2^\eps$ be the respective approximations of the distributions $\chi_{R}\s\delta_{S_1}$ and $\delta_{S_2}$ as described in~\eqref{regu}-\eqref{solution_with_delta_source} compactly supported in $\PP^+M$. (We do not multiply $\delta_{S_2}$ with a cutoff function, since $S_2$ is just a point.) %--~\eqref{approx_sol_prop}. 
For $j=1,2$, let $u_j^\eps$ be the solutions corresponding to $h_j^\eps$: % to
\begin{equation}\label{regularized_equation}
\begin{split}
\XX u_j^\eps  &= h_j^\epsilon \text{ on } \SP M \\
u_j^\eps &= 0 \text{ on } \SP \mathcal{C}^-.
\end{split}
\end{equation}
%as described~\ref{delta_dist_of_subm}. 
By Lemma \ref{deriv} we have that the second linearization $\Phi''$ of the source to solution map $\Phi$ satisfies 
\begin{equation}\label{second_lin_solves}
\begin{split}
\Phi'' (0\;h_1^\epsilon, h_2^\epsilon)  \circ P  =  \big(\IX\mathcal{Q} [ u_1^\eps , u_2^\eps ]\big)\circ P +  \big(\IX\mathcal{Q} [u_2^\eps , u_1^\eps ]\big)\circ P, \\
 %=  \IX \pi^* \big( \mathcal{Q} [ u_1^\eps , u_2^\eps ]^P \big) +  \big(\IX\mathcal{Q} [u_2^\eps , u_1^\eps ]\big)\circ P,
\end{split}
\end{equation}
where $\IX$ is the solution operator to the Vlasov equation~\eqref{vlasov1}. % on $\OVS M$.
We first study the limit $\epsilon \to 0$ of 
\[
 \mathcal{Q} [ u_1^\eps , u_2^\eps ]\circ P +  \mathcal{Q} [u_2^\eps , u_1^\eps ]\circ P.
\]


%\tbg{We will control the singularities of the limit above and use the microlocal properties of the operator $\IX$ to keep track of their propagation.}
%
Since $h^{\epsilon}_{1}$ and $h^{\epsilon}_{2}$ are supported on $\SP M$ and since $P(x)$ is light-like, we find that 
\begin{equation}\label{tyhja123}
\mathcal{Q}_{loss} [ u_1^\eps , u_2^\eps ] \circ P(x) = \mathcal{Q}_{loss} [u_2^\eps , u_1^\eps ] \circ P(x)=0 .
\end{equation}
Therefore, the light which scatters from the collisions arises only from the terms %~\f{Where did the reversed $1$ and $2$ term go?} 
\[
\mathcal{Q}_{gain}^P [ u_1^\eps , u_2^\eps ]= \mathcal{Q}_{gain} [ u_1^\eps , u_2^\eps ] \circ P \ \ \text{and} \ \ \mathcal{Q}_{gain}^P [ u_2^\eps , u_1^\eps ]= \mathcal{Q}_{gain} [ u_2^\eps , u_1^\eps ] \circ P.
\]
%We can therefore replace $\mathcal{Q}$ above by $\mathcal{Q}_{gain}$. 

% {\color{blue}

\antti{By the discussion in Section~\ref{approx_delta_dists} we have that, away from $S_1$ and $S_2$, the element $  \IX(\chi_R\s \delta_{S_1})$ lies in $ I^{n/2-1/4}(\SP M; N^*K_{S_1})$ and $  \IX(\delta_{S_2})$ lies in $ I^{1-1/4}(\SP M; N^*K_{S_2})$. 
%where $\text{supp}(\chi_1),\text{supp}(\chi_2)\subset\subset \SP M\setminus (S_1\cup S_2)$ and $\chi_1$ and $\chi_2$ equal $1$ on $\SP U$. 
Therefore, if $\Gamma$ is any conical neighborhood of $\Lambda_1\cup\Lambda_2$, where $\Lambda_1$ and $\Lambda_2$ are as in Property~\ref{intersection_coords}, we have by \antti{Corollary} \ref{sofisti_further} that 
\begin{equation}\label{thiscvo}
\begin{split}
   \mathcal{Q}_{gain}^P& [ \IX \delta_{S_2} , \IX (\chi_R\s\delta_{S_1}) ] +  \mathcal{Q}_{gain}^P [ \IX (\chi_R\s \delta_{S_1}) ,  \IX \delta_{S_2}  ]  \\
 &\in I^l(\Lambda_0 \setminus (\Lambda_1 \cup \Lambda_2)\;U) + \mathcal{D}_\Gamma'(U) \subset \mathcal{D}'(U),
 \end{split}
 \end{equation}
 where $l=(n/2-1/4)+(1-1/4)+3n/4-1/2=5n/4$ \antti{and $U$ is a small neighbourhood around $z_1$. }
 Here we use the standard notation to denote 
 \[
 \begin{split}
%& \Lambda_1 = \Lambda_{(\hat{x},\hat{p})}, \quad \Lambda_2 = \Lambda_M, \quad
%
 \mathcal{D}_\Gamma'(U) = \{ u \in \mathcal{D}'(U)\s:\s WF(u) \subset \Gamma \}.
% \in I ( \Lambda_M ,  \Lambda_{\{ (\hat{x} , \hat{p}) \}}  ) +  I (    \Lambda_{\{ (\hat{x} , \hat{p}) \}}  , \Lambda_M)
 \end{split}
\]
 %See discussion in Section~\ref{approx_delta_dists}. % and $\supp(\chi_1)\in \SP M\setminus S_2$
%up to a residual with singular support in a small neighbourhood of $ (\Lambda_1 \cup \Lambda_2)$. 
By continuity of $\IX$ (see Section~\ref{approx_delta_dists}) and $\mathcal{Q}_{gain}$ (Corollary \ref{sofisti_further}), the distribution~\eqref{thiscvo} equals the limit
\begin{equation}\label{implieslimit}
\lim_{\epsilon\rightarrow 0} \big( \mathcal{Q}_{gain}^P [ u_1^\epsilon , u_2^\epsilon ] +  \mathcal{Q}_{gain}^P [ u_2^\epsilon,  u_1^\epsilon  ]\big),
\end{equation}
\tbl{ in $\mathcal{D}'(\SP M)$.} It also follows by definition of the collision operator and $\text{supp} (u_j^\epsilon ) \subset K_{\text{supp}(h_j^\epsilon)}$ that the support of \eqref{implieslimit} focuses close to the intersection point $z_1$ as $\epsilon \to 0$. In particular, we may consider it as a compactly supported distribution in $U$.
Now let $P$ be a restriction of a section in Lemma \ref{ooiiuu} for $k=2$, $(x_1,p_1)=(z_1, \dot\gamma(0))$ and $(x_2,p_2) = (e,\dot\gamma(T))$ where $\gamma$ is the optimal geodesic connecting $z_1$ to $e$. Then the terms in \eqref{second_lin_solves} satisfy
\begin{align}
 (  \IX  \mathcal{Q}_{gain} [ u_1^\eps,u_2^\eps ]  ) \circ P   &= P^{-1}  \mathcal{Q}_{gain}^P [ u_1^\eps,u_2^\eps ]  ,
 % \longrightarrow P^{-1} \mathcal{Q}_{gain} [ \IX \delta_{S_2} , \IX (\chi_R\s\delta_{S_1}) ]  , 
 \\
 ( \IX  \mathcal{Q}_{gain} [ u_2^\eps,u_1^\eps ]  ) \circ P &=   P^{-1} \mathcal{Q}_{gain}^P [ u_2^\eps,u_1^\eps ] ,
 %\longrightarrow P^{-1} \mathcal{Q}_{gain} [ \IX \delta_{S_2} , \IX (\chi_R\s\delta_{S_1}) ]
\end{align}
where $P^{-1} : C_c^\infty (U) \to C^\infty(V_e)$, $P^{-1} \phi (x) := \int  \phi ( \gamma_{x,p(x)} (t) ) dt$, i.e. the integration along integral curves of the light-like field $P$. Here $V_e$ is a small neighbourhood of $e$ in the domain of the field. 
% and $f_1$ and $f_2$ are initial values invariant in the flow of $P$. 
The canonical relation of the Fourier integral operator $P^{-1}$ is
\[
C= \{ ( x, \xi ; y  , \eta) \in T^*V_e \setminus \{0\} \times T^*U \setminus \{0\} : x = \gamma_{y,p(y)} (t) , \ \xi,\eta \perp \gamma_{y,p(y)}   \}
\]
 and the symbol is a non-vanishing constant. 
Since light-like geodesics intersect cleanly the time-like flow-outs $G_{S_1} = \pi \Lambda_1$ and $G_{S_2} = \pi \Lambda_2$ and a single point $\pi \Lambda_0$, it is straightforward to check that the expressions above extend also to the limit $\epsilon \to 0$ (See e.g. \cite{duistermaat2010fourier}). Hence, 
\begin{align}
 ( \IX  \mathcal{Q}_{gain} [ u_1^\eps,u_2^\eps ]  ) \circ P  \longrightarrow P^{-1} \mathcal{Q}_{gain}^P [\IX (\chi_R\s\delta_{S_1}),  \IX \delta_{S_2}  ], 
 %\\
 %(  \IX  \mathcal{Q}_{gain} [ u_2^\eps,u_1^\eps ]  ) \circ P   \longrightarrow P^{-1} \mathcal{Q}_{gain} [ \IX \delta_{S_2} , \IX (\chi_R\s\delta_{S_1}) ]  , 
\end{align}
and away from $\Lambda_1$ and $\Lambda_2$ we have the standard principal symbol formulas (cf. \cite[(4.2.10)]{duistermaat2010fourier}
\begin{align}
&\sigma ( P^{-1} \mathcal{Q}_{gain}^P [\IX (\chi_R\s\delta_{S_1}),  \IX \delta_{S_2}  ]  )  
= \sum  \sigma ( P^{-1} )\sigma (\mathcal{Q}_{gain}^P [\IX (\chi_R\s\delta_{S_1}),  \IX \delta_{S_2}  ] )  \\
&= c  \sum \sigma (\mathcal{Q}_{gain}^P  [\IX (\chi_R\s\delta_{S_1}),  \IX \delta_{S_2}  ]  )   , 
%\\
%\sigma ( P^{-1} \mathcal{Q}_{gain} [ \IX \delta_{S_2} , \IX (\chi_R\s\delta_{S_1}) ]  ) = \sigma ( P^{-1} ) \sigma (\mathcal{Q}_{gain} [ \IX \delta_{S_2} , \IX (\chi_R\s\delta_{S_1}) ]  ) \\
%\simeq \sigma (\mathcal{Q}_{gain} [ \IX \delta_{S_2} , \IX (\chi_R\s\delta_{S_1}) ]  ) 
\end{align}
for composition of Fourier integral operators. 
Analogous identities hold for the other term. Thus, following the standard composition calculus for Fourier integral operators, it suffices to show that the symbol of $\mathcal{Q}_{gain}^P  [\IX (\chi_R\s\delta_{S_1}),  \IX \delta_{S_2}  ] + \mathcal{Q}_{gain}^P  [  \IX \delta_{S_2}, \IX (\chi_R\s\delta_{S_1})  ] $ is not of order $-\infty$ at any direction in $\Lambda_0= T_{z_1}^* M$ away from $\Lambda_1$ and $\Lambda_2$. This, however, follows from Theorem \ref{sofisti} together with the  formulas $\sigma(\IX \delta_j )  \simeq \sigma(\delta_{S_2}) \simeq 1$ and $\sigma(\IX \chi_R \delta_{S_1} )  \simeq \chi_R \sigma(\delta_j) \simeq \chi_R$ for principal symbols.
}
\end{proof}
%\[
%\sigma(\IX f ) = \sigma (\IX ) \sigma(f) \simeq \sigma(f).
%\]
%for principal symbol.  
% % % % % % % % % % % % % % % % % % % % % % % % % %  \end{proof}
 
Let $S_1$ and $S_2$ be as earlier. Then, $G_{S_1} =  \pi K_{S_1} $ and $G_{S_2} = \pi K_{S_2}$ intersect in $ \pi(\text{supp}(A))$ only finitely many times and at discrete points. Given that the intersections exist, we can write  $\{z_1, \dots, z_k\} = \pi(K_{S_1})\cap \pi(K_{S_2})\cap \pi(\text{supp}(A))$.
\begin{lemma}\label{estupido}
\antti{As above, denote the points in $\pi(K_{S_1})\cap \pi(K_{S_2})\cap \pi(\text{supp}(A))$ by $z_1,\dots, z_k$ (if exist) and  \tbl{arrange them so that $z_1\ll z_2\ll\cdots\ll z_k$. %Let $V$ be an~\f{What is $V$ suppose to be here? Add}% be the intersections of $\gamma_{(\hat{x},\hat{p})}(s)$, $s > 0$, and $\gamma_{(\hat{y},\hat{q})}(s')$, $s'>0$, inside $\text{supp}(x \mapsto A(x, \cdot,\cdot,\cdot, \cdot))$ if they exist. 
For every section} $P$ of the bundle $L^+V$ } we have
\[
\text{supp}( \sslimit_P) \subset
%\mathcal{L}^+   \big[ \gamma_{(\hat{x},\hat{p})} (0,\infty) \cap  \gamma_{(\hat{y},\hat{q})}(0,\infty) \cap \text{supp}(x \mapsto A(x, \cdot,\cdot,\cdot, \cdot)) \big]=
\bigcup_{l=1}^k \mathcal{L}^+(z_l) \subset  J^+(z_1),
\]
or $\text{supp}( \sslimit_P) = \emptyset$ if $\pi(K_{S_1})\cap \pi(K_{S_2})\cap \pi(\text{supp}(A)) = \emptyset$. 
Here we denote
\[
\sslimit_P := \lim_{\epsilon \rightarrow 0} (\Phi''( 0 ; h_1^\epsilon, h_2^\epsilon) \circ P ).
\]
\tbl{In particular, if for some section $P$ we have that $\text{supp}( \sslimit_P) \neq \emptyset$,} then the first intersection point $z_1$ exists.  
\begin{proof}
\antti{Let us adopt the notation of the proof of Proposition \ref{kooasu}.
One checks that}
\[
 \text{supp}\big(\mathcal{Q}_{gain}^P [u_1^\eps , u_2^\eps ] +  \mathcal{Q}_{gain}^P [ u_2^\eps,  u_1^\eps  ]\big) \subset E_\epsilon 
\]
\tbl{and
\[
\Phi''( 0 ; h_1^\epsilon, h_2^\epsilon) \circ P %= \IX \mathcal{Q}_{gain}^P [u_1^\eps , u_2^\eps ] +  \IX \mathcal{Q}_{gain}^P [u_2^\eps,  u_1^\eps  ]
=\int_{-\infty}^0  \mathcal{Q}_{gain}^{\tbl{P}} [ u_1^\eps , u_2^\eps ]  ( \gamma_{(x,p(x))} (s) ) + \mathcal{Q}_{gain}^{\tbl{P}} [ u_2^\eps , u_1^\eps  ]  ( \gamma_{(x,p(x))} (s) ) ds, 
\]
}
where for $\epsilon>0$ 
\[
E_\epsilon := G_{\text{supp} ( h_1^\epsilon)}^+ \cap G_{\text{supp} ( h_2^\epsilon)}^+ \cap \pi(\text{supp}(A)) .
% (x \mapsto A(x, \cdot,\cdot,\cdot,\cdot)), %\ \ \epsilon>0, %\text{supp} (x \mapsto A(x, \cdot,\cdot,\cdot,\cdot))
\]
%\tbl{satisfy $E_{\eps_1}\subset E_{\eps_2}$, $0< \eps_1\leq \eps_2$. }
\antti{As $E_\epsilon$ is a monotone sequence }it has the limit which is $\bigcap_{\epsilon>0} E_\epsilon = \{z_1,\dots,z_k\}$.
Thus, we obtain 
\[
\text{supp}( \Phi''( 0 ; h_1^\epsilon, h_2^\epsilon) \circ P ) \subset  \mathcal{L}^+ E_\epsilon
\]
and hence
\[
\text{supp}( \sslimit_P ):= \text{supp}(  \lim_{\epsilon \rightarrow 0} (\Phi''( 0 ; h_1^\epsilon, h_2^\epsilon) \circ P ) ) \subset \bigcap_{\tbl{\epsilon>0}} \mathcal{L}^+ E_\epsilon = \mathcal{L}^+ \{ z_l, \dots, z_k \} = \bigcup_{l=1}^k \mathcal{L}^+ (z_l)
\]
%By transitivity property of the past and future relation we have 
\tbl{It also follows from the definition of $\mathcal{L}^+$ and $J^+$ that $\bigcup_{l=1}^k \mathcal{L}^+ (z_l) \subset J^+(z_1)$.}
\end{proof}
\end{lemma}
In our inverse problem we will observe the $\text{supp}(\sslimit_P)$ and use the last claim of Lemma~\ref{estupido} to detect the collision of particles in a subset $W\subset M$.

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  Time separation fuctions
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 
 \subsection{Separation time functions }\label{time_sep_fnct}
Let $(M,g)$ be a $C^\infty$-smooth, globally hyperbolic, Lorentzian manifold. Also, let $\hat{\mu}:[-1,1]\to M$ be a given smooth, future-directed, timelike geodesic, and $V$ be an open neighbourhood of $\hat{\mu}$.  In this subsection we will use $g|_V$, $\hat{\mu}$ and $V$ to introduce a useful representation for certain points in $M$. 
%the causal diamond $W :=  I^-(\hat{\mu}(1)) \cap I^+(\hat{\mu}(-1))\subset M$. 
Our representation scheme will associate a point $w\in M$ to a subset $\mathcal E_{\mathcal U}(w)\subset {\mathcal U}$, where ${\mathcal U}\subset V$ is an open set. Loosely speaking, the subset $\mathcal{E}_{\mathcal U}(w)$ will be comprised of points in ${\mathcal U}$ which lie on a \tbl{optimal} lightlike geodesic emanating from $w$. This representation was first introduced by Kurylev, Lassas, and Uhlmann in~\cite{Kurylev2018}; we reproduce a summary of it here for the reader's convenience. We later will use this representation to construct the desired isometry $F:W_1\to W_2$ described in Theorem \ref{themain}.
%We introduce concepts from the paperWe do the introduction on a single geodesically complete globally hyperbolic~\f{Do we need global hyperbolicity here?} Lorentzian manifold $(M,g)$. In the subsequent sections, we will use the introduced concepts on two (possibly) different manifolds to ultimately prove Theorem~\ref{themain}.%, these concepts will be relative to two different manifolds. 


% \begin{definition}[Smaller Observation Domain]

To begin, as shown in \cite[Section II]{manasse-misner}, there exists a bounded, connected, open set $\mathcal{A}\subset \R^{n-1}$ and a  neighbourhood $\mathcal{U}\subset V$ of $\hat{\mu}$ on which we may define \tbl{coordinates}
\[
x\in \mathcal{U}\mapsto (s,a^1,a^2,\dots,a^{n-1})\in [-1,1]\times\mathcal{A} %(y^0,y^1,\dots,y^{n-1})\in (-1,1)\times\mathcal{A}.
\]
These coordinates have the property that $\hat\mu(s) =(s,0,\dots,0)$ and for fixed $a= (a^1,a^2,\dots,a^{n-1}) \in \mathcal{A}$ the map $\mu_a(s) = (s,a^1,a^2,\dots,a^{n-1})$ is a $C^\infty$-smooth timelike curve. Further, writing $\mu_{\hat{a}} = \hat{\mu}$ where $\hat{a} = (0,\dots,0)\in \mathcal{A}$, we have
\[
\mathcal{U} = \bigcup_{a\in \mathcal{A}}\mu_a[-1,1].
\]
Let $\overline{\mathcal{A}}$ be the closure of $\mathcal{A}$ in $\R^{n-1}$.
Below, we will assume that for all $a\in \overline{\mathcal{A}}$ we have $\hat{\mu}(s_+)\ll \mu_a(1)$ and 
 $\mu_a(-1)\ll \hat{\mu}(s_-)$.
%
%let $\mathcal{A}\subset V$ be a connected, open, and relatively compact set which parametrizes a smooth variation of $\hat{\mu}$ in $V$.
%

 Given $\mathcal{U}$ and the family of curves $\mu_a$, ${a\in \overline{\mathcal{A}}}$ (which may be defined by replacing $\mathcal{A}$ above by a smaller open subset if necessary), we will next define the notions of time separation functions and observation time functions. 

Consider $-1< s^{-} < s^{+} < 1$ and set $x^{\pm}:= \hat\mu(s^{\pm})\in V$. As in \cite[Definition 2.1]{Kurylev2018}, for each $a\in \overline{\mathcal{A}}$ and corresponding path $\mu_a$, we define the \emph{observation time functions} $f_a^\pm:J^- (x^+) \setminus I^- (x^- )\to \R$ by the formulas
\[
f_a^+ (x) := \inf(  \{ s \in (-1,1) : \tau(x, \mu_a(s) ) > 0 \}  \cup \{1\} ) 
\]
and
\[
f_a^- (x) := \sup(  \{ s \in (-1,1) : \tau(\mu_a(s),x ) > 0 \}  \cup \{-1\} ).
\]
\tbl{Here $\tau$ is the time separation function defined in Section~\ref{sca123}. We note that if $x\in M$ and  $a\in \mathcal{A}$ are such that at least one point in $\mu_a(-1,1)$ can be reached from $x$ by a future-directed timelike curve
we obtain $\tau(x, \mu_a( f_a^+ (x) ) ) = 0$, see \cite{Kurylev2018}.~\f{Check that this is found from the paper, add location. -Tony} In this case, there also
%there 
exists a future-directed optimal light-like geodesic that connects $x$ to $\mu_a(f_a^+(x))$ as discussed in Section \ref{sca123}.} 

The  earliest time observation functions  $f_a^+:J^- (x^+) \setminus I^- (x^- )\to \R$
determine the set
\begin{equation}\label{eioreiie-eq}
\mathcal{E}_{\mathcal{U}} (w) = \{ \mu_a (f_a^+ (w) ) : a\in \mathcal{A} \}\subset U,
\end{equation}
that is the \emph{earliest light observation set} of $w\in J^- (x^+) \setminus I^- (x^- )$.

Finally, as shown in \cite[Proposition 2.2.]{Kurylev2018}, we may construct the conformal type of the open, relatively compact set $W\subset J^- (x^+) \setminus I^- (x^- )$ when we are given the collection
of all earliest light observation sets associated to points $w\in W$, that is, 
\[
\mathcal{E}_{\mathcal{U}}(W) =\{ \mathcal{E}_{\mathcal{U}} (w)\,:\, w\in W\} \subset 2^{\mathcal{U}}.
\]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%. Determination of light obs sets from SS map
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 \subsection{Source-to-Solution map determines earliest light observation sets}\label{ss_elos}
 %\antti{
 %\\
% --------------------------------------------------------------- 
% \\
% EDITING THIS SECTION AT THE MOMENT. GOT TIRED OF USING THE COLORS. --Antti \\
% \\
% ---------------------------------------------------------------
%  \\
% --------------------------------------------------------------- \\
% --------------------------------------------------------------- \\
% --------------------------------------------------------------- \\
% --------------------------------------------------------------- \\
% }
 
In this section, we prove that the source-to-solution map for light observations (see \eqref{light-source-soln})
of the Boltzmann equation on a subset $V$ of a manifold determines the earliest light observation sets on a  subset of the manifold which properly contains $V$. We will define such a set below. % The set $W$ depends on $V$ set by a causality condition. %the location of the sources and where measurements are made. %determined by casuality conditions. that depends o, which depends naturally on the set where  described in Section \ref{time_sep_fnct} for subsets of the manifold satisfying causuality properties. 
After proving this, the main result of this paper, Theorem \ref{themain}, will follow by applying~\cite[Theorem 1.2]{Kurylev2018}, which states that the earliest light observation sets determine the Lorentzian metric structure of the manifold up to conformal class. % Theorem 1.2 of Kurylev, Lassas, and Uhlmann \cite{Kurylev2018}. 
%In contrast to the result, in our setting the source-to-solution data allows us to recover the conformal factor, and hence the complete metric on the unknown set. This is shown in the last section. 
 
% \subsection{Diffeomorphism $W_1 \cong W_2$}\label{uptocon}
  
 %To prove the uniqueness statement of Theorem \ref{themain}, we now consider the following setting. 
 
From this point onwards, we assume that $(M_1,g_1)$ and $(M_2, g_2)$ are two geodesically complete, globally hyperbolic, $C^\infty$-smooth, Lorentzian manifolds, which contain a common open subset $V$ and %~\f{I did this assumption here early on, since we will use it anyhow.} 
 \[
g_1|_V=g_2|_V.  
 \]
 We assume that $\hat\mu:[-1,1]\to V$ is a given future-directed timelike geodesic. Let $\mathcal{A}\subset \R^{n-1}$, the family of paths $(\mu_a)_{a\in \mathcal{A}}$, and the subset $\mathcal{U}\subset V$ be as in the Section \ref{time_sep_fnct}.

% % %  
 For $-1< s^{-} < s^{+} < 1$, we set $x^{\pm}:= \hat\mu(s^{\pm})\in V$ and define%~\f{Removed $\lambda$ from the notation. } %subset of $M_1$ and $M_2$  and let 
 \begin{align}
 W_1 &:=  I^-(x^{+}) \cap I^+(x^{-})\subset M_1 \ \ \text{defined with respect to $(M_1,g_1)$},\label{ppa1}
 \\
 W_2 &:=  I^-(x^{+}) \cap I^+(x^{-})\subset M_2 \ \ \text{defined with respect to $(M_2,g_2)$}\label{ppa2}.
 \end{align}
 Additionally, for $\lambda=1,2$, let $A_\lambda$ be an admissible collision kernel (see Definition \ref{good-kernels}) with respect to the space $(M_\lambda,g_\lambda)$ and write $\Phi_{\lambda,L^+V}$ for the source-to-solution map for light observations (see Equation \eqref{light-source-soln}) associated to the relativistic Boltzmann equation \eqref{boltzmann} with respect to $g_\lambda$.  The notation $\Phi_\lambda$ denotes the full source to solution map for \eqref{boltzmann}.%Likewise, let $A_2$ be an admissible collision kernel with respect to $(M_2,g_2)$ and write $\Phi_2$ for the source-to-solution map for light observations associated to the relativistic Boltzmann problem \eqref{boltzmann} with respect to $g_2$. 
 
% We use the following shorthand notation throughout the rest of this paper: if there exists an isometry $\Xi: (V,g_1|_V) \to (V,g_2|_V)$ such that $\Phi_{2,L^+V}  =  (T \Xi^{-1})^* \circ \Phi_{1,L^+V} \circ T\Xi^*$, we write $\Phi_{1,L^+V}=\Phi_{2,L^+V}$ (and likewise for the maps $\Phi_\lambda$).
 
In the above setting we prove:
\begin{repproposition}{ss_map_first_obs}
Let $\Phi_{1,L^+V}$ and $\Phi_{2, L^+V}$ be the above source-to-solution maps for light observations.  
%Assume that the conditions of Theorem \ref{themain} are satisfied for $(M_j,g_j)$, $j=1,2$. %, fix $w_{M_1}\in W_1$ and let $w_{M_2}\in W_2$ be as described above. 
Then  $\Phi_{1,L^+V}=\Phi_{2, L^+V}$ implies
%\[
%\mathcal{E}_{\mathcal{U}} (w_{M_1}) = \mathcal{E}_{\mathcal{U}} (w_{M_2})
%\]
\[
\mathcal{E}^1_{\s\mathcal{U}}({W_1}) = \mathcal{E}^2_{\s\mathcal{U}}({W_2}). % (w_{M_2})
\]
\end{repproposition}
%   

We prove Proposition~\ref{ss_map_first_obs} by showing that $\Phi_{1,L^+V}=\Phi_{2,L^+V}$ implies the existence of a diffeomorphism
\[
F:W_1 \rightarrow W_2 \]
 which satisfies 
 \[
 \mathcal{E}_{\s\mathcal{U}}^1(w_1) = \mathcal{E}_{\s\mathcal{U}}^2(F(w_1)),\quad w_1\in W_1.\]
 
To construct the map $F:W_1 \rightarrow W_2$, consider the observation time functions on $(M_j,g_j)$, $j=1,2$ which we denote by $f_{a,j}^{\pm}$. For each 
\[
w_1 \in W_1\subset M_1,
\]
we define $\eta_{w_1}$ to be an optimal future-directed light-like geodesic in $M_1$ such that
\begin{equation}\label{9090sdj}
\eta_{\s {w_1}} (0) = \hat\mu (f_{\hat{a},1}^- (w_1) ) \text{ and }\eta_{\s {w_1}}(T) = w_1 \text{ for some }T>0.
\end{equation}
%and $a\in \mathcal{A} \setminus \hat{a}$.
By the definition of $W_1$ such $\eta_{\s {w_1}}$ exists. In the following, $w_1$ will be fixed and we abbreviate
\[
 \eta_1:=\eta_{\s w_1}.
\]

% We also use the notation
% \[
%  \eta_{\s w_1}:=\eta_1
% \]
% to remind about the dependence of $\eta_1$ on the point $w_1\in M_1$.

Since $\mathcal{U}$ is open and $\text{dim}(M_1)=\nnn>2$, we may choose
%\begin{equation}\label{9090sdjl}
%$a \in \mathcal{A} $ such that $a\neq \hat a$ and on the maximal (inextensible) domain $\eta_{\s {1}}$ does not hit  $\mu_a(-1,1)$.  %\quad \eta_{\s {1}} \cap \mu_a(-1,1) = \emptyset ,
%\end{equation}
%We fix 
another future-directed optimal light-like geodesic $\widetilde{\eta}_{\s 1}$ that is not tangential to $\eta_1$ and satisfies
\begin{equation}\label{9090sdjlk}
\widetilde{\eta}_{\s {1}}(0) = \mu_a (f_{a,1}^-(w_1)) \text{ and }\widetilde{\eta}_{\s {1}}(\widetilde{T}) = w_1\text{ for some }\widetilde{T}>0,  \quad  a\in \mathcal{A} \setminus \hat{a}.
\end{equation}
%One may also assume that the initial value $\widetilde{\eta}_{\s {1}}(0)$ belongs to the same Cauchy surface as $\eta_1(0)$. 
Since both segments $\eta_1|_{[0,T]},\tilde\eta_1|_{[0, \widetilde{T}]}$ are optimal, the shortcut argument implies that $\eta_{\s {1}}(s)$, $s>0$ and $\widetilde{\eta}_{\s {1}}(s')$, $s'>0$ intersect the first time at $w_1$. 

% % % % 

In the lemma below we approximate the light-like geodesics $\eta_{1}$ and $\tilde{\eta}_{1}$ by  time-like geodesics
\[
\gamma_{(\hat{x},\hat{p})}(s) \text{ and } \gamma_{(\hat{y},\hat{q})}(s) ,  \quad s>0, \quad (\hat{x}, \s \hat{p})\in \mathcal{P}^+V, \quad  (\hat{y}, \s \hat{q})  \in \mathcal{P}^+V
\]
that \underline{intersect for the first time at $w_1$ as geodesics in $M_1$}.
%that as geodesics in $M_1$ intersect first time at $w_1$ and  satisfy 
%respectively. 
%This is done as follows. %Here $(\hat{x}_l,\hat{p}_l)\in P^{m_1}M_1$ and $(\hat{x}_l,\hat{p}_l)\in P^{m_2}M_1$.~\f{Can we replace $M_1$ by $W_1$ or $V$ here?} 
%By Lemma \ref{druqks} in Appendix, % given $m_1,m_2>0$  and $\mathcal{U}\subset V$ as defined in section \ref{time_sep_fnct}, 
%there exists a sequences $(\hat{x}_l,\hat{p}_l) \in P^{m_1} (\mathcal{U} \cap W_1 \cap W_2) $ and $(\hat{y}_l,\hat{q}_l) \in  P^{m_2} (\mathcal{U} )$, and positive numbers $\lambda_l$ and $\lambda_l'$ (which tend to infinity along $l$), such that 
One may always fix the geodesics such that $\hat{x}$ and $\hat{y}$ belong to a  same  Cauchy surface and 
%\[
$(\hat{x}, \s \hat{p}) $ is arbitrarily near the curve   $(\gin,\dgin)$, and $(\hat{y}, \s \hat{q})  $ is arbitrarily near the curve $  (\ginp, \dginp)$.
%\]
%as $l\to \infty$.
Notice the abuse of notation: $\gamma_{(\hat{x},\hat{p})}$, $\gamma_{(\hat{y},\hat{q})}$ may refer to a pair of geodesics either in $(M_1,g_1)$ or $(M_2,g_2)$. 
 Due to global hyperbolicity we may always redefine the initial vectors by sliding them along the geodesic flow so that $\hat{x}$ and $\hat{y}$ lie in a Cauchy surface. 
% The reason why we need to consider approximative geodesics is that our 
 Let $\eta_2$ and $\tilde{\eta}_2$ be the geodesics in $(M_2,g_2)$, which %let $\tgin$ and $\tginp$ be the analogous geodesics 
 have the same initial data  with $\eta_{1}$ and $\tilde{\eta}_{1}$ respectively:
 \begin{equation}\label{last_geo}
  \dot{\eta}_2(0)=\dot{\eta}_{1}(0)\in T_{\eta_{1}(0)}\mathcal{U} \text{ and } \dot{\tilde{\eta}}_2(0)=\dot{\tilde{\eta}}_{1}(0)\in T_{\tilde{\eta}_{1}(0)}\mathcal{U}.
 \end{equation}
 (Recall that $ \mathcal{U} \subset V$ is a mutual set of $M_1$ and $M_2$ so that this makes sense.)

 %$(\gin(0), \dgin(0)) = ( \tgin(0),\dtgin(0))$ and $(\ginp(0), \dginp|_{s=0}) = ( \tginp(0),\dtginp|_{s=0})$. 
% %  {\color{gray}
% %  Let $w_{M_2}$ (which at this point may or may not lie in $W_2$ or even exist) be the first intersection of $\tgin (s)$, $s>0$ and $\tginp (s') $, $s'>0$.
% %  Assuming that the conditions of Theorem \ref{themain} are satisfied, each $w_{M_1}$ in $W_1$ is connected to corresponding $w_{M_2}$ in $W_2$. This is mainly due to identical source-to-solution operators. 
% %  }
 
 %By assuming the conditions of Theorem~\ref{themain},~\f{Write precisely after the claim of Theorem~\ref{themain} is fixed/finalized.} 
We thus define  
 \[
F :W_1 \rightarrow W_2  
 \]
as the map which assigns a given point $w_1\in W_1$ to the first intersection of $\eta_2(s)$, $s>0$ and $\tilde{\eta}_2(s')$, $s'>0$ denoted by $w_2\in M_2$.  For the assignment $w_1\mapsto w_2$ to be well-defined, we of course need to show that the first intersection $w_2$ exists and lies in $W_2$. There are also many choices for the geodesics $\eta_1$ and $\tilde{\eta}_1$ on $(M_1,g_1)$, which are used to define $\eta_2$ and $\tilde{\eta}_2$ on $(M_2,g_2)$. Therefore we need also to show that $w_2$ is independent of our choices of $\eta_1$ and $\tilde{\eta}_1$. These necessities are proven in Lemma~\ref{ss_map_determines_intersection} below. %After proving the lemma,  %In this geometry, we use the same source data as constructed % in the case of $(M_1,g_1)$.
 \begin{figure}[h]
\begin{tikzpicture}[scale=2]
%ELLIPSE:
    \draw[fill=gray!20] (0,0) ellipse (0.5cm and 2.7cm); 
%SMALL DETAIL TO CREATE 3D PERSPECTIVE :   
    % \draw[gray,dashed] (0,0) ellipse (0.5cm and 0.1cm);
%VERTICAL LINES:    
    \draw (0,-2.7) -- (0,2.7);
    \draw (0.25,-1.5) -- (0.25,1.5);
%RAYS:    
    \draw[thick] (0,-0.5) -- (1,0.5);
      \draw[blue,thick] (-0.03,-0.7) -- (1,0.5) -- (1.515,1.1);
    \draw[thick] (0.25,-0.5) -- (1,0.5);
      \draw[blue,thick] (0.27,-0.7) -- (1.365,1.1);
%DIAMOND:
    \draw (0,1.8) -- (2,0) -- (0,-1.8) -- (-2,0) -- (0,1.8);
%INTERSECTION POINT:  
    \filldraw[red] (1,0.5)  circle (1pt);
%LABEL OF THE INTERSECTION POINT:    
  \node[red] at (1.3,0.3) {$w_{1}$};
\end{tikzpicture}
\caption{Given $w_{1} \in W_1$ (in red) the light-like geodesics $\gin,\ginp$ (in black) are chosen such that they maximize distance between their initial points in $\mathcal{U}$ (in gray) and $w_{1}$. The timelike geodesics $\gamma_{(\hat{x},\hat{p} )}$ and $\gamma_{(\hat{x},\hat{p} )}$ (in blue) intersect first time at $w_{1}$ and approximate the light-like segments.
%{\color{red}(This is a tikz picture so you can modify it directly in the tex file here. --Antti)}
}
\end{figure}
 
 %To prove Proposition~\ref{ss_map_first_obs} we begin with a lemma.
 \begin{lemma}\label{ss_map_determines_intersection}%there is an isometry $\Xi: (V,g_1|_V) \to (V,g_2|_V)$ such that $\Phi_{2}  =  (T \Xi^{-1})^* \circ \Phi_{1} \circ T\Xi^*$
 
 Let $(M_j,g_j)$, $\mathcal{U}\subset V \subset M_j$, $W_j \subset M_j$, $\Phi_{j}$ for $j=1,2$ be as described above. %the source-to-solution maps described above and assume that the conditions of Theorem \ref{themain} are satisfied for both $M_j$, $j=1,2$.~\f{Write precisely after the claim of Theorem~\ref{themain} is fixed/finalized. Let's use two manifolds $M_1$ and $M_2$ in the statement.} 
 Let $w_{1} \in W_1$  and consider light-like future-directed geodesics $\eta_{1}(s)$, $s>0$, $ \tilde{\eta}_{1}(s')$, $s'>0$ in $(M_1,g_1)$ with \eqref{9090sdj} and \eqref{9090sdjlk} intersecting the first time at $w_1$. Let $\eta_2$ and $\widetilde\eta_2$ be the associated light-like geodesics in $(M_2,g_2)$ with the initial conditions $( \eta_2(0), \dot\eta_2(0)) = ( \eta_1(0), \dot\eta_1(0))$ and $( \tilde\eta_2(0), \dot{\tilde\eta}_2(0)) = ( \tilde\eta_1(0), \dot{\tilde\eta}_1(0))$. 
% \[
%\eta_{1},\  \tilde{\eta}_{1},\ \eta_2,\ \tilde{\eta}_2,\ \gamma_{(\hat{x}_l,\hat{p}_l)} \text{ and } \gamma_{(\hat{y}_l,\hat{q}_l)}
% \]
%be the geodesics described above in the lines between \eqref{9090sdj} and \eqref{last_geo}. 
Then the condition $\Phi_{1,L^+V}=\Phi_{2,L^+V}$ implies the following:
\begin{enumerate}
\item %For every $w_{M_1}\in W_1$ 
There exists the first intersection  $w_2$  of $\tgin(s)$, $s>0$ and $\tginp(s')$, $s'>0$ in $(M_2,g_2)$. Moreover, $w_2 \in W_2$.  % the point $w_{2}$ exists.  
\item The first intersection point $w_{2}$ is independent from the choice of the geodesics $\gin $, $\ginp $ satisfying the required conditions above. %  yields  the same $w_{2}$. 
\item For every  pair $(\hat{x},\hat{p}) \in \mathcal{P}^+ V$ and $(\hat{y},\hat{q}) \in   \mathcal{P}^+ V $ 
%(elements of the sets (\ref{linea1}),(\ref{linea2})) 
with the geodesics $\gamma_{(\hat{x},\hat{p})}(s)$, $s>0$, and $\gamma_{(\hat{y},\hat{q})}(s')$, $s'>0$ in $(M_1,g_1)$ intersecting the first time at $w_{1}$, the associated geodesics in $(M_2,g_2)$ intersect for the first time at $w_2$. 
%$w_{M_2}$ above is the first intersection of the timelike estimates $\gamma_{(\hat{x},\hat{p})}$ and $\gamma_{(\hat{y},\hat{q})}$ in the space $(M_2,g_2)$. 
%(In your notation above you've used tildes to distinguish gammas in $M_2$ from those in $M_1$. I haven't). -Antti}   
\end{enumerate}

\end{lemma}




%In this section, we show that our source-to-solution map data captures information about the earliest light observation sets for points in $W_{1}$ and $W_{2}$. That is,







%\begin{lemma}\label{ewekk}
%Under the assumptions of Theorem \ref{themain}, for every $w_{M_1}\in W_1$ the geodesics $\tgin (s)$, $s>0$ and $\tginp (s') $, $s'>0$ of the space $(M_2,g_2)$ intersect in $W_2$.
%Further, the first intersection point $w_{M_2}$ in $(M_2,g_2)$ is independent of the choice of the light-like future directed geodesics $\gin $, $\ginp $ defined as above and satisfies
%\[
%\mathcal{E}_{\mathcal{U}} (w_{M_1}) = \mathcal{E}_{\mathcal{U}} (w_{M_2})
%\]
%\end{lemma}

%\tjb{TB: I suggest splitting Lemma \ref{ewekk} into the following:}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Proof of Lemma for SS map determines intersection points
%

%Now are ready to prove Lemma \ref{ss_map_determines_intersection}:
\begin{proof}[Proof of Lemma \ref{ss_map_determines_intersection}]
%As $\Phi_{1}=\Phi_{2}=:\Phi$, by Lemma
%Again, simplify the nomenclature by denoting the image (set) of a geodesic in $M$ with the same symbol as the geodesic. 
 Let $w_1\in W_1$ and let $e \in \mathcal{L}^+ ( w_{1} )$ be a first observation of $w_{1}$ in $\mathcal{U}\subset V \subset M_1$. That is, $e\in \mathcal{E}_{\mathcal{U}}^1(w_1)$. By the fact \eqref{eioreiie-eq} there is a point $a\in \mathcal{A}$ and the corresponding path $\mu_a$ such that
 \begin{equation}\label{diieee4}
 e= \mu_{a}(f_{a,1}^+(w_{1} ) ) \in (M_1,g_1).
 \end{equation}
Let $\gamma_{1}$ be the \tbl{optimal} geodesic in $(M_1,g_1)$ as in Proposition~\ref{kooasu} such that $ \gamma_1(0)=w_{1}$ and $ \gamma_1(1)=e$. %that connects $w_{1}$ to $e$.
%$\eta_1$~\f{The claim of this lemma needs to rewritten.} in $(M_1,g_1)$  $ \gamma_1(0)=w_{1}$ that connects $w_{1}$ to $e$.~\f{Should it be maximizing geodesic as in ?}

We approximate the light-like geodesics $\eta_1$ and $\tilde{\eta}_1$ by time-like geodesics from $(\hat{x},\hat{p})\in  \mathcal{P}^+  V $ and $(\hat{y},\hat{q})\in \mathcal{P}^+ V$ as described earlier by requiring that for the geodesics in $(M_1,g_1)$ their first intersection for positive parameter values is at $w_1$. 
%To simplify the notation let us fix $l=l_0$ for now and write
%\begin{equation}\label{eq:shorthand_not_for_xj_pj}
% (\hat{x},\hat{p}) :=(\hat{x}_{l_0},\hat{p}_{l_0}) \text{ and } (\hat{y},\hat{q}):=(\hat{y}_{l_0},\hat{q}_{l_0}).
%\end{equation}
\tbl{Let $S_2=\{\hat{x},\hat{p}\}\subset P^{m_1}V$. By Corollary \ref{coro_renerew} 
%Lemma~\ref{two_manifold_jacobi_const},
 there exists a submanifold $S_1\subset \mathcal{P}^+ V$ with $(\hat{y},\hat{q})\in S_1$ such that the geodesic flowouts $Y_{j,1} := K_{S_1;M_j} \subset \mathcal{P}^+M_j$ of $S_1$ and $Y_{j,2}:= K_{S_2;M_j} \subset  \mathcal{P}^+M_j$ of $S_2$ in $(M_j ,g_j)$ have an admissible intersection property in the sense of Definition \ref{intersection_coords}} for both $j=1,2$. Therefore, we are in the setting for which the earlier results of this this section and Section~\ref{microlocal-collision} are valid. %Here $K_{1,S_j}$, $j=1,2$, are the geodesic flowouts of $S_j$ in $(M_1,g_1)$. %The intersection of $\pi(Y_{1,1})$ and $\pi(Y_{1,2})$  $z_{1,a}$, $a=1,\ldots, k_1$, as
With this in mind, let us write  
\begin{equation}\label{3249reeeredfds}
 \pi(Y_{1,1})\cap\pi(Y_{1,2})=\{z_{1,1},z_{1,2},\ldots,z_{1,k_1}\}\subset M_1,
\end{equation}
where the intersection points $z_{1,l}$, $l=1,\ldots, k_1$, of $\pi(Y_{1,1})$ and $\pi(Y_{1,2})$ are ordered causally as $z_{1,1}\ll z_{1,2}\ll\cdots \ll z_{1,k_1}$. (The index $1$ in $z_{1,l}$ 
%, $K_{1,S_j}$ and $Y_{1,j}$ 
refers to the manifold $(M_1,g_1)$)
Notice that $z_{1,1} = w_1$. 
For $\eps>0$, let 
\[
 h_1^\eps\in C_c^\infty(\SP V)\text{ and } h_2^\eps\in C_c^\infty(\SP V)                                                                                                                                                                                                                                                                                            \]
be the sequences of approximative delta functions of $S_1$ and $S_2$ described in~\eqref{regu}. 





%by 
%$\hat\mu ( f_{\hat{a}}^+ (w_{M_1}) )$ 
%in the space $(M_1,g_1)$.~\f{Remind why exists.} 
% % % % % %Let $\tilde{\eta}_1$ be another geodesic in $(M_1,g_1)$ with the properties described in~\eqref{9090sdjl}--\eqref{9090sdjlk}. Let also $\eta_2$ and $\tilde{\eta}_2$ be geodesics in $(M_2,g_2)$ described in~\eqref{last_geo}. %Since the geodesic segment maximizes the length function, 
%We denote by $\gout$ also the image of the geodesic. 

%We denote the images of geodesics by the symbol of the geodesics. 
%We also consider geodesics only for positive geometric parameter values if not otherwise stated. Especially, 
%\tbl{When we say that geodesics intersect, we mean that the geodesics intersect for some positive geodesic parameter values.}
%We also consider without further  consider geodesic  for non-negative geodesic parameters.
By Proposition \ref{kooasu} there is a neighbourhood $V_e\subset V$ of $e$ and a section $P_e:V_e\to  L^+V_e$ %,  $x\in V_e$, 
%$e:=\hat\mu ( f_{\hat{a}}^+ (w_{M_1}) )$ 
 such that the distribution %~\f{Do we want here $j=1$ or $j=1,2$?} 
 \[
  \sslimit_1:=\lim_{\epsilon \rightarrow 0} (  \Phi_1'' (0;\s h_1^\epsilon,\s h_2^\epsilon)  \circ P_e )\in \mathcal{D}'(V_e),
 \]
%\sslimit_j:=\lim_{\epsilon \rightarrow 0} (  \Phi_j'' (0;h_1^\epsilon, h_2^\epsilon)  \circ P_e )$, $j=1,2$ 
 satisfies
\[
\text{singsupp}( \sslimit_1) = \gout  \cap V_e.
\]

%Since $V$ is a mutual set of $M_1$ and $M_2$, we also have that $S_1\subset  \mathcal{P}^+M_2$ and $S_2\subset  \mathcal{P}^+M_2$. We denote the respective geodesic flowouts of $S_1$ and $S_2$ with respect to the metric $g_2$ on $M_2$ by $Y_{2,1}$ %and $Y_{2,1}$. 
The index $2$ in $Y_{2,j}$, and in $z_{2,l}$, $\mathcal{L}_2^+$ and $J_2^+$ below, refers to corresponding quantities on the manifold $(M_2,g_2)$. The submanifolds of $Y_{2,1}$ and $Y_{2,2}$ have admissible intersection property by their definition above. %~\f{Need to change notation of Lemma~\ref{two_manifold_jacobi_const}, since $\Phi$ is also the source to solution map.} 


The condition \tbl{$\Phi_{1,L^+V}=\Phi_{2,L^+V}$} %~\f{Do we actually want $\Phi_{j,L}$ here?} 
implies 
\[
 \sslimit_1:=\lim_{\epsilon \rightarrow 0} ( \Phi_1'' (0;\s h_1^\epsilon,\s h_2^\epsilon)  \circ P_e )=\lim_{\epsilon \rightarrow 0} ( \Phi_2'' (0;\s h_1^\epsilon,\s h_2^\epsilon)  \circ P_e ) =:\sslimit_2.
\]
%\sslimit_1= \sslimit_2$ and 
Therefore, we have $\text{singsupp}( \sslimit_2) = \gamma_1 \cap V_e\subset V$ and
\[
 e \in \text{supp} (\sslimit_1)\cap \text{supp} (\sslimit_2).
\]
%   e \in \text{supp} (\sslimit_j )$ for both $j=1,2$.  
Consequently,  the sets $\pi(Y_{2,1})$ and $\pi(Y_{2,2})$ intersect by Lemma \ref{estupido}. Let us denote 
\[
 \pi(Y_{2,1})\cap\pi(Y_{2,2})=\{z_{2,1},z_{2,2},\ldots,z_{2,k_2}\}\subset M_2,
\]
where the intersection points of $\pi(Y_{2,1})$ and $\pi(Y_{2,2})$ are ordered as $z_{2,1}\ll z_{2,2}\ll\cdots \ll z_{2,k_2}$.
At this point we do not know whether $z_{2,1}$ is $w_2$ or not. 
% Let us denote the intersection points of $\eta_2$ and $\tilde{\eta}_2$ by $z_{l,2}$, $l=1,2\ldots, k_2<\infty$, where $z_{1,2}$ is the first intersection point.
%first intersection point by $z_{1,2}$ and the other possible intersection points of $\eta_2$ and $\tilde{\eta}_2$ by $z_{l,2}$, $l=2,\ldots, k_2<\infty$. %, where $k_2<\infty$. 
%re is the first intersection point ~\f{What are? Some geodesics? This part should likely be after defining $\varphi_2$} $z_{1,2}$ in $M_2$  and
By applying Lemma~\ref{estupido} again, we conclude for both $j=1,2$ that
\begin{equation}\label{tytyt}
\gamma_1  \cap V_e \subset \bigcup_{l=1}^{k_j} \mathcal{L}_2^+ (z_{j,l}) \subset J_j^+ (z_{j,1})  \subset (M_j,g_j).
\end{equation}
%(The index $2$ in $z_{l,2}$, $\mathcal{L}_2^+$ and $J_2^+$ refers to corresponding quantities on the manifold $(M_2,g_2)$.~\f{Write better.})
 %$z_{l,2}\in M_2$, $l=1,\ldots,k$. 
In particular, 
\begin{equation}\label{ralksd347}
%  \hat\mu ( f_{\hat{a} }^+ (w_{M_1})) =: 
  e \in  J_j^+(z_{j,1}) \subset (M_j,g_j).
\end{equation}
%for both $j=1,2$.  
%As Lemma~\ref{estupido} also holds for the space $(M_1,g_1)$, the conclusions \eqref{tytyt} and \eqref{ralksd347} hold in both spaces $(M_1,g_1)$ and $(M_2,g_2)$. 

Recall that $V\subset M_j$ for both $j=1,2$ and $g_1|_V=g_2|_V$. Let $\gamma_2$ be the geodesic in $(M_2,g_2)$, which has the same initial condition as $\gamma_1$ at $e$, that is, $(\gamma_2(1) , \dot\gamma_2(1)) = (\gamma_1(1) , \dot\gamma_1(1))$. 
%~\f{Is this the correct definition for $\gamma_2$? It was missing. Write precisely.} %Since by assumption $V\subset M_1\cap M_2$ and $g_1|_V=g_2|_V$, 
%By the assumptions, the manifolds $M_j$, $j=1,2$, and hence 
It follows that the geodesics 
%$\eta_2(t)$ and $\eta_2(t)$ coincide near $e \in V_e \subset V$. 
$\gamma_1$ and $\gamma_2$ coincide in $ V_e \subset V$. 
%By redefining the neighbourhood $V_e \subset V$ of $e$ smaller, if necessary, we may assume that $\gamma_1 \cap V_e =\gamma_2 \cap V_e $. 
Thus,
\begin{equation}\label{uuipaa}
\gamma_l  \cap V_e \subset  \bigcup_{h=1}^{k_j} \mathcal{L}_2^+ (z_{j,h}) \subset J_j^+(z_{j,1}) \subset  (M_j,g_j)
\end{equation}
for every combination of $l=1,2$ and $j=1,2$. 
%
%Thus $\Phi_1=\Phi_2$ provides a link between the first light observations in the spaces $W_1$ and $W_2$. 
%Notice that $\gamma_{(\hat{x},\hat{p})}=\gamma_{(\hat{x},\hat{p}),M_j}$ and $\gamma_{(\hat{y},\hat{q})}=\gamma_{(\hat{y},\hat{q}),M_j}$ above depend on $j=1,2$.  
%As $\Phi_1=\Phi_2$ we can repeat the argument on $M_2$ to obtain 
%\begin{equation}\label{ralksd3472}
%%  \hat\mu ( f_{\hat{a} }^+ (w_{M_1})) =: 
%  e \in \mathcal{L}^+ \big[ \gamma_{(\hat{x},\hat{p})} (0,\infty) \cap  \gamma_{(\hat{y},\hat{q})}(0,\infty) \cap W_{2} \big] 
%  \end{equation}
%in the geometry $(M_2,g_2)$. 
%In particular, the first intersection point $z_1$ of the approximative geodesics $\gamma_{(\hat{x},\hat{p})} (s) $ and $  \gamma_{(\hat{y},\hat{q})} (s')$ exists in $(M_2,g_2)$ although it is not necessarily the point $w_{M_2}$. 
%
%\end{proof}
%
%



\noindent\textbf{Proof of (1):} We prove 
%the first claim of Lemma \ref{ss_map_determines_intersection} 
that $\tgin$ and  $\tginp$ intersect in $W_2\subset M_2$ the first time at geodesic parameter times $s>0$ and $s'>0$. %The first intersection will be then the % $s>0$ and $s'>0$ respectively. 
%and i$W_2$ (see~\eqref{ppa2}).
%The  proof of (3) follows from the construction.

%Let us show the existence of the intersection of $\tgin(s)$, $s>0$ and $\tginp(s)$, $s>0$ in $W_2$. 
%First, we show that if the intersection point exists, it must lie in $W_2$. As $\tgin(0) = \hat{\mu}(f_{\hat{a}} (w_{M_1}) )$ it is a consequence of the shortcut lemma (Lemma \ref{shortcut_lemma}) that also the first intersection belongs to $W_2$. 

Fix $e:= \hat\mu( f_{\hat{a}}^+ (w_{1} ) )$, that is, $a= \hat{a}$ in \eqref{diieee4}.  
%From our source-to-solution map data and Lemma \ref{estupido}, we have (\ref{ralksd347}) and \eqref{ralksd3472} holds. This implies 
%Thus, 
%\[
%J^- ( e )
%%f_{\hat{a} }^+ (w_{M_1}) + \delta)
%  % \cap \big[ \gamma_{(\hat{x},\hat{p})}(0,\infty) \cap  \gamma_{(\hat{y},\hat{q})}(0,\infty) \cap K_1 \big] \neq \emptyset
% \cap \{ z_1, \dots, z_k \} \neq \emptyset, \quad (z_l = z_{l,M_j}, \quad j=1,2)
%\]
%which holds in both spaces $(M_j,g_j)$, $j=1,2$.
%viewed in $(M_1,g_1)$ and 
%\[
%J^- ( e )
%%f_{\hat{a} }^+ (w_{M_1}) + \delta)
%   \cap \big[ \gamma_{(\hat{x},\hat{p})}(0,\infty) \cap  \gamma_{(\hat{y},\hat{q})}(0,\infty) \cap K_2 \big] \neq \emptyset
%\]
%in $(M_2,g_2)$.
% and $s^-< f_{\hat{a} }^+ (w_{M_1}) + \delta < s^+$ for $\delta>0$  sufficiently small by the shortcut argument. 
We approximate the light-like geodesics $\eta_1$ and  $\tilde{\eta}_1$ with  sequences $\gamma_{(\hat{x}_l,\hat{p}_l)}$ and $\gamma_{(\hat{y}_l,\hat{q}_l)}$, $l \in \mathbb{N}$ of time-like geodesics $\gamma_{(\hat{x},\hat{p})}$ and $\gamma_{(\hat{y},\hat{q})}$. 
In other words, we choose the geodesics such that for every $l\in \N $ the first intersection $z_{1,1}$ of $\gamma_{(\hat{x}_l,\hat{p}_l)}$ and $\gamma_{(\hat{y}_l,\hat{q}_l)}$ as geodesics in $M_1$ is $w_1$ and the initial values $(\hat{x}_l,\hat{p}_l)$ and $  (\hat{x}_l,\hat{p}_l)$ converge to some points in $ ( \eta_1, \dot\eta_1 ) \cap \OVS V$ and $( \tilde\eta_1, \dot{\tilde\eta}_1 )  \cap  \OVS V$, respectively.  
%\[
%(\hat{x}_l,\hat{p}_l) \to ( \eta_1(t), \dot\eta_1(t) )  \quad \text{and}  \quad  (\hat{x}_l,\hat{p}_l) \to ( \tilde\eta_1(\tilde{t}), \dot{\tilde\eta}_1(\tilde{t}) ) 
%\]
%for some $t<T$ and $\tilde{t} < \widetilde{T}$.
%as $l$ grows.
We may take $\hat{x}_l$ and $\hat{y}_l$ to lie in a fixed Cauchy surface $\mathcal{C}$ in $M_2$ 
and  $\hat{x}_l \in  W_2$ by removing the first terms in the sequence, if necessary.  
One applies the shortcut argument (Lemma \ref{shortcut_lemma}) and convergence of $\hat{x}_l$ to show that $\hat{x}_l \in J^+_2( \hat\mu(s_0) )$ for all indices $l$ and some $s_0\in (s^-,s^+)$. 
%there is $s_0\in (s^-,s^+)$ and a time-like future-directed geodesic in $(M_2,g_2)$ that connects $\hat\mu(s_0)$ to $\hat{x}$. 
Moreover,  $\gamma_{(\hat{x}_l,\hat{p}_l)}(s) \in J^+_2( \hat\mu(s_0) )$ in $M_2$, for all $s>0$, by a similar argument. 
%\begin{figure}
%    \centering
%    \includegraphics[scale=0.25]{pictures/light_obs_indep_IC.pdf}
%    \caption{Temporary picture to help illustrate the geodesics and points in claim 1. {\color{red}What's the message here? To me it looks like $\hat{x}$ is not in the right place. Is this %intentional (e.g. an indirect proof)?--antti}}
%    \label{fig:claim1_setup}
%\end{figure}
Consequently, we have for the first intersections $z_{2,1} = z_{2,1}(l)$ of $\gamma_{(\hat{x}_l,\hat{p}_l)}$ and $\gamma_{(\hat{y}_l,\hat{q}_l)}$ in $M_2$ the condition
\[
z_{2,1} \in \pi(Y_{2,1})\cap \pi(Y_{2,2})=\{\gamma_{(\hat{x},\hat{p})}(s)\in (M_2,g_2): s\geq 0 \}\cap \pi(Y_{2,2}) \subset J^+_2( \hat\mu(s_0) ) \quad \text{in} \quad (M_2,g_2),
 \]
 where we omitted the index $l$. 
% where $l$ refers to 
% Here $\gamma_{2,(\hat{x},\hat{p})}$ is a geodesic in $(M_2,g_2)$ with initial data $(\hat{x},\hat{p})$.
%Notice that the existence of $z_{1,2}$ in $(M_2,g_2)$ is already proven.~\f{Since? Or write differently ``We have proven the existence of $z_{1,2}$.}
From (\ref{ralksd347}) we obtain 
\[
 z_{2,1}(l)\in J^+_2( \hat\mu(s_0) ) \cap J^-_2(e)  \text{ in } (M_2,g_2),
\]
where $z_{2,1}(l)$ is the first intersection of the geodesics $\gamma_{(\hat{x}_l,\hat{p}_l)}$ and $\gamma_{(\hat{y}_l,\hat{q}_l)}$ in $(M_2,g_2)$. 
%Notice that due to convergence of $\hat{x}_l$ in $W_2$ we may choose $s_0$ such that it does not depend on $l$.  
%considerer only for positive geodesic parameter times. 
% and
% \[
%  pi(Y_{2,1}(j))\cap\pi(Y_{2,2}(j))=\{z_{2,1}(j),z_{2,2},\ldots,z_{2,k_2}\}\subset M_2
% \]
% 
% 
% I wo
% Now, by using Lemma \ref{druqks} in the appendix, we construct sequences~\f{Change the indices. $l$ for the sequence $a$ for the intersections $j$ for the manifolds.} $(\hat{x}_j, \hat{p}_j)\in P^{r_1}(\mathcal{U} \cap W_1 \cap W_2)$, and $(\hat{y}_j, \hat{q}_j)\in P^{r_2}  \mathcal{U}$, $j\in \N$,~\f{Note that $\mathcal{U}\cap W_1\cap W_2\subset V\subset M_1\cap M_2$.} such that as $j\to\infty$ 
% %\[
% \begin{equation}\label{kouihy5}
% (\hat{x}_j, \lambda_j \hat{p}_j)\to(\gin(0),\dgin(0)), \text{ and } (\hat{y}_j, \lambda_j \hat{q}_j)\to  (\ginp(0), \dginp(0)).
% \end{equation}
% %\]
% for strictly positive coefficients~\f{Does this mean that $\lambda_j,\lambda_j' >c>0$?}  $\lambda_j,\lambda_j' >0$. These are related to the normalisation coefficients $c_j,c_j'$ of the lemma via $\lambda_j = c_j^{-1}$ and $\lambda_j' = (c_j')^{-1}$.~\f{Just state $\lambda_j = c_j^{-1}$. It's best to out $\lambda_j$ in the lemma.}
%\longrightarrow \infty$. 
%and so that there is a $j_0\ge 1$ with $(\hat{x}_{j_0},\hat{p}_{j_0})= (\hat{x},\hat{p})$ and $(\hat{y}_{j_0},\hat{q}_{j_0}) = (\hat{y},\hat{q})$. 
%
% Notice that \eqref{intersection_nonempty} holds for arbitrary elements $(\hat{x},\hat{p})$, $(\hat{y},\hat{q})$ of the sequences $(\hat{x}_j,\hat{p}_j), (\hat{y}_j,\hat{q}_j)$ and that the first intersection $z_1 = z_1(j)$ remains the same when scaling the initial vector by $\lambda_j$ or $\lambda_j'$. 
Thus, there exist sequences $(s_l)$ and $(s_l')$ of positive numbers such that 
\begin{equation}\label{324234325346}
 z_{2,1}(l)= \gamma_{(\hat{x}_l, \s \hat{p}_l)} (s_l) =   \gamma_{(\hat{y}_l, \s \hat{q}_l)}(s_l') \in   J^+_2( \hat\mu(s_0) ) \cap J^-_2(e). % \subset (M_2,g_2)
\end{equation}
Here $s_l>0$ and $s_l'>0$ are so that the geodesics $\gamma_{(\hat{x}_l,\hat{p}_l)}$,  $ \gamma_{(\hat{y}_l,\hat{q}_l)}$ intersect the first time at the geodesic parameter times $s_l$ and $s_l'$. % $s,s'>0$. 
To finish the prove of $(1)$, we show that a subsequence of $z_{2,1}(l)\in M_2$ converges to the first intersection of $\eta_2$ and $\tilde{\eta}_2$. 
% \begin{enumerate}
% \item $z_1^{(2)}(l):= \gamma_{(\hat{x}_l, \lambda_l \hat{p}_l)} (s_l) =   \gamma_{(\hat{y}_l, \lambda_l' \hat{q}_l)}(s_l') \in   J^+( \hat\mu(s_0) ) \cap J^-(e) \text{ in }(M_2,g_2),$ for some sequences $s_l'>0$ and $s_l>0$, and
% \item as $l\to\infty$, the sequence $z_1^{(2)}(l)
% %= \gamma_{(\hat{x}_l,\hat{p}_l)} (s_l))= \gamma_{(\hat{y}_l,\hat{q}_l)}(s_l')
% $ converges in the space $J^+( \hat\mu(s_0) ) \cap J^-(e)$.
% \end{enumerate}

Since $(M_2,g_2)$ is globally hyperbolic, the set $J^+_2( \hat\mu(s_0) ) \cap J^-_2(e)$ is compact. Thus, we may pass to a subsequence so that 
\[
z_{2,1}(l) \text{ converges in } J^+_2( \hat\mu(s_0) ) \cap J^-_2(e)\subset W_2 \text{ as } l\to \infty.
%as $l\to\infty$, the sequence $z_1^{(2)}(l)
% %= \gamma_{(\hat{x}_l,\hat{p}_l)} (s_l))= \gamma_{(\hat{y}_l,\hat{q}_l)}(s_l')
% $ converges in the space $J^+( \hat\mu(s_0) ) \cap J^-(e)$.
% \end{enumerate}
\]
%By the shortcut argument $J^+_2( \hat\mu(s_0) ) \cap J^-_2(e) \subset W_2$ so the limit lies in $W_2$.  
%
%Notice that we may assume that the sequence $\hat{x}_l$ (resp. $\hat{y}_l$) lie in a Cauchy surface in $M_2$  which we denote by $\mathcal{C}$. 
Applying the parametrisation $\overline{\mathcal{P}}^+ \mathcal{C} \times \R \to \overline{\mathcal{P}}^+ M_2$, $(x,p,t) \mapsto \gamma_{x,p}(t)$ near the curve $\eta_2$ (resp. $\tilde{\eta}_2$) to \eqref{324234325346} implies that $s_l$ and $s_l'$ must converge. 
Thus, as the time-like curves in $M_2$ with initial values $(\hat{x}_l,\hat{p}_l)$ and $(\hat{y}_l,\hat{q}_l)$ approximate $\eta_2$ and $\tilde{\eta}_2$, respectively, it follows that there must exist the first intersection point of $\eta_2$ and $\tilde{\eta}_2$ in $W_2$ at the limit of $z_{2,1}(l)$. This is the point $w_2$. 
%Since 
%By moving the points along geodesic flow inside $V$ we may also assume that $(\hat{x}_l,\hat{p}_l)$ for large $l$ are on a same Cauchy surface $\mathcal{C}$
%\Big[ 
%of $ J^+( \hat\mu(s_0) ) \cap J^-(e)$  
%subsequence $l$ of indices $j$~\f{Write better.}
%
%By (\ref{intersection_nonempty}), the convergent sequence $z_{2,1}(l)$
%%$\gamma_{(\hat{x}_l,\hat{p}_l)} (s_l) $ and $ \gamma_{(\hat{y}_l,\hat{q}_l)}(s_l')$ 
%also lies in $\OVS W_2$. 
%% {\color{gray} 
%% By Lemma \ref{uuiisok}, $\XX$ is strictly hyperbolic over $\OVS(W_2)$,
%% } {\color{red}($\leftarrow$ Could you please explain this and why it was added here? Doesn't this actually follow from global hyperbolicity of $M$ toghether with (\ref{kouihy5})? How does strict hyperbolicity of an operator tell us about convergence? --Antti)}
%Hence there is an interval $[0,S]$ such that $s_l,s_l'\in [0,S]$ for all indices $l$.
%%
%% By passing on to a subsequence we can assume that $s_l$ converges.
%It follows that $ \gamma_{(\hat{x}_l,\lambda_l \hat{p}_l)} \to \tgin$ and $ \gamma_{(\hat{y}_l,\lambda_l'\hat{q}_l)} \to \tginp$ uniformly on $[0,S]$ as $l\to \infty$. We obtain 
%%\begin{enumerate}
%%\item $\gamma_{(\hat{x}_l,\lambda_l \hat{p}_l)} (s_l)  
%%$z_1(l) \in J^+( \hat\mu(s_0) ) \cap J^-(e) $ and 
%\[
%\lim_{l \rightarrow \infty} z_{2,1}(l)  \in \tgin ([0,S])   % = \tgin [0,S)
%\quad 
%\text{and}
%\quad 
%\lim_{l \rightarrow \infty} z_{2,1}(l)  \in \tginp ([0,S]).  %= \tginp [0,\infty). 
%\]
%(If the geodesic $\eta_2$ or $\tilde{\eta}_2$ does not exist for all positive geodesic parameters, we replace $S$ above by the supremum of values where the geodesic exists and consider the closure of the graph of the geodesic.)
%%where $0< S \leq \infty$, $0< \tilde{S} \leq \infty$ are such that $[0,S)$ and $[0,\tilde{S})$ are inextendible domains of $\tgin$ and $\tginp$, respectively. 
%%\item $\gamma_{(\hat{y}_l\lambda_l'\hat{q}_l)} (s_l')  \in J^+( \hat\mu(s_0) ) \cap J^-(e)$ and $\gamma_{(\hat{y}_l, \lambda_l'\hat{q}_l)} (s_l')  \in \overline{\tginp [0,\infty) }  = \tginp [0,\infty)$.
%%\end{enumerate}
%%
%In conclusion,  
%\begin{equation}\label{ydisp}
%\lim_{l \rightarrow \infty} z_{2,1}(l) \in \tgin ([0,S]) \cap  \tginp ([0,S]) \cap [ J^+( \hat\mu(s_0) ) \cap J^-(e) ] .
%% \lim_{l \rightarrow \infty} z_1(l) \in \overline{\tgin (0,S) } \cap  \overline{\tginp (0,\tilde{S} ) } \cap [ J^+( \hat\mu(s_0) ) \cap J^-(e) ] .
%%\subset \left(\tgin [0,\infty) \cap  \tginp [0,\infty) \cap  W_2\right) .
%\end{equation}
%
%%Since $(M_2,g_2)$ is globally hyperbolic, 
%The geodesics $\tgin$ and $\tginp$ escape the compact set $[ J^+_2( \hat\mu(s_0) ) \cap J^-_2(e) ] \subset W_2$ permanently in finite geodesic parameter times. 
%Thus, (\ref{ydisp}) implies 
%\[
%\lim_{l \rightarrow \infty} z_{2,1}(l) \in \tgin ([0,S])  \cap  \tginp ([0,S])  \cap [ J^+_2( \hat\mu(s_0) ) \cap J^-_2(e) ] 
%\subset  \tgin ([0,S])  \cap  \tginp ([0,S]) \cap  W_2 
%%\lim_{l \rightarrow \infty} z_1(l) \in \tgin [0,S)  \cap  \tginp [0,\tilde{S} )  \cap [ J^+( \hat\mu(s_0) ) \cap J^-(e) ] 
%%\subset  \tgin [0,S)  \cap  \tginp [0,\tilde{S} ) \cap  W_2 .
%\]
%By using this and the fact that the graphs of $\tgin$ and $\tginp$ are different, we
%% 
%% As , we 
%% 
%conclude that there is the first intersection point $w_2\in W_2\subset M_2$ of $\tgin$ and  $\tginp$ which happens at some positive geodesic parameter times. Since the geodesics $\gamma_{(\hat{x}_l, \lambda_l\s \hat{p}_l)}$ and $\gamma_{(\hat{x}_l, \lambda_l\s \hat{p}_l)}$ converge to $\eta_2$ and $\tilde{\eta}_2$ uniformly on $[0,S]$ we also have that %approximate these rays arbitrarily well 
%%on compact intervals we conclude that the limit of $ z_1(l)$ is the first one of the intersections, that is, 
%\begin{equation}\label{pqwehhert}
%\lim_{l \rightarrow \infty} z_{2,1}(l) = w_{2}.
%\end{equation}
%This completes the proof of (1).
  

 %\textbf{Claim 2: The first intersection point $w_{M_2}$ does not depend on the choice of $\gin$ and $\ginp$.} 
 
 \noindent\textbf{Proof of (2) and (3):} 
 %To prove that the first intersection point $w_{2}$ does not depend on the choice of $\gin$ and $\ginp$, we first 
%  To prove this, we first 
%  
%  
%prove the condition (3). % which is then applied to prove the condition 2.~\f{Change the order in the statement of the lemma.} 
 %By excluding a finite number of the first elements in the sequences above, we may localize 
 Recall that the first intersection $w_1\in W_1$ of  the time-like approximations $\gamma_{ (\hat{x},\hat{p}) }$ and $\gamma_{(\hat{y},\hat{q})}$
 %$\gamma_{ (\hat{x},\hat{p}) } (s)$, $s>0$ and $\gamma_{(\hat{y}',\hat{q}')} (s')$, $s'>0$ in $(M_1,g_1)$ 
 %sufficiently close to $w_{M_1}$ so that local injectivity of the exponential map at $w_{M_1}$ guarantees that the first intersection of these curves 
 %takes place exactly at the point $w_{M_1}$ 
 %(cf. proof of Lemma \ref{druqks}). 
%By definition, 
%which, also by definition, 
is also the first intersection $w_1$ of $\gin$ and $\tilde{\eta}_1$ in $(M_1,g_1)$ by definition.  We also know that the first intersection exist for the associated time-like geodesics in $(M_2,g_2)$. 
%takes also place at $w_{M_1}$ and these geodesics are approximated by $\gamma_{ (\hat{x},\hat{p}) } (s)$, $s>0$ and $\gamma_{(\hat{y}',\hat{q}')} (s')$, $s'>0$ intersecting first time at $w_{M_1}$. 
  To prove (2), let $\gino$ and $\ginpo$ be another pair of geodesics that satisfies the  conditions  of $\gin$ and $\ginp$. 
  % replaced with $\gino$ and $\ginpo$ respectively. 
 The first part of the proof above applies also for $\gino$ and $\ginpo$ and the first intersection is obtained as a limit of first intersections for some pair of time-like geodesics $\gamma_{ (\hat{x}_l',\hat{p}_l') }$ and $\gamma_{(\hat{y}_l',\hat{q}_l')}$ 
 that as geodesics in $M_1$ intersect first time in $w_1$ for every $l$ and approximate the light-like geodesics $\gino$ and $\ginpo$. 
 Thus it suffices to show that for two pairs 
 %$\gamma_{ (\hat{x},\hat{p}) }$, $\gamma_{(\hat{y},\hat{q})}$ and $\gamma_{ (\hat{x}',\hat{p}') }$, $\gamma_{(\hat{y}',\hat{q}')}$ of time-like geodesics with  
 $(\hat{x},\hat{p}),(\hat{y},\hat{q})\in \mathcal{P}^+V$ and $(\hat{x}',\hat{p}'), (\hat{y}',\hat{q}')  \in \mathcal{P}^+V$ with the associated pairs of geodesics  in $(M_1,g_1)$  intersecting the first time at $w_1$ have the property that both pairs $\gamma_{ (\hat{x},\hat{p}) }$, $\gamma_{(\hat{y},\hat{q})}$ and $\gamma_{ (\hat{x}',\hat{p}') }$, $\gamma_{(\hat{y}',\hat{q}')}$ of geodesics in $(M_2,g_2)$ intersect the first time at a mutual point. Note that this point must be the limit $z_{2,1}(l) \to w_2$ of the first intersection points 
 constructed in the proof of $(1)$. In fact, the sequence is a constant sequence. 
 
 
 As earlier, let $\gamma_1$ be a light-like optimal geodesic in $M_1$ from $w_1= \gamma_1 (0 )$ to $e = \gamma_1(1)$ and define the geodesic $\gamma_2$ in $M_2$ by the condition $(\gamma_2(1) , \dot\gamma_2(1)) = (\gamma_1(1) , \dot\gamma_1(1))$.
%
Let us then consider three pairs of initial vectors 
\begin{align}\label{vector-pairs}
\{ (\hat{x},\hat{p}), (\hat{y},\hat{q}) \},\ \ \{(\hat{x},\hat{p}), (\hat{y}',\hat{q}')\},  \text{ and }  \{(\hat{x}',\hat{p}'), (\hat{y}',\hat{q}') \}. 
\end{align}
constructed from the pairs  $(\hat{x},\hat{p}),(\hat{y},\hat{q})\in \mathcal{P}^+V$ and $(\hat{x}',\hat{p}'), (\hat{y}',\hat{q}')  \in \mathcal{P}^+V$ above. 
To each of these pairs of vectors, we may associate a pair of geodesics in $(M_1,g_1)$ which have the vectors as initial data. Each pair of geodesics has the property that they intersect for first time (for positive geodesic parameter times) at $w_{1}\in W_1$. On the other hand, to each pair of vectors in \eqref{vector-pairs}, we may achieve a pair of geodesics in $(M_2,g_2)$ that have the vectors as initial conditions at  $s=0$. 
As shown earlier, each pair of geodesics has the property that they intersect in $M_2$ and for the first time (for positive geodesic parameter times) it happens in $W_2$. 
%We aim at showing that the intersection point corresponding to the first 
We label these first intersection points in $W_2$ by $z^{(1)}$, $z^{(2)}$ and $z^{(3)}$, respectively. These intersections points lie in $\{ \gamma_2(s) : s<1 \}$ according to Lemma \ref{intersection_lightlike_geo} below. %~\f{Remove Lemma \ref{intersection_lightlike_geo} and copy the argument here.} 
%
Before proving the lemma let us assume that it holds and show that the intersection points $z^{(1)}$, $z^{(2)}$, $z^{(3)}\in M_2$ ($z^{(1)} = z_{2,1}$ in the proof of (1)) are actually identical. The claim (2) then follows from this  since the first intersections  of the approximative time-like geodesics accumulate arbitrarily near $w_2$, as shown in the proof of (1). 
%which is analogous to the corresponding curves in $(M_1,g_1)$. 


We argue by contradiction and suppose that $z^{(1)}\neq z^{(2)}$.   % by assuming the opposite and 
%Contrary to the claim, assume that for two of the pairs the associated first intersections in $(M_2,g_2)$ are distinct. 
That is, we suppose the first intersection of the pairs of geodesics 
\[
\{ \gamma_{(\hat{x},\hat{p})}, \gamma_{(\hat{y},\hat{q})}\} \text{ and } \{  \gamma_{(\hat{x},\hat{p})}, \gamma_{(\hat{y}',\hat{q}')}\}.
\]
in $(M_2,g_2)$ are distinct. 
The proof for the case $z^{(2)}\neq z^{(3)}$ is analogous. 
Applying Lemma \ref{intersection_lightlike_geo} we deduce that  $\gamma_{(\hat{x},\hat{p})}(s)$, $s>0$ hits $\{ \gamma_2(s) : s<1 \}$ twice, first at one of the points $z^{(1)}$, $z^{(2)}$ and then after at the other. 
%For the other cases the proofs are analogous. 
% for positive geodesic parameter times. 
%(As before, we consider all geodesic to be defined only for non-negative geodesic parameter times so that the intersections happen when the geodesic parameters times are positive.)   
%
We may assume that $\tau(z^{(1)} ,z^{(2)})>0$ in $M_2$. For $\tau(z^{(2)} ,z^{(1)})>0$ one simply swaps the roles of the points in the proof. 
The shortcut lemma (Lemma \ref{shortcut_lemma}) implies that there is a time-like future-directed segment connecting $z^{(1)}$ to $e$ in $M_2$.
%$\tgout$ can not maximise the length function over the causal curves between the intersection $\tgout(T_1)$ and $e= \tgout(T)$. In particular, 
Thus, there is some point $e'$ in the curve $\hat\mu$ that satisfies $\tau(e',e)>0$ and which can be reached from $z^{(1)}$ along a future-directed lightlike geodesic segment. %We repeat the argument in the end of the proof of Lemma \ref{intersection_lightlike_geo}: 
We can now apply Corollary \ref{coro_renerew}  and 
 Proposition \ref{kooasu} to get $e' \in\text{singsupp} ( \lim_{\epsilon \rightarrow 0} ( \Phi''(0;  h_1^\epsilon ,  h_2^\epsilon) \circ P_{e'} ) ) $ in both spaces from which by Lemma \ref{estupido} one obtains $e' \in  J^+ (w_{1})$ in the space $(M_1,g_1)$. Since $\tau(e',e)>0$, we have $e \neq \hat\mu ( f_{\hat{a}}^+(w_{1}) )$ which is a contradiction. 
 %
 %One arrives similarly into a contradiction by assuming instead $z^{(1)}\neq z^{(2)}$ or $z^{(2)}\neq z^{(3)}$. 
 Thus, we have that 
 \[
  z^{(1)}=z^{(2)}.
 \]
 In a similar way one shows that $ z^{(2)}=z^{(3)}$.
  
 
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now prove the following auxiliary lemma:

\begin{lemma}\label{intersection_lightlike_geo}
 % Under the conditions of Theorem \ref{themain} and the assumptions above 
   Let $\gamma_1$ be \tbl{an optimal future-directed lightlike geodesic in $(M_1,g_1)$ between the points $w_{1}= \gamma_1(0)\in W_1$  and $e=\hat\mu( f_{\hat{a}}^+ (w_{1} ) ) = \gamma_1(1)$.} 
   Let $\gamma_2$ be the geodesic in $(M_2,g_2)$ with $(\gamma_2 (1) , \dot\gamma_2(1))= (\gamma_1 (1) , \dot\gamma_1(1))$. Let $(x,p),(y,q) $ be elements in $ \mathcal{P}^+   V $ for both $j=1,2$ such that in $(M_1,g_1)$ the geodesics $\gamma_{(x,p)}(s)=\gamma_{(x,p);M_1}(s)$, $s>0$ and $\gamma_{(y,q)}(s')= \gamma_{(y,q);M_1}(s')$, $s'>0$ intersect the first time at $w_1 \in W_1$. 
  %Let $\tgout$ be the geodesic in $(M_2,g_2)$ having the same initial data as $\eta_1$. %: % that is,
  %\[
  %(\tgout (T), \dot{\eta}_2 (T)) = (\gout (T),\dot{\eta}_1 (T) ).
  %\] 
  Then, $\Phi_1 = \Phi_2$ implies that the first intersection point $z=z_{2,1}$ of $\gamma_{ (x,p) }(s) = \gamma_{ (x,p);M_2 }(s)$, $s>0$ and $\gamma_{(y,q)}(s')= \gamma_{(y,q);M_2}(s')$, $s'>0$  in $(M_2,g_2)$ belongs to $\{ \gamma_2(s) : s<1 \}$.  
  %for $s>0$ and $s'>0$, in the space $(M_2,g_2)$ lies in 
 % in $(M_2,g_2)$ lies in 
%\[
% \{ \gamma_1(t) : t < 1 \}.
%\] 
%where $[0,S)$, $0 < S \leq \infty$, is the inextendible domain of $t \mapsto \tgout (-t)$. 
 \end{lemma}
 \begin{proof}
Following the construction in page \pageref{3249reeeredfds} one puts together Corollary \ref{coro_renerew}, Proposition \ref{kooasu} to show that 
 for certain sources $h_1^\epsilon ,  h_2^\epsilon$ and a vector field $P_e$ on neighbourhood $U_e$ around $e$ we have 
 \[
 \text{singsupp} ( \lim_{\epsilon \rightarrow 0} ( \Phi''(0;  h_1^\epsilon ,  h_2^\epsilon) \circ P_{e} ) ) =  \gamma_2 \cap U_e.
 \]
Moreover, Lemma \ref{estupido} implies that $ \gamma_2 (1-\delta)$ belongs to the causal future of $z$ for sufficiently small $\delta >0$. Hence there is a causal geodesic $\nu$ connecting $z$ to $ \gamma_2 (1-\delta)$. 
If $z_1 \notin \{ \gamma_2(s) : s<1 \}$ we may combine $\nu$ with $\gamma|_{[1-\delta,1]}$ and apply shortcut argument to show that $z$ can be connected to $e$ with a timelike curve in $(M_2,g_2)$. 
Thus, $\hat{\mu}$ contains a point $e' \ll e$ that can be reached from $z$ with an optimal lightlike geodesic $\tilde\gamma_2$. We can then repeat the construction above with some vector field $P_{e'}$ tangent to $\tilde\gamma_2$ to derive that $e' \in J^+_1(w_1)$. Thus $\gamma_1$ does not define optimal segment from $w_1$ to $e$ which is in conflict with the assumptions. 

% 
\end{proof}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Quick proof of the proposition for determining E.L.O.S
%
The determination of the earliest light observation sets from the knowledge of the source-to-solution map data follows from %is an easy consequence of 
Lemma \ref{ss_map_determines_intersection}: %and the definition of earliest light observation set:



Below, let $f_{a,1}^+$ 
and $f_{a,2}^+$ be the earliest observation time functions on $M_1$ and $M_2$, respectively.
 Lemma~\ref{ss_map_determines_intersection} shows that there is a mapping 
%We prove that the mapping
% Using these lemmas, for $w_{M_{1}}\in W_{1}$ and $w_{M_{2}}\in W_{2}$ the corresponding intersection point, define
% 
\begin{equation}\label{F_map}
F : W_1 \rightarrow W_2 , \quad F(w_{1}) := w_{2},
\end{equation}
which maps the first intersection $w_1$ of $\eta_1$ and $\tilde{\eta}_1$ to the first intersection $w_2$ of $\eta_2$ and $\tilde{\eta}_2$. Here $\eta_j$ and $\tilde{\eta}_j$, $j=1,2$, are defined as in~\eqref{9090sdj}--\eqref{last_geo}. 
%Thus $F$ 
%is well defined.

\begin{proposition}\label{prof: Map F preserves E-sets}
Let $\Phi_{1,L^+V}$ and $\Phi_{2,L^+V}$ be as earlier in Section~\ref{main-proof} and assume that $\Phi_{1,L^+V}=\Phi_{2,L^+V}$. Assume also that the conditions of Theorem \ref{themain} are satisfied for the Lorentzian manifolds $(M_1,g_1)$ and $(M_2,g_2)$.

Then, the map~\eqref{F_map}
\[
F : W_1 \rightarrow W_2 
\]
 is a bijection and
 %satisfies. Further, the first light observations of the points in $W_j$, $j=1,2$ measured in $\mathcal{U} \subset V$ are invariant under the transformation $F$. That is,
\begin{eqnarray}\label{eq: F and E sets}
f_{a,1}^+( w_1 ) = f_{a,2}^+ (F(w_1)),
\end{eqnarray}
for every $w_1\in W_1$ and $a\in \mathcal A$. 
%Especially, $\mathcal{E}_{\mathcal{U}}^1(W_1)=\mathcal{E}_{\mathcal{U}}^2(W_2)$.
\end{proposition}
\begin{proof}
Let $w_1\in W_1$ and $w_2=F(w_1)$. 
%Using Lemma \ref{ss_map_determines_intersection}, we can define the corresponding point $w_2\in W_2$. 
We show that the earliest observation time functions $f_{a,1}^+$ on $M_1$
and $f_{a,2}^+$ on $M_2$  satisfy $f_{a,1}^+(w_1)=f_{a,2}^+(w_2)$.
%$\mathcal{E}_{\mathcal{U}}^1 (w_{1} )  =\mathcal{E}_{\mathcal{U}}^2  (w_{2} ) $.

Let  $a\in \mathcal A$ and  $f_{a,1}^+:W_1\to \R$ 
be {an earliest observation time function} on $M_1$.
 %(not necessarily the one corresponding to $a= \hat{a}$) such that 
Moreover, let 
 $e= \mu_a (f_{a,1}^+ (w_{1} ) )$. (This means that $e$ can be reached by a lightlike future-directed geodesic from $w_{1}$.) 
Let $(\hat{x},\hat{p})$ and $(\hat{y},\hat{q})$ be timelike initial vectors as in the last condition of Lemma \ref{ss_map_determines_intersection}. In the space $(M_1,g_1)$ the first intersection of the associated geodesics is $w_1$ whereas the first intersection $z_{2,1}$ in $(M_2,g_2)$ is $w_2$. 
%intersect first time at $w_{M_1}$ as before. 
As in the proof of Lemma \ref{ss_map_determines_intersection} %one combines Proposition \ref{kooasu} and Lemma \ref{estupido} to 
we deduce from  $\Phi_{1,L^+V}=\Phi_{2,L^+V}$  that 
%As $\Phi_1=\Phi_2$ we deduce
%\[
$e \in J_2^+(z_{2,1})$ in $(M_2,g_2)$ and hence $w_2 \in J^-_2(e)$. 
%\mathcal{L}^+ \big[ \gamma_{(\hat{x},\hat{p})} (0,\infty) \cap  \gamma_{(\hat{y},\hat{q})}(0,\infty) \cap W_{2} \big].
%\]
%Since $z_1 = w_{2}$, we conclude $e \in J_1^+(w_{1})$.
%Lemma \ref{estupido}. 
%Applying the last condition of Lemma \ref{ss_map_determines_intersection} we can assume $z_1 = w_{M_2}$ so $e \in J^+(w_{M_2})$. 
Thus, the earliest light observation from $w_{2}$ on the path $\mu_a$ occurs either at $e$ or at a point that is in the past of $e$. In particular, 
\begin{equation}\label{ff}
f_{a,2}^+ (w_{2} ) \leq  f_{a,1}^+ (w_{1}). 
\end{equation}

To see that $F$ has an inverse, note that we may change the roles of $(M_1,g_1)$ and $(M_2,g_2)$ in Lemma~\ref{ss_map_determines_intersection} to have a mapping 
\[
 W_2\to W_1,
\]
which maps the first intersection of $\eta_2$ and $\tilde{\eta}_2$ to the first intersection of $\eta_1$ and $\tilde{\eta}_1$. Here $\eta_j$ and $\tilde{\eta}_j$, $j=1,2$, are defined as in~\eqref{9090sdj}--\eqref{last_geo}. This mapping is the inverse of $F$ and 
$F:W_1\to W_2$ is a bijection.

By interchanging the roles of $(M_1,g_1)$ and $(M_2,g_2)$ and repeating the above construction we see as in
\eqref{ff} that
\[
 f_{a,1}^+ (w_{1}) \leq  f_{a,2}^+ (w_{2}).
\]
Thus, we have
$f_{a,1}^+ (w_{1} ) =  f_{a,2}^+ (w_{2} )=  f_{a,2}^+ (F(w_{1}) )$ for all $w_1\in W_1$. 
Hence,
$F:W_1\to W_2$ is a bijection
 satisfying $f_{a,1}^+ (w_{1} ) = f_{a,2}^+ (F(w_{1}) )$ for all $w_1\in W_1$. 
 
\end{proof}

This result implies  Proposition \ref{ss_map_first_obs}:


\begin{proof}[Proof of Proposition \ref{ss_map_first_obs}]
By definition \eqref{eioreiie-eq} of the sets  
$\mathcal{E}_{\mathcal{U}}^j (w )$,
Proposition \ref{prof: Map F preserves E-sets}  proves that 
$\mathcal{E}_{\mathcal{U}}^1 (w_{1} )  = \mathcal{E}_{\mathcal{U}}^2  (w_{2} ) $ for
all $w_1\in W_1$ and $w_2=F(w_1)$. As $F:W_1\to W_2$ is a bijection,
%By changing the roles of manifolds $M_1$ and $M_2$, we see that
this proves $\mathcal{E}_{\mathcal{U}}^1  (W_1)= \mathcal{E}_{\mathcal{U}}^2 (W_2) $.
% which proves the claim.
%by (\ref{eioreiie-eq}).
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  Metric uniqueness from source-to-solution map
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Determination of the metric from the source-to-solution map}
% .

 In this section we prove that $F$ is in fact an isometry,
\[
 F^*g_2=g_1.
\]
This will prove our main theorem, Theorem~\ref{themain}.
% The definition is valid by Lemma \ref{ss_map_determines_intersection}. Putting together the results above yields the following:



To this end, we apply Proposition \ref{prof: Map F preserves E-sets} to have the following implication of \cite[Theorem 1.2]{Kurylev2018}:

\begin{theorem}\label{oo1}
Let $\Phi_{1}$ and $\Phi_{2}$ be as earlier in Section~\ref{main-proof} and assume that $\Phi_{1,L^+V}=\Phi_{2,L^+V}$. Assume also that the conditions of Theorem \ref{themain} are satisfied for the Lorentzian manifolds $(M_1,g_1)$ and $(M_2,g_2)$.
%Let $\Phi_1 = \Phi_2$  and assume that the conditions of Theorem \ref{themain} are satisfied for the Lorentzian manifolds $(M_j,g_j)$, $j=1,2$. 
Then, the map 
\[
{F} : W_1 \rightarrow W_2
\]
is a diffeomorphism  and the metric ${F}^* g_2$ is conformal to $g_1$ in $W_1$. 
\end{theorem}


\begin{proof} The claim follows from the proof of~\cite[Theorem 1.2]{Kurylev2018}. However,
let us briefly explain the main steps of the proof as we need the construction in the proof to determine the conformal factor between $F^*g_2$ and $g_1$ in the next section.

On the manifold $(M_j,g_j)$, let $\mathcal F_j:W_j\to C(\mathcal A)$ be the map from the point $q$
to the corresponding earliest observation time function, that is,  $\mathcal F_j(w)=f_{a,j}^+(w)$, $j=1,2$.
Then formula \eqref{eq: F and E sets} and \cite[Lemma 2.4 (ii)]{Kurylev2018} imply that
\begin{eqnarray}\label{eq: F and f maps }\mathcal F_1(w)=\mathcal F_2(F(w)),\quad
\hbox{for every $w\in W_1$}.
\end{eqnarray}
 In particular, the sets $\mathcal F_j(W_j)\subset C(\mathcal A)$, $j=1,2$, satisfy $\mathcal F_1(W_1)=\mathcal F_2(W_2)$, since $F:W_1\to W_2$ is a bijection by Proposition~\ref{prof: Map F preserves E-sets}. 
Thus we can write
$F=(\mathcal F_2)^{-1}\circ \mathcal F_1:W_1\to W_2$. By~\cite[Proposition  2.2]{Kurylev2018},
this implies that $F:W_1\to W_2$  is a homeomorphism. Hence the sets
$\mathcal F_j(W_j)$ can be considered as topological submanifolds of
the infinite dimensional vector space $C(\mathcal A)$.  It is shown in~\cite[Section 5.1.2]{Kurylev2018} 
that using the knowledge of the set $\mathcal F_1(W_1)$, we can construct 
for any point $Q\in \mathcal F_1(W_1)$ a neighborhood $U\subset  \mathcal F_1(W_1)$ of $Q$ and the values $a_1,a_2,\dots,a_n\in \mathcal A$ such that the following holds:
The point $q=\mathcal F_1^{-1}(Q)\in W_1$ has
a neighborhood $\mathcal F_1^{-1}(U)\subset W_1$,   
where the map $f_{a_1,\dots,a_n}:x\mapsto (f_{a_k,1}^+(x))_{k=1}^n$ defines smooth local coordinates on $W_1$. Observe that for $P\in U$, we have 
$f_{a_k,1}^+\circ \mathcal F_1^{-1}(P)=P(a_k)$. Thus when $E_a:C(\mathcal A)\to \R$, $a\in \mathcal A$ are the evaluation functions $E_a(P)=P(a)$ and $E_{a_1,\dots,a_n}(P)=(E_{a_j}(P))_{j=1}^n$, the above constructed pairs $(U,E_{a_1,\dots,a_n})$ determine on $\mathcal F_1(W_1)$ an atlas 
 of differentiable coordinates
on $\mathcal F_1(W_1)$ which makes $\mathcal F_1:W_1\to \mathcal F_1(W_1)$ a diffeomorphism. As noted above, such atlas can be constructed using only the knowledge of the set  $\mathcal F_1(W_1).$
Thus, as $\mathcal F_1(W_1)=\mathcal F_2(W_2)$, the atlases constructed on these sets
coincide. %, that is, the map  $Id:\mathcal F_1(W_1)\to \mathcal F_2(W_2)$ is a diffeomorhpsim.
This implies that the homeomorphism $F=(\mathcal F_2)^{-1}\circ\mathcal F_1:W_1\to W_2$  is actually a diffeomorhpsim.
  
  Let us next consider the conformal classes of the metric tensors $g_1$ and $g_2$.  Let
 $(x,\eta)\in L^+\mathcal{U}$ be a future directed lightlike vector.
 Let us consider the lightlike geodesics $ \gamma^{\s j}_{(x,\eta)}(\R_-)$, $j=1,2$, on $(M_j,g_j)$ that lie in the causal past of the point $x$,
and let $s_1>0$ be such that $ \gamma^{\s j}_{(x,\eta)}([-s_1,0])\subset \mathcal{U}$.
 By~\cite[Proposition 2.6 ]{Kurylev2018} we have that a point $w_j\in W_j$ satisfies
 $w_j\in  \gamma^{\s j}_{(x,\eta)}((-\infty,-s_1])$  if and only if $ \gamma^{\s j}_{(x,\eta)}((-s_1,0))\subset \mathcal{E}_{\mathcal{U}}^j ( w_j )$. In other words, for a point $w_j\in W_j $ 
 the set $\mathcal{E}_{\mathcal{U}}^j ( w_j )$ determines whether $w_j\in  \gamma^{\s j}_{(x,\eta)}((-\infty,-s_1])$.
 By formula \eqref{eq: F and E sets}, this implies that $F$ maps the lightlike geodesic
  $\gamma^{\s 1} ((-\infty,-s_1])\cap W_1$ on to $\gamma^{\s 2} ((-\infty,-s_1])\cap W_2$,
  \begin{equation}\label{F_preserve_light_geos}
   F\big(\gamma^{\s 1} ((-\infty,-s_1])\cap W_1\big) \subset \gamma^{\s 2} ((-\infty,-s_1])\cap W_2
  \end{equation}

  
  
  Let 
 $w_1\in W_1$ and $\xi_1\in L^+_{w_1}M_1$  be such that $\gamma^{\s 1}_{(w_1,\xi_1)}(\R_+)\cap \mathcal{U}\not=\emptyset$,
 so that there is $t_1>0$ so that $\gamma^{\s 1}_{(w_1,\xi_1)}(t_1)\in \mathcal{U}$. Let $x=\gamma^{\s 1}_{(w_1,\xi_1)}(t_1)$  and 
 $\eta=\dot\gamma^{\s 1}_{(w_1,\xi_1)}(t_1)$.
   Then~\eqref{F_preserve_light_geos} implies that there is $t_0\in (0,t_1)$  such that 
 \begin{eqnarray}\label{eq: light-like geodesics}
 F\big(\gamma^{\s 1}_{(w_1,\xi_1)}((-t_0,t_0))\big)\subset F\big(\gamma^{\s 1}_{(x,\eta)}((-\infty,-t_1+t_0))\cap W_1\big)
\subset \gamma^{(2)}_{x,\eta}(\R)\cap W_2.
 \end{eqnarray}
Thus for any $w_1\in W_1$ and $\xi_1\in L^+_{w_1}M_1$  
 such that $\gamma_{w_1,\xi_1}(\R_+)\cap \mathcal{U}\not=\emptyset$, formula \eqref{eq: light-like geodesics}
 implies that 
  $F$ restricted to a neighborhood of $w_1$ maps the lightlike geodesic $\gamma^{\s 1}_{(w_1,\xi_1)}$ 
 to a segment of a light-like geodesic of $(M_2,g_2)$.
%  $F$  maps  near $w_1$ the light-like geodesic $\gamma^{\s 1}_{(w_1,\xi_1)}$ 
%  to a light-like geodesic of $(M_2,g_2)$. 
% 
Hence, $F_*\xi_1\in L_{w_2}M_2$, where $w_2=w_1$.
 Thus for any $w_1\in W_1$ there are infinitely many vectors $\xi_1\in L^+_{w_1}M_1$  
  such that $\gamma_{(w_1,\xi_1)}^{\s 1}(\R_+)\cap \mathcal{U}\not=\emptyset$, and for which $F_*w_1\in L_{w_2}M_2$,
  we see that $F$  maps $L^+_{w_1}M_1$ to $L_{w_2}M_2$. Thus the metric tensor $g_1$ is conformal to $F^*g_2$ at $w_1$. As $w_1\in W_1$ is arbitrary, this implies that $g_1$ and $F^*g_2$  are conformal  
 \end{proof}
 




%In particular, this proves the uniqueness statement of . 
%
To complete the proof of Theorem \ref{themain} it ~ remains to show that the conformal factor is $1$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  Determination of the conformal factor and proof finish
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Determination of the conformal factor}\label{det-of-conform}
Here we prove that also the conformal factor of the metric is the same. This is the final step in the proof of Theorem \ref{themain}.
% 
% 

\begin{proposition}\label{conformii}
Let $(M,g), (\widetilde{M}, \widetilde{g})$ be globally hyperbolic $C^\infty$ manifolds with metrics $g$ and $\tilde{g}$.  
%= g_{ij}dx^i dx^j$, $\widetilde{g} = \widetilde{g}_{ij} dx^i dx^j$ and 
Let the subsets $W \subset M$ and $\widetilde{W} \subset \widetilde{M}$ be open. Let $c \in C^\infty (W)$ be a strictly positive function and assume there is a diffeomorphism 
$
F : W \rightarrow \widetilde{W} 
$ 
such that $(F^* \widetilde{g})(x) = c(x) g(x)$, $\forall x \in W$. % where $ F^* \widetilde{g}$ is the pull-back of $\widetilde{g}$. 
%Assume that there are no closed timelike geodesics (e.g. $X$ globally hyperbolic). 
%Let $B \subset X$ be open. 
Let $\gamma_{(x,p)}$ be the geodesic in $(M,g)$ with initial condition $\dot\gamma_{(x,p)} (0) = (x,p)$, where $(x,p) \in TW$. 
Also let $\sigma_{(x,p)}$ be the geodesic in the manifold $(W, F^*\widetilde{g})$ with $\dot\sigma_{(x,p)}(0) = (x,p)$.
%
Assume that for every $x \in W$ there exist two linearly independent timelike vectors $p_1,p_2\in T_x W$, real numbers $\epsilon_1,\epsilon_2>0$ and two smooth functions $\alpha_j: (-\epsilon_j,\epsilon_j) \rightarrow \R$, $j=1,2$, such that 
\begin{equation}\label{d77jlp}
\gamma_{(x,p_j)} (t) = \sigma_{(x,p_j)} ( \alpha_j (t) ) , \quad \text{for every} \quad t \in (-\epsilon_j , \epsilon_j), \quad j=1,2. 
\end{equation}

Then $c$ is a constant function on $W$. In particular, if the metrics $g$ and $F^*\widetilde{g}$ equal at some point $x \in W$, then they equal everywhere in $W$.
\end{proposition}


\begin{proof}
Let us write $c(x) = e^{\varphi(x)}$ for some smooth function $\varphi$, and $\Gamma_{ij}^k$ and $\widetilde\Gamma_{ij}^k$ for the Christoffel symbols of the metrics $g$ and $F^*\tilde{g}$ respectively. Denote the associated pair of covariant derivatives by $\nabla$ and $\widetilde\nabla$. 
%In local coordinates we distinguish the two sets Christoffel symbols from each other by writing $\Gamma_{ij}^k := ( \nabla_{\partial_i} \partial_j )^k$ and $\widetilde\Gamma_{ij}^k := ( \widetilde\nabla_{\partial_i} \partial_j )^k$. 
%and for vector fields along curves by $D_t$ and $\widetilde{D}_t$. 
%Denote $\Gamma_{ij} := \Gamma_{ij}^k \partial_k$.
The Christoffel symbols of the conformal metrics $g$ and $F^*\tilde{g}=c\s g$ are connected to each other by 
\[
\begin{split}
\widetilde\Gamma_{ij}^k
% \frac{1}{2} \tilde{g}^{kl} ( \partial_i \tilde{g}_{lj} +  \partial_j \tilde{g}_{li}- \partial_l \tilde{g}_{ij}) \\
% &= \frac{1}{2} e^{-\varphi} g^{kl} \big( \partial_i (e^{\varphi} g_{lj} )+  \partial_j (e^{\varphi} g_{li} )- \partial_l (e^{\varphi} g_{ij}) \big) \\
% &= \frac{1}{2} g^{kl} \big( \partial_i  g_{lj} +  \partial_j  g_{li} - \partial_l  g_{ij} \big) + \frac{1}{2} g^{kl} \big(  g_{lj} \partial_i  \varphi +   g_{li}\partial_j \varphi- g_{ij}\partial_l  \varphi  \big)  \\
= \Gamma_{ij}^k +  \frac{1}{2}  \big(  \delta_j^k \partial_i  \varphi +  \delta_i^k \partial_j \varphi-  g_{ij} g^{kl} \partial_l  \varphi  \big).  %\\
\end{split}
\]
(See  \cite[Ch. 3, Proposition 13.]{oneill1983semiriemannian}). 
Thus, for any smooth curve $\gamma$ in $W$, 
\begin{equation}\label{123hhheiq}
\begin{split}
\widetilde\nabla_{\dot\gamma} \dot\gamma =&  \ddot\gamma^k\partial_k  + \widetilde\Gamma_{ij}^k (\gamma)  \dot\gamma^i \dot\gamma^j  \partial_k\\
=&   \ddot\gamma^k \partial_k +\Big( \Gamma_{ij}^k(\gamma) +  \frac{1}{2}  \big(  \delta_j^k \partial_i  \varphi |_\gamma +  \delta_i^k \partial_j \varphi|_\gamma-  g_{ij}(\gamma) g^{kl}(\gamma) \partial_l  \varphi|_\gamma  \big)  \Big) \dot\gamma^i \dot\gamma^j  \partial_k\\
=&   \ddot\gamma^k \partial_k + \Gamma_{ij}^k(\gamma)  \dot\gamma^i \dot\gamma^j   \partial_k +     \partial_j \varphi |_\gamma \dot\gamma^j \dot\gamma^k  \partial_k -    \frac{1}{2}g_{ij}(\gamma) \dot\gamma^i \dot\gamma^j  g^{kl}(\gamma) \partial_l  \varphi |_\gamma \partial_k   \\
=&   \nabla_{\dot\gamma} \dot\gamma +      \langle d\varphi , \dot\gamma \rangle  \dot\gamma -    \frac{1}{2} g (\dot\gamma,\dot\gamma) \nabla \varphi  .  \\
\end{split} 
\end{equation}
%\begin{equation}\label{123hhheiq}
%\begin{split}
%\widetilde\nabla_V V =&  V^i \partial_i V^k \partial_k + \widetilde\Gamma_{ij}^k  V^i V^j  \partial_k\\
%=&  V^i \partial_i V^k \partial_k +\Big( \Gamma_{ij}^k +  \frac{1}{2}  \big(  \delta_j^k \partial_i  \varphi +  \delta_i^k \partial_j \varphi- % g_{ij} g^{kl} \partial_l  \varphi  \big)  \Big) V^i V^j  \partial_k\\
%=&  V^i \partial_i V^k \partial_k + \Gamma_{ij}^k  V^i V^j  \partial_k +     \partial_j \varphi  V^j    V^k \partial_k -    \frac{1}{2}g_{ij} %V^iV^j g^{kl} \partial_l  \varphi  \partial_k   \\
%=&   \nabla_V V +      \langle d\varphi , V \rangle  V -    \frac{1}{2} g (V,V) \nabla \varphi  . \\
%\end{split} 
%\end{equation}
Let $x \in W$ and,  for $j=1,2$, let 
%let $p$ be one of the vectors 
$p_j\in T_xW$, $\eps_j>0$ and $\alpha_j: (-\epsilon_j,\epsilon_j) \rightarrow \R$ be as in the claim of this proposition. Let us relax the notation by omitting the indices $j=1,2$ from subscripts. 
By differentiating~\eqref{d77jlp} in the variable $t$ we obtain
\begin{equation}\label{ghus}
\dot\gamma_{(x,p)} (t) = \alpha'(t) \dot\sigma_{(x,p)} ( \alpha (t) )
\end{equation}
%for every $x\in W$ 
%future-directed timelike $(x,p)$ 
%and 
for $t \in (-\epsilon , \epsilon)$. 
Since 
\[
\sigma_{(x,p)}( \alpha(0)) = \gamma_{(x,p)} (0) = x = \sigma_{(x,p)} (0)
\]
and since the causal geodesics $\sigma_{(x,p)}$ does not have self-intersection by global hyperbolicity (recall that $F$ identifies $ \sigma_{(x,p)}$ with a causal geodesic in the globally hyperbolic manifold $\widetilde{M}$), we obtain $\alpha(0) = 0$. 
%(The Lorentz manifold $(W,F^*\tilde{g})$ is globally hyperbolic since it is conformal to $(W,c\s g)$.) 
Substituting $\alpha(0) = 0$ to (\ref{ghus}) yields
\[
p = \dot\gamma_{(x,p)} (0) = \alpha'(0) \dot\sigma_{(x,p)} ( \alpha (0) ) = \alpha'(0) \dot\sigma_{(x,p)} ( 0 )  = \alpha'(0)\s p,
\]
that is, $\alpha'(0) = 1$. Thus, $\alpha(t) = t + O(t^2)$ near $t=0$. In particular,
\[
\tilde\nabla_{\dot\gamma_{(x,p)}} \big[ \dot\sigma_{(x,p)}( \alpha(t)) \big]|_{t=0 }  = \tilde\nabla_{\dot\sigma_{(x,p)}} \dot\sigma_{(x,p)}( t) |_{t=0 } = 0.
\]
%In particular, $\alpha'(0) \neq 0$ for $p \neq 0$ so dividing by $\alpha'(0)$ is valid. 
%Let $(x,p) \in TX$ be such that $g(p,p) \neq 0$ (possibly space-like).
%and
%\[
%\ddot\gamma_{(x,p)} (t) = \alpha''(t) \dot\sigma_{(x,p)} ( \alpha (t) )+  (\alpha'(t))^2 \ddot\sigma_{(x,p)} ( \alpha (t) )
%\]
Substituting this to (\ref{123hhheiq}) and using that $\gamma_{(x,p)}$ is a geodesic imply 
\[
\begin{split}
0 =& \nabla_{\dot\gamma_{(x,p)}} \dot\gamma_{(x,p)} (t) |_{t=0} =    \widetilde{\nabla}_{\dot\gamma_{(x,p)} } [  \alpha'(t) \dot\sigma_{(x,p)} ( \alpha (t) ) ] |_{t=0} -    \langle d\varphi , \dot\gamma_{(x,p)} (0) \rangle  \dot\gamma_{(x,p)} (0) \\
&+    \frac{1}{2} g (\dot\gamma_{(x,p)} (0), \dot\gamma_{(x,p)} (0) ) \nabla \varphi ( \gamma_{(x,p)} (0))  \\
=&  \alpha''(0)  \dot\sigma_{(x,p)} ( 0 ) +  \widetilde\nabla_{\dot\gamma_{(x,p)}}[ \dot\sigma_{(x,p)}( \alpha(t))] |_{t=0 }    -    \langle d\varphi (x) , p \rangle p+    \frac{1}{2} g (p,p ) \nabla \varphi(x)  \\
%=&  \alpha''(0)  \dot\sigma_{(x,p)} ( 0 ) +  \widetilde\nabla_{\dot\sigma_{(x,p)}(t)} \dot\sigma_{(x,p)}( t) |_{t=\alpha(0) }    -    \langle d\varphi (x) , %p \rangle p+    \frac{1}{2} g (p,p ) \nabla \varphi(x)  \\
=& \big( \alpha''(0)      -    \langle d\varphi (x) , p \rangle \big)p+    \frac{1}{2} \underbrace{g (p,p )}_{\neq 0} \nabla \varphi(x).    \\
%=& \Big( \frac{\alpha''(0)}{\alpha'(0)}     -    \langle d\varphi (x) , p \rangle \Big) p+    \frac{1}{2} g (p,p ) \nabla \varphi(x) .   \\
\end{split}
\]
In particular, $ \nabla \varphi(x) $ lies in the line spanned by $p$ in the space $T_xW$. Since this holds for every $x\in W$ and for the corresponding two linearly independent $p_1,p_2  \in T_xW$ (recall that we omitted the subscripts in the calculation above), we conclude that $\nabla \varphi(x) = 0$ for every $x \in W$. That is, the function $ \varphi$, and hence $c= e^\varphi$ is a constant function on $W$. 
\end{proof}
%\end{proposition}


%Recall from Theorem \ref{oo1} that the metric $F^* g_2$ is conformal to $g_1$ in $W_1$. 
We finish the proof Theorem~\ref{themain} by showing that the conformal factor is $1$; that is, $g_1 = F^* g_2$ on $W_1$.

\begin{theorem}
Assume that the conditions of Theorem \ref{themain} are satisfied and $\Phi_{1,L^+V} = \Phi_{2,L^+V}$ for Lorentzian manifolds $(M_j,g_j)$, $j=1,2$. 
Equip the associated spaces $W_j$, $j=1,2$ with the canonical metrics $g_j|_{W_j}$ induced by the trivial inclusions $W_j \hookrightarrow M_j$.
%Then,
%the conformal factor (cf. Theorem \ref{oo1}) between ${F}^* g_2$ and $g_1|_{W_1}$ is $1$. 
Then, the map 
\[
{F} : W_1 \rightarrow W_2
\]
is an isometry. 
\end{theorem}

\begin{proof}
Let $w_{1} \in W_1$ be arbitrary and choose two time-like vectors $(\hat{x},\hat{p} ), (\hat{y},\hat{q} )$ based in $\mathcal{U}$ such that the geodesics $\gamma_{(\hat{x},\hat{p} )}$ and $\gamma_{(\hat{y},\hat{q} )}$ intersect first time at $w_{1}$ in $(M_1,g_1)$ as earlier.
By Lemma \ref{ss_map_determines_intersection} we may fix them such that the corresponding  geodesics in $(M_2,g_2)$ intersect first time at $F(w_{1}) = w_{2}$. For $(x,p) \in TW_1$ let us denote by $\sigma_{(x,p)}$ the geodesic in $(W_1,F^*g_2)$ that satisfies $\dot\sigma_{(x,p)}(0) = (x,p) $.
While keeping $(x,p)$ fixed, we can vary the initial direction $(y,q)$ so that the intersection point of the geodesics $\gamma_{(y,q)}$ and $\gamma_{(x,p)}$ varies along the geodesic $\gamma_{(x,p)}$ through an open geodesic segment.  
% If we vary $w_{1}$ slightly along  the graph of $\gamma_{(\hat{x},\hat{p} )}$ the vector $(\hat{x},\hat{p} )$ can be kept still~\f{What does this mean? Why we want to keep $(\hat{x},\hat{p})$ still?} while moving only $(\hat{y},\hat{q} )$.
Since the geodesics $\gamma_{(\hat{x},\hat{p} )}$ and $\gamma_{(\hat{y},\hat{q} )}$ intersect in both geometries, this variation of $w_{2}=F(w_{1})$ corresponds to a path through $w_{2}$ that is some reparametrisation of the geodesic  $\gamma_{(\hat{x},\hat{p} )}$ in $(W_2,g_2)$. 
Mapping this reparametrised geodesic segment to $M_1$ using $F^{-1}$ implies that there is a vector $p_1 \in T_{w_{1}} W_1$ and a smooth reparametrisation $\alpha_1(s)$ such that the geodesic $\gamma_{(w_{1},p_1)}$ in $(M_1,g_1)$ satisfies $\gamma_{(w_{1},p_1)}(s) = \sigma_{(w_{1},p_1)}( \alpha_1(s) )$  on some interval $s\in (-\epsilon_1,\epsilon_1)$. Further, by exchanging the roles of $(\hat{x},\hat{p} )$ and $(\hat{y},\hat{q} )$ and then repeating the construction above one obtains another linearly independent vector $p_2 \in T_{w_{1}} W_1$ and a smooth  reparametrisation $\alpha_2(s)$, $s\in (-\epsilon_2, \epsilon_2)$ such that $\gamma_{(w_{1},p_2)}(s) = \sigma_{(w_{1},p_2)}( \alpha_2(s) )$, for $s\in (-\epsilon_2, \epsilon_2)$. By Theorem \ref{oo1}, we have $g_1|_{W_1}=c\s F^* g_2$. Consequently by Proposition \ref{conformii} we have that $c>0$ is constant. % $g_1|_{W_1}$ equals $c F^* g_2$ with some constant $c>0$. 
Since $F^* g_2 = g_1$ on $V$ we conclude that $c=1$. Thus $F$ is an isometry.
\end{proof}












==> Sections/prelim.tex <==
% Preliminary section
%
\section{Preliminaries}\label{prelim}
\subsection{Notation}\label{notation}
Throughout this paper, $(M,g)$ will be an $n$-dimensional Lorentzian spacetime with $\nnn \geq 3$. We additionally assume that $(M,g)$ is globally hyperbolic. Globally hyperbolicity (see e.g.~\cite{bernal2005}) implies that \tbl{$M=\R \times N$}, for some smooth $n-1$ dimensional submanifold $N\subset M$, and that the metric takes the form
\[
g (x)  = -g_{00}(x) dx^0 \otimes dx^0  + g_{N}(x), \ \ x=(x^0,\overline{x}), \  x^0 \in \R, \ \overline{x} \in N,
\]
where $g_{00} \in C^{\infty} (M)$ is a positive function and $g_{N} (x^0, \, \cdot  \,  )   $ is a smooth Riemannian metric on $N$, for each $x^0 \in \R$.
Global hyperbolicity implies that the manifold $(M,g)$ has a global smooth timelike vector field $\tau$. This vector field  defines the causal structure for $(M,g)$. Further, a globally hyperbolic manifold is both causally disprisoning and \antti{causally} pseudoconvex (see for example \cite{MR1216526}). \tjb{Causally disprisoning means that for each inextendible causal geodesic $\gamma: (a,b)\to M$, $-\infty\le a<b\le \infty$, and any $t_{0}\in(a,b)$, the closures in $M$ of the sets $\gamma(a,t_{0}]$ and $\gamma[t_{0},b)$ are not compact in $M$. }%Causally disprisoning means that for each inextendible causal geodesic $\gamma: (a,b)\to M$,\tbl{ $-\infty\le a<b\le \infty$}, and every compact set $K\subset M$, there are parameter values $a<t_1<t_2<b$ such that $\gamma(t)\in M\setminus K$ for all $a<t<t_1$ and $t_2<t<b$.
The manifold $M$ is pseudoconvex if % on the inextendible (i.e. maximal) domain of parameters and 
for every compact set of $M$, there is a geodesically convex compact set which properly contains it.  %another compact set that is convex with respect to causal geodesic segments.%~\footnote{\tbl{Remove starting from ``That is...'' if this is not needed later.}} 


%Let $N$ be a given a smooth manifold of dimension $n-1$, and consider the manifold $\R\times N$.
%The Cartesian product trivially splits each point $x\in \R \times N$ into two components:
%\[
%x= (x^0,\overline{x} ) , \ \  x^0 \in \R, \ \overline{x} \in N.
%\]
%We set
%\[
%g (x)  = -g_{00}(x) dx^0 \otimes dx^0  + g_{N}(x), \ \ x=(x^0,\overline{x}), \  x^0 \in \R, \ \overline{x} \in N
%\]
%to be a globally hyperbolic, geodesically complete, pseudo-Riemannian metric on $\R \times N$, where  $g_{00} \in C^{\infty} (\R \times N ; (0,\infty) )$, and $g_{N} (x^0, \ \cdot  \  )   $ is  a smooth Riemannian metric on $N$, for each $x^0 \in \R$.

We use standard notation for the causal structure of $(M,g)$. For $x,y\in M$ we write $x\ll y$ (respectively $x\gg y$) if  $x\ne y$ and there is a future directed timelike geodesic from $x$ to $y$ (respectively from $y$ to $x$). We write $x < y$ (respectively $x > y$) if  $x\ne y$ and there is a future directed causal geodesic from $x$ to $y$ (respectively from $y$ to $x$).


 Given $x\in M$, let  $J^{+}(x):=\{y\, :\, x< y \text{ or } x=y\}\subset M$ and $I^{+}(x):=\{y\, :\, x\ll y\}\subset M$ denote respectively the causal and chronological future of $x$. Similarly, let $J^{-}(x)$ and $I^{-}(x)$ denote the causal and chronological past of $x$.  %Analogously, we define the causal and chronological past $J^-(x)$ and $I^-(x)$ for points and $J^-(U)$ and $I^-(U)$ for subsets in $\R \times N$.
The set of points in $M$ which may be reached by lightlike geodesics emanating from a point $x \subset M$ is 
\[
\mathcal{L}^{\pm}(x):= \{  y \in TM : y=\exp_x (sp) , \, p \in L_x^\pm M, \, s \in [0,\infty) \}, 
\]
where $L^\pm_x M \subset TM$ is the set of future ($+$) or past ($-$) directed lightlike vectors in $T_xM$.
%
%In the settings where we consider the causal regions of a set $U\subset M$, w
If $U\subset M$, we also write 
\begin{equation}\label{causal_spaces}
J^{\pm}(U) = \bigcup_{x\in U}  J^{\pm}(x), \quad I^{\pm}(U) = \bigcup_{x\in U}  I^{\pm}(x), \quad \mathcal{L}^{\pm}(U)= \bigcup_{x\in U}  \mathcal{L}^{\pm}(x).
\end{equation}
 
We express the elements of $TM$ as $(x,p)$ where $x\in M$ and $p\in T_xM$. Since $TM=  T\R \times TN$, each $(x,p)\in TM$ can be written in the form
\[
x=(x^{0}, \bar{x}), \ \ \text{ and } \ \ p = (p^{0},\bar{p}), 
\]
for $ x^{0} \in \R$, $\bar{x} \in N$, $p^{0}\in T_{x^{0}} \R$, and $\bar{p} \in T_{\bar{x}} N$.
% and 
% \[
% p = (p^{0},\bar{p}), \ \ p^{0}\in T_{x^{0}} \R, \ \ \bar{p} \in T_{\bar{x}} N.
% \] 
%Local coordinates in $\R \times N$ generate a local frame $\partial_\alpha : U \rightarrow T(\R \times N)$, $\alpha = 1,\dots, \nnn$ on the corresponding coordinate neighbourhood $U \subset \R \times N$. Using the ordered set 
%$\{ \partial_\alpha|_x \}_{\alpha=0}^{\nnn-1}
%% \subset T_x(\R \times N)
%$ as a coordinate basis in each fiber $T_x (\R \times N)$, $x\in U$ one identifies $TU \subset T(\R \times N)$ with the cartesian product $U \times \R^{\nnn}$. 
%Such a construction is called a local trivialization of the bundle $T(\R \times N)$. % We shall use the symbol $\approx$ when referring to local treatment. 
Given a local coordinate frame $\partial_\alpha : U\subset M \rightarrow TM$, $\alpha = 1,\dots, \nnn$, we identify $TU \approx  U \times \R^{\nnn}$. We use $(x,p^\alpha)$ to denote this local expression.%\footnote{\tbl{look for where we actually use this notaion}}

For $(x,p)\in TM$, we denote by $\gamma_{(x,p)}$ the geodesic with initial position $x$ and initial velocity $p$. 
% 
%Explicitly, such a geodesic is given locally by $\gamma_{(x,p)}(s)= \exp_x(sp)$. % where $\exp_x$ is the exponential map defined on an open neighbourhood of the origin in $T_xM$. 
%In this paper $M$ is considered to be geodesically complete which, by definition, implies that the exponential map is well defined on the whole fiber $T_x M$. That is, the curve  $\gamma_{(x,p)}$ is well defined as a function on $\R$. 
The velocity of $\gamma_{(x,p)}$ at $s\in \R$ is denoted by $\dot\gamma_{(x,p)}(s) \in T_{\gamma_{(x,p)}(s)} M$, $s\in \R$. To simplify the notation we occasionally refer also to the curve $s\mapsto ( \gamma_{(x,p)}(s), \dot\gamma_{(x,p)}(s) ) \in TM$ by $\dot\gamma_{(x,p)}(s)$. 

%$(p^0, \dots, p^{\nnn-1}) \in \R^{\nnn}$, an element $(x,p)\in TU$ takes the form $(x,p^0, \dots, p^{\nnn-1 } )$; we often simply write $(x,p^\alpha)$ for this local expression.

% local trivialization $T(\R \times N) \approx U \times \R^{\nnn}$ we use $(x,p^\alpha)$ as a shorthand for $(x,p^0, \dots, p^{\nnn-1 } )$, where $(p^0, \dots, p^{\nnn-1}) \in \R^{\nnn}$ are the local coordinates.


The appropriate phase spaces for our particles will be comprised of the following subbundles of $TM$. %; below are the various notation we use for these spheres. 
Let $U\subset M$ be open and let $m\geq 0$. The mass shell of mass $m$ on $U$ is  %{\color{red} (Problematic notation. cf. $TQ$ when $Q$ submanifold of $M$. Confusion could maybe be avoided by saying that the meaning is usually clear from the context. What do you think? --Antti)}
%The hyperbolic sphere bundle of radius $r$ over a set $U$ is the set of timelike vectors 
\[
%S_r (\R \times N ) :=
P^m U := \{ (x,p) \in TM \setminus \{0\} : \sqrt{- g( p,p) } = m, \ \ \pi(x,p)=x  \in U \} \subset TM ,
\] 
where $\pi :TM \rightarrow M$ is the canonical projection. The time-like bundle on $U$ is
\[
\mathcal{P}U :=  \bigcup_{m>0}P^{m}U.
\]
We denote the inclusion of the light-like bundle $LU := P^0 U$ to this union as
\[
\overline{\mathcal{P}}U  :=  \bigcup_{m\geq 0}P^{m}U
\]
which is the bundle of causal vectors on $U$. 
%As we will often will consider these sphere bundles and collections thereof  over the whole space $M$, 
Notice that $\overline{\mathcal{P}}U$ excludes the zero section; that is, a zero vector is not causal in our conventions.
We also write for $t \in \R$, $ x\in \R \times N$
%{\color{red} ( I've replaced the shorthands $P^r$, $\OVS$, $\SP$,... with $P^r M$, $\OVS M $, $\SP M$,... If/when you find some remains of the old notation, please update them. I've also tried to reduce unnecessary brackets when there is no danger of confusion, so expressions like $P^r (U)$ should be just $P^r U$ etc. The new nomenclature is also in line with the standard notation for bundles in differential geometry (cf. $TU$, $\mathcal{T} U$, etc.).  --Antti)}
\begin{alignat*}{2}
%P^r := P^rM, \ \ 
P^r_t U &:= (T_t\R  \times TN) \cap P^r U ,   \quad &&P^r_x U :=T_x M \cap P^r U \\%\overline{\mathcal{P}}_{t} := ( T_{t} \R \times  T N )\cap \overline{\mathcal{P}},
%\mathcal{P} := \mathcal{P}M, 
%\ \ \overline{\mathcal{P}} := \overline{\mathcal{P}}(M), 
\ \ \mathcal{P}_{t} U &:= ( T_{t} \R \times  T N )\cap \mathcal{P}U , \quad  &&\mathcal{P}_{x}U := ( T_{x} M )\cap \mathcal{P}U,
\end{alignat*}
and write similarly for $\overline{\mathcal{P}}_x U$ and $\overline{\mathcal{P}}_t U$.%, is considered for the causal vectors.
%
%\begin{align*}
%S^r &:= S^r(M), \\
% S^r_t &:= (T_t\R  \times TN) \cap S^r \ \  \text{for} \ \ t \in \R, \\
%  S_x^r&:= T_xM \cap S^r \ \ \text{for} \ \   x\in \R \times N,\\ \intertext{and} 
% \PP_{t} &:= ( T_{t} \R \times  T N )\cap \PP \ \ \text{for} \ \   t\in \R,\\
% \PP&:= \PP(M),\\
% \overline{\PP}&:= \overline{\PP}(\R \times N).
% \end{align*}
%We only consider the cases when $r > 0$ and $r=0$ which correspond to time-like and light-like mass shells in the context of general relativity.
%In particular, $S^0$ is the collection of light-like vectors in $T( \R \times N)$. 

Each one of the bundles above consists of future-directed and past-directed components which are distinguished by adding ``$+$'' or ``$-$'' to the superscript.
For example, we denote the manifold of future-directed causal vectors on an open set $U \subset M$ by %\footnote{\tbl{check sign of $g(T,p)$ below}}
\[
\OVS U := \{ (x ,p) \in TM \setminus \{0\} : x \in U, \,  -g(p,p)|_x \geq 0 , \, g(\tau,p)<0 \} \subset \overline{\mathcal{P}} U.
\]
%For $U = M$, once again we simply write $\OVS  := \OVS M$. 

%
%\begin{figure}
%    \centering
%    \includegraphics[width=\textwidth]{pictures/mass-shells1.pdf}
%    \caption{The light cone $L(x) = S^0_x$ (in red) and mass shells $S^r_x$ (in black) for different values of $r>0$ and fixed $x\in \R \times N$. The upper and  lower halves of the space indicate the future- and past-directed vectors, respectively. They differ by sign of the coordinate $p^0:= \langle dx^0, p \rangle $ whose absolute value corresponds to the energy in physics.}
%    \label{fig:my_label}
%\end{figure}
%   

%\tjb{TB: relabel manifolds below later. Any ideas for good names?} \\ 
%{\color{red} My (=Antti) suggestion : 
%\\
%$K_S$: (two-sided/complete/open)  flowout of $S$ in $TM$, \\
%$G_S$: (two-sided/complete/open) flowout of $S$ in $M$ --Antti }

Let $S \subset \overline{\mathcal{P}}_t M$, $t \in \R$ be a submanifold of $TM$. The \emph{geodesic flowout} of $S$ in $TM$ is the set
\[
K_S := \{ (x,p) \in TM : (x,p) = \dot\gamma_{(y,q)} (s), \ s\in (-T(y,-q),T(y,q)), \ (y,q) \in S \} \subset \overline{\mathcal{P}} M.
\]
Here the interval $(-T(y,-q),T(y,q))$ is inextendible, i.e. the maximal interval where the geodesic $\gamma_{(y,q)}$ is defined. 
\begin{remark}\label{flowout-is-manifold}
The geodesic flowout $K_S$ is a smooth manifold. To see this, note that $K_S$ is the image of the map $(s,(y,q))\mapsto \varphi_s(y,q)$, where $\varphi_s(y,q)$ is the integral curve of the geodesic vector field $\XX$ at parameter time $s$ starting from $(y,q)\in S$. Since $\XX$ is transversal to $\overline{\mathcal{P}}_t M$ (see the  proof of Lemma~\ref{uuiisok}) we have that this map is an immersion, see e.g.~\cite[Theorem 9.20]{Lee_2013}. Given that $M$ is globally hyperbolic, there are no closed causal geodesics. From this it follows that this map is also injective and thus an embedding. Consequently, its image $K_S$ is a smooth submanifold of $TM$.
\end{remark}


% To see this, recall first that $M$ is causally disprisoning as described above. % first that causal vectors on a globally hyperbolic manifold escape compact sets.  
% %Since the manifold $M$ is globally hyperbolic, causal geodesics escape compact sets. 
% It follows that the intersection $K_S \cap TU$ with a relatively compact open set $U \subset M$ is a submanifold of $TM$. As a smooth manifold has a countable basis of regular coordinate balls \cite[Proposition 1.19]{Lee_2013}, we conclude that $K_S$ is a smooth manifold. ~\footnote{\tbl{Antti, can you elaborate your proof that $K_S$ is a submanifold?}}
%which splits up into the positive and negative halves, 
%\[
%K_S^{\pm} = \{ (x,p) \in TM : (x,p) = \dot\gamma_{(y,q)} (s), \ \pm s\in [0,\infty), \ (y,q) \in S \}.
%\]
We denote $G_S:=\pi(K_S)$, which is the set 
\[
G_S = \{ x \in M : x = \gamma_{(y,q)} (s), \ s\in (-T(y,-q),T(y,q)), \ (y,q) \in S \} \subset M. %G_M
\]
%where $\gamma_{(y,q)}$ is a geodesic in $M$ with the initial value $\dot\gamma_{(y,q)} (0) = (y,q)$. 
Unlike $K_S$, the set $G_S$ might not be a manifold since the geodesics describing this set might have conjugate points.%~\footnote{\tbl{Do we ever use $G_S^\pm$. The part about $G_S^\pm$ here is commented away.}} %due to possible presence conof caustics. 
%We refer to $G_S$ as the  geodesic flowout of $S$ in $M$. 
% % It splits up into the two halves,  
% % \[
% % G_S^\pm := \{ x \in M : x = \gamma_{(y,q)} (s), \ \pm s\in [0,T(y,\pm q) ), \ (y,q) \in S \},
% % \]
% % corresponding to the trajectories of half-closed geodesic segments with initial($+$) or final($-$) velocity in $S$. We only consider the case where $S$ consists of future directed vectors, i.e. $S\subset \OVS M$. In that case the set $G_S^\pm$ consists of the causal future($+$) or the past($-$) of the elements with initial position and velocity described by $S$.

If $X$ is a smooth manifold and $Y$ is a submanifold of $X$, the conormal bundle of $Y$ is defined as
\[
 N^*Y=\{(x,\xi)\in T^*X\setminus \{0\}: x\in Y,\, \xi \perp T_xY\}.
\]
Here $\perp$ is understood with respect to the canonical pairing of vectors and covectors. %We also define%~\footnote{\tbl{Check that this is what $\Lambda_S$ is supposed to be?}}
%\[
%\Lambda_S := \{ (x, \xi ) \in T^* M : \text{ there is } (x,p)\in K_S \text{ such that } (x,p\, ; \, \pi^*(\xi ))   \in N^* K_S\}.
%\]
%For a relatively compact open set $U \subset M$, 
%Here $\pi:T^*M\to M$ and $\pi^*:T^*T^*M\to T^*M$ is the pullback. The set $\Lambda_S$ is a Lagrangian manifold which equals the conormal bundle of $G_S$ in the open regions $U \subset M$ where the set $G_S \cap U$ is a manifold. 
%where $\pi : T(\R \times N) \rightarrow \R \times N$ is the projection $(x,p) \mapsto x$. %The definition is equivalent to if $G_M$ is a manifold.

%The set $T(\R \times N) \setminus ( \R \times \{ 0\} \times TN)$  is denoted by $\PP$. Here we identify $T_{\{ t \}} \R = \{ t \} \times \R$ for each $t \in \R$. '

%\subsection{Light Observations}\label{light-obs}
%
%%\subsection{The System}
%Fix a smooth future pointing time-like curve $\mu (s) \in \R \times N $, $s \in [-1,1]$, $j=1,2$, let $-1 < s^-,s^+ < 1$ and assume that $V \subset  \R \times N $ is a neighbourhood of the curve $\mu ([0,1])$.  Set $x^{\pm}:=\mu(s^{\pm})$.
%% and $TV \cap (Q_1 \cup Q_2) = \emptyset$.  
%We consider $V$ as the known observation space in which we make measurements.  The curve $\mu(s)$ can be thought of as a part of the world line of a measurement device (for example a photon detector carried by a satellite). 
%The region we aim to construct is the open, relatively compact set 
%\begin{equation}\label{unknown}
%W :=  I^+(x^{-}) \cap I^-(x^{+}) \subset \R \times N.% \ \ S^{r_j} (Q_j ) := S^{r_j} \cap T Q_j
%\end{equation}
%By construction, each point of $W$ can be connected to the observation space with a ray of light.  Hence, it is possible (see Lemma \ref{druqks}) to reach and receive information from locations in the unknown region by sending particles of invariant masses $r_1$ and $r_2$ with initial velocities in $S^{r_1}(V)$ and $S^{r_2}(V)$, respectively. 
%
%In fact, it is possible to record multiple instances of light information from a single location. We adopt the following definitions from \cite{Kurylev2018} for the sets of measured light signals.
%
%Let $x\in \R \times N$ and $U\subset \R\times N$ be open.
%\begin{enumerate}[(i)]
%\item The future directed light cone emanating from the point $x\in \R \times N$:
%\[
% \mathcal{L}^+(x) :=  \{ z \in \R \times N : z= \gamma_{(x,p)} (s), \ s \geq 0, \ p\in L^+(x), \}  .
%\]
%\item The light observation set of $x$ in the set $U$:
%%simply the collection of future-directed light-like vectors which reach $U$:
%\[
%\mathcal{P}_U (x) :=  \mathcal{L}^+ ( x )  \cap U \in 2^U.
%\]
%\item The earliest light observation set of a $x$ in the set $U$ is the collection
%\[
%\mathcal{E}_U (x) :=  \left\{ y \in \mathcal{P}_U (x) : \begin{array}{l}
% \text{there are no } z\in \mathcal{P}_U (x) \text{ and future-pointing time-like geodesics }\\
% \gamma : [0,1] \rightarrow U \text{ with } \gamma(0) = z \text{ and } \gamma(1) = y
%\end{array}
% \right\}.
%\]
%
%%\[
%%\mathcal{E}_V (x)  := \{  y \in \mathcal{P}_V (x) : \text{}  \}t
%%\]
%\item The family of earliest light observation sets in $U$ of points in $W \subset \R \times N$:
%\[
%\mathcal{E}_U (W) := \{ \mathcal{E}_U (x) : x \in W \}.
%\]
%\end{enumerate}
%As shown in \cite[Theorem 1.2]{Kurylev2018}, the conformal class of the metric in $W$ is uniquely described by the associated earliest light observation set in $V$ for $\nnn \geq 3$. 
%


\subsection{Lagrangian distributions and Fourier integral operators}\label{lagrangian-dist}\tjb{Here we define the classes of distributions and operators we work with in this paper. We will follow the notation in Duistermaat's book ~\cite{duistermaat2010fourier}. }%; see also \cite{hormander1971fourier1}.% for thorough exploration of the field. 
\antti{See also the original sources \cite{hormander1971fourier1, MR388464}. }

Let $X$ be a smooth manifold of dimension $n \in \mathbb{N}$ and $\Lambda\subset T^*X\setminus \{0\}$ be a conic Lagrangian manifold~\cite[Section 3.7]{duistermaat2010fourier}. We denote the space of symbols  \cite[Definition 2.1.2]{duistermaat2010fourier} of order $\mu \in \R$ (and type $1,0$) on the conic manifold $X \times \R^k \setminus \{0 \}$ by $S^\mu(X \times \R^k \setminus \{0 \})$. 
The H\"ormander space  of Lagrangian distributions of order $m\in \R$ over $\Lambda$  is denoted by $I^m (X ; \Lambda )$, and consists of locally finite sums $u=\sum_j u_j \in \mathcal{D}' (X)$ of oscillatory integrals
\[
u_j(x) = \int_{\R^{k_j}} e^{i\varphi_j (x, \xi) } a_j(x,\xi) d\xi , \quad x\in X.
\]
Here $a_j \in S^{m - k_j/2+ n/4} (X\times \R^{k_j}\setminus \{0\} )$. The phase function $\varphi_j$ is defined on an open cone $\Gamma_j\subset X\times \R^{k_j}$ and satisfies the following two conditions: (a) it is nondegenerate, $d\varphi_j\neq 0$ on $\Gamma_j$ and (b) the mapping % on an open cone $\Gamma_j\subset X\times \R^{k_j}$ satisfying the following: The mapping 
\[
\Gamma_j \rightarrow \Lambda, \ \  (x,\xi) \mapsto (x,d_x \varphi_j (x,\xi) ) 
\]
defines a diffeomorphism between the set $\{ (x,\xi) \in \Gamma_j : d_\xi \varphi_j (x,\xi)=0 \}$ and some open cone in $\Lambda$. 
%We also assume that $\chi a \in S^{-\infty} (X\times \R^k\setminus \{0\} )$ for any smooth cut-off function $\chi$ that vanishes on $\Gamma_j$. 
When the base manifold $X$ is clear, we abbreviate $I^m (\Lambda) = I^m (X ; \Lambda )$. %Elements of $I^m(\Lambda)$ for some Lagrangian manifold $\Lambda$ are referred to as \emph{Lagrangian distributions}.
%For example, $\varphi (x^1,x^2, \xi_1,\xi_2) = \varphi(x) \xi_1 $

\tjb{Below we let $X,Y,Z$ be $C^\infty$-smooth manifolds.  }% of dimension $n_X$ and $n_Y$ respectively. 
Let $\Lambda$ be a conic Lagrangian manifold in $T^*(X \times Y) \setminus \{0\}$.  
The manifold corresponds to a \tbl{canonical} relation $\Lambda'$ defined by
\begin{align}\label{relation_defn}
 \Lambda' = \{ (x,y  \;  \xi_x,\xi_y) \in T^*(X \times Y) :  (x,y \;  \xi_x,-\xi_y) \in \Lambda \}.
\end{align}
Equivalently, one may start with a canonical relation and obtain a Lagrangian manifold. In this paper we chose to represent canonical relations as twisted manifolds $\Lambda'$ of Lagrangian manifolds. 
%and  $G \in I^m (X \times Y ; \Lambda)$. We define 
%a Fourier integral 
%We define 
%an operator $F$ as %of order $m$ as
%\[
%F : C_c^\infty (Y, \Omega_{\frac{1}{2}}) \rightarrow \mathcal{D} (X, \Omega_{\frac{1}{2}})
%\]
Considering an element in $I^m (X \times Y ; \Lambda)$ as a Schwartz kernel defines an operator
\[
F : C_c^\infty (Y) \rightarrow \mathcal{D}' (X).%\qquad \langle \langle F ,\phi \rangle  , \psi \rangle = \langle G , \phi \otimes \psi  \rangle, 
\]
%\tbl{where $\psi\in C_c^\infty(X)$. 
%as a Schwartz kernel. 
%Here also $(\phi\otimes \psi)(y,x)=\phi(y)\psi(x)$ and we use the same notation for the tensor product of distributions (see e.g.~\cite{HormanderVol1}) over different spaces. Tensor product of distribution is defined
 %call $G$ the distribution kernel of $F$. 
%The manifold $\Lambda$ corresponds to a \tbl{canonical} relation $\Lambda'$ defined by
%\begin{align}\label{relation_defn}
% \Lambda' = \{ (x,y  \;  \xi_x,\xi_y) \in T^*(X \times Y) :  (x,y \;  \xi_x,-\xi_y) \in \Lambda \}.
%\end{align}
%We sometimes denote $\Lambda'$ by $C$.\footnote{\tbl{Why two labels? Remove this an explain when used.}} 
The class of operators of this form are called  Fourier integral operators of order $m \in \R $ associated with the relation $\Lambda'$. We denote this class of operators by % is denoted by
\[
I^m (X,Y ; \Lambda').
\]
We may also identify the space $ I^m (X ; \Lambda)$, $\Lambda \subset T^*X$, with \tbl{$I^m (X,\{0\}  ;  \Lambda \times \{ (0,0)\})$.}~\f{$\Lambda_0$ has another meaning later in the text.} % where $\Lambda' = \Lambda \times \{ (0,0)\}$. 
%Notice that canonical relations and Lagrangian manifolds in $X \times Y$ are in 

The wavefront set of $F$ is denoted by $WF'(F)$ and it is the set
\begin{align}
WF'(F)&=\{(x,\xi^x,y,\xi^y)\in (T^*X\times T^*Y)\setminus \{0\} \,:\, (x,y,\xi^x,-\xi^y)\in WF(G)\},\label{wf_set_fio}
\end{align}
where $WF(G)$ is the wavefront set of the distribution kernel  $G$ of $F$. We also define 
%the restricted wavefront sets of $F$ as 
\begin{align}
WF'_X(F)&= \{(x,\xi^x)\in (T^*X)\setminus \{0\} \,:\, (x,y,\xi^x,0)\in WF(G)\},\label{wf_set_fio_image}\\
%
WF'_Y(F)&= \{(y,\xi^y)\in (T^*Y)\setminus \{0\} \,:\, (x,y,0,\xi^y)\in WF(G)\}\label{wf_set_fio_domain}.
\end{align}




%for conic Lagrangian manifold $\Lambda \subset T^*X$.
\tjb{Consider two Fourier integral operators} \antti{ $u_1 \in I^{m_1} (X , Y ; \Lambda_1')$ and $u_2 \in I^{m_2} (Y , Z ; \Lambda_2')$ (i.e. Schwartz kernels in $  I^{m_1} (X \times  Y ; \Lambda_1)$ and $ I^{m_2} (Y \times  Z ; \Lambda_2)$, respectively)}
%\footnote{\antti{Removed ''Schwartz kernels''. Kernels are Lagrangian distributions on $X \times Y$. Not in the operator classes.}} 
with respective orders $m_1$ and $m_2$ and relations $\Lambda_1'$ and $\Lambda_2'$. Sufficient conditions for $u_1$ and $u_2$ to form a well defined composition $u_1\circ u_2 \in I^{m_1+m_2} (X,Z ; \Lambda_1' \circ \Lambda_2')$ are described in  \antti{theorems \cite[Theorem 2.4.1, Theorem 4.2.2]{duistermaat2010fourier} which provide the rules of basic microlocal operator calculus, often referred to as transversal intersection calculus.} 
%\antti{The operator calculus generated by the theorems is often referred to as transversal intersection calculus. }
 The relation $\Lambda_1' \circ \Lambda_2'$ is defined as % given by those elements $ (x,z \ ; \ \xi_x,\xi_z ) \in T^*( X \times Z)$ that satisfy 
\begin{align}\label{relation_of_composition}
\Lambda_1' \circ \Lambda_2':=\{ (x,z \, ; \, \xi^x,\xi^z ) &\in T^*( X \times Z): \nonumber\\
&(x,y \, ; \, \xi^x,\xi^y) \in \Lambda_1' , \ \ (y,z \, ; \, \xi^y,\xi^z) \in \Lambda_2' , \  \text{for some}  \ (y \, ; \, \xi^y) \in T^*Y \}.
\end{align}

Lastly, we remark that products of Lagrangian distributions are naturally defined as distributions over an interesting pair of conic Lagrangian manifolds $\Lambda_0,\Lambda_1 \in T^*X\setminus \{0\}$, \tjb{ which are described next. We refer to \cite{ES-thesis, guillemin1981, melrose-uhlmann1979, greenleaf_uhlmann1990, greenleaf-uhlmann} for a thorough presentation of such distributions.} 


\tjb{To begin, a pair $(\Lambda_0,\Lambda_1)$ of conic Lagrangian manifolds} $\Lambda_0,\Lambda_1 \in T^*X\setminus \{0\}$, \tjb{is called an intersecting pair if their} intersection is clean: $\Lambda_0\cap \Lambda_1$ is a smooth manifold and 
\begin{align*}
%&\Lambda_0\cap \Lambda_1\text{ is smooth}\\
T^*_\lambda(\Lambda_0\cap \Lambda_1) = T^*_\lambda\Lambda_0 \cap T^*_\lambda\Lambda_1 \text{ for all } \lambda\in \Lambda_0\cap\Lambda_1.
\end{align*}

\tjb{Let $(\Lambda_0,\Lambda_1)$ be an intersecting pair of conic Lagrangians with $\text{codim}(\Lambda_{0}\cap \Lambda_{1})=k$, and $\mu,\nu\in \R$. For $\ell \in \mathbb{Z}_{+}$, we denote by $S^{\mu,\nu}(X\times (\R^{\ell}\setminus\{0\})\times \R^{k})$ the space of symbol-valued symbols on $X\times (\R^{\ell}\setminus\{0\})\times \R^{k}$ (see \cite{ES-thesis,greenleaf_uhlmann1990}). We say that $u\in \mathcal{D}'(X)$ is a paired Lagrangian distribution of order $(\mu,\nu)$ associated to $(\Lambda_0,\Lambda_1)$ if $u$ can be expressed as a locally finite sum of the form}
\[
u= u_0 +u_1 + v,
\]
where $u_0\in I^{\mu+\nu}(\Lambda_0)$, $u_1\in I^{\nu}(\Lambda_1)$, and 
\[
v(x) = \int_{\R^{\ell}}\int_{\R^{k}} e^{i\varphi(x;\theta;\sigma)}a(x;\theta;\sigma)\,d\theta d\sigma
\]
for $a(x;\theta;\sigma)\in S^{\tilde\mu,\tilde\nu}(X\times (\R^{\ell}\setminus\{0\})\times \R^{k})$,  some $\ell\in \mathbb{Z}_+$, \tjb{$\mu = \tilde\mu + \tilde\nu + \frac{\ell+k}{2} - \frac{n}{4}$, and $\nu = -\tilde\nu - \frac{n}{2}$}\f{fixed tildes}. Above, the multiphase function $\varphi(x;\theta;\sigma)$ satisfies the following three conditions: for any $\lambda_{0} \in \Lambda_{0}\cap \Lambda_{1}$, (a) there is an open conic set $\Gamma \subset X\times (\R^{\ell}\setminus\{0\})\times \R^{k}$~\f{Brackets added.} such that $\varphi(x;\theta,\sigma) \in C^{\infty}(\Gamma)$, (b) $\varphi(x;\theta,0)$ is a phase function parametrizing $\Lambda_{0}$ in a conic neighbourhood of $\lambda_{0}$, and (c) $\varphi(x;0,\sigma)$ is a phase function parametrizing $\Lambda_{1}$ in a conic neighbourhood of $\lambda_{0}$. 
\antti{In particular,
\begin{align}
u\in I^{\mu,\nu}(\Lambda_0,\Lambda_1) \Longrightarrow WF(u)\subset \Lambda_0\cup\Lambda_1.
\end{align}
}
%\footnote{\antti{removed repetition and incorrect statements}}
\tjb{We denote the set of paired Lagrangian distributions of order $(\mu,\nu)$, $\mu,\nu\in \R$, associated to $(\Lambda_0,\Lambda_1)$ by $I^{\mu,\nu}(\Lambda_0,\Lambda_1)$.} 
%These distribution classes have the property that 
%\begin{align}
%u\in I^{\mu,\nu}(\Lambda_0,\Lambda_1) \Longrightarrow WF(u)\subset \Lambda_0\cup\Lambda_1,
%\end{align}
%and \antti{ for a conic $\Gamma \subset T^*X$ containing $\Lambda_0 \cap  \Lambda_1$, 
%%microlocally away from $\Lambda_0\cap \Lambda_1$,
%\begin{align}\label{lagrangian_pairs}
%& I^{\mu,\nu}(\Lambda_0,\Lambda_1)\subset I^{\mu+\nu}(\Lambda_0 ) +  I^{\mu}(\Lambda_1) + \mathcal{D}_{\Gamma}' (X)
%% \text{ microlocally away from }\Lambda_1,\text{ and}\\
%%&I^{\mu,\nu}(\Lambda_0,\Lambda_1) \subset I^{\mu}(\Lambda_1) \text{ microlocally away from }\Lambda_0.
%\end{align}
%}
%For more details, see~\cite{greenleaf-uhlmann,melrose-uhlmann1979,guillemin1981} and references therein.

% 
% 
% \subsection{$C^k$ function spaces}
% 
% We will also have need of the following function spaces of continuous functions.\footnote{\tbl{Is there a reference for this?}}
% 
% Let $\compp$ be a closed set in a smooth manifold $X$. 
% %or the set $[0,\infty) \times N$, and let $I\subset \R$ be an interval. 
% %Note that since $(\R\times N,g)$ is globally hyperbolic,  $J^+(\compp)$ is closed.
% %In the topology of $C^k ( J^+( \R \times N ) )$, 
% For integers $k\ge0$, we define 
% \[
% C_{\compp}^k ( X ) := \{ h \in C^k ( X )  :  \text{supp}(h) \subset \compp \}.
% \]
%where $\pi : T(\R \times N) \rightarrow \R \times N$, $\pi(x,p) := x$. 
%and
%\[
%C^{j,k}_{I,\compp}(J^+( \R \times N )) := \{ h:t\mapsto h(t)\in C_{\compp}^k ( J^+( \R\times N ) ): h(t)\in C^{j}(I) \}. %C^j (\R, C_{\compp }^k ( J^+( \R \times N ) ))
%\]
%and
%\[
%C_{+}^k ( J^+( \R \times N ) ) := \{ h \in C^k ( J^+( \R \times N ) )  : \text{supp}(h) \subset J^+( [0,\infty)\times N ) \}
%\]
%\end{definition}



%Define 
%$l(x,p)  \geq 0$ by  $\gamma_{(x,p)} (-l(x,p) ) \in \{0\} \times N$ (See Lemma \ref{app_lemma1}) for $(x,p) \in \OVS([0,\infty) \times N)$ and $l(x,p)=0$, for $(x,p) \in \OVS ((-\infty,0) \times N)$.












==> Sections/transversal-collision.tex <==
%
% Last edited: July 2, 2019
%
% This file contains the proof of transversal collisions
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Existence of transversal collisions}\label{travserse-collisions-section}

%\color{magenta}

In this section, we construct a particular submanifold $S$ of $TM$. %which performs three roles. % in our main proof.
%The flowout $K_S$ of the submanifold $S$ under the geodesic vector field will be used in Section \ref{approx_delta_dists} to define the microlocal support of a source of particles. 
In the proof of our main theorem, Theorem~\ref{themain}, we will construct particle sources in a common open set $V$ of two manifolds $M=M_l$,  $l=1,2$ such that they send information into the unknown region $W_l \subset M_l$ to create point singularities produced by using the nonlinearity. We use the source-to-solution map to study the propagation of that singularity.
The idea is that for two time-like future pointing vectors with distinct base-points in $V$ we build a manifold $S$ around one of the vectors such that the flowouts $Y_1= Y_{1,M_l,g_l} := K_{S;M_l,g_l} $ and $Y_2=Y_{2,M_l,g_l} :=K_{\{(x,p)\} ; M_l,g_l}$ of $S$ and the other vector $(x,p)$ will satisfy the admissible intersection property (Definition~\ref{intersection_coords}) in  $ \pi \text{supp}A_l \supset W_l $ in both $M_l$ simultaneuously. 
Here $A_l$ is an admissible collision kernel. 
The Corollary \ref{lemma_renerew} below states that such a manifold $S$ exists.  
Consequently, %about the intersection of conditions in 
Corollary \ref{sofisti_further} will be applicable in both manifolds for sources conormal to $S_1 = S$ and $S_2 = \{x,p\}$. 
%That is, the collision operator for two particle sources with their microlocal support on $Y_1$ and on a given time-like geodesic arc $Y_2$ will be well-defined in both $M_l$ simultaneously. 
%\tbl{In the inverse problem, we consider $K_S$ related to a geodesic $\gamma$ and another geodesic. In the next lemma, the points $z_{l,j}$ correspond to the intersection points of the projection of $K_S$ and the other geodesic. The vectors $V_k$ correspond to the tangent vectors of the other geodesic at the points $x_k$.}


 \begin{figure}
 \includegraphics[width=0.4\textwidth]{intersection}
 \caption{An admissible intersection of $K_{S}$ and a single geodesic path $K_{(x,p)}$. The initial vector $(x,p)$ and the manifold $S$ are indicated in red and blue, respectively. Near the intersection point $G_S$ behaves as a manifold transversal to $\gamma_{(x,p)}$.}
 \end{figure}

Below $\SP \mathcal{C}\subset TM$ stands for set of future directed time-like vectors with base points in given Cauchy surface $\mathcal{C}$. 

\begin{lemma}\label{lemma_renerew}
Let $(M_l,g_l)$, $l=1,2$ be two globally hyperbolic manifolds containing open sets $V_l \subset M_l$ and assume that there is a diffeomorphism $\Psi : V_1 \rightarrow V_2$ such that $g_1|_{V_1} = \Psi^* g_2$. 
For $l=1,2$ consider $(x_l,p_l) \in \mathcal{P}^+ V_l$ with $(x_2,p_2) = D\Psi (x_1,p_1)$. Let $\{ (z_{l,j},v_{l,j}) : j \in J_l \}$ $($possibly $J_l  = \emptyset)$ be a countable  family of vectors in 
\[
\big\{ (z,v) \in  \mathcal{P}^+M_l  \ \big| \  \exists t \ : \ z= \gamma_{(x_l,p_l)} (t) , \   v \in   \mathcal{P}^+_z M_l  \setminus \text{span}\{ \dot\gamma_{(x_l,p_l)}(t) \} \big\} . 
\]
Let $\mathcal{C}$ be a space-like Cauchy surface through $x_l$ in one of the manifolds $M_l$, $l=1,2$ and copy its restriction $\mathcal{C}_l := \mathcal{C} \cap V_l$ to the other by setting $\mathcal{C}_2 = \Psi \mathcal{C}_1$. 
Then there exist $(2n-2)$-dimensional submanifolds $S_l \subset \mathcal{P}^+  \mathcal{C}_l$, $l=1,2$  
such that $(x_l,p_l) \in S_l$, $S_2 = D\Psi S_1$ and the following two conditions hold for every $j\in J_l$:
\begin{enumerate}[(i)]
%\item $(x_l,p_l) \in S_l$, 
%\item $S_2 = D\Psi S_1$,
\item The point $z_{l,j}$ has an open neighbourhood $U_{l,j} \subset M_l$ such that the intersection $U_{l,j} \cap G_{S_l}$, where $G_{S_l} := \pi K_{S_l}$, is a $(n-1)$-dimensional submanifold of $M_l$. 
\item
$ v_{l,j} \notin  T_{z_{l,j}}G_{S_l}  $.
\end{enumerate}
%Moreover, we can fix $S_l$, $l=1,2$ above such that for any space-like Cauchy surface $\mathcal{C}$ through $x_1$ $($resp. $x_2)$ the  $S_1$ $($resp. $S_2)$ lies in $\mathcal{P}^+  \mathcal{C} $. 
\end{lemma}

%The lemma above implies the following corollary:

\begin{corollary}\label{coro_renerew}
Let $(M_l,g_l)$, $l=1,2$ be globally hyperbolic manifolds with a mutual open set $ V  \subset M_l$,
$l=1,2$ and assume that $g_1|_V = g_2|_V$. Consider $(x,p),(y,q)  \in \mathcal{P}^+ V$ with distinct base points $x\neq y$.  Assume that the geodesics $\gamma_l$ and $\tilde\gamma_l$ in $M_l$, defined by 
%Then, for a pair $\gamma_l $, $\tilde\gamma_l$ of time-like future-directed geodesics distinguishable as paths (on their maximal domains) and entangled in $V$ via the initial values 
\begin{align}
&  (\gamma_2(0) ,\dot\gamma_2(0) ) =   (\gamma_1(0) ,\dot\gamma_1(0) )=(x,p) , \\
 %\\
%(\hat{y}_l,\hat{q}_l):= (\tilde\gamma_l(0) ,\dot{\tilde\gamma}_l(0) ) \in \mathcal{P}^+V_l, \quad (\hat{y}_2,\hat{q}_2) = D\Psi (\hat{y}_1,\hat{q}_1) 
%\\
&(\tilde\gamma_2(0) ,\dot{\tilde\gamma}_2(0) ) = (\tilde\gamma_1(0) ,\dot{\tilde\gamma}_1(0) ) =(y,q) , 
% \quad 
%y \neq x, 
\end{align} 
are distinguishable as paths (on their maximal domains), that is, $(x,p)$ and $(y,q)$ are not tangent to the same geodesic. Let $\mathcal{C}$ be a space-like Cauchy surface through $x$ $($resp. $y)$ in one of the manifolds $M_l$ and let $X_l \subset M_l$ be compact. $($e.g. $X_l = \pi \text{supp} A_l$ for admissible collision kernels $A_l$,   $l=1,2)$
%\footnote{Sets $W_l$
%are added as well as intersections of $K_S$ with $TW_l$ on  Sep. 6, 2021- Matti. 
%This is done as we may have infinitely many intersection points on $M_l$ and to get transversal intersection of $K_S$ and $K_{(x,p)}$ we may have to make $S$ ``smaller'' in every intersection point.
%Antti, could you please check if you agree with this change?}  
%$X_l\subset M_l$ be relatively compact sets, $l=1,2$. 
Then, there is a $(2n-2)$-dimensional
%\footnote{Dimension of $S$ is added on  Sep. 6, 2021- Matti} 
submanifold $S \subset \mathcal{P}^+ ( \mathcal{C} \cap V)$ containing $(x,p) $ $(\text{resp. }(y,q) )$ such that 
% $ K_S = K_{S;M_l,g_l}$, $l=1,2$ 
%satisfy that 
the pair consisting of the flowouts $K_S = K_{S;M_l,g_l}$ and $K_{(y,q)}= K_{\{ (y,q)\};M_l,g_l}$ $($resp.  $K_{(x,p)} = K_{\{(x,p)\};M_l,g_l})$ have admissible intersection property in $X_l$ for both $l=1,2$. 
%of the curve $(\tilde\gamma_l, \dot{\tilde\gamma}_l)$ $(\text{resp. } (\gamma_l ,\dot\gamma_l ) )$. 
%Moreover, if $\mathcal{C} \subset V$ is a restriction of a space-like Cauchy surface through $x$ in either $M_l$, $j=1,2$, we can choose $S$ such that $S \subset \mathcal{P}^+  \mathcal{C}$. 
 \end{corollary} 
 
 
 
 \begin{proof}[Proof of Lemma \ref{lemma_renerew}]
%Let us first omit the index $l=1,2$. 
%Let $C$ be a Cauchy surface through $x_1$ in $M_1$ and define $ \mathcal{C}_l \subset V_l$, $l=1,2$ by $\mathcal{C}_1 := C \cap V_1$ and $\mathcal{C}_2 :=\Psi (C \cap V_1) $.  
 Since $M_l$ is globally hyperbolic, the space $\mathcal{P}^+M_l$  can locally near the curve $(\gamma_{x_l,p_l}, \dot\gamma_{x_l,p_l})$ be written  as the product $\mathcal{P}^+\mathcal{C}_l   \times \R$ by identifying $(x,p,t)  $ with $ ( \gamma_{(x,p)}(t), \dot\gamma_{(x,p) }(t) )$. 
 %It suffices to construct suitable  $S_l$ in the initial vector manifold $ \mathcal{P}^+\mathcal{C}_l$. 
 Denote by $\phi_l $ be the projection from the neighbourhood of $(\gamma_{x_l,p_l}, \dot\gamma_{x_l,p_l})$ to $ \mathcal{P}^+\mathcal{C}_l$ that in terms of the identification above equals the cartesian projection $(x,p,t) \mapsto (x,p) $. 
 That is; $\phi_l$ takes each $(x,p)$ in the neighbourhood into the unique intersection of $(\gamma_{(x,p)}, \dot\gamma_{(x,p)})$ and $\mathcal{P}^+\mathcal{C}_l $. Let 
 $\phi_l(x,p)=(z_{l,j},p_{l,j})\in \mathcal{P}^+\mathcal{C}_l$, 
 that is,
 $p_{l,j}$ stand for the velocity $\dot\gamma_{x_l,p_l}$ at $z_{l,j}$. We define 
  $L_{j,l} \subset T_{z_{l,j} } M_l $ to be the 2-plane spanned by $ p_{l,j} $ and $ v_{l,j}$.  Let $\pi :  \mathcal{P}^+M \to M$ be the canonical projection. 
We see that the linear space
 \[
 E_{l,j} :=  D_{(z_{l,j},p_{l,j})}  \phi_l  (  D_{(z_{l,j},p_{l,j})} \pi )^{-1}  L_{l,j}   \subset T_{(x_l,p_l)} \mathcal{P}^+\mathcal{C}_l , 
  \]
   is $(n+1)$-dimensional. There are only countable many of such manifolds so 
 there is a small submanifold $S_1 \subset  \mathcal{P}^+\mathcal{C}_1 $ through $(x_1,p_1)$ of dimension $\dim T_{(x_1,p_1)} \mathcal{P}^+\mathcal{C}_1 - (n+1) = n-2$ such that each of the spaces $ E_{1,j}$, $j\in J_1$ and $D\Psi^{-1}   E_{2,j}$, $j\in J_2$ intersect $T_{x_1,p_1} S_1$ transversally. By considering the dimension of these linear spaces, we observe that the intersection occurs only at the origin.  
  This implies the analogous condition also for $S_2 := D\Psi S_1$.
   It is straightforward to check that
   \[
   \text{ker} ( D_{(z_{l,j}, p_{l,j})} \pi )  \cap T_{(z_{l,j}, p_{l,j})} K_{S_l} = \{ 0 \} 
   \]
which ensures that $D_{(z_{l,j}, p_{l,j})} \pi $ defines an isomorphism from $T_{(z_{l,j}, p_{l,j})} K_{S_l}$ to its image. This implies that $G_{S_l} = \pi  K_{S_l}$ near $(z_{l,j}, p_{l,j})$ is a manifold of dimension $\dim K_{S_l} =\dim S_l +1 = n-1$. 
Let us deduce the condition $ v_{l,j} \notin  T_{z_{l,j}}G_{S_l}  = \emptyset$.  
By the construction above, 
\[
T_{(x_l,p_l)} S_l \cap   E_{l,j}= \{0\}.
\]
Hence, 
\[
  ( D_{(z_{l,j},p_{l,j})} \phi_l )^{-1} (  T_{(x_l,p_l)} S_l \  \cap \     E_{l,j}  )\subset     \text{ker} ( D_{(z_{l,j},p_{l,j})} \phi_l )  .
\]
We check that
\[
 ( D_{(z_{l,j},p_{l,j})} \phi_l )^{-1} (  T_{(x_l,p_l)} S_l )= T_{(z_{l,j},p_{l,j})} K_{S_l}
 \]
  and 
  \[
   ( D_{(z_{l,j},p_{l,j})} \phi_l )^{-1}  E_{l,j}  =  (D_{(z_{l,j},p_{l,j})} \pi)^{-1}  L_{l,j}.
   \] 
By substitution we conclude 
%\footnote{Antti, please add details in \eqref{a numbered formula}.}
\begin{equation}\label{a numbered formula}
T_{(z_{l,j},p_{l,j})} K_{S_l}  \ \cap \   (D_{(z_{l,j},p_{l,j})} \pi)^{-1}  L_{l,j}  \subset   \text{ker} ( D_{(z_{l,j},p_{l,j})} \phi_l ). 
\end{equation}
Applying $D_{(z_{l,j},p_{l,j})} \pi$ gives 
\[
T_{z_{l,j}} G_{S_l}  \ \cap \    L_{l,j}  \subset  D_{(z_{l,j},p_{l,j})} \pi  (  \text{ker} ( D_{(z_{l,j},p_{l,j})} \phi_l ) )  =  \R p_{l,j}
\] 
which implies $v_{l,j} \notin  T_{z_{l,j}} G_{S_l} $ by the definition of $ L_{l,j}$.  


 \end{proof}

\color{black}


%\begin{figure}
%\begin{tikzpicture}
%
%\pgfplotsset
%{
%colormap
%={Anders}{rgb255(0cm)=(180,180,180); rgb255(1cm)=(255,255,255)}
%}
%
%  \begin{axis}[
%  width=0.8\textwidth,
%    hide axis,
%    view = {0}{40}
%  ]
%  \addplot3 [
%    surf,
%    %mesh,
%    %colormap/blackwhite,
%    %shader     = faceted interp,
%    point meta = x,
%    samples    = 40,
%    samples y  = 5,
%    z buffer   = sort,
%    domain     = 0:360,
%    y domain   =-50:50
%  ] (
%    {x +y*cos(x)},
%    {x},
%    {x }
%  );
%
%
%%THE RAYS:
%
%
%  \addplot3 [
%  	black,
%    samples=50,
%    domain=0:360, %
%                     %
%    samples y=0,
%    thick
%  ] (
%    {x},
%    {x},
%    {x}
%  );
%  
%    \addplot3 [
%  	black,
%    samples=50,
%    domain=0:360, %
%                     %
%    samples y=0,
%   % thick
%   dashed
%  ] (
%    {x + 25*cos(x)},
%    {x},
%    {x}
%  );
%  
%      \addplot3 [
%  	black,
%    samples=50,
%    domain=0:360, %
%                     %
%    samples y=0,
%   % thick
%   dashed,
%  ] (
%    {x + 50*cos(x)},
%    {x},
%    {x}
%  );
%  
%          \addplot3 [
%  	black,
%    samples=50,
%    domain=0:360, %
%                     %
%    samples y=0,
%  %  thick
%  dashed
%  ] (
%    {x - 25*cos(x)},
%    {x},
%    {x}
%  );
%  
%        \addplot3 [
%  	black,
%    samples=50,
%    domain=0:360, %%,
%                     % %
%    samples y=0,
%  %  thick
%  dashed
%  ] (
%    {x - 50*cos(x)},
%    {x},
%    {x}
%  );
% 
% 
% %THE Vs :
% 
%
% \draw [->,black,thick] (180,80,180) -- (120,200,200);
% \draw [->,black,thick] (250,200,200) -- (200,300,200);
%  \draw [->,black,thick] (350,300,300) -- (330,300,400);
%  
%  %THE Js
%    \draw [->,black,thick] (50,0,0) -- (120,0,0);
%      \draw [->,black,thick] (180,80,180) -- (230,80,180);
%          \draw [->,black,thick] (250,200,200) -- (310,200,200);
%            \draw [->,black,thick] (350,300,300) -- (380,300,300);
% 
% 
% 
% 
% %THE MANIFOLD S:
% 
%%  \draw [-,black,thick] (0,0,0) -- (100,0,0); %horisontal line
%   % \draw [-,black,dashed] (100,0,0) -- (300,0,0); %horisontal line
% %   \draw [->,black,thick] (0,0,0) -- (25,25,25);
%    %    \draw [->,black,thick] (25,0,0) -- (50,25,25);
%          \draw [->,thick] (50,0,0) -- (100,50,50);
%                 %   \draw [->,black,thick] (75,0,0) -- (100,25,25);
%                       %       \draw [->,black,thick] (100,0,0) -- (125,25,25);
%                              
%                              
%                              
%                              
%                              %TEXTS:
%                              \node at (110,200,140) {$V_1$};
%                               \node at (180,300,180) {$V_2$};
%                                 \node at (310,300,400) {$V_3$};
%                                 \node at (160,0,0) {$J_1(0)$};
%                                  \node at (270,80,180) {$J_1(t_1)$};
%                                   \node at (350,200,200) {$J_1(t_2)$};
%                                     \node at (420,300,300) {$J_1(t_3)$};
% 
%  \end{axis}
%\end{tikzpicture}
%\caption{A geodesic variation of $\gamma$ in the direction defined by the Jacobi field $J_1$. The vectors $V_1,V_2$, and $V_3$ are transversal to $J_1$ and their base points are located in regions where the field, and hence the surface drawn by the variation (in gray) is not degenerated. {\color{red}(This is a tikz picture so you can modify it directly in the .tex file if you are not satisfied. See the picture in colors below. I wasn't sure whether you want it B\&W or in colors. Traceys pics seem to be B\&W. --Antti)}}
%%\end{figure}

%\begin{comment}
%\begin{figure}
%\begin{tikzpicture}
%
%%%%Custom colormap:
%\pgfplotsset
%{
%colormap
%={Anders2}{rgb255(0cm)=(180,180,180); rgb255(1cm)=(255,255,255)}
%}
%
%
%%%%The surface:
%  \begin{axis}[
%  width=0.8\textwidth,
%    hide axis,
%    view = {0}{40}
%  ]
%  \addplot3 [
%    surf,
%    %colormap/Anders,
%    shader     = faceted interp,
%    point meta = x,
%    samples    = 40,
%    samples y  = 5,
%    z buffer   = sort,
%    domain     = 0:360,
%    y domain   =-50:50
%  ] (
%    {x +y*cos(x)},
%    {x},
%    {x }
%  );
%
%
%%%%THE RAYS:
%
%
%  \addplot3 [
%  	red,
%    samples=50,
%    domain=0:360, %
%                     %
%    samples y=0,
%    thick
%  ] (
%    {x},
%    {x},
%    {x}
%  );
%  
%    \addplot3 [
%  	black,
%    samples=50,
%    domain=0:360, %
%                     %
%    samples y=0,
%   % thick
%   dashed
%  ] (
%    {x + 25*cos(x)},
%    {x},
%    {x}
%  );
%  
%      \addplot3 [
%  	black,
%    samples=50,
%    domain=0:360, %
%                     %
%    samples y=0,
%   % thick
%   dashed,
%  ] (
%    {x + 50*cos(x)},
%    {x},
%    {x}
%  );
%  
%          \addplot3 [
%  	black,
%    samples=50,
%    domain=0:360, %
%                     %
%    samples y=0,
%  %  thick
%  dashed
%  ] (
%    {x - 25*cos(x)},
%    {x},
%    {x}
%  );
%  
%        \addplot3 [
%  	black,
%    samples=50,
%    domain=0:360, %%,
%                     % %
%    samples y=0,
%  %  thick
%  dashed
%  ] (
%    {x - 50*cos(x)},
%    {x},
%    {x}
%  );
% 
% 
% %%%THE Vs :
% 
%
% \draw [->,blue,thick] (180,80,180) -- (120,200,200);
% \draw [->,blue,thick] (250,200,200) -- (200,300,200);
%  \draw [->,blue,thick] (350,300,300) -- (330,300,400);
%  
%  %%%THE Js
%    \draw [->,black,thick] (50,0,0) -- (120,0,0);
%      \draw [->,black,thick] (180,80,180) -- (230,80,180);
%          \draw [->,black,thick] (250,200,200) -- (310,200,200);
%            \draw [->,black,thick] (350,300,300) -- (380,300,300);
% 
% 
% 
% 
% %THE MANIFOLD S:
% 
%%  \draw [-,black,thick] (0,0,0) -- (100,0,0); %horisontal line
%   % \draw [-,black,dashed] (100,0,0) -- (300,0,0); %horisontal line
% %   \draw [->,black,thick] (0,0,0) -- (25,25,25);
%    %    \draw [->,black,thick] (25,0,0) -- (50,25,25);
%    
%    
%          \draw [->,thick, red] (50,0,0) -- (100,50,50);
%          
%          
%                 %   \draw [->,black,thick] (75,0,0) -- (100,25,25);
%                       %       \draw [->,black,thick] (100,0,0) -- (125,25,25);
%                              
%                              
%                              
%                              
%                              %TEXTS:
%                              \node[blue] at (110,200,140) {$V_1$};
%                               \node[blue] at (180,300,180) {$V_2$};
%                                 \node[blue] at (310,300,400) {$V_3$};
%                                 \node at (160,0,0) {$J_1(0)$};
%                                  \node at (270,80,180) {$J_1(t_1)$};
%                                   \node at (350,200,200) {$J_1(t_2)$};
%                                     \node at (420,300,300) {$J_1(t_3)$};
% 
%  \end{axis}
%\end{tikzpicture}
%\caption{A geodesic variation of $\gamma$ in the direction defined by the Jacobi field $J_1$. The vectors $V_1,V_2$, and $V_3$ are transversal to $J_1$ and their base points are located in regions where the field, and hence the surface drawn by the variation (in gray) is not degenerated.}
%
%\end{figure}
%\end{comment}
%
%
%\begin{lemma}[]\label{manifold_jacobi_const}
%Let $(M, g)$ be a $C^\infty$-smooth globally hyperbolic geodesically complete Lorentzian manifold with a Cauchy surface $\mathcal{C}\subset M$. 
%Let $r>0$, $x_0\in \mathcal{C}$, and let $p_0\in P^r_{x_0}M$. % be a future-directed vector. 
%Let $T>0$ and let $\gamma: [0,T] \to M$ to be the timelike geodesic with the initial data  $(\gamma(0),\dot{\gamma}(0)) = (x_0, p_0)$.
%
%Let $K\in \N$ and choose 
%\begin{itemize}
%\item $K+1$ locations along $\gamma$, denoted by $x_k:= \gamma(t_k)$, with $0=t_0<t_1<\dots < t_K<T$.
%\item $K+1$ causal vectors $0\neq V_k\in T_{x_k}M$, $k\in\{0,1,\dots, K\}$, with the property that $V_k$ is not parallel to $\dot{\gamma}(t_k)$.
%%\[ z_k:= \gamma(t_k), \text{ with } t_0<t_1<\dots < t_K<T. \]
%\end{itemize}
%%Choose $0=t_0<t_1<\dots < t_{\tilde{K}}<T$ be given; write $z_k:= \gamma(t_k)$.\\
%%Suppose we are given vectors $V_k\in T_{z_k}M$ with the property that for each $k\in\{0,1,\dots, \tilde{K}\}$, $V_k$ is not a multiple of $\dot{\gamma}(t_k)$. 
%
%Then, there exist $n-2$ Jacobi fields $J_1,\dots, J_{n-2}$ along $\gamma$ such that the vectors
%\begin{equation}\label{lin_indep_J}
% V_k, \,\dot{\gamma}(t_k),\, J_1(t_k),\ldots, J_{n-2}(t_k)
%\end{equation}
%span $T_{x_k}M$ for each $k\in\{0,1,2,\dots,K\}$.
%% which satisfy %such that  
%%  \begin{equation}\label{lin_indep_J}
%%  V_k \wedge\dot{\gamma}(t_k)\wedge J_1(t_k)\wedge\cdots J_{n-2}(t_k)\neq 0
%%  \end{equation}
% 
%%  , and % and the vectors $\dot{J}_1(0), \dots, \dot{J}_{n-2}(0)$ are transversal to the hypersurface $\{t_0\}\times N$.
%%  %\tbl{
%%  \begin{equation}\label{Js_tangent}
%%  J_{1}(0),\dots,J_{n-2}(0)\in T_{x_0}M.
%%  \end{equation}
% %}
% %(Here $T(\{t_{0}\}\times N)$ is the $n-1$ dimensional tangent space of $\{t_{0}\}\times N$.)
% %}
% 
%% % % % %  Moreover, there exists a submanifold $S$ of $T\mathcal{C}\cap P^rM\subset TM$ such that $(x_0,p_0)\in S$ and that the projection of the geodesics flowout $G_S$ of $S$ has the following property: If $k=0,\ldots, K$, then on a neighbourhood of $\gamma(t_k)$ the  projection of $G_S$ is a submanifold of $M$ of dimension $n-1$ which is transversal to $V_k$.
%%  
%%  $\eps>0$ and smooth maps $\alpha:(-\epsilon,\epsilon)^{n-2}\to \{t_{0}\}\times N $ and $W: (-\epsilon,\epsilon)^{n-2}\to TM$ with $W(s)\in P_{\alpha(s)}^r$%}
%% %  \[
%% %  \alpha :s\in (-\epsilon,\epsilon)^{n-2}\mapsto exp_{t_0;x_0}\left(\sum_{i=1}^{n-2}s^iJ_i(0)\right)\ \ \text{and }\ \ W:s\in (-\epsilon,\epsilon)^{n-2}\mapsto W(s)\in \PP^r_{t_0}
%% %  \]
%% %}
%% such that the set~\footnote{\tbl{The current notation is that $P^r_{t_0}$ is used instead of $\PP^r_{t_0}$.}}
%%   \[
%%   S =\left\{s\in (-\epsilon,\epsilon)^{n-2}: \left(\alpha(s),W(s)\right)\in \tbl{P^r_{t_0}}\right\}
%%  \]
%% is a submanifold of $P^r_{t_0}$ of dimension $n-2$. %; here $\exp_{t_0;x_0}$ is the exponential map defined on an open neighbourhood of $T_{x_0}(\{t_0\}\times N)$.
%% }
%% %  \[
%% %  S =\left\{s\in (-\epsilon,\epsilon)^{n-2}: \left(\exp_{t_0;x_0}\left(\sum_{i=1}^{n-2}s^iJ_i(0)\right),T(s)\right)\in \PP^r_{t_0}\right\}
%% % \]
%% %is a submanifold of $\PP^r_{t_0}$ of dimension $n-2$; here $s=(s^1,\dots,s^{n-2})$ are local coordinates, $\exp_{t_0;x_0}$ is the exponential map defined on an open neighbourhood of $T_{x_0}(\{t_0\}\times N)$, and $T(s)\in \PP^r_{t_0}$ is a vector field depending on $J_1,\dots, J_{n-2}$.
%% %$i=1,\dots,n-2$ are vector fields along $\exp_{t_0;x_0}$ each satisfying $\frac{d}{ds}W_i(s^i)|_{s^i=0} = \frac{d}{dt}J_i(t)|_{t=0}$ ($i$ not summed).
%
%%$W_i(s^i) \in TM$, $i=1,\dots,n-2$ are vector fields along $\exp_{x_0}\left(s^iJ_i(0)\right)$ ($i$ not summed), each satisfying $\frac{d}{ds}W_i(s^i)|_{s^i=0} = \dot{J}_i(0)$.
%% 
%% Additionally, the geodesic flowout $G_S\subset M$ of $S$ is a subset of $M$ which is a submanifold of $M$ on a neighbourhood of each $\gamma(t_k)$, $k=0,\ldots, K$, of dimension $n-1$.
% \end{lemma}
%
%
%\begin{proof}
%%Without loss of generality, we may assume that $t_0=0$.
%%First we define some auxiliary vector fields and curves. Let $\{E_i\}_{i\in\{1,\dots, n-2\}}$, be a collection of vector fields along $\gamma$ which satisfy
%% \[ g(E_i(t),E_j(t))=\delta_{ij}, \text{ and  } g(E_i(t),\dot{\gamma}(t))=0\]
%% for all $t\in [t_0,T]$.
% 
% %For every $i\in\{1,\dots, n-2\}$ and every $k\in\{0,1,2,\dots,K\}$, set $\alpha_{i,k}: [0,1]\to M $ to be a smooth curve satisfying
% %\[ \alpha_{i,k}(t_k)= \gamma(t_k), \ \ \dot{\alpha}_{i,k}(t_k) = E_i.\]
% Let $\{E_l\}_{l=1}^{n-2}\subset  T_{x_0}M$ be vectors such that for $j,l=1,\ldots, n-2$ we have
% % the tangent vectors at $\gamma(0)=x_0$ which satisfy
% \begin{equation}\label{initial_vectors} 
% g(E_l,E_j)=\delta_{lj}, \quad g(V_0,E_l)=0  \quad \text{and} \quad g(E_l,\dot{\gamma}(0))=0.
% \end{equation}
%
% 
%Let $J_l: \R\to TM$, $l=1,\dots,n-2$, be the Jacobi fields along $\gamma$ with the initial data
% \begin{align*}
%% &\ddot{J_i}+ R\left(\dot{\gamma}, J_i\right)\dot{\gamma} = 0\\
% & J_l(0)=E_l(0) \text{ and } \dot{J}_l(0)= 0,%\dot{\gamma}(0).
% \end{align*}
% where $\dot{J}_l(0):=\nabla_{\partial_t}J_l(0)$ is the covariant derivative along the geodesic $\gamma$.
% %for some choice of $a_i, b_i\in (0,\epsilonilon_{0})$. %$a_i, b_i\in \mathbb{R}\setminus\{0\}$. 
%%  The variation through geodesics of $\gamma$ induced by $J_i$ is the 1-parameter family of curves
%%  \[ \gamma_i(s,t) := \exp_{\alpha_{{i}}(s)}\left(t W_{i}(s)\right) \]
%%  where $\exp_{\alpha_{i}(s)}$ is the exponential map defined on an open set of $T_{\alpha_{i}(s)}M$, and \[ \alpha_{i}(s):= \exp_{0;x_0}\left( sJ_{i}(0) \right), \]
%%  where $\exp_{0; x_0}$ is the exponential map defined on an open set of $T_{x_0}(\{0\}\times N)$,
%%  %$\alpha_i(s)$, $s\in [0,2\epsilonilon_0)$ is a smooth curve satisfying
%%  %\[ \alpha_{i}(0)= \gamma(0), \ \ \dot{\alpha}_{i}(0) = a_iE_i\]
%%  $W_{i}(s)$ is the parallel transport of the vector $\dot{\gamma}(0)+s\dot{J}_i(0)$ along $\alpha_i(s)$, and $s\in [0,2\epsilon_{0})$.
% We show that we may perturb the Jacobi fields $J_l$ so that the  vectors 
% %\begin{equation}\label{lin_indep_J}
% \[
% V_k, \,\dot{\gamma}(t_k),\, J_1(t_k),\ldots, J_{n-2}(t_k)
%\]
% %\end{equation}
% %in~\eqref{lin_indep_J} 
% span $T_{x_k}M$ for all $k=0,\ldots, K$. % is by recursion on the index $k$. 
% This is shown by using a recursion argument. When $k=0$, this is true by~\eqref{initial_vectors}. 
%%that 
%%  \[
%%   V_0\wedge\dot{\gamma}(0)\wedge J_1(0)\wedge\cdots \wedge J_{n-2}(0)\ne 0.
%%  \]
%% Thus~\eqref{lin_indep_J} holds for $k=0$.  
% 
% Assume next that we have found $n-2$ Jacobi fields so that the vectors in~\eqref{lin_indep_J} span $T_{x_k}M$ for all $k<K^*$. If at the time $t_{K^*}$ we have that $V_{K^*},\, \dot{\gamma}(t_{K^*}),\, J_1(t_{K^*}),\ldots, J_{n-2}(t_{K^*})$ are linearly dependent, that is $V_{K^*}\wedge \dot{\gamma}(t_{K^*})\wedge J_1(t_{K^*})\wedge\cdots \wedge J_{n-2}(t_{K^*})= 0$, we proceed as follows. For $k=0,\ldots, K^*-1$, we have by the assumption that
% \begin{equation}\label{deltak}
%  \delta=\min_{k=0,\ldots,K^*-1}\left|\left| V_k\wedge \dot{\gamma}(t_k)\wedge J_1(t_{k})\wedge\cdots \wedge J_{n-2}(t_{k})\right|\right|>0.
% \end{equation}
% Here the norm is with respect to some auxiliary Riemannian metric.
%%\delta_k := \left|\left| V_k\wedge \dot{\gamma}(t_k)\wedge J_1(t_{k})\wedge\cdots \wedge J_{n-2}(t_{k})\right|\right|_{g}^{\frac1n}>0$, for $k=0,\ldots,K^*-1$, 
%%Define $\delta=\min_{k=0,\ldots,K^*-1}\delta_k>0$. 
%Let $R\ge2$ be the largest integer $\leq n-2$ such that after possibly relabeling of the Jacobi fields $J_l$ we have that
%%  , up to relabeling of the vectors, when $R=2$ all $J_{l}(t_{K^*})$ for $l=1,\dots,n-2$ are parallel to $V_{K^*}$ or $\dot{\gamma}(t_{K^*})$, when $R=3$ we have
%% \[ 
%% V_{K^*}\wedge \dot{\gamma}(t_{K^*})\wedge J_{1}(t_{K^*})\ne 0,
%% \]
%% and when $R>3$ 
% \[ 
% V_{K^*}\wedge \dot{\gamma}(t_{K^*})\wedge J_1(t_{K^*})\wedge\cdots \wedge J_{R-2}(t_{K^*})\ne 0.
% \]
% 
% We proceed by using a perturbation argument. Let us define a matrix 
% \[
%  A:= [ V_{K^*}\,  \gamma(t_{K^*})\,  J_1(t_{K^*})\, \cdots\,  J_{n-2}(t_{K^*})]
% \]
% in columnar form. Let us choose tangent vectors $\{e_1,\dots, e_{n-2}\}\in T_{x_{K^*}}M$ such that the set  $\{V_{K^*}, \gamma(t_{K^*}), e_1, \dots, e_{n-2}\}$ of vectors form a basis for $T_{x_{K^*}}M$. By using this basis, the matrix $A$ becomes
% \[ 
% A= \begin{pmatrix}
%        I_{2\times 2} & A_0\\
%        0 & A_1
%        \end{pmatrix}.
% \]
% 
%\tbl{Next, we will perturb} $A_1$ slightly so that after the pertubation the determinant of $A_1$ is nonzero. Note that
% $\det(A)=\det(A_1)$. %Consider the matrix $A_1$, and let $\epsilon>0$. 
% By using the singular value decomposition of matrices we may find invertible matrices $P$ and $Q$ such that 
% \[
%PA_1Q:= \begin{pmatrix}
%        I_{(R-2)\times (R-2)} & 0\\
%        0 & 0
%        \end{pmatrix}.
% \]
% We choose a perturbation of $A_1$ of the form 
% \[
% A_1(h) :=  P^{-1}\begin{pmatrix}
%       I_{(R-2)\times (R-2)} & 0\\
%        0 & h\s I_{(n-R+2)\times (n-R+2)}
%        \end{pmatrix} Q^{-1},
%        \]
%        where $h>0$ is a small number. This induces a perturbation of $A$ of the form
% \[
% A(h) :=  \begin{pmatrix}
%         I_{2\times 2} & A_0\\
%        0 & A_1(h)
%        \end{pmatrix}.
%        \]        
%%By continuity of the matrix multiplication, 
%We have that $A(h)$ converges to $A$ in the space of matrices as $h\to 0$. 
%
%Denote by ${J}_l^h$ the $l^{\textrm{th}}$ column of $A(h)$. We therefore have for all $h>0$ that
% \[
%  V_{K^*}\wedge\dot{\gamma}(t_{K^*})\wedge {J}_1^h\wedge\cdots \wedge {J}_{n-2}^h\neq 0
% \]
% since in this case $\det(A(h))\neq 0$. 
%Let $\widetilde{J}_l^{\,h}:\R\to TM$, $l=1,\ldots,n-2$, be the solutions to the Jacobi equation on the geodesic $\gamma$ with initial conditions given at the time $t_{K^*}\in (0,T)$ by
%\[
% \widetilde{J}_l^{\,h}(t_{K^*})=J_l^h \text{ and } \dot{\widetilde{J}_l^{\,h}}(t_{K^*})= {J}_l(t_{K^*}).
%\]
%%We inspect the Jacobi fields $\widetilde{J}_i^h$ at times $t< t_{K^*}$. 
%By the continuous dependence of the Jacobi equation on its initial data we have that 
%\[
% \widetilde{J}_l^{\,h}\to J_l, \text{ as } h\to 0
%\]
%in the space of vector fields over $\gamma([0,T])$ in the $C^0$ norm. Thus, by using~\eqref{deltak} there exists $h_0>0$ so that
%\[
%\norm{V_k\wedge \dot{\gamma}(t_k)\wedge \widetilde{J}_1^{\,h_0}(t_{k})\wedge\cdots \wedge \widetilde{J}_{n-2}^{\,h_0}(t_{k})}>0
%\]
%for all $k=0,\ldots, K^*$. This shows that the Jacobi fields $\widetilde{J}_1^{\,h_0}, \ldots, \widetilde{J}_{n-2}^{\,h_0}$ span $T_{x_k}M$ at times $t_k$  for all $k=0,\ldots, K^*$. Renaming the Jacoci fields $\widetilde{J}_l^{\,h_0}$ as $J_l$, $l=1,\ldots,n-2$, concludes the recursion argument. \qedhere
%% 
%% Then, for $\delta$ chosen as above, by continuity of the Jacobi equation there exists $\epsilon_0>0$ so that if $\epsilon<\epsilon_{0}$, we have $||{{J}_l(t_{K^*},\epsilon)-J_l(t_{K^*})}||_{g}<\delta$. Let $\tilde{J}_l(t)$, $t\leq t_{K^*}$, denote the solution to the Jacobi equation with initial data $({J}_l(t_{K^*},\epsilon_0), \dot{J}_l(t_{K^*}))$ backwards in the parameter $t$. Again, by continuous dependence on initial conditions, for all $\tilde \epsilon>0$, $||{{J}_l(t_{K^*},\epsilon)-J_l(t_{K^*})}||_{g}<\delta$ implies $||\tilde{J}_l-J_l(\cdot)||_{g}<\tilde\epsilon$. 
% 
%%   Moreover, \eqref{lin_indep_J} still holds for $\tilde{J}_l(t_{k})$, with $k=0,\ldots, K^*-1$ and $l=1,\ldots,n-2$. 
%%  Thus we have
%% \[
%%  V_k\wedge\dot{\gamma}(t_k)\wedge \tilde{J}_1(t_{k})\wedge\cdots \tilde{J}_{n-2}(t_k)\neq 0, \quad k=1,\ldots,K^*.
%% \]
%
%%  It only remains to show \eqref{Js_tangent}. For the Jacobi fields $\tilde{J}_{1},\dots,\tilde{J}_{n-2}$ constructed above, we may further adjust $\epsilon$ in the above construction so that the projection of $\tilde{J}_{l}(0)$ to $T(\{t_{0}\}\times N)$, denoted by $\tilde{J}^{\top}_{l}(0)$, is nonzero for each $l=1,\dots,n-2$. Let $J_{l}$ be the Jacobi fields arising from the initial data $(\tilde{J}^{\top}_{l}(0), \dot{\tilde{J}}_{l}(0))$, $l= 1,\dots,n-2$.
%%  As the projection map is continuous, by the perturbation procedure above, we may achieve Jacobi fields $J_{1},\dots, J_{n-2}$ satisfying both \eqref{Js_tangent} for $t=0$ and \eqref{lin_indep_J} at each $t_{k}$ for $k=1,\ldots,K^*$.
%%  
%%   This completes the recursive proof.
%%   
%%   We have found $n-2$ Jacobi fields and next we define a variation of the original geodesic as follows. If $s\in (-a,a)^{n-2}$, $a>0$ sufficiently small, then we define a path $r mapsto \alpha(rv)$, $v$ by
%%   \[
%%    \alpha (r) := \exp_{0;x_0}\left(r \frac{s^1}{\abs{s}J_1(0) + \dots + s^{n-2}J_{n-2}(0)\right)
%%   \]
%% % % % % 
%% % % % %   
%% % % % % We move on to constructing a submanifold $S$ of $TC\cap P^rM$ with the desired properties. % mappings $\alpha$ and $W$ and the submanifold $S$ in the second claim of this lemma. 
%% % % % % Let $\eps>0$ and 
%% % % % %  %Next, we construct the submanifold $S$ in local coordinates ad show that the flowout $G_S\subset M$ has dimension $n-1$ at the points $x_k$, $k=0,\dots,K$. 
%% % % % %  let $s = (s^1, \dots , s^{n-2})\in (\epsilon,\epsilon)^{n-2}$. We define a variation $\Gamma$ of the geodesic $\gamma$ by
%% % % % %  \[
%% % % % %   \Gamma(t,s) := \exp_{\alpha(s)}\left(t\,W(s)\right),
%% % % % %  \]
%% % % % % %\gamma(t,s) := \exp_{\alpha(s)}\left(t\tilde{W}(s)\right)$ be an induced variation of $\gamma$ by the chosen Jacobi fields $J_1,\dots, J_{n-2}$. 
%% % % % % where $\alpha$ and $W$ are defined as follows. We define $\alpha:(-\eps,\eps)^{n-2}\to M$ as
%% % % % %  \[
%% % % % %  \alpha(s) := \exp_{x_0}\left(s^1J_1(0) + \dots + s^{n-2}J_{n-2}(0)\right).
%% % % % %  \]
%% % % % %  Let $\beta_s:(-\eps,\eps)\to M$ be the geodesic $\beta_s(r)=\alpha(rs/\abs{s})$. We define $W:(-\eps,\eps)^{n-2}\to TM$ by
%% % % % %  \[
%% % % % %   W(s) \text{ is the parallel transport of } \dot{\gamma}(0) + \sum_{l=1}^{n-2} s^l\dot{J}_l(0) \text{ along the geodesic } \beta_s \text{ to } T_{\beta(\abs{s})}M.
%% % % % %  \]
%% % % % %  An alternative way to write the definition of $W$ would be $W(s)=\text{PT}_{\beta}^{\,\abs{s}}\big(\dot{\gamma}(0) + \sum_{l=1}^{n-2} s^l\dot{J}_l(0)\big)$, where $\text{PT}_{\beta}^r$ is the parallel transport along the geodesic $\beta_s$ at the time $r$.
%% % % % % % Let us extend $\gamma$ and the Jacobi fields $J_i$ to be defined for $t\in \R$, and extend $\Gamma$ likewise. 
%% % % % % % Since $\gamma$ intesects the time-slice at time $t_0$, we have that the set
%% % % % % %  \[
%% % % % % %   \Gamma(\R,(-\eps,\eps)^{n-2})\subset M
%% % % % % %  \]
%% % % % % %  intersects the time-slice. 
%% % % % %  
%% % % % %  We show next that if $k\in \{0,\ldots, K\}$, then the set
%% % % % %  \[
%% % % % %   \Gamma(\R,(-\eps,\eps)^{n-2})\subset M
%% % % % %  \]
%% % % % %  is a submanifold of $M$ on a neighbourhood of the point $\gamma(t_k)$. To prove this, we let $k\in \{0,\ldots, K\}$ and we calculate 
%% % % % %  the differential of $\Gamma(t,s)$ at the points $(t_k,0)$. We have by the standard properties of the geodesic variation (see e.g.~\cite[Theorem 5.2.1]{Jost_book}) that
%% % % % % % 
%% % % % % % 
%% % % % % % 
%% % % % % %  
%% % % % % %  where once again $\exp_{0; x_0}$ is the exponential map defined on an open set of $T_{x_0}(\{0\}\times N)$. As the space of Jacobi fields on $\gamma$ splits naturally into those tangent to $\gamma$ and those normal to $\gamma$, \eqref{lin_indep_J} implies that $J_l\in T_{x_0}(\{0\}\times N)$ for each $l$.
%% % % % % %  
%% % % % % % We define vectors $\tilde{W}(s)$ along $\alpha$ to be the parallel transport of the vector $\dot{\gamma}(0) + \sum s^l\dot{J}_l(0)$ along the image of $\alpha(s)$. Set 
%% % % % % %  \[
%% % % % % % W(0):= r\frac{\tilde{W}(s)}{||\tilde{W}(s)||_g}.
%% % % % % %  \] 
%% % % % % % %of the form 
%% % % % % % % \[
%% % % % % % % W(s):=r\frac{W_1(s^1) + \dots + W_{n-2}(s^{n-2})}{||W_1(s^1) + \dots + W_{n-2}(s^{n-2})||_g},
%% % % % % % % \] 
%% % % % % % % where $W_l(s^l)$ ($l$ not summed) is the parallel transport of the vector $\dot{\gamma}(0) + s_l \dot{J}_l(0)$ along the curve $\alpha(0, \dots, 0 , s_l, 0, \dots, 0)$. 
%% % % % % %  Note that $W_l(0)=  r\frac{\dot{\gamma}(0)}{||\dot{\gamma}(0)||_g}$, and by our choice of scaling, $W(s)\in \PP^r_{t_0}$.
%% % % % % %  % Now we show that the flowout $G_S\subset M$ has dimension $n-1$ at the points $x_k$, $k=0,\dots,K$. 
%% % % % % %  
%% % % % % %  Set 
%% % % % % %  \[
%% % % % % %   S =\left\{s\in (-\epsilon,\epsilon)^{n-2}: \left(\alpha(s),W(s)\right)\right\}.
%% % % % % %  \]
%% % % % % %  By construction of the curve $\alpha$ and the vector field $W(s)$, we see that $S\subset \PP^r_{0}$. It remains to show that $S$ and $G_S$ are manifolds.
%% % % % % % 
%% % % % % %  At each $k$, we have by construction 
%% % % % %  \begin{align}\label{Ds}
%% % % % %   &\frac{\partial }{\partial s^l} \Gamma(t,s^1, \dots , s^{n-2})\big|_{t=t_k,\,s=0} = \frac{\partial }{\partial s^l} \exp_{\alpha(s)}\left(t\,W(s)\right)\big|_{t=t_k,\,s=0}  \\
%% % % % %   &=\frac{d}{dr}\exp_{\hat{\alpha}(r)}\left(t\,\widetilde{W}(r)\right)\big|_{t=t_k,\,r=0}=J_{l}(t_k),\nonumber
%% % % % %  \end{align}
%% % % % %  where we have denoted $\hat{\alpha}(r)= \exp_{x_0}\left(rJ_l(0)\right)$ and $\widetilde{W}(r)=PT_{\alpha'}^{\,r}(\dot{\gamma}(0)+r\dot{J}_l)$. We also have that
%% % % % % \begin{equation}\label{Dt}
%% % % % %   \frac{\partial }{\partial t} \Gamma(t,s^1, \dots , s^{n-2})\big|_{t=t_k,\,s=0} = \dot{\gamma}(t_k).
%% % % % %  \end{equation}
%% % % % %  Since the vectors $J_1(t_k),\dots, J_{n-2}(t_k)$ and $\dot{\gamma}(t_k)$ are linearly independent by the first part of this lemma,
%% % % % %  the equations~\eqref{Ds} and~\eqref{Dt} imply that the mapping $\Gamma$ is of full rank $n-1$ on a neighbourhood of the point $(t_k,0)$.  As the map $\Gamma(t,s)$ is also smooth, %and %the vector fields $J_1,\dots, J_{n-2}$ and $\dot{\gamma}$ are linearly independent by~\eqref{lin_indep_J} at each $t_k$, 
%% % % % %  the constant rank theorem implies that $\Gamma(\R,(-\eps,\eps)^{n-2})$ is a smooth manifold of dimension $n-1$ on a neighbourhood $U_k\subset M$ the point $\gamma(t_k)$. Moreover, there is a neighbourhood $\Omega_k$ of $(t_k,0)\in (\R\times (-\eps,\eps)^{n-2})$ such that $\Gamma:\Omega_k\to \Gamma(\Omega_k)$ is a diffeomorphism.
%% % % % %  
%% % % % %  Let us then find a submanifold $S$ of $P_{t_0}^{\,r}M \subset  TM$ such that the projection $G_S\subset TM$ of the geodesic flowout of $S$ is the set $\Gamma(\R,(-\eps,\eps)^{n-2})$. For this, let us first define
%% % % % %  \[
%% % % % %   I=\Gamma(\R,(-\eps,\eps)^{n-2})\cap \mathcal{C}\neq \emptyset,
%% % % % % \]
%% % % % % where $\mathcal{C}$ is a Cauchy surface.
%% % % % % The set $\Gamma(\R,(-\eps,\eps)^{n-2})$ and the Cauchy surface $\mathcal{C}$ are $n-1$ dimensional $C^\infty$ submanifolds (see~\cite{bernal2005} for the latter) on a neighbourhood of $x_0\in M$ that intersect each other transversally. By redefining $\eps>0$ smaller, if necessary, it follows that $I$ is an $n-2$ dimensional submanifold of $M$ by the standard transverality result~\cite[Theorem 6.30]{Lee_DG_book}, and that $I\subset \Gamma(\Omega_0)$. %Thus $\Psi_0$ is defined on $I$. 
%% % % % % Let us next define a smooth vector field $p:I\to TM$ on $I$ by
%% % % % % \[
%% % % % %  p(x)=\frac{d}{dr}\Big|_{r=0}\Gamma\big(\Gamma^{-1}_0(x)+r,\Gamma_1^{-1}(x),\ldots, \Gamma_{n-1}^{-1}(x)\big), \quad x\in I,
%% % % % % \]
%% % % % % where $\Gamma^{-1}_l$, $l=0,1,\ldots,n-2$, are the component functions of the inverse of $\Gamma|_{\Omega_0}$.
%% % % % % Define
%% % % % % \[
%% % % % %  S:=\big\{(x,\widetilde{p}(x))\in TM: x\in I, \ \widetilde{p}(x)=rp(x)/\sqrt{-g(p(x),p(x))}\big\}.
%% % % % % \]
%% % % % %  It follows that $G_S$ equals $\Gamma(\R,(-\eps,\eps)^{n-2})$, since if $x\in \Gamma(\R,(-\eps,\eps)^{n-2})$, then $x$ is a point on a geodesic $t\mapsto \exp_{\alpha(s)}\left(t\,W(s)\right)$ that intersects $\mathcal{C}$ for some $s$. Moreover, $S$ is submanifold of $T\mathcal{C}\cap P^{r}M$ since $p$ is smooth and the norm of $p$ is nonzero (by redefining $\eps>0$ smaller if necessary). %\qedhere
%\end{proof}
%
%% % % % % \begin{lemma}[]\label{manifold_jacobi_const2}
%% % % % % Assume as in Lemma~\ref{manifold_jacobi_const} and adopt its notation. There exists a submanifold $S$ of $T\mathcal{C}\cap P^rM\subset TM$ such that $(x_0,p_0)\in S$ and that the projection of the geodesics flowout $G_S$ of $S$ has the following property: If $k=0,\ldots, K$, then on a neighbourhood of $\gamma(t_k)$ the  projection of $G_S$ is a submanifold of $M$ of dimension $n-1$ which is transversal to $V_k$.
%% % % % %  \end{lemma}
%% % % % % \begin{proof}
%% % % % %  a
%% % % % % \end{proof}
%
%
%
%%  
%% If the intersection happens at $t that has the initial velocity $\frac{d}{dr}\Big|_{r=0}
%% % \[
%% %  x=\Gamma(t,s)
%% % \]
%
%\tbl{TONY: The formulation of the next lemma needs to be checked so that we can apply it in the proof of Lemma \ref{ss_map_determines_intersection}. At the moment I think it can not be applied, at least as it is, and thus it is marked in gray for removal.}
%We also formulate Lemma~\ref{manifold_jacobi_const} above for the situation where we consider two distinct Lorentzian manifolds.
%{\color{gray}
%\begin{lemma}[]\label{two_manifold_jacobi_const}
%Let $(M_1, g_1)$ and $(M_2,g_2)$ be $C^\infty$-smooth globally hyperbolic Lorentzian manifolds. Assume that $B_j$, $j=1,2$, are open subsets of $M_j$, and assume that $\mathcal{C}_j\subset M_j$ are Cauchy surfaces such that $\mathcal{C}_j\cap B_j\neq \emptyset$. Assume also that there is an isometry $\Psi: B_1\to B_2$ such that $\Psi(\mathcal{C}_1\cap B_1)=\mathcal{C}_2\cap B_2$.%~\footnote{We need to assume at some point of the paper that $\Psi(\mathcal{C}_1)=\mathcal{C}_2$?  TB: is this not given by the fact the isometry must preserve the foliation $\R\times N$?}}
%
%Let $r>0$, $x_0\in C_1$, and let $p_0\in P^r_{x_0}(M_1)$. % be a future-directed vector. 
%%Let $\gamma_1: \R \to M$ to be the timelike geodesic with initial data given as $(\gamma(0),\dot{\gamma}(0)) = (x_0, p_0)$.
%Let $T>0$ and let $\gamma_1,\gamma_2:[0,T]\to M_j$, be geodesics with the initial data $(\gamma_1(0),\dot{\gamma}_1(0)) = (x_0, p_0)$ and $(\gamma_2(0),\dot{\gamma}_2(0)) = (\Psi(x_0), \Psi_*(p_0))$ respectively.
%% 
%% and that ther with a Cauchy surface $C$. %$\{t_0\}\times N\subset M$. 
%% Let $r>0$, $x_0\in C$, and let $p_0\in P^r_{x_0}$ be future-directed vector. Let $\gamma: \R \to M$ to be the timelike geodesic with initial data given as $(\gamma(0),\dot{\gamma}(0)) = (x_0, p_0)$.
%For $a=1,2$, let $K_a\in \N$ and $T>0$ and choose
%\begin{itemize}
%\item $K_a+1$ locations $x_{a,k}:= \gamma_a(t_{a,k})$, with $t_{a,0}<t_{a,1}<\dots < t_{a,K}<T$.
%\item $K_a+1$ causal vectors $V_{a,k}\in T_{x_{a,k}}M_a$, $k_a\in\{0,1,\dots, K_a\}$, with the property that $V_{a,k}$ is not parallel to $\dot{\gamma}_a(t_{a,k})$.
%%\[ z_k:= \gamma(t_k), \text{ with } t_0<t_1<\dots < t_K<T. \]
%\end{itemize}
% Then there exists a submanifold $S$ of $T\mathcal{C}\,\cap\, P^r(M_1)\subset TM_1$ such that the projections of the geodesic flowouts $G_S$ and $G_{\Psi_*S}$ of $S$ and $\Psi_*S$ in $M_1$ and $M_2$ respectively have the following property: The sets $G_S$ and $G_{\Psi_*S}$ are submanifolds near the points $x_{k_1}$ and $x_{k_2}$, $k_j\in\{0,1,\dots, K_j\}$ that are transversal to $V_{j,k}$ respectively, $j=1,2$. %Moreover $\Phi(G_S)=G_{\Phi_*(S)}$. 
% \end{lemma}
%\begin{proof}
%We first prove the claim in the special case $(M_1,g_1)=(M_2,g_2)$. %After that we argue for the general case. 
%For this, we denote $(M,g)=(M_1,g_1)$, $\gamma=\gamma_1$ and $t_k=t_{1,k}$ etc. 
%
%Let us construct a submanifold $S$ of $TC\cap P^rM$ with the desired properties. 
%% mappings $\alpha$ and $W$ and the submanifold $S$ in the second claim of this lemma. 
%Let $J_1,\dots, J_{n-2}$ be $n-2$ Jacobi fields along $\gamma$ with the properties as in Lemma~\ref{manifold_jacobi_const}. %such that the vectors
%Let $\eps>0$ and 
% %Next, we construct the submanifold $S$ in local coordinates ad show that the flowout $G_S\subset M$ has dimension $n-1$ at the points $x_k$, $k=0,\dots,K$. 
% let $s = (s^1, \dots , s^{n-2})\in (\epsilon,\epsilon)^{n-2}$. We define a variation $\Gamma$ of the geodesic $\gamma$ by
% \[
%  \Gamma(t,s) := \exp_{\alpha(s)}\left(t\,W(s)\right),
% \]
%%\gamma(t,s) := \exp_{\alpha(s)}\left(t\tilde{W}(s)\right)$ be an induced variation of $\gamma$ by the chosen Jacobi fields $J_1,\dots, J_{n-2}$. 
%where $\alpha$ and $W$ are defined as follows. We define $\alpha:(-\eps,\eps)^{n-2}\to M$ as
% \[
% \alpha(s) := \exp_{x_0}\left(s^1J_1(0) + \dots + s^{n-2}J_{n-2}(0)\right).
% \]
% Let $\beta_s:(-\eps,\eps)\to M$ be the geodesic $\beta_s(r)=\alpha(rs/\abs{s})$. We define $W:(-\eps,\eps)^{n-2}\to TM$ by
% \[
%  W(s) \text{ is the parallel transport of } \dot{\gamma}(0) + \sum_{l=1}^{n-2} s^l\dot{J}_l(0) \text{ along the geodesic } \beta_s \text{ to } T_{\beta(\abs{s})}M.
% \]
% An alternative way to write the definition of $W$ would be $W(s)=\text{PT}_{\beta}^{\,\abs{s}}\big(\dot{\gamma}(0) + \sum_{l=1}^{n-2} s^l\dot{J}_l(0)\big)$, where $\text{PT}_{\beta}^r$ is the parallel transport along the geodesic $\beta_s$ at the time $r$.
%% Let us extend $\gamma$ and the Jacobi fields $J_i$ to be defined for $t\in \R$, and extend $\Gamma$ likewise. 
%% Since $\gamma$ intesects the time-slice at time $t_0$, we have that the set
%%  \[
%%   \Gamma(\R,(-\eps,\eps)^{n-2})\subset M
%%  \]
%%  intersects the time-slice. 
% 
% We show next that if $k\in \{0,\ldots, K\}$, then the set
% \[
%  \Gamma(\R,(-\eps,\eps)^{n-2})\subset M
% \]
% is a submanifold of $M$ on a neighbourhood of the point $\gamma(t_k)$. To prove this, we let $k\in \{0,\ldots, K\}$ and we calculate 
% the differential of $\Gamma(t,s)$ at the points $(t_k,0)$. We have by the standard properties of the geodesic variation (see e.g.~\cite[Theorem 5.2.1]{Jost_book}) that
%% 
%% 
%% 
%%  
%%  where once again $\exp_{0; x_0}$ is the exponential map defined on an open set of $T_{x_0}(\{0\}\times N)$. As the space of Jacobi fields on $\gamma$ splits naturally into those tangent to $\gamma$ and those normal to $\gamma$, \eqref{lin_indep_J} implies that $J_l\in T_{x_0}(\{0\}\times N)$ for each $l$.
%%  
%% We define vectors $\tilde{W}(s)$ along $\alpha$ to be the parallel transport of the vector $\dot{\gamma}(0) + \sum s^l\dot{J}_l(0)$ along the image of $\alpha(s)$. Set 
%%  \[
%% W(0):= r\frac{\tilde{W}(s)}{||\tilde{W}(s)||_g}.
%%  \] 
%% %of the form 
%% % \[
%% % W(s):=r\frac{W_1(s^1) + \dots + W_{n-2}(s^{n-2})}{||W_1(s^1) + \dots + W_{n-2}(s^{n-2})||_g},
%% % \] 
%% % where $W_l(s^l)$ ($l$ not summed) is the parallel transport of the vector $\dot{\gamma}(0) + s_l \dot{J}_l(0)$ along the curve $\alpha(0, \dots, 0 , s_l, 0, \dots, 0)$. 
%%  Note that $W_l(0)=  r\frac{\dot{\gamma}(0)}{||\dot{\gamma}(0)||_g}$, and by our choice of scaling, $W(s)\in \PP^r_{t_0}$.
%%  % Now we show that the flowout $G_S\subset M$ has dimension $n-1$ at the points $x_k$, $k=0,\dots,K$. 
%%  
%%  Set 
%%  \[
%%   S =\left\{s\in (-\epsilon,\epsilon)^{n-2}: \left(\alpha(s),W(s)\right)\right\}.
%%  \]
%%  By construction of the curve $\alpha$ and the vector field $W(s)$, we see that $S\subset \PP^r_{0}$. It remains to show that $S$ and $G_S$ are manifolds.
%% 
%%  At each $k$, we have by construction 
% \begin{align}\label{Ds}
%  &\frac{\partial }{\partial s^l} \Gamma(t,s^1, \dots , s^{n-2})\big|_{t=t_k,\,s=0} = \frac{\partial }{\partial s^l} \exp_{\alpha(s)}\left(t\,W(s)\right)\big|_{t=t_k,\,s=0}  \\
%  &=\frac{d}{dr}\exp_{\hat{\alpha}(r)}\left(t\,\widetilde{W}(r)\right)\big|_{t=t_k,\,r=0}=J_{l}(t_k),\nonumber
% \end{align}
% where we have denoted $\hat{\alpha}(r)= \exp_{x_0}\left(rJ_l(0)\right)$ and $\widetilde{W}(r)=PT_{\alpha'}^{\,r}(\dot{\gamma}(0)+r\dot{J}_l)$. We also have that
%\begin{equation}\label{Dt}
%  \frac{\partial }{\partial t} \Gamma(t,s^1, \dots , s^{n-2})\big|_{t=t_k,\,s=0} = \dot{\gamma}(t_k).
% \end{equation}
% Since the vectors $J_1(t_k),\dots, J_{n-2}(t_k)$ and $\dot{\gamma}(t_k)$ are linearly independent by the first part of this lemma,
% the equations~\eqref{Ds} and~\eqref{Dt} imply that the mapping $\Gamma$ is of full rank $n-1$ on a neighbourhood of the point $(t_k,0)$.  As the map $\Gamma(t,s)$ is also smooth, %and %the vector fields $J_1,\dots, J_{n-2}$ and $\dot{\gamma}$ are linearly independent by~\eqref{lin_indep_J} at each $t_k$, 
% the constant rank theorem implies that $\Gamma(\R,(-\eps,\eps)^{n-2})$ is a smooth manifold of dimension $n-1$ on a neighbourhood $U_k\subset M$ the point $\gamma(t_k)$. Moreover, there is a neighbourhood $\Omega_k$ of $(t_k,0)\in (\R\times (-\eps,\eps)^{n-2})$ such that $\Gamma:\Omega_k\to \Gamma(\Omega_k)$ is a diffeomorphism.
% 
% Let us then find a submanifold $S$ of $P_{t_0}^{\,r}M \subset  TM$ such that the projection $G_S\subset TM$ of the geodesic flowout of $S$ is the set $\Gamma(\R,(-\eps,\eps)^{n-2})$. For this, let us first define
% \[
%  I=\Gamma(\R,(-\eps,\eps)^{n-2})\cap \mathcal{C}\neq \emptyset,
%\]
%where $\mathcal{C}$ is a Cauchy surface.
%The set $\Gamma(\R,(-\eps,\eps)^{n-2})$ and the Cauchy surface $\mathcal{C}$ are $n-1$ dimensional $C^\infty$ submanifolds (see~\cite{bernal2005} for the latter) on a neighbourhood of $x_0\in M$ that intersect each other transversally. By redefining $\eps>0$ smaller, if necessary, it follows that $I$ is an $n-2$ dimensional submanifold of $M$ by the standard transverality result~\cite[Theorem 6.30]{Lee_DG_book}, and that $I\subset \Gamma(\Omega_0)$. %Thus $\Psi_0$ is defined on $I$. 
%Let us next define a smooth vector field $p:I\to TM$ on $I$ by
%\[
% p(x)=\frac{d}{dr}\Big|_{r=0}\Gamma\big(\Gamma^{-1}_0(x)+r,\Gamma_1^{-1}(x),\ldots, \Gamma_{n-1}^{-1}(x)\big), \quad x\in I,
%\]
%where $\Gamma^{-1}_l$, $l=0,1,\ldots,n-2$, are the component functions of the inverse of $\Gamma|_{\Omega_0}$.
%Define
%\[
% S:=\big\{(x,\widetilde{p}(x))\in TM: x\in I, \ \widetilde{p}(x)=rp(x)/\sqrt{-g(p(x),p(x))}\big\}.
%\]
% It follows that $G_S$ equals $\Gamma(\R,(-\eps,\eps)^{n-2})$, since if $x\in \Gamma(\R,(-\eps,\eps)^{n-2})$, then $x$ is a point on a geodesic $t\mapsto \exp_{\alpha(s)}\left(t\,W(s)\right)$ that intersects $\mathcal{C}$ for some $s$. Moreover, $S$ is submanifold of $T\mathcal{C}\cap P^{r}M$ since $p$ is smooth and the norm of $p$ is nonzero (by redefining $\eps>0$ smaller if necessary). This ends the proof of the special case $(M_1,g_1)=(M_2,g_2)$.
%
%To prove the general case, we argue as follows. 
%We first use Lemma~\ref{manifold_jacobi_const} to find $n-2$ Jacobi fields $J_{1,l}$, $l=1,\ldots,n-2$, on $M_1$ such that 
%\begin{equation}\label{span_eq}
%V_{1,k}, \,\dot{\gamma_1}(t_{1,k}),\, J_{1,1}(t_{1,k}),\ldots, J_{1,n-2}(t_{1,k})
%\end{equation}
%%the vectors corresponding to the ones in~\eqref{lin_indep_J} 
%span $T_{x_{1,k}}M_1$, $k=1,\ldots, K_1$. % by using the construction in  %To do this, we first do the exact same construction for the Jacobi fields on $M_1$ as we did in the proof of
%%Lemma~\ref{manifold_jacobi_const}. 
%
%We move on study the situation on the manifold $M_2$. We transform the initial data of the Jacobi fields $J_{1,k}$ %the already found Jacobi fields 
%%
%on $M_1$ onto $M_2$ by the diffeomorphisms $\Psi$. Using this initial data, we construct $n-2$ Jacobi fields on $(M_2,g_2)$. By perturbing the the initial data 
%as in the proof of Lemma~\ref{manifold_jacobi_const}, we may assume that $V_{2,k}, \,\dot{\gamma_2}(t_{2,k}),\, J_{2,1}(t_{2,k}),\ldots, J_{2,n-2}(t_{2,k})$
%%the vectors corresponding to the ones in~\eqref{lin_indep_J} 
%span $T_{x_{2,k}}M_1$, $k=1,\ldots,K_2$. For this, it sufficient to have an arbitrary small perturbation of the initial data.
%%we use again the recursion argument in the proof of Lemma~\ref{manifold_jacobi_const} to perturb the initial Jacobi fields on $M_2$. As a result of the pertubation argument, the vectors corresponding to the ones in~\eqref{lin_indep_J} span $T_{x_{k_2}}M_2$. 
%After this pertubation we have by using $\Psi^{-1}$ updated initial data for Jacobi fields on $(M_1,g_1)$. Since it was sufficient to do an arbitrarily small perturbation we may assume that~\eqref{span_eq} still holds.  % Taking the perturbations of the Jacobi fields on $M_2$ small enough, the Jacobi fields on $M_1$ corresponding to the updated initial data still have the property that the vectors corresponding to the ones in~\eqref{lin_indep_J} span $T_{x_{k_1}}M_1$. 
%
%The submanifold $S$ of $T\mathcal{C}\cap P^r_{x_0}(M_1)\subset TM_1$ is constructed as in the special case above. %exactly as in the proof of Lemma~\ref{manifold_jacobi_const} and has the claimed properties. 
%Since $\Psi$ is an isometry, also $\Psi_*(S)$ have the claimed properties. %is a submanifold of $T\Phi_*(C)\cap P^r_{x_0}(M_2)\subset TM_2$ with the claimed properties. %That $\Phi(G_S\cap B_1)=G_{\Phi_*(S)}$ follows from the assumption that $\Phi$ is an isometry.
%\end{proof}
%}




==> Sections/vlasov-boltz.tex <==
%
% Last edited: June 4, 2019 TB
%
%
\section{Vlasov and Boltzmann Kinetic Models}\label{LB-models}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  The Vlasov model
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{The Vlasov model}\label{Vlasov}

We consider a system of particles on a Lorentzian manifold $(M,g)$ having positions $x\in M$ and momenta $p\in \PP_xM$ in a statistical fashion as a density distribution $u\in \mathcal{D}'( \PP M )$. We assume that the support of $u$ is contained in some compact and proper subset $K\subset \overline{\PP} M$. %{\color{red}( $\leftarrow$ Here you had $ \mathcal{D}'( K )$ which I changed since I believe you actually mean the distributions $\mathcal{D}_K'( \PP M )$. Notice that $\mathcal{D}_K'( \PP M ) \neq \mathcal{D}'( K ) $ in general. --Antti)} 
The Vlasov model describes the trajectories of a system of particles in a relativistic setting where there are no external forces and where collisions between particles are negligible. In this situation, the individual particles travel along geodesics determined by initial positions and velocities. % to by those conditions. 
On the level of density distributions, the behaviour of the system of particles is captured by the \emph{Vlasov equation} %(see \cite{ \tjb{add citations to CB, HR, AR})
%
\begin{align}
\mathcal{X}u&=f,
\end{align}
%
where $f\in \mathcal{D}'( \PP M )$ is a source of particles and $\mathcal{X} : TM \rightarrow TTM$ on $TM$ is the geodesic vector field. Locally, this vector field has the expression~\f{$x$ added.}  
\[
\mathcal{X} =   p^\alpha  \frac{\partial}{\partial x^\alpha}  -  \Gamma^\alpha_{\lambda \mu}(x)   p^\lambda  p^\mu  \frac{\partial}{\partial p^\alpha }.
\]
Above the functions $\Gamma^\alpha_{\lambda \mu}$, $\lambda,\mu,\alpha = 0,\dots, \nnn=\dim(M)-1$, are the Christoffel symbols of the Lorentz metric $g$.

The geodesic vector field  $-i\mathcal{X}:C^\infty(\PP M ) \rightarrow C^\infty(\PP M )$ may be viewed as Fourier Integral Operator (FIO) with principal symbol 
\begin{align}\label{principal_symbol_of_X}
\sigma_\mathcal{X}  : T^* TM \rightarrow \R, \ \ 
\sigma_\mathcal{X} (x,p^\alpha \, ; \, \xi^x_\alpha,  \xi_\alpha^p ) =   p^\alpha \xi^x_\alpha   - \Gamma^\alpha_{\lambda \mu} (x)  p^\lambda  p^\mu  \xi^p_\alpha.  %= \langle \xi ,  i\mathcal{X}  \rangle
\end{align}
Writing $\langle \ccdot, \ccdot \rangle$ for the dual paring between $TTM$ and $T^*TM$, $\sigma_\mathcal{X}$ takes the form
\[
\sigma_\mathcal{X} (x,p \, ; \, \xi) =  \langle \xi , \mathcal{X} \rangle |_{(x,p)} =  \big\langle \xi , \partial_s \dot\gamma_{(x,p)} (s)  \big\rangle\big|_{s=0}.
\]
Therefore, a function $\phi \in C^\infty ( TM )$ satisfies $\sigma_\mathcal{X} (x,p,d\phi |_{(x,p)} ) = 0$ at each $(x,p) \in TM$ if and only if $\phi$ is constant along geodesic velocity curves $s\mapsto \dot\gamma_{(x,p)}(s)$. Thus the bicharacteristic strip of $-i\mathcal{X}$ with initial data $(\tilde{x},\tilde{p} \; \tilde\xi )\in \sigma_\mathcal{X}^{-1} (0)$ is the parametrized curve
%\[
%s\mapsto (x(s),p(s) \ ; \ \xi(s) ) \in T^* T(\R \times N),
%\]
\[
s\mapsto (x(s),p(s)) = \dot\gamma_{(\tilde{x},\tilde{p})}(s) , \ \  \xi(s) = d \phi|_{\dot\gamma_{(\tilde{x},\tilde{p})} (s) }, 
\]
where $\phi \in C^\infty(TM)$ is any smooth function which is constant along geodesic velocity curves and satisfies $d \phi|_{(\tilde{x},\tilde{p})} = \tilde{\xi}$. We denote by $\Lambda_\XX$ the collection of pairs 
\begin{equation}\label{lambda_XX}
 ((x,p \, ; \, \xi) ,(y,q \, ; \, \eta)) \in T^* TM \times T^*  TM
 \end{equation}
% that are characteristic (i.e. belong to $\sigma_\mathcal{X}^{-1} (0)$) and 
that lie on the same bicharacteristic strip of $\XX$. 


 \begin{lemma}\label{uuiisok}
Let $(M,g)$ be a globally hyperbolic $C^{\infty}$-smooth Lorentzian manifold and write it in the standard 
%$($global time $\times$ space$)$ 
form $M = \R \times N$ of global time and space. Let $t \in \R$. 
The geodesic vector field $-i\mathcal{X}$ on $\PP M$ is a strictly hyperbolic operator of multiplicity $1$ with respect to the submanifold $\PP_{t}M:= (T_t\R  \times TN) \cap \PP M$. 

%Likewise, $\mathcal{X}^0$ is a strictly hyperbolic operator of multiplicity $1$ with respect to the submanifold $P_{t}^0M= P^0M \cap ( T_{t} \R \times  T N )$. %(T_t\R  \times TN) \cap \PP M$.
%\end{lemma}
\end{lemma}
\tbl{We omit the proof of the lemma, which is a straightforward verification of the conditionsin~\cite[Definition 5.1.1]{duistermaat2010fourier}.}
%{\color{gray} We have placed the proof of the above lemma in Appendix \ref{appendix-al}.}~\f{We omit the proof from the journal version.}

% {\color{blue}

In this section, the space $(M,g)$ is assumed to be globally hyperbolic
%geodesically complete 
$C^\infty$-smooth Lorentzian manifold, but not necessarily geodesically complete. 
%, and 
%$A:
%(TM)^{\otimes4}
%\Sigma \to \mathbb{R}$ an admissible collision kernel. 
 Given \tbl{the initial data that $u$ vanishes in the past of a Cauchy surface and a source $f$}, we will show that the Vlasov equation $\mathcal{X}u=f$ has a unique solution. There is a substantial amount of literature on this topic (see for example \cite{Choquet-Bruhat}, \cite{Andreasson}, \cite{Ringstrom}, and \cite{Rendall}). 
For example, Lemma \ref{uuiisok} together with standard results for hyperbolic Cauchy problems (see e.g.~\cite[Theorem 5.1.6]{duistermaat2010fourier}) demonstrates uniqueness of solutions to the Vlasov equation. 

Let us denote by $\gamma_{(x,p)}:(-T_1,T_2)\to M$ the inextendible geodesic which satisfies
\begin{equation}
\gamma_{(x,p)}(0)=x \text{ and } \dot{\gamma}_{(x,p)}(0)=p.                                                                                                                            
\end{equation}
Since $(M,g)$ is not necessarily geodesically complete, we might have that $T_1<\infty$ or $T_2<\infty$. Existence of solutions to $\XX u =f$, with initial data $u=0$, in the case where $f(x,p)$ is a smooth function on $\OVS M$ with compact support in the base variable $x\in M$, can be shown by checking that 
\begin{equation}\label{integrate_over_flow}
u(x,p) := \int_{-\infty}^0 f( \gamma_{(x,p)}(t) , \dot\gamma_{(x,p)}(t) )  dt \quad \text{on} \quad (x,p) \in \OVS M
\end{equation}
 is well-defined and satisfies $\XX u =f$. 
%  
%  Indeed, this integral is well-defined since on a globally hyperbolic Lorentzian manifold any causal geodesic $\gamma$ exits a given compact set $K_\pi\subset M$ permanently after finite parameter times. That is, there are parameter times $t_1,t_2$ such that $\gamma(\{t<t_1\}),\gamma(\{t>t_2\})\subset M\setminus K_\pi$. Thus the integral above is actually an integral of a smooth function over a finite interval. 
%  
%  
\tbl{Indeed, on a globally hyperbolic Lorentzian manifold for a given compact set $K_\pi\subset M$ and a causal geodesic $\gamma$, there are $t_1,t_2\in \R$ such that for parameter times $t\notin[t_1,t_2]$ we have $\gamma(t)\notin K_\pi$. Thus the integral above is actually over a finite interval. 
Because $f$ and the geodesic flow on $(M,g)$ are smooth, the function $u(x,p)$ is smooth.  If $(M,g)$ is not geodesically complete, and if $\gamma_{(x,p)}:(-T_1,T_2)\to M$, we interpret the integral above to be over $(-T_1,0]$. % when $\gamma_{(x,p)}:(-T_1,T_2)\to M$. 
 We interpret similarly for all similar integrals without further notice.}

% -----------------------------------
% 
% Given initial data $u=0$, and source $f$, we will show that the Vlasov equation $\mathcal{X}u=f$ has a unique solution. There is a substantial amount of literature on this topic (see for example \cite{Choquet-Bruhat}, \cite{Andreasson}, \cite{Ringstrom}, and \cite{Rendall}).  %Below is a summary of this literature relevant for the purposes of this paper. 
% % \begin{remark}\label{uuiisok-2}
% % Instead consider the restriction of $\mathcal{X}$ to $P^0 M$, denoted $\mathcal{X}^0$. By the argument of lemma \ref{uuiisok}, we also discover $-i\mathcal{X}^0$ is strictly hyperbolic of multiplicity $1$ with respect to $P^0_{t} M :=P^0M \cap ( T_{t} \R \times  T N )$. Thus, in the analysis that follows, the results also hold when replacing $\mathcal{X}$ with $\mathcal{X}^0$, $\PP M$ with $P^0 M$, and   $\PP_t M$ with $P_t^0 M$.
% % \end{remark}
% %and $\mathcal{X}^0$ on $S^0$ and $S^0_{t_0} :=S^0 \cap ( T_{t_0} \R \times  T N )$
% For example, Lemma \ref{uuiisok} together with standard results for hyperbolic Cauchy problems (see e.g.~\cite[Theorem 5.1.6]{duistermaat2010fourier}) show uniqueness of solutions to the Vlasov equation in the case of smooth initial data and a smooth source. Existence of solutions to this problem in the case where $f(x,p)$ is a smooth function on $\OVS M$ with compact support in the base variable $x\in M$ can be shown by checking that $u(x,p) =  \IX f(x,p)$ for
% \begin{equation}\label{integrate_over_flow}
% \IX f: (x,p) \mapsto \int_{-\infty}^0 f( \gamma_{(x,p)}(t) , \dot\gamma_{(x,p)}(t) )  dt \quad \text{on} \quad (x,p) \in \OVS M
% \end{equation}
%  is well defined\footnote{If $(M,g)$ is not geodesically complete and if $\gamma_{(x,p)}:(-T_1,T_2)\to M$, we interpret the integral to be defined on the interval $(-T_1,0]$.} and satisfies $\mathcal{X}u=f$. We note here that the map $u(x,p) =  \IX f(x,p)$ is well-defined since on the globally hyperbolic Lorentzian manifold $(M,g)$ causal geodesics exit compact sets in finite parameter time and do not return to the compact set. Thus $\IX f(x,p)$ is an integral of a smooth function over a finite interval. 
%  
% Further, since $f$ and the geodesic flow on $(M,g)$ are smooth the map~\eqref{integrate_over_flow} is smooth.  
 

%: Let $\rho_0$ be the restriction operator, defined as the the pullback of the inclusion $ \PP_0 M \hookrightarrow \PP M$. Recall that $\PP_0 M := (T_0\R  \times TN) \cap \PP M$. For every $f\in C^\infty(\PP M)$, the Cauchy problem~\footnote{\tbl{See where the restriction operator is used the next time. Define it there and remove it here.}}
%\begin{align}\label{vlasov-smooth}
%\begin{cases}
%\mathcal{X}u = f, \\
%%\rho_0  \partial_t u = g_1 \\
%\rho_0 u = 0
%\end{cases}
%\end{align}
%has a unique solution.


If $\mathcal{C}$ is a Cauchy surface of $M$, we write $\mathcal{C}^\pm$ for the causal future ($+$) or the causal past ($-$) of $\mathcal{C}$:
\[
 \mathcal{C}^\pm=J^\pm(\mathcal{C}).
\]
In particular, the notation $\OVS \mathcal{C}^\pm$ refers to the subset of $TM$ of future directed causal vectors on the causal future ($+$) or past ($-$) of the Cauchy surface $\mathcal{C}$, i.e. $\OVS \mathcal{C}^\pm=\OVS [J^\pm(\mathcal{C})]$ (see~\eqref{causal_spaces} for more details). If $K\subset \OVS \mathcal{C}^+$ is compact and $k\geq 0$ is an integer, we define the Banach space
%by $C_K^k(\OVS M)$ the Banach space of functions $f$ with $f\in C^k(\OVS \mathcal{C}^+)$ with $\supp{f}\subset K$:
\[
C_K^k(\OVS \mathcal{C}^+) := \{f\in C^k(\OVS \mathcal{C}^+)\,:\, \text{supp}(f)\subset K\},
\]
equipped with the norm of $C^k$.


For our purposes it is convenient to have explicit formulas for solutions to the Vlasov equation and therefore we give a proof using the solution formula~\eqref{integrate_over_flow}.
\begin{theorem}\label{vlasov-exist}
Assume that $(M, g)$ is a globally hyperbolic $C^\infty$-smooth Lorentzian manifold. Let $\mathcal{C}$ be a Cauchy surface of $(M,g)$, $K\subset \OVS \mathcal{C}^+$ be compact and $k\ge 0$.
Let also $f\in C_K^k(\OVS M)$. Then, the problem
\begin{alignat}{2}\label{vlasov1}
%\begin{gathered}
\mathcal{X}u(x,p)&= f(x,p) \quad &&\text{on} \quad \OVS M \nonumber \\
u(x,p)&= 0 \quad &&\text{on} \quad  \OVS \mathcal{C}^- 
%\end{gathered}
\end{alignat}
has a unique solution $u$ in $C^k ( \OVS M )$. We write $u=\IX(f)$ and call $\IX: C^k_K(\OVS M)\to C^k(\OVS M)$ the solution operator \tbl{to~\eqref{vlasov1}}. In particular, \tbl{if $Z\subset \OVS M$ is compact, there is a constant $c_{k,K,Z}>0$ such that  
\begin{align} \norm{u|_Z}_{C^k ( Z)}\le c_{k,K,Z}\|f\|_{C^{k}
( \OVS M )}. \label{est-vlasov1}
\end{align}
If $k=0$, the estimate above is independent of $Z$: 
\[
 \norm{u}_{C ( \OVS M)}\le c_{K}\|f\|_{C( \OVS M )}.
\]
}
\end{theorem}
% \begin{theorem}\label{vlasov-exist}
% Assume that $(M, g)$ is a globally hyperbolic $C^\infty$-smooth Lorentzian manifold. Let $k\ge 0$ and $\mathcal{C}$ be a Cauchy surface of $M$. % $\mathcal{X}: TM\to TTM$ be the geodesic vector field, and let $\compp \subset  \OVS ( (0,\infty) \times N)$ be a compact set. 
% %Then, there is an open neighbourhood $V_K \subset C_K^k (\OVS M)$ of $0$ such that if $f \in V_K$, the Cauchy problem
% Let also $f\in C_c^k(\OVS \mathcal{C}^+)$. Then, the problem %~\footnote{Note that this problem equivalent to Duistermaat Theorem 5.1.6 p.123 formulation with $m=1$ and $g_1=0$.} %Note that this does not mean $E=\IX$
% \begin{alignat}{2}\label{vlasov1}
% %\begin{gathered}
% \mathcal{X}u(x,p)&= f(x,p) \quad &&\text{on} \quad \OVS M \nonumber \\
% u(x,p)&= 0 \quad &&\text{on} \quad  \OVS \mathcal{C}^- %((-\infty,0] \times N)
% %\end{gathered}
% \end{alignat}
% has a unique solution $u=\IX f$ in $C^k ( \OVS M )$. %~\footnote{\tbl{What is this? Where it is needed?}}
% % \[
% % \text{supp}(u) \subset \{ (x,p) \in TM :  (x,p) := (\gamma_{(y,q)}(s), \dot\gamma_{(y,q)}(s)) , \ \ s\geq 0, \ \ (x,p) \in \compp \}.
% % \]
% %and 
%  In particular, there is a constant $c_k>0$ such that  
% \begin{align} \norm{u}_{C^k ( \OVS M)}\le c_k\|f\|_{C^{k}
% ( \OVS M )}. %\label{est-vlasov1}
% \end{align}
% %
% % Moreover, we may also consider the problem~\eqref{vlasov1} for $f\in \mathcal{E}'(\OVS \mathcal{C}^+)$ and still obtain a unique solution $u\in \mathcal{D}'(\OVS \mathcal{C}^+)$. If in this case we have $f\in I^m(S)$ for some submanifold $S\subset \OVS M$ and $m\in \R$, then $u\in I^{m- 1/4}(K_S)$.
We have placed the proof of the theorem in Appendix \ref{appendix-ss}. The proof follows from the explicit formula~\eqref{integrate_over_flow} for the solution. We call $\IX$ the solution operator to~\eqref{vlasov1}. The source-to-solution map $\Phi^L$ of the Vlasov equation~\eqref{vlasov1} is defined as %by $\Phi^L$ as 
% 
% \begin{remark}
% Note that Theorem \ref{vlasov-exist} gives the existence of the source-to-solution map %$C_c^k(\OVS M)$, $k\ge 0$, such that the map 
% {\color{blue}
\[ \Phi^L: C_K^k (\OVS M) \to C^k  ( \OVS M ), \ \ \Phi^L(f) = u,\]
% of the Vlasov equation.
where $u$ is the unique solution to \eqref{vlasov1} with the source $f\in C^k_K(\OVS M)$ and $k\geq 0$. As we will soon see, the Vlasov equation is the linearization of the Boltzmann equation with a source-to-solution map $\Phi$.
We also consider the setting where we relax the condition that the source $f$ above is smooth and show that the solution operator to~\eqref{vlasov1} (when considering separately timelike and lightlike vectors) has a unique continuous extension to the class of distribution $f$, which satisfy $WF(f)\cap N^*(\SP \mathcal{C})=\emptyset$. For the precise statement and  proof thereof, please see Appendix \ref{appendix-ss}.



%------- EDITED THIS BEGINNING - TONY November 10 2020

% Given initial data $u=0$, and source $f$, we will show that the Vlasov equation $\mathcal{X}u=f$ has a unique solution. There is a substantial amount of literature on this topic (see for example \cite{Choquet-Bruhat}, \cite{Andreasson}, \cite{Ringstrom}, and \cite{Rendall}).  %Below is a summary of this literature relevant for the purposes of this paper. 
% % \begin{remark}\label{uuiisok-2}
% % Instead consider the restriction of $\mathcal{X}$ to $P^0 M$, denoted $\mathcal{X}^0$. By the argument of lemma \ref{uuiisok}, we also discover $-i\mathcal{X}^0$ is strictly hyperbolic of multiplicity $1$ with respect to $P^0_{t} M :=P^0M \cap ( T_{t} \R \times  T N )$. Thus, in the analysis that follows, the results also hold when replacing $\mathcal{X}$ with $\mathcal{X}^0$, $\PP M$ with $P^0 M$, and   $\PP_t M$ with $P_t^0 M$.
% % \end{remark}
% %and $\mathcal{X}^0$ on $S^0$ and $S^0_{t_0} :=S^0 \cap ( T_{t_0} \R \times  T N )$
% For example, Lemma \ref{uuiisok} together with standard results for hyperbolic Cauchy problems (see e.g.~\cite[Theorem 5.1.6]{duistermaat2010fourier}) show uniqueness of solutions to the Vlasov equation in the case of smooth initial data and a smooth source. Existence of solutions to this problem in the case where $f(x,p)$ is a smooth function on $\OVS M$ with compact support in the base variable $x\in M$ can be shown by checking that $u(x,p) =  \IX f(x,p)$ for
% \begin{equation}\label{integrate_over_flow}
% \IX f: (x,p) \mapsto \int_{-\infty}^0 f( \gamma_{(x,p)}(t) , \dot\gamma_{(x,p)}(t) )  dt \quad \text{on} \quad (x,p) \in \OVS M
% \end{equation}
%  is well defined\footnote{If $(M,g)$ is not geodesically complete and if $\gamma_{(x,p)}:(-T_1,T_2)\to M$, we interpret the integral to be defined on the interval $(-T_1,0]$.} and satisfies $\mathcal{X}u=f$. We note here that the map $u(x,p) =  \IX f(x,p)$ is well-defined since on the globally hyperbolic Lorentzian manifold $(M,g)$ causal geodesics exit compact sets in finite parameter time and do not return to the compact set. Thus $\IX f(x,p)$ is an integral of a smooth function over a finite interval. Further, since $f$ and the geodesic flow on $(M,g)$ are smooth the map~\eqref{integrate_over_flow} is smooth.  
 

% %: Let $\rho_0$ be the restriction operator, defined as the the pullback of the inclusion $ \PP_0 M \hookrightarrow \PP M$. Recall that $\PP_0 M := (T_0\R  \times TN) \cap \PP M$. For every $f\in C^\infty(\PP M)$, the Cauchy problem~\footnote{\tbl{See where the restriction operator is used the next time. Define it there and remove it here.}}
% %\begin{align}\label{vlasov-smooth}
% %\begin{cases}
% %\mathcal{X}u = f, \\
% %%\rho_0  \partial_t u = g_1 \\
% %\rho_0 u = 0
% %\end{cases}
% %\end{align}
% %has a unique solution.

% We relax the condition of smooth data above and prove the following local existence and uniqueness result for the Vlasov source problem. First we set a shorthand notation for causal sets in $M$.

% If $\mathcal{C}$ is a Cauchy surface of $M$, we write $\mathcal{C}^\pm$ for the causal future ($+$) or the causal past ($-$) of $\mathcal{C}$:
% \[
%  \mathcal{C}^\pm=J^\pm(\mathcal{C}).
% \]
% In particular, the notation $\OVS \mathcal{C}^\pm$ refers to the subset of $TM$ of future directed causal vectors on the causal future ($+$) or past ($-$) of the Cauchy surface $\mathcal{C}$, i.e. $\OVS \mathcal{C}^\pm=\OVS [J^\pm(\mathcal{C})]$ (see~\eqref{causal_spaces} for more details).


% \begin{theorem}\label{vlasov-exist}
% Assume that $(M, g)$ is a globally hyperbolic $C^\infty$-smooth Lorentzian manifold. Let $k\ge 0$ and $\mathcal{C}$ be a Cauchy surface of $M$. % $\mathcal{X}: TM\to TTM$ be the geodesic vector field, and let $\compp \subset  \OVS ( (0,\infty) \times N)$ be a compact set. 
% %Then, there is an open neighbourhood $V_K \subset C_K^k (\OVS M)$ of $0$ such that if $f \in V_K$, the Cauchy problem
% Let also $f\in C_c^k(\OVS \mathcal{C}^+)$. Then, the problem~\footnote{Note that this problem equivalent to Duistermaat Theorem 5.1.6 p.123 formulation with $m=1$ and $g_1=0$.} %Note that this does not mean $E=\IX$
% \begin{alignat}{2}\label{vlasov1}
% %\begin{gathered}
% \mathcal{X}u(x,p)&= f(x,p) \quad &&\text{on} \quad \OVS M \nonumber \\
% u(x,p)&= 0 \quad &&\text{on} \quad  \OVS \mathcal{C}^- %((-\infty,0] \times N)
% %\end{gathered}
% \end{alignat}
% has a unique solution $u=\IX f$ in $C^k ( \OVS M )$. %~\footnote{\tbl{What is this? Where it is needed?}}
% % \[
% % \text{supp}(u) \subset \{ (x,p) \in TM :  (x,p) := (\gamma_{(y,q)}(s), \dot\gamma_{(y,q)}(s)) , \ \ s\geq 0, \ \ (x,p) \in \compp \}.
% % \]
% %and 
%  In particular, there is a constant $c_k>0$ such that  
% \begin{align} \norm{u}_{C^k ( \OVS M)}\le c_k\|f\|_{C^{k}
% ( \OVS M )}. %\label{est-vlasov1}
% \end{align}

% Moreover, we may also consider the problem~\eqref{vlasov1} for $f\in \mathcal{E}'(\OVS \mathcal{C}^+)$ and still obtain a unique solution $u\in \mathcal{D}'(\OVS \mathcal{C}^+)$. If in this case we have $f\in I^m(S)$ for some submanifold $S\subset \OVS M$ and $m\in \R$, then $u\in I^{m- 1/4}(K_S)$.
% \end{theorem}

% For the proof, please see Appendix \ref{appendix-ss}.

% \begin{remark}
% Note that Theorem \ref{vlasov-exist} gives the existence of the source-to-solution map %$C_c^k(\OVS M)$, $k\ge 0$, such that the map 
% \[ \Phi^L: C_c^k (\OVS M) \to C^k  ( \OVS M ), \ \ \Phi^L(f) = u,\]
% of the Vlasov equation.
%  Here $u$ is the unique solution to \eqref{vlasov1} with the source $f$ and $k\geq 0$.
% \end{remark}

% %{\color{red} (Why is this emphasized? I also got confused 'cus this is not actually the ss-map of boltzmann but is called ss-map and looks like it. --Antti)}

% %The rest of this subsection, written for the operator $\mathcal{X}$ on $\PP$ holds also for $\mathcal{X}^0$ by replacing $\PP$ with $S^0$ and $\PP_0$ with $S^0_0$. 



%------- EDITED THIS END - TONY November 10 2020



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  The Boltzmann model
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The Boltzmann model}\label{Bman-model}

The Boltzmann model of particle kinetics in $(M,g)$ modifies the Vlasov model to take into account collisions between particles. This modification is characterized by the (relativistic) \emph{Boltzmann equation}
\begin{align*}
\mathcal{X} u(x,p) - \COLOP [u,u ] (x,p) &= 0.
\end{align*}
Here $\COLOP[\ccdot,\ccdot]$ is called the \emph{collision operator}. It is explicitly given by
\begin{align}\label{colop}
 \COLOP&:  C_c^\infty (\overline\PP M ) \times C_c^\infty (\overline\PP M)
%L^\infty(T(\R \times N) ) \times L^\infty(T(\R \times N) )  
\rightarrow C^\infty (\overline\PP M )\\
\COLOP[u_1,u_2](x,p) &=\int_{\Sigma_{x, p }} \left[ u_1 (x,p) u_2 (x,  q )  - u_1 (x,p' ) u_2 (x,  q' )\right]  A(x,p,q, p', q') dV_{x,p} (q,p',q'), \nonumber
\end{align}
where $ dV_{x,p} (q,p',q')$ for fixed $(x,p)$ is a volume form defined on 
\begin{align}\label{Sigma_Set}
\Sigma_{x,p} &= \{ (p, q, p', q' ) \in   (\overline{\mathcal{P}}_{x}M)^4 : p + q = p' + q' \} \subset T_xM^4,
\end{align} 
which is induced by a volume form $dV(x,p, q,p',q')$ on the manifold
\begin{align}\label{Sigma_union}
\Sigma &= \bigcup_{(x,p)\in \OVS} \Sigma_{x,p}.
%\Sigma_{x,p} &= \{ (q, p', q' ) \in   (T_{x}M)^3 : p + q = p' + q' \}.
\end{align}
We call $A=A(x,p,q,p',q')$ the \emph{collision kernel} and assume that it is admissible in the sense of Definition~\ref{good-kernels}. 
% satisfies $A \in C^\infty(\Sigma)$, $A\geq 0$.

Heuristically, $\COLOP$ describes the average density of particles with position and momentum $(x,p)$, which are gained and lost from the collision of two particles $u_1,u_2$. The contribution to the average density from the gained particles is
\begin{align}\label{Q-gain}
\COLOP_{gain} [u_1, u_2] (x,p) :=- \int_{\Sigma_{x, p }} u_1 (x,p' ) u_2 (x,  q' )  A(x,p,q, p', q') dV_{x,p} (q,p',q'), %dV (x,p \ ; \ q,p',q'), 
\end{align}
and the contribution from the lost particles is % as a result of the collision, given by the first term in \eqref{colop}
\begin{align}
\COLOP_{loss}[u_1, u_2] (x,p):= u_1 (x,p) \int_{\Sigma_{x, p }}   u_2 (x,  q ) A(x,p,q, p', q') dV_{x,p} (q,p',q'). %dV (x,p \ ; \ q,p',q') 
\end{align}



%Though we do not consider them, the physical quantities of invariant mass, total energy, and total momentum can be defined and shown to be conserved under the Boltzmann kinematic model (see \cite{Choquet-Bruhat}, \cite{Ringstrom}, or \cite{Rendall} for more details).~\footnote{\tbl{Move this to intro.}}

%\begin{remark}
%One could also define the collision operator on causal particle densities by choosing the domain of the collision operator to be $ C_c^\infty (\overline\PP M ) \times C_c^\infty %(\overline\PP M)$ instead of $C_c^\infty (\PP M ) \times C_c^\infty (\PP M)$. This is not necessary here. Notice that the outgoing particle distribution, i.e. the range of the collision %operator, covers also the photons. 
%\end{remark}

The existence and uniqueness to the initial value problem for the Boltzmann equation has been studied in the literature under various assumptions on the geometry of the Lorentzian manifold, properties of the collision kernel and assumptions on the data, see for example~\cite{Bichteler,Bancel,Glassey}. These references consider the Boltzmann equation on $L^2$-based function spaces.
%to \eqref{boltz-smooth}, global existence and uniqueness to \eqref{boltz-smooth} has been shown; see
% (as opposed to $L^2$ based function spaces.)
%As we are not concerned with controlling the energy of solutions (i.e. we do not require $u$ to lie in some Sobolev space), 

We consider the following initial value problem for the Boltzmann equation on a globally hyperbolic manifold $(M,g)$ with a source $f$ % and initial data $f_0$ 
\begin{align*}%\label{boltz-smooth}
%\begin{cases}
\mathcal{X} u - \COLOP [u,u ] &= f, \quad \text{on }\OVS M\\
%\rho_0  \partial_t u = g_1 \\
 u  &= 0, \quad \text{on }\OVS \mathcal{C}^{-},
%\end{cases}
\end{align*}
%where we recall that $\rho_0$ is the restriction operator to $\PP_0 M$. 
where $\mathcal{X}$ is the geodesic vector field on $TM$, $\mathcal{C}$ is a Cauchy surface of $M$ and $\mathcal{C}^{\pm}$ denotes the causal future (+)/past (-) of $\mathcal{C}$. %The condition $u=0$ on $\OVS [J^-(\mathcal{C})]$ is equivalent to $u=0$, for $\mathcal{T}\leq 0$ if $\mathcal{T}$ is a time function on $(M,g)$ with $\mathcal{C}=\{\mathcal{T}=0\}$. %ifold $\overline\PP M$ with boundary $P^0 M$. 
%In this paper, 
%We will mostly consider the Boltzmann model of kinematics with the presence of a smooth particle source $f \in C_c^\infty (\PP^+ M)$, considered as an element of $C^\infty(\overline\PP M )$, and trivial initial data $f_0 = 0$. 
%The existence (local or global) and uniqueness of solutions to \eqref{boltz-smooth} is highly dependent on the choice of collision kernel for $\COLOP$. %At the time of writing, the properties collision kernel should posses are not satisfactorily understood. 
We assume that $(M,g)$ is globally hyperbolic and that the collision kernel of $\COLOP$ is admissible in the sense of Definition~\ref{good-kernels}. Our conditions on the collision kernel allow us to consider the Boltzmann equation in the space of continuous functions. We also assume that the sources $f$ are supported in a fixed compact set $K\subset \OVS C^+$. Note that (since $0\notin \OVS M$) this especially means that $f$ is supported outside a neighbourhood of the zero section of $TM$. We work with the following function spaces, each equipped with the supremum norm:
\begin{align*}
C_b(\OVS \mathcal{C}^+) &:= \{h\in C(\OVS \mathcal{C}^+)\,:\,h \text{ is bounded}\},
\end{align*}
and 
\[
C_K(\OVS \mathcal{C}^+) := \{h\in C(\OVS \mathcal{C}^+)\,:\, \text{supp}(h)\subset K\}.
\]

%We prove the following existence result to the Boltzmann equation Cauchy problem under the assumption that the collision kernel $A$ is admissible in the sense of Definition \ref{good-kernels}.


% \begin{theorem}\label{boltz-exist}
% Let $(M, g)$ be a globally hyperbolic $C^\infty$-smooth Lorentzian manifold and $\XX$ its associated geodesic vector field. %$\compp$ be a compact set in $\OVS ((0, \infty) \times N) $ and set 
% Let $A: \Sigma \to \mathbb{R}$ to be an admissible collision kernel in the sense of Definition \ref{good-kernels}.
% %Assume also that $\text{supp}(x \mapsto A(x,\cdot,\cdot,\cdot,\cdot))$ is compact. 
% 
% Then, there are open neighbourhoods $B_1 \subset C_c (\OVS M )$ and $B_2\subset C( \OVS  M )$~\footnote{\tbl{Figure out a better notation for the space $C_{\OVS( [0,\infty)\times N )} ( \OVS  M )$}} of the origins such that if $f \in B_1$, the Cauchy problem
% \begin{equation}\label{boltz1}
% \begin{gathered}
% \mathcal{X}u(x,p)-\COLOP[u,u](x,p)= f(x,p) \quad \text{on} \quad 
% \OVS((0,\infty)\times N)
% \\
% u(x,p)= 0 \quad \text{on} \quad \OVS (J^-[\pi(\supp{f})])
% \end{gathered}
% \end{equation}
% has a unique solution $u\in B_2$. Here $\pi$ is the canonical projection.~\footnote{\tbl{Figure out decent notation regardind the support of $f$.}}
% Further, 
% \[ \|u\|_{C( \OVS M )}\le C\|f\|_{C_c(\OVS M)},\]
% for some constant $C>0$. 
% % % 
% % % 
% % % 
% % % Let $(M, g)$ be a globally hyperbolic $C^\infty$-smooth Lorentzian manifold and $\XX$ its associated geodesic vector field. %$\compp$ be a compact set in $\OVS ((0, \infty) \times N) $ and set 
% % % Let $A: \Sigma \to \mathbb{R}$ to be an admissible collision kernel in the sense of Definition \ref{good-kernels}.
% % % %Assume also that $\text{supp}(x \mapsto A(x,\cdot,\cdot,\cdot,\cdot))$ is compact. 
% % % 
% % % Then, there are $\delta>0$ and $\eps>0$ and open balls $B(0,\delta) \subset C_c (\OVS M )$ and $B(0,\eps)\subset C_{\OVS( [0,\infty)\times N )} ( \OVS  M )$ %  ~\footnote{\tbl{Figure out a better notation for the space $C_{\OVS( [0,\infty)\times N )} ( \OVS  M )$}} of the origins 
% % % such that if $f \in B(0,\delta)$, the Cauchy problem
% % % \begin{equation}\label{boltz1}
% % % \begin{gathered}
% % % \mathcal{X}u(x,p)-\COLOP[u,u](x,p)= f(x,p) \quad \text{on} \quad 
% % % \OVS((0,\infty)\times N)
% % % \\
% % % u(x,p)= 0 \quad \text{on} \quad \OVS ((-\infty,0]\times N)
% % % \end{gathered}
% % % \end{equation}
% % % has a unique solution $u\in B(0,\eps)$. 
% % % Further, 
% % % \[ \|u\|_{C_{\OVS( [0,\infty)\times N )} ( \OVS M )}\le C\|f\|_{C_c(\OVS M)},\]
% % % for some constant $C>0$. 
% % Let $(M, g)$ be a globally hyperbolic $C^\infty-$smooth Lorentzian manifold and $\XX$ its associated geodesic vector field. Let $\compp$ be a compact set in $\OVS ((0, \infty) \times N) $ and set  $A: \Sigma \to \mathbb{R}$ to be an admissible collision kernel.
% % %Assume also that $\text{supp}(x \mapsto A(x,\cdot,\cdot,\cdot,\cdot))$ is compact. 
% % 
% % Then, there is an open neighbourhood $V_K \subset C_K^\zerok (\OVS M)$, $0 \in V_K$ such that if $f \in V_K$, the Cauchy problem
% % \begin{equation}\label{boltz1}
% % \begin{gathered}
% % \mathcal{X}u(x,p)-\COLOP[u,u](x,p)= f(x,p) \quad \text{on} \quad 
% % \OVS M
% % \\
% % u(x,p)= 0 \quad \text{on} \quad x \in (-\infty,0]\times N
% % \end{gathered}
% % \end{equation}
% % has a unique small~\footnote{\tbl{Define what means ``small''.}} solution $u\in  C^\zerok (\OVS M )$. 
% % Further, 
% % \[ \|u\|_{C^\zerok ( \OVS M )}\le c_\compp\|f\|_{C^{\zerok}_K(\OVS M )},\]
% % for some constant $c_\compp>0$. 
% \end{theorem}


 

\begin{reptheorem}{boltz-exist}
% Assume that $(M, g)$ is a globally hyperbolic $C^\infty$-smooth Lorentzian manifold. Let $k\ge 0$ and $\mathcal{S}$ be a Cauchy surface of $M$. % $\mathcal{X}: TM\to TTM$ be the geodesic vector field, and let $\compp \subset  \OVS ( (0,\infty) \times N)$ be a compact set. 
% %Then, there is an open neighbourhood $V_K \subset C_K^k (\OVS M)$ of $0$ such that if $f \in V_K$, the Cauchy proble

\tjb{Let $(M, g)$ be a globally hyperbolic $C^\infty$-smooth Lorentzian manifold. Let also $\mathcal{C}$ be a Cauchy surface of $M$ and $K\subset \OVS \mathcal{C}^+$ be compact. % and $\XX$ its associated geodesic vector field. %$\compp$ be a compact set in $\OVS ((0, \infty) \times N) $ and set 
Assume that $A: \Sigma \to \mathbb{R}$ is an admissible collision kernel in the sense of Definition \ref{good-kernels}.}
%Assume also that $\text{supp}(x \mapsto A(x,\cdot,\cdot,\cdot,\cdot))$ is compact. 

\tjb{There are open neighbourhoods $B_1 \subset C_K(\OVS \mathcal{C}^+ )$ and $B_2\subset C_b( \OVS  M )$ of the respective origins such that if $f \in B_1$, the Cauchy problem}
\begin{alignat}{2}\label{boltz1}
%\begin{gathered}
\mathcal{X}u(x,p)-\COLOP[u,u](x,p)&= f(x,p) \quad && \text{ on } 
\OVS M \nonumber \\
u(x,p)&= 0 \quad &&\text{ on } \OVS \mathcal{C}^-
%\end{gathered}
\end{alignat}
\tjb{has a unique solution $u\in B_2$. There is a constant $c_{A,K}>0$ such that}
\[ \|u\|_{C( \OVS M )}\le c_{A,K}\|f\|_{C(\OVS M)}.\]

% Let $(M, g)$ be a globally hyperbolic $C^\infty$-smooth Lorentzian manifold. Let also $\mathcal{C}$ be a Cauchy surface of $M$ and $K\subset \OVS \mathcal{C}^+$ be compact. Assume that $A: \Sigma \to \mathbb{R}$ is an admissible collision kernel in the sense of Definition \ref{good-kernels}. 

% There are open neighbourhoods $B_1 \subset C_K(\OVS \mathcal{C}^+ )$ and $B_2\subset C_b( \OVS  M )$ of the respective origins such that if $f \in B_1$, the Cauchy problem
% \begin{alignat}{2}\label{boltz1}
% %\begin{gathered}
% \mathcal{X}u(x,p)-\COLOP[u,u](x,p)&= f(x,p) \quad && \text{ on } 
% \OVS M \nonumber \\
% u(x,p)&= 0 \quad &&\text{ on } \OVS \mathcal{C}^-
% %\end{gathered}
% \end{alignat}
% has a unique solution $u\in B_2$. There is a constant $C>0$ such that
% \[ \|u\|_{C_b( \OVS M )}\le C\|f\|_{C_K(\OVS M)}.\]
\end{reptheorem}

%\begin{theorem}\label{boltz-exist}
%% Assume that $(M, g)$ is a globally hyperbolic $C^\infty$-smooth Lorentzian manifold. Let $k\ge 0$ and $\mathcal{C}$ be a Cauchy surface of $M$. % $\mathcal{X}: TM\to TTM$ be the geodesic vector field, and let $\compp \subset  \OVS ( (0,\infty) \times N)$ be a compact set. 
%% %Then, there is an open neighbourhood $V_K \subset C_K^k (\OVS M)$ of $0$ such that if $f \in V_K$, the Cauchy proble
%
%Let $(M, g)$ be a globally hyperbolic $C^\infty$-smooth Lorentzian manifold. Let also $\mathcal{C}$ be a Cauchy surface of $M$. % and $\XX$ its associated geodesic vector field. %$\compp$ be a compact set in $\OVS ((0, \infty) \times N) $ and set 
%Assume that $A: \Sigma \to \mathbb{R}$ is an admissible collision kernel in the sense of Definition \ref{good-kernels}.
%%Assume also that $\text{supp}(x \mapsto A(x,\cdot,\cdot,\cdot,\cdot))$ is compact. 
%
%There are open neighbourhoods $B_1 \subset C_c(\OVS \mathcal{C}^+ )$ and $B_2\subset C( \OVS  M )$ of the respective origins such that if $f \in B_1$, the Cauchy problem
%\begin{alignat}{2}\label{boltz1}
%%\begin{gathered}
%\mathcal{X}u(x,p)-\COLOP[u,u](x,p)&= f(x,p), \quad && (x,p)\in
%\OVS M \nonumber \\
%u(x,p)&= 0, \quad && (x,p)\in \OVS \mathcal{C}^-
%%\end{gathered}
%\end{alignat}
%has a unique solution $u\in B_2$. There is a constant $C>0$ such that
%\[ \|u\|_{C( \OVS M )}\le C\|f\|_{C(\OVS M)}.\]
%\end{theorem}

We give a proof of Theorem \ref{boltz-exist} in Appendix \ref{appendix-ss}.
%
As a direct consequence, we find:
\begin{corollary}\label{ss-corollaari}
Assume as in Theorem \ref{boltz-exist} and adopt its notation. % Under the assumptions of Theorem \ref{boltz-exist} % and by using its notaion $B_1 Then the $B \subset C_c (\OVS  M)$ about the origin such that we have a well-defined 
The source-to-solution map
\[
\Phi : B_1 \rightarrow B_2 , \quad \Phi(f) = u
\]
is well-defined.
Here $u \in  B_2\subset C_b( \OVS M )$ is the unique solution to the Boltzmann equation~\eqref{boltz1} with the source $f\in B_1\subset C_K(\OVS M)$.
\end{corollary}

The proof of Corollary \ref{ss-corollaari} appears in Appendix \ref{appendix-ss}.

Given the existence of the source-to-solution map $\Phi$ associated to the Boltzmann equation, we now formally calculate the first and second Frech\'et differentials of $\Phi$, which will correspond to the first and second linearizations of the Boltzmann equation. %This correspondence is explained heuristically as follows. % is nonlinear
%As metioned in the introduction, we want to relate the source to solution map $\Phi$ for the Boltzmann equation to the source to solution map of the 
%collision kernel through a 
%second linearization of $\Phi$. 
%We recall the formal argument from the introduction. 
Let $\mathcal{C}$ be a Cauchy surface in $M$, and $f_1,f_2 \in C_c^\infty(\OVS \mathcal{C}^+)$, and consider the $2$-parameter family of functions
 \[
(\epsilon_1, \epsilon_2 ) \mapsto \Phi ( \epsilon_1 f_1 + \epsilon_2 f_2  )
\]
where $\eps_1,\eps_2$ are small enough so that $\eps_1f_1+\eps_2f_2\in B_1$.
Formally expanding in $\epsilon_1$ and $\epsilon_2$, we obtain
\[
\Phi(\epsilon_1 f_1 + \epsilon_2 f_2) = \epsilon_1 \Phi^L(f_1) + \epsilon_2 \Phi^L(f_2) + \epsilon_1\epsilon_2 \Phi^{2L}(f_1,f_2)  + \text{higher order terms},
\]
where the higher order terms tend to zero as $(\epsilon_1, \epsilon_2 )\to (0,0)$ \tbl{in $C_b(\OVS M)$}. Substituting this expansion of $\Phi(\epsilon_1 f_1 + \epsilon_2 f_2)$ into the Boltzmann equation and  %$\Phi(\epsilon_1 f_1 + \epsilon_2 f_2)$ solves \eqref{boltz1} with source $ \epsilon_1 f_1 + \epsilon_2 f_2$, we obtain by 
differentiating in the parameters $\eps_1$ and $\eps_2$ at $\eps_1=\eps_2=0$ yields the equations
\[
\XX \Phi^L(f_j) = f_j, \quad j=1,2,
\]
and
\[
\XX \Phi^{2L}(f_1,f_2) =  \COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]+  \COLOP [ \Phi^L (f_2),  \Phi^L( f_1)] . \label{second-ss}
%\in C^\infty (\mathcal{C}),
\]
We call these equations the first and second linearizations of the Boltzmann equation. Notice that the first and second linearizations are a Vlasov-type equation \eqref{vlasov1} with a source term.

The next lemma makes the above formal calculation precise. We have placed the proof of the lemma in Appendix \ref{appendix-ss}.

% \begin{lemma}\label{deriv}
% Consider the setting of Theorem \ref{boltz-exist} above, and let $\Phi$ be the source-to-solution map for \eqref{boltz1}. Given $f,h\in C^\zerok_K (\OVS((0,\infty)\times N))$, we have:
% \begin{enumerate}
% \item the source to solution map $\Phi^{L}$ for the Vlasov Cauchy problem \eqref{vlasov1} (the first linearization of \eqref{boltz1} about $0$), satisfies \[ \Phi'(0;f):= \lim_{\epsilon\to0}\frac{\Phi(\epsilon f)-\Phi(0)}{\epsilon} = \Phi^{L}(f).\]
% \item the source to solution map $\Phi^{2L}$ for the second linearization of \eqref{boltz1} about $(0,0)$ satisfies \[ \Phi''(0;f,h):= \lim_{\epsilon\to0}\frac{\Phi'(\epsilon h;f)-\Phi'(0;f)}{\epsilon} = \Phi^{2L}(0).\]
% \end{enumerate}
% 
% \end{lemma}
\begin{lemma}\label{deriv}
Assume as in Theorem \ref{boltz-exist} and adopt its notation. Let $\Phi:B_1 \to B_2 \subset C_b(\OVS M)$, $B_1\subset C_K(\OVS \mathcal{C}^+)$, be the source-to-solution map of the Boltzmann equation. % as in Corollary~\ref{}.

The map $\Phi$ is twice Frech\'et differentiable at the origin of $C_K(\OVS \mathcal{C}^+)$. If $f,\, h\in B_1$, then:
\begin{enumerate}
\item The first Frech\'et derivative $\Phi'$ of the source-to-solution map $\Phi$ at the origin satisfies %for the Vlasov equation \eqref{vlasov11} (the first linearization of \eqref{boltz11} about $u=0$), 
%satisfies 
\[ \Phi'(0;f)
%\lim_{\epsilon\to0}\frac{\Phi(\epsilon f)-\Phi(0)}{\epsilon} 
= \Phi^{L}(f),\]
where $\Phi^L$ is the source-to-solution map of the Vlasov equation~\eqref{vlasov1}. %the limit is in $C(\OVS M)$.% $\Phi'$ denotes the Frech\'et derivative of $\Phi$
\item The second Frech\'et derivative $\Phi''$ of the source-to-solution map $\Phi$ at the origin satisfies %for the Vlasov equation \eqref{vlasov11} (the first linearization of \eqref{boltz11} about $u=0$), 
%satisfies
%The source to solution map $\Phi^{2L}$ for the second linearization of \eqref{boltz11} about $u=0$ and $v=0$, satisfies 
\[ \Phi''(0;f,h)%= \lim_{\epsilon\to0}\frac{\Phi'(\epsilon h;f)-\Phi'(0;f)}{\epsilon} 
= \Phi^{2L}(f,h),\]
where $\Phi^{2L}(f,h)\in C(\OVS M)$ is the unique solution to the equation 
\begin{alignat}{2}\label{second_lin_bman}
%\begin{gathered}
\mathcal{X}\Phi^{2L}(f,h)&= \COLOP[\Phi^L(f),\Phi^L(h)] + \COLOP[\Phi^L(h),\Phi^L(f)], \quad &&\text{ on }
\OVS M,\\
\Phi^{2L}(f,h)&= 0, \quad && \text{ on }\OVS \mathcal{C}^-.  \nonumber 
%\end{gathered}
\end{alignat}
 %is the source-to-solution map of the second linearization (see ~\eqref{} below) of the Boltzmann equation.
\end{enumerate}

\end{lemma}
% We note that technically speaking solvability of~\eqref{second_lin_bman} does not follow from Theorem~\ref{vlasov-exist}, since the term $\COLOP[\Phi^L(f),\Phi^L(h)] + \COLOP[\Phi^L(h),\Phi^L(f)]$ might not have compact support. However, this term is compactly supported in the base variable on $M$ and we may thus use the formula 
% 
% The first linearization of the Boltzmann equation about $u=0$ is the Vlasov equation \eqref{vlasov1}. Here, the second linearization of \eqref{boltz1} about the origin is 
% \begin{alignat}
%  \XX w &= \COLOP[v_1,v_2] + \COLOP[v_2,v_1]\quad \OVS M\\
%  w&=0,\quad \OVS \mathcal{C}^-,
% \end{alignat}
% where $v_1,v_2$ solve \eqref{vlasov1} with source data . The associated source to solution map is defined as 
% \begin{align}
%  \Phi^{2L}:=\IX\left(\COLOP[v_1,v_2] + \COLOP[v_2,v_1]\right).
% \end{align}
% 
% 
% 
% To define the second linearization, consider two smooth sources , 


%We call Equation~\ref{second_lin_bman} the second linearization of the Boltzmann equation.
We remark that the terms $\COLOP[\Phi^L(f),\Phi^L(h)] + \COLOP[\Phi^L(h),\Phi^L(f)]$ in~\eqref{second_lin_bman} might not have compact support in $\OVS M$, and thus unique solvability of~\eqref{second_lin_bman} does not follow directly from Theorem~\ref{vlasov-exist}. However, a unique solution to~\eqref{second_lin_bman} is shown to exist in the proof of the above lemma.

In our main theorem, Theorem~\ref{themain}, the measurement data consists of solutions to the Boltzmann equation restricted to our measurement set $V$. By Lemma~\ref{deriv} above, we obtain that the measurement data also determines the solutions to the first and second linearization of the Boltzmann equation restricted to  $V$. We will see from \eqref{second_lin_bman} that the second linearization $\Phi^{2L}$ captures information about the (singular) behaviour of the collision term $\COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]$. In the next section we will analyze the microlocal behaviour of $\COLOP [ \Phi^L(f_1),  \Phi^L( f_2) ]$. Then, in Section~\ref{main-proof}, we use this analysis to recover information about when particles collide in the unknown region $W$. From such particle interactions in $W$, we will parametrize points in the unknown set $W$ by light signals measured in $V$, which are obtained by restricting $\Phi^{2L}$ to lightlike vectors.































